Changes in zonal surface temperature gradients and Walker circulations in a wide range of climates

Variations in zonal surface temperature gradients and zonally asymmetric tropical overturning circulations (Walker circulations) are examined over a wide range of climates simulated with an idealized atmospheric general circulation model (GCM). The asymmetry in the tropical climate is generated by an imposed ocean energy flux, which does not vary with climate. The range of climates is simulated by modifying the optical thickness of an idealized longwave absorber (representing greenhouse gases). The zonal surface temperature gradient in low latitudes generally decreases as the climate warms in the idealized GCM simulations. A scaling relationship based on a two-term balance in the surface energy budget accounts for the changes in the zonally asymmetric component of the GCM-simulated surface temperature gradients. The Walker circulation weakens as the climate warms in the idealized simulations, as it does in comprehensive simulations of climate change. The wide range of climates allows a systematic test of energetic arguments that have been proposed to account for these changes in the tropical circulation. The analysis shows that a scaling estimate based on changes in the hydrological cycle (precipitation rate and saturation specific humidity) accounts for the simulated changes in the Walker circulation. However, it must be evaluated locally, with local precipitation rates. If global-mean quantities are used, the scaling estimate does not generally account for changes in the Walker circulation, and the extent to which it does is the result of compensating errors in changes in precipitation and saturation specific humidity that enter the scaling estimate.

==> bibliography/references <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Tapio Schneider at 2010-08-19 18:04:48 -0700 


%% Saved with string encoding Unicode (UTF-8) 



@article{Chang01a,
	Author = {E. K. M. Chang},
	Date-Added = {2010-08-17 15:57:14 -0700},
	Date-Modified = {2010-08-17 15:58:27 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {1784--1800},
	Title = {{GCM} and observational diagnoses of the seasonal and interannual variations of the {P}acific storm track during the cool season},
	Volume = {58},
	Year = {2001},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxjaGFuZzAxYS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAetAJx1QPrwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx1SALwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhbmcwMWEucGRmAAAOABoADABjAGgAYQBuAGcAMAAxAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2NoYW5nMDFhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9jaGFuZzAxYS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Black98a,
	Author = {Black, R. X.},
	Date-Added = {2010-08-17 10:44:11 -0700},
	Date-Modified = {2010-08-17 10:50:43 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {3159--3175},
	Title = {The maintenance of extratropical intraseasonal transient eddy activity in the {GEOS-1} assimilated dataset},
	Volume = {55},
	Year = {1998},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxibGFjazk4YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAes/CyJAYnwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyJB7DwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmxhY2s5OGEucGRmAAAOABoADABiAGwAYQBjAGsAOQA4AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2JsYWNrOThhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9ibGFjazk4YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Broccoli92a,
	Author = {Broccoli, A. J. and Manabe, S.},
	Date-Added = {2010-08-17 10:16:57 -0700},
	Date-Modified = {2010-08-17 10:19:07 -0700},
	Journal = {J. Climate},
	Pages = {1181--1201},
	Title = {The effects of orography on midlatitude Northern Hemisphere dry climates},
	Volume = {5},
	Year = {1992},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9icm9jY29saTkyYS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAes/xyJASiQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyJB0+QAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnJvY2NvbGk5MmEucGRmAA4AIAAPAGIAcgBvAGMAYwBvAGwAaQA5ADIAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvYnJvY2NvbGk5MmEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvYnJvY2NvbGk5MmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Branstator95a,
	Author = {Branstator, G.},
	Date-Added = {2010-08-17 10:08:39 -0700},
	Date-Modified = {2010-08-17 10:10:07 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {207--226},
	Title = {Organization of storm track anomalies by recurring low-frequency circulation anomalies},
	Volume = {52},
	Year = {1995},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXgAAAAAAXgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhFicmFuc3RhdG9yOTVhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAes/DyJAQbQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyJBy3QAAAAEADAAJDH4ACE6zAACS8wACADBNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnJhbnN0YXRvcjk1YS5wZGYADgAkABEAYgByAGEAbgBzAHQAYQB0AG8AcgA5ADUAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACRVc2Vycy90YXBpby9QYXBlcnMvYnJhbnN0YXRvcjk1YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHi4uLy4uL1BhcGVycy9icmFuc3RhdG9yOTVhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIcAh4CIwIsAjcCOwJJAlACWQJ6An8CggKPApQAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACpg==}}

@article{Chang09a,
	Author = {Chang, E. K. M.},
	Date-Added = {2010-08-16 16:05:20 -0700},
	Date-Modified = {2010-08-16 16:06:08 -0700},
	Journal = {J. Climate},
	Pages = {670--688},
	Title = {Diabatic and orographic forcing of northern winter stationary waves and storm tracks},
	Volume = {22},
	Year = {2009},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxjaGFuZzA5YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAeiwVxdb2nwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxddnHwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhbmcwOWEucGRmAAAOABoADABjAGgAYQBuAGcAMAA5AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2NoYW5nMDlhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9jaGFuZzA5YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Lee95a,
	Author = {Lee, S.},
	Date-Added = {2010-08-16 16:00:57 -0700},
	Date-Modified = {2010-08-16 16:01:33 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {977--989},
	Title = {Localized storm tracks in the absence of local instability},
	Volume = {52},
	Year = {1995},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpsZWU5NWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAeixXyI8RZAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyI9z1AAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGVlOTVhLnBkZgAADgAWAAoAbABlAGUAOQA1AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2xlZTk1YS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvbGVlOTVhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Lee93a,
	Author = {Lee, S. and Held, I. M.},
	Date-Added = {2010-08-16 15:56:51 -0700},
	Date-Modified = {2010-08-16 15:58:40 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {1413--1428},
	Title = {Baroclinic wave packets in models and observations},
	Volume = {50},
	Year = {1993},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpsZWU5M2EucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAeixGyI8QagAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyI9y2gAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGVlOTNhLnBkZgAADgAWAAoAbABlAGUAOQAzAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2xlZTkzYS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvbGVlOTNhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Chang93b,
	Author = {E. K. M. Chang},
	Date-Added = {2010-08-16 15:54:44 -0700},
	Date-Modified = {2010-08-16 15:55:53 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {2038--2053},
	Title = {Downstream development of baroclinic waves as inferred from regression analysis},
	Volume = {50},
	Year = {1993},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxjaGFuZzkzYi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAeiwxyI8P+wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyI9yawAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhbmc5M2IucGRmAAAOABoADABjAGgAYQBuAGcAOQAzAGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2NoYW5nOTNiLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9jaGFuZzkzYi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Chang93a,
	Author = {E. K. M. Chang and I. Orlanski},
	Date-Added = {2010-08-16 15:50:58 -0700},
	Date-Modified = {2010-08-16 15:54:02 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {999-1015},
	Title = {On the dynamics of a storm track},
	Volume = {50},
	Year = {1993},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxjaGFuZzkzYS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAeiwjyI8PSwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyI9xuwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhbmc5M2EucGRmAAAOABoADABjAGgAYQBuAGcAOQAzAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2NoYW5nOTNhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9jaGFuZzkzYS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{McShane10a,
	Author = {B. B. McShane and A. J. Wyner},
	Date-Added = {2010-08-16 10:37:29 -0700},
	Date-Modified = {2010-08-16 10:39:10 -0700},
	Journal = {Ann. Appl. Stat.},
	Title = {A statistical analysis of multiple temperature proxies: {Are} reconstructions of surface temperatures over the last 1000 years reliable?},
	Year = {2010},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5tY3NoYW5lMTBhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAeTDwyI6/dAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyI8h5AAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWNzaGFuZTEwYS5wZGYAAA4AHgAOAG0AYwBzAGgAYQBuAGUAMQAwAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL21jc2hhbmUxMGEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL21jc2hhbmUxMGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Showman10a,
	Author = {A. P. Showman and L. M. Polvani},
	Date-Added = {2010-08-02 23:09:39 -0700},
	Date-Modified = {2010-08-02 23:11:02 -0700},
	Journal = {Geophys. Res. Lett.},
	Title = {The {Matsuno}-{Gill} Model and Equatorial Superrotation},
	Year = {2010},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zaG93bWFuMTBhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAZhWFyH0AkwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyH1jAwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hvd21hbjEwYS5wZGYAAA4AHgAOAHMAaABvAHcAbQBhAG4AMQAwAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3Nob3dtYW4xMGEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3Nob3dtYW4xMGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Friedson10a,
	Author = {A. J. Friedson and R. A. West and E. H. Wilson and F. Oyafuso and G. S. Orton},
	Date-Added = {2010-07-21 13:15:51 -0700},
	Date-Modified = {2010-07-21 13:17:52 -0700},
	Journal = {Planet. Space Sci.},
	Pages = {1931--1949},
	Title = {A global climate model of {Titan}'s atmosphere and surface},
	Volume = {57},
	Year = {2010},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9mcmllZHNvbjEwYS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAPnSRyGyhhQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyG0D9QAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnJpZWRzb24xMGEucGRmAA4AIAAPAGYAcgBpAGUAZABzAG8AbgAxADAAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZnJpZWRzb24xMGEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZnJpZWRzb24xMGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Mingalev06a,
	Author = {Mingalev, I. V. and Mingalev, V. S. and Mingalev, O. V. and Kazeminejad, B. and Lammer, H. and Biernat, H. K. and Lichtenegger, H. I. M. and Schwingenschuh, K. and Rucker, H. O.},
	Date-Added = {2010-07-21 13:13:28 -0700},
	Date-Modified = {2010-07-21 13:18:40 -0700},
	Journal = {Ann. Geophys.},
	Pages = {2115--2129},
	Title = {First simulation results of {Titan}'s atmosphere dynamics with a global 3-D non-hydrostatic circulation model},
	Volume = {24},
	Year = {2006},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9taW5nYWxldjA2YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAPniRyGyi0wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyG0FQwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWluZ2FsZXYwNmEucGRmAA4AIAAPAG0AaQBuAGcAYQBsAGUAdgAwADYAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbWluZ2FsZXYwNmEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbWluZ2FsZXYwNmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Tokano09a,
	Author = {T. Tokano},
	Date-Added = {2010-07-21 13:11:01 -0700},
	Date-Modified = {2010-07-21 13:12:18 -0700},
	Journal = {Icarus},
	Pages = {619--636},
	Title = {Impact of seas/lakes on polar meteorology of {T}itan: {S}imulation by a coupled {GCM}-Sea model},
	Volume = {204},
	Year = {2009},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg10b2thbm8wOWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAPnHKyGye9AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyG0BZAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dG9rYW5vMDlhLnBkZgAOABwADQB0AG8AawBhAG4AbwAwADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvdG9rYW5vMDlhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3Rva2FubzA5YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Griffith09a,
	Author = {Caitlin Griffith and Paulo Penteado and Sebastien Rodriguez and Stephanie Le Mouelic and Kevin H. Baines and Bonnie Buratti and Roger Clark and Phil Nicholson and Ralf Jaumann and Christophe Sotin},
	Journal = {Astrophys. J.},
	Pages = {L105-109},
	Title = {Charaterization of clouds in {Titan's} tropical atmosphere},
	Volume = {702},
	Year = {2009},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9ncmlmZml0aDA5YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAALF10yFwmbgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyFyI3gAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3JpZmZpdGgwOWEucGRmAA4AIAAPAGcAcgBpAGYAZgBpAHQAaAAwADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZ3JpZmZpdGgwOWEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZ3JpZmZpdGgwOWEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Tokano05a,
	Author = {Tokano, T.},
	Date-Added = {2010-07-07 04:19:34 -0700},
	Date-Modified = {2010-07-07 04:20:58 -0700},
	Journal = {Icarus},
	Pages = {222--242},
	Title = {Meteorological assessment of the surface temperatures on {Titan}: {C}onstraints on the surface type},
	Volume = {173},
	Year = {2005},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg10b2thbm8wNWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAKoTwyFmxDwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyFoTfwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dG9rYW5vMDVhLnBkZgAOABwADQB0AG8AawBhAG4AbwAwADUAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvdG9rYW5vMDVhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3Rva2FubzA1YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Jennings09a,
	Author = {Jennings, D. E. and Flasar, F. M. and Kunde, V. G. and Samuelson, R. E. and Pearl, J. C. and Nixon, C. A. and Carlson, R. C. and Mamoutkine, A. A. and Brasunas, J. C. and Guandique, E. and others},
	Date-Added = {2010-07-07 04:01:22 -0700},
	Date-Modified = {2010-07-07 04:04:49 -0700},
	Journal = {Astrophys. J.},
	Pages = {L103--L105},
	Title = {Titan's surface brightness temperatures},
	Volume = {691},
	Year = {2009},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9qZW5uaW5nczA5YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAKkswyFms8AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyFoPYAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6amVubmluZ3MwOWEucGRmAA4AIAAPAGoAZQBuAG4AaQBuAGcAcwAwADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvamVubmluZ3MwOWEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvamVubmluZ3MwOWEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Hayes08a,
	Author = {Hayes, A. and Aharonson, O. and Callahan, P. and Elachi, C. and Gim, Y. and Kirk, R. and Lewis, K. and Lopes, R. and Lorenz, R. and Lunine, J. and others},
	Date-Added = {2010-07-07 03:44:38 -0700},
	Date-Modified = {2010-07-07 03:46:56 -0700},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2008GL033409},
	Pages = {L09204},
	Title = {Hydrocarbon lakes on {Titan}: Distribution and interaction with a porous regolith},
	Volume = {35},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxoYXllczA4YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAKkZKyFmo+gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyFoLagAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGF5ZXMwOGEucGRmAAAOABoADABoAGEAeQBlAHMAMAA4AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2hheWVzMDhhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9oYXllczA4YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Elachi05a,
	Author = {Elachi, C. and Wall, S. and Allison, M. and Anderson, Y. and Boehmer, R. and Callahan, P. and Encrenaz, P. and Flamini, E. and Franceschetti, G. and Gim, Y. and others},
	Date-Added = {2010-07-07 03:41:32 -0700},
	Date-Modified = {2010-07-07 03:43:08 -0700},
	Journal = {Science},
	Pages = {970--974},
	Title = {Cassini radar views the surface of {Titan}},
	Volume = {308},
	Year = {2005},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1lbGFjaGkwNWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAKkWOyFmoLwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyFoKnwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZWxhY2hpMDVhLnBkZgAOABwADQBlAGwAYQBjAGgAaQAwADUAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZWxhY2hpMDVhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2VsYWNoaTA1YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Lunine08a,
	Author = {J. I. Lunine and C. Elachi and S. D. Wall and M. A. Janssen and M. D. Allison and Y. Anderson and R. Boehmer and P. Callahan and P. Encrenaz and E. Flamini and G. Franceschetti and Y. Gim and G. Hamilton and S. Hensley and W. T. K. Johnson and K. Kelleher and R. L. Kirk and R. M. Lopes and R. Lorenz and D.O. Muhleman and R. Orosei and S.J. Ostro and F. Paganelli and P. Paillou and G. Picardi and F. Posa and J. Radebaugh and L. E. Roth and R. Seu and S. Shaffer and L. A. Soderblom and B. Stiles and E. R. Stofan and S. Vetrella and R. West and C. A. Wood and L. Wye and H. Zebker and G. Alberti and E. Karkoschka and B. Rizk and E. McFarlane and C. See and B. Kazeminejad},
	Date-Added = {2010-07-07 03:32:53 -0700},
	Date-Modified = {2010-07-07 03:37:01 -0700},
	Doi = {DOI: 10.1016/j.icarus.2007.12.022},
	Journal = {Icarus},
	Pages = {415--433},
	Title = {Titan's diverse landscapes as evidenced by {Cassini} {RADAR}'s third and fourth looks at {Titan}},
	Volume = {195},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1sdW5pbmUwOGEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAKii2yFmmfAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyFoI7AAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bHVuaW5lMDhhLnBkZgAOABwADQBsAHUAbgBpAG4AZQAwADgAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbHVuaW5lMDhhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2x1bmluZTA4YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/B6WGF-4RM1KY4-2/2/60dc6a26071d138a4b59304d0814ae06},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.icarus.2007.12.022}}

@article{Pauluis10a,
	Author = {O. Pauluis and A. Czaja and R. Korty},
	Date-Added = {2010-07-04 06:08:07 -0700},
	Date-Modified = {2010-07-04 06:12:07 -0700},
	Journal = {J. Climate},
	Pages = {3077--3093},
	Title = {The Global Atmospheric Circulation in Moist Isentropic Coordinates},
	Year = {2010},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5wYXVsdWlzMTBhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAJ2o8yFXVdQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyFY35QAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGF1bHVpczEwYS5wZGYAAA4AHgAOAHAAYQB1AGwAdQBpAHMAMQAwAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3BhdWx1aXMxMGEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3BhdWx1aXMxMGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Manabe69a,
	Author = {S. Manabe},
	Date-Added = {2010-06-30 10:54:29 -0700},
	Date-Modified = {2010-06-30 10:56:36 -0700},
	Journal = {Mon. Wea. Rev.},
	Pages = {739--773},
	Title = {Climate and the ocean circulation: {I. The} atmospheric circulation and the hydrology of the Earth's surface},
	Volume = {97},
	Year = {1969},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1tYW5hYmU2OWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIFxPmopwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxPoLFwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFuYWJlNjlhLnBkZgAOABwADQBtAGEAbgBhAGIAZQA2ADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbWFuYWJlNjlhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL21hbmFiZTY5YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Park10a,
	Author = {H.-S. Park and J. C. H. Chiang and S.-W. Son},
	Date-Added = {2010-06-25 10:30:24 -0700},
	Date-Modified = {2010-06-25 10:30:57 -0700},
	Journal = {J. Atmos. Sci.},
	Title = {The role of the {C}entral {A}sian mountains on the midwinter suppression of {N}orth {P}acific storminess},
	Year = {2010},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtwYXJrMTBhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAF3sRyEo1BAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEqXdAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGFyazEwYS5wZGYADgAYAAsAcABhAHIAawAxADAAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvcGFyazEwYS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9wYXJrMTBhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Boos10a,
	Author = {W. R. Boos and Z. Kuang},
	Date-Added = {2010-06-23 16:05:07 -0700},
	Date-Modified = {2010-06-23 16:07:24 -0700},
	Journal = {Nature},
	Pages = {218--222},
	Title = {Dominant control of the {S}outh {A}sian monsoon by orographic insulation versus plateau heating},
	Volume = {463},
	Year = {2010},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtib29zMTBhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzxx48VQAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx4+FwAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9vczEwYS5wZGYADgAYAAsAYgBvAG8AcwAxADAAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYm9vczEwYS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9ib29zMTBhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==},
	Bdsk-File-2 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtib29zMTBiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzyx5Wt9AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx5YedAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9vczEwYi5wZGYADgAYAAsAYgBvAG8AcwAxADAAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYm9vczEwYi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9ib29zMTBiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Dirmeyer98a,
	Author = {Dirmeyer, P. A.},
	Date-Added = {2010-06-23 00:56:33 -0700},
	Date-Modified = {2010-06-23 00:57:14 -0700},
	Journal = {J. Geophys. Res.},
	Pages = {11555--},
	Title = {Land-sea geometry and its effect on monsoon circulations},
	Volume = {103},
	Year = {1998},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9kaXJtZXllcjk4YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2WyEcM6AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEdvWAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGlybWV5ZXI5OGEucGRmAA4AIAAPAGQAaQByAG0AZQB5AGUAcgA5ADgAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZGlybWV5ZXI5OGEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZGlybWV5ZXI5OGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Clement04a,
	Author = {A. C. Clement and A. Hall and A. J. Broccoli},
	Date-Added = {2010-06-23 00:11:37 -0700},
	Date-Modified = {2010-06-23 00:12:49 -0700},
	Journal = {Climate Dyn.},
	Pages = {327--341},
	Title = {The importance of precessional signals in the tropical climate},
	Volume = {22},
	Year = {2004},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5jbGVtZW50MDRhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1exUCLuwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxUD8OwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2xlbWVudDA0YS5wZGYAAA4AHgAOAGMAbABlAG0AZQBuAHQAMAA0AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2NsZW1lbnQwNGEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2NsZW1lbnQwNGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@incollection{Bretherton07a,
	Address = {Princeton, NJ},
	Author = {C. S. Bretherton},
	Booktitle = {The Global Circulation of the Atmosphere},
	Date-Added = {2010-06-22 19:50:14 -0700},
	Date-Modified = {2010-06-22 19:51:30 -0700},
	Editor = {T. Schneider and A. H. Sobel},
	Pages = {302--330},
	Publisher = {Princeton University Press},
	Title = {Challenges in Numerical Modeling of Tropical Circulations},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXgAAAAAAXgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhFicmV0aGVydG9uMDdhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0HyEbEXgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEcmzgAAAAEADAAJDH4ACE6zAACS8wACADBNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnJldGhlcnRvbjA3YS5wZGYADgAkABEAYgByAGUAdABoAGUAcgB0AG8AbgAwADcAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACRVc2Vycy90YXBpby9QYXBlcnMvYnJldGhlcnRvbjA3YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHi4uLy4uL1BhcGVycy9icmV0aGVydG9uMDdhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIcAh4CIwIsAjcCOwJJAlACWQJ6An8CggKPApQAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACpg==}}

@article{Zhang06a,
	Author = {G. J. Zhang and H. Wang},
	Date-Added = {2010-06-22 19:01:12 -0700},
	Date-Modified = {2010-06-22 19:02:54 -0700},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2005GL025229},
	Pages = {L06709},
	Title = {Toward mitigating the double {ITCZ} problem in {NCAR} {CCSM3}},
	Volume = {33},
	Year = {2006},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx6aGFuZzA2YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRS9yEaxOQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEcTqQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6emhhbmcwNmEucGRmAAAOABoADAB6AGgAYQBuAGcAMAA2AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3poYW5nMDZhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy96aGFuZzA2YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Broccoli06a,
	Author = {Broccoli, A. J. and Dahl, K. A. and Stouffer, R. J.},
	Date-Added = {2010-06-22 16:05:27 -0700},
	Date-Modified = {2010-06-22 16:11:18 -0700},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2005GL024546},
	Pages = {L01702},
	Title = {Response of the {ITCZ} to {N}orthern {H}emisphere cooling},
	Volume = {33},
	Year = {2006},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9icm9jY29saTA2YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0KyEaQMQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEbyoQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnJvY2NvbGkwNmEucGRmAA4AIAAPAGIAcgBvAGMAYwBvAGwAaQAwADYAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvYnJvY2NvbGkwNmEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvYnJvY2NvbGkwNmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{kang08a,
	Author = {Kang, S. M. and Held, I. M. and Frierson, D. M. W. and Zhao, M.},
	Date-Added = {2010-06-22 13:32:20 -0700},
	Date-Modified = {2010-06-22 14:33:03 -0700},
	Journal = {J. Climate},
	Pages = {3521--3532},
	Title = {The response of the {ITCZ} to extratropical thermal forcing: {I}dealized slab-ocean experiments with a {GCM}},
	Volume = {21},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtrYW5nMDhhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFqxLyS8wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxLz1YwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2FuZzA4YS5wZGYADgAYAAsAawBhAG4AZwAwADgAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMva2FuZzA4YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9rYW5nMDhhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Delworth06a,
	Author = {Delworth, T. L. and Broccoli, A. J. and Rosati, A. and Stouffer, R. J. and Balaji, V. and Beesley, J. A. and Cooke, W. F. and Dixon, K. W. and Dunne, J. and Dunne, K. A. and Durachta, J. W. and Findell, K. L. and Ginoux, P. and Gnanadesikan, A. and Gordon, C. T. and Griffies, S. M. and others},
	Date-Added = {2010-06-22 13:08:14 -0700},
	Date-Modified = {2010-06-22 14:33:29 -0700},
	Journal = {J. Climate},
	Pages = {643--674},
	Title = {{GFDL}'s {CM2} global coupled climate models. {Part I}: {F}ormulation and simulation characteristics},
	Volume = {19},
	Year = {2006},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9kZWx3b3J0aDA2YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2EyDXFkAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDYoAAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGVsd29ydGgwNmEucGRmAA4AIAAPAGQAZQBsAHcAbwByAHQAaAAwADYAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZGVsd29ydGgwNmEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZGVsd29ydGgwNmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Boos08b,
	Author = {Boos, W. R. and Emanuel, K. A.},
	Date-Added = {2010-06-21 13:52:14 -0700},
	Date-Modified = {2010-06-21 13:53:38 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {3758--3778},
	Title = {Wind-evaporation feedback and the axisymmetric transition to angular momentum conserving {Hadley} flow},
	Volume = {65},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtib29zMDhiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzwxW1P3gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxW3AXgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9vczA4Yi5wZGYADgAYAAsAYgBvAG8AcwAwADgAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYm9vczA4Yi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9ib29zMDhiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Boos08a,
	Author = {Boos, W. R. and Emanuel, K. A.},
	Date-Added = {2010-06-21 13:49:29 -0700},
	Date-Modified = {2010-06-22 14:34:23 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {2194--2214},
	Title = {Wind-evaporation feedback and abrupt seasonal transitions of weak, axisymmetric {Hadley} circulations},
	Volume = {65},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtib29zMDhhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzvxKoP5AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxKpyVAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9vczA4YS5wZGYADgAYAAsAYgBvAG8AcwAwADgAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYm9vczA4YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9ib29zMDhhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Burns06a,
	Author = {Burns, S. P. and Sobel, A. H. and Polvani, L. M.},
	Date-Added = {2010-06-21 13:22:45 -0700},
	Date-Modified = {2010-06-21 13:23:49 -0700},
	Journal = {Theor. Comput. Fluid Dyn.},
	Number = {5},
	Pages = {443--467},
	Title = {Asymptotic solutions of the axisymmetric moist {Hadley} circulation in a model with two vertical modes},
	Volume = {20},
	Year = {2006},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxidXJuczA2YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0XyEUX4wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEV6UwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnVybnMwNmEucGRmAAAOABoADABiAHUAcgBuAHMAMAA2AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2J1cm5zMDZhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9idXJuczA2YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Xian08a,
	Author = {Xian, P. and Miller, R. L.},
	Date-Added = {2010-06-20 22:18:14 -0700},
	Date-Modified = {2010-06-22 14:34:05 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {1878--1895},
	Title = {Abrupt seasonal migration of the {ITCZ} into the summer hemisphere},
	Volume = {65},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt4aWFuMDhhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSXxHKxGlBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxHMTigAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eGlhbjA4YS5wZGYADgAYAAsAeABpAGEAbgAwADgAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMveGlhbjA4YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy94aWFuMDhhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Hourdin95a,
	Author = {Hourdin, F. and Talagrand, O. and Sadourny, R. and Courtin, R. and Gautier, D. and Mckay, C. P.},
	Date-Added = {2010-06-20 08:29:09 -0700},
	Date-Modified = {2010-06-20 08:29:49 -0700},
	Journal = {Icarus},
	Pages = {358--374},
	Title = {Numerical simulation of the general circulation of the atmosphere of Titan},
	Volume = {117},
	Year = {1995},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5ob3VyZGluOTVhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6ewYSX+VBERiAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwYUIeQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG91cmRpbjk1YS5wZGYAAA4AHgAOAGgAbwB1AHIAZABpAG4AOQA1AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2hvdXJkaW45NWEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2hvdXJkaW45NWEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Rannou02a,
	Author = {Rannou, P. and Hourdin, F. and McKay, C. P.},
	Date-Added = {2010-06-20 08:18:01 -0700},
	Date-Modified = {2010-06-20 08:20:32 -0700},
	Journal = {Nature},
	Pages = {853--856},
	Title = {A wind origin for {Titan}'s haze structure},
	Volume = {418},
	Year = {2002},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1yYW5ub3UwMmEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLVyEN/eAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEPh6AAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmFubm91MDJhLnBkZgAOABwADQByAGEAbgBuAG8AdQAwADIAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcmFubm91MDJhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3Jhbm5vdTAyYS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Rannou06a,
	Author = {Rannou, P. and Montmessin, F. and Hourdin, F. and Lebonnois, S.},
	Date-Added = {2010-06-20 08:15:49 -0700},
	Date-Modified = {2010-06-20 08:17:39 -0700},
	Journal = {Science},
	Pages = {201--205},
	Title = {The latitudinal distribution of clouds on {Titan}},
	Volume = {311},
	Year = {2006},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1yYW5ub3UwNmEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLWwNRH0wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwNSqQwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmFubm91MDZhLnBkZgAOABwADQByAGEAbgBuAG8AdQAwADYAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcmFubm91MDZhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3Jhbm5vdTA2YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=},
	Bdsk-File-2 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1yYW5ub3UwNmIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLXwNRH8wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwNSqYwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmFubm91MDZiLnBkZgAOABwADQByAGEAbgBuAG8AdQAwADYAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcmFubm91MDZiLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3Jhbm5vdTA2Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@book{ipcc07,
	Address = {Cambridge and New York},
	Date-Added = {2010-06-18 15:55:51 -0700},
	Date-Modified = {2010-06-18 15:59:13 -0700},
	Editor = {Solomon, S. and Qin, D. and Manning, M. and Chen, Z. and Marquis, M. and Averyt, K. B. and Tignor, M. and Miller, H. L.},
	Publisher = {Cambridge University Press},
	Title = {Climate Change 2007: {The} Physical Science Basis},
	Year = {2008}}

@article{Semtner76a,
	Author = {Semtner, A. J.},
	Date-Added = {2010-06-18 15:43:22 -0700},
	Date-Modified = {2010-06-18 16:01:19 -0700},
	Doi = {10.1175/1520-0485(1976)006<0379:AMFTTG>2.0.CO;2},
	Journal = {J. Phys. Oceanogr.},
	Pages = {379--389},
	Title = {A Model for the Thermodynamic Growth of Sea Ice in Numerical Investigations of Climate},
	Url = {http://journals.ametsoc.org/doi/abs/10.1175/1520-0485%281976%29006%3C0379%3AAMFTTG%3E2.0.CO%3B2},
	Volume = {6},
	Year = {1976},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zZW10bmVyNzZhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNcyEFDxAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEGmNAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2VtdG5lcjc2YS5wZGYAAA4AHgAOAHMAZQBtAHQAbgBlAHIANwA2AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3NlbXRuZXI3NmEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3NlbXRuZXI3NmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ},
	Bdsk-Url-1 = {http://dx.doi.org/10.1175/1520-0485(1976)006%3C0379:AMFTTG%3E2.0.CO;2}}

@article{Wang04a,
	Author = {Wang, X. and Auler, A. S. and Edwards, R. L. and Cheng, H. and Cristalli, P. S. and Smart, P. L. and Richards, D.A. and Shen, C.-C.},
	Date-Added = {2010-06-17 16:01:32 -0700},
	Date-Modified = {2010-06-17 16:03:49 -0700},
	Journal = {Nature},
	Pages = {740--743},
	Title = {Wet periods in northeastern {Brazil} over the past 210 kyr linked to distant climate anomalies},
	Volume = {432},
	Year = {2004},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt3YW5nMDRhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRcyD/3mwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEBaCwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2FuZzA0YS5wZGYADgAYAAsAdwBhAG4AZwAwADQAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvd2FuZzA0YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy93YW5nMDRhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@incollection{Koutavas04a,
	Author = {Koutavas, A. and Lynch-Stieglitz, J.},
	Booktitle = {The Hadley Circulation: Present, Past, and Future},
	Date-Added = {2010-06-17 15:44:32 -0700},
	Date-Modified = {2010-06-17 16:04:06 -0700},
	Editor = {Diaz, H. F and Bradley, R. S.},
	Pages = {347--369},
	Publisher = {Springer},
	Series = {Advances in Global Change Research},
	Title = {Variability of the marine {ITCZ} over the eastern {P}acific during the past 30,000 years: Regional perspective and global context},
	Volume = {21},
	Year = {2004}}

@article{Peterson00a,
	Author = {Peterson, L. C. and Haug, G. H. and Hughen, K. A. and Rohl, U.},
	Date-Added = {2010-06-17 13:54:33 -0700},
	Date-Modified = {2010-06-17 15:40:56 -0700},
	Journal = {Science},
	Pages = {1947--1951},
	Title = {Rapid changes in the hydrologic cycle of the tropical {A}tlantic during the last glacial},
	Volume = {290},
	Year = {2000},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9wZXRlcnNvbjAwYS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKfyD/yTwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEBUvwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGV0ZXJzb24wMGEucGRmAA4AIAAPAHAAZQB0AGUAcgBzAG8AbgAwADAAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvcGV0ZXJzb24wMGEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvcGV0ZXJzb24wMGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Porco05b,
	Author = {Porco, C. C. and Baker, E. and Barbara, J. and Beurle, K. and Brahic, A. and Burns, J. A. and Charnoz, S. and Cooper, N. and Dawson, D. D. and Del Genio, A. D. and others},
	Date-Added = {2010-06-14 14:17:07 -0700},
	Date-Modified = {2010-06-14 14:19:12 -0700},
	Journal = {Science},
	Pages = {1243--1247},
	Title = {Cassini imaging science: Initial results on {Saturn}'s atmosphere},
	Volume = {307},
	Year = {2005},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxwb3JjbzA1Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLHwst5ZwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsvb1wAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cG9yY28wNWIucGRmAAAOABoADABwAG8AcgBjAG8AMAA1AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3BvcmNvMDViLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9wb3JjbzA1Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Porco05a,
	Author = {Porco, C. C. and Baker, E. and Barbara, J. and Beurle, K. and Brahic, A. and Burns, J. A. and Charnoz, S. and Cooper, N. and Dawson, D. D. and Del Genio, A. D. and others},
	Date-Added = {2010-06-14 14:09:08 -0700},
	Date-Modified = {2010-06-14 14:13:56 -0700},
	Journal = {Nature},
	Number = {7030},
	Pages = {159--168},
	Title = {Imaging of {Titan} from the {Cassini} spacecraft},
	Volume = {434},
	Year = {2005},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxwb3JjbzA1YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLGyDvpRAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDxLtAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cG9yY28wNWEucGRmAAAOABoADABwAG8AcgBjAG8AMAA1AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3BvcmNvMDVhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9wb3JjbzA1YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{mitchell08a,
	Author = {Mitchell, J.L.},
	Date-Added = {2010-06-14 13:39:53 -0700},
	Date-Modified = {2010-06-14 13:49:32 -0700},
	Journal = {J. Geophys. Res},
	Pages = {E08015},
	Title = {The drying of {Titan}'s dunes: {Titan}'s methane hydrology and its impact on atmospheric circulation},
	Volume = {113},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9taXRjaGVsbDA4YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIyyDZ5pgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDbcFgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWl0Y2hlbGwwOGEucGRmAA4AIAAPAG0AaQB0AGMAaABlAGwAbAAwADgAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbWl0Y2hlbGwwOGEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbWl0Y2hlbGwwOGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Mitchell09a,
	Author = {J. L. Mitchell and R. T. Pierrehumbert and D. M. W. Frierson and R. Caballero},
	Date-Added = {2010-06-14 12:05:23 -0700},
	Date-Modified = {2010-06-14 12:07:32 -0700},
	Doi = {10.1016/j.icarus.2009.03.043},
	Issn = {00191035},
	Journal = {Icarus},
	Pages = {250--264},
	Title = {The impact of methane thermodynamics on seasonal convection and circulation in a model {Titan} atmosphere},
	Volume = {203},
	Year = {2009},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9taXRjaGVsbDA5YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIzx/25MwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx/4bowAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWl0Y2hlbGwwOWEucGRmAA4AIAAPAG0AaQB0AGMAaABlAGwAbAAwADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbWl0Y2hlbGwwOWEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbWl0Y2hlbGwwOWEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc},
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.icarus.2009.03.043}}

@article{Barnes09,
	Abstract = {We analyze observations of Titan's south polar lake Ontario Lacus obtained by Cassini's Visual and Infrared Mapping Spectrometer during the 38th flyby of Titan (T38; 2007 December 5). These near-closest-approach observations have the highest signal-to-noise, the finest spatial resolution, and the least atmospheric influence of any near-infrared lake observation to date. We use the large, spatially flat, and low-albedo interior of Ontario Lacus as a calibration target allowing us to derive an analytical atmospheric correction for emission angle. The dark lake interior is surrounded by two separate annuli that follow the lake interior's contours. The inner annulus is uniformly dark, but not so much as the interior lake, and is generally 5--10 kilometers wide at the lake's southeastern margin. We propose that it represents wet lakebed sediments exposed by either tidal sloshing of the lake or seasonal methane loss leading to lower lake-volume. The exterior annulus is bright and shows a spectrum consistent with a relatively low water-ice content relative to the rest of Titan. It may represent fine-grained condensate deposits from a past era of higher lake level. Together, the annuli seem to indicate that the lake level for Ontario Lacus has changed over time. This hypothesis can be tested with observations scheduled for future Titan flybys.
},
	Author = {Barnes, J. W. and Brown, R. H. and Soderblom, J. M. and Soderblom, L. A. and Jaumann, R. and Jackson, B. and Le Mou{\'e}lic, S. and Sotin, C. and Buratti, B. J. and Pitman, K. M. and Baines, K. H. and Clark, R. N. and Nicholson, P. D. and Turtle, E. P. and Perry, J.},
	Date-Modified = {2010-06-13 22:12:20 -0700},
	Journal = {Icarus},
	Pages = {217--225},
	Title = {Shoreline features of {Titan}'s {O}ntario {L}acus from {Cassini}/{VIMS} observations},
	Url = {http://www.sciencedirect.com/science/article/B6WGF-4V9S471-4/2/a9a172414a8e47ddb761dbf00e6ddc8c},
	Volume = {201},
	Year = {2009},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1iYXJuZXMwOWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQy6yDsIVwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDtqxwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmFybmVzMDlhLnBkZgAOABwADQBiAGEAcgBuAGUAcwAwADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvYmFybmVzMDlhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2Jhcm5lczA5YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/B6WGF-4V9S471-4/2/a9a172414a8e47ddb761dbf00e6ddc8c}}

@artice{Barnes08,
	Author = {Barnes, J. W. and Brown, R. H. and Soderblom, L. and Sotin, C. and Le Mou{\'e}lic, S. and Rodriguez, S. and Jaumann, R. and Beyer, R. A. and Buratti, B. J. and Pitman, K. and Baines, K. H. and Clark, R. and Nicholson, P.},
	Journal = {Icarus},
	Pages = {400--414},
	Title = {Spectroscopy, morphometry, and photoclinometry of {Titan}'s dunefields from {Cassini}/{VIMS}},
	Url = {http://www.sciencedirect.com/science/article/B6WGF-4RH380F-2/2/9ab3fc3eebb61da51a8a900f61a5033c},
	Volume = {195},
	Year = {2008},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/B6WGF-4RH380F-2/2/9ab3fc3eebb61da51a8a900f61a5033c}}

@article{Bird05,
	Author = {Bird, M. K. and Allison, M. and Asmar, S. W. and Atkinson, D. H. and Avruch, I. M. and Dutta-Roy, R. and Dzierma, Y. and Edenhofer, P. and Folkner, W. M. and Gurvits, L. I. and Johnston, D. V. and Plettemeier, D. and Pogrebenko, S. V. and Preston, R. A. and Tyler, G. L.},
	Comment = {10.1038/nature04060},
	Journal = {Nature},
	Pages = {800--802},
	Title = {The vertical profile of winds on {Titan}},
	Url = {http://dx.doi.org/10.1038/nature04060},
	Volume = {438},
	Year = {2005},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature04060}}

@article{Brown02,
	Author = {Brown, M. E. and Bouchez, A. H. and Griffith, C. A.},
	Comment = {10.1038/nature01302},
	Journal = {Nature},
	Pages = {795--797},
	Title = {Direct detection of variable tropospheric clouds near {Titan}'s south pole},
	Url = {http://dx.doi.org/10.1038/nature01302},
	Volume = {420},
	Year = {2002},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxicm93bjAyYS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0OyDsI5AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDtrVAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnJvd24wMmEucGRmAAAOABoADABiAHIAbwB3AG4AMAAyAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2Jyb3duMDJhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9icm93bjAyYS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature01302}}

@article{Brown10a,
	Abstract = {We use data from the VIMS instrument on board the Cassini spacecraft to construct high sensitivity and high spatial-resolution maps of the locations of tropospheric clouds on Titan in the late northern winter season during which the Cassini prime mission took place. These observations show that, in this season, clouds on Titan are strongly hemispherically asymmetric. Mid-latitude clouds, in particular, occur only in the southern hemisphere and have not ever been observed in the north. Such an asymmetry is in general agreement with circulation models where sub-solar surface heating controls the locations of clouds and appears in conflict with models where perennial polar hazes prevent significant summertime polar heating from affecting the circulation. The southern mid-latitude clouds appear to be distributed uniformly in longitude, in contrast to some previous observations. Southern high-latitude clouds exhibit a significant concentration, however, between about 180$\,^{\circ}$ and 270$\,^{\circ}$E longitude. A spatially and temporally uniform cloud always appears northward of 50$\,^{\circ}$N latitude. This cloud appears unchanged over the course of the observations, consistent with the interpretation that it is caused by continuous ethane condensation as air subsides and radiatively cools through the tropopause. The location of this cloud likely provides a direct tracer of elements of north polar atmospheric circulation, potentially allowing continuous monitoring of circulation changes as Titan passes through equinox into north polar spring and summer. We show that a similar analysis of this dataset by Rodriguez et al. (2009) contains substantial errors and should not be used.},
	Author = {Brown, M. E. and Roberts, J. E. and Schaller, E. L.},
	Date-Modified = {2010-06-13 22:06:49 -0700},
	Journal = {Icarus},
	Pages = {571--580},
	Title = {Clouds on {Titan} during the {Cassini} prime mission: A complete analysis of the {VIMS} data},
	Url = {http://www.sciencedirect.com/science/article/B6WGF-4X5JSVF-1/2/81c34c45a663b43c80558506173e1da7},
	Volume = {205},
	Year = {2010},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxicm93bjEwYS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0RyDsGuAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDtpKAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnJvd24xMGEucGRmAAAOABoADABiAHIAbwB3AG4AMQAwAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2Jyb3duMTBhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9icm93bjEwYS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/B6WGF-4X5JSVF-1/2/81c34c45a663b43c80558506173e1da7}}

@article{Brown09a,
	Abstract = {Images from instruments on Cassini as well as from
                  telescopes on the ground reveal the presence of
                  sporadic small-scale cloud activity in the cold
                  late-winter north polar region of Saturn's large
                  moon Titan. These clouds lie underneath the
                  previously discovered uniform polar cloud attributed
                  to a quiescent ethane cloud at {\^a}¼40 km and
                  appear confined to the same latitudes as those of
                  the largest known hydrocarbon lakes at the north
                  pole of Titan. The physical properties of these
                  clouds suggest that they are due to methane
                  convection and condensation. Such convection could
                  be caused by a process in some ways analogous to
                  terrestrial lake-effect clouds. The lakes on Titan
                  could be a key connection between the surface and
                  the meteorological cycle.},
	Author = {Brown, M. E. and Schaller, E. L. and Roe, H. G. and Chen, C. and Roberts, J. and Brown, R. H. and Baines, K. H. and Clark, R. N.},
	Date-Modified = {2010-06-13 22:10:13 -0700},
	Journal = {Geophys. Res. Lett.},
	Pages = {L01103},
	Title = {Discovery of lake-effect clouds on {Titan}},
	Url = {http://dx.doi.org/10.1029/2008GL035964},
	Volume = {36},
	Year = {2009},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxicm93bjA5YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0PyDsHrwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDtqHwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnJvd24wOWEucGRmAAAOABoADABiAHIAbwB3AG4AMAA5AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2Jyb3duMDlhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9icm93bjA5YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=},
	Bdsk-Url-1 = {http://dx.doi.org/10.1029/2008GL035964}}

@article{Brown08,
	Author = {Brown, R. H. and Soderblom, L. A. and Soderblom, J. M. and Clark, R. N. and Jaumann, R. and Barnes, J. W. and Sotin, C. and Buratti, B. and Baines, K. H. and Nicholson, P. D.},
	Comment = {10.1038/nature07100},
	Journal = {Nature},
	Pages = {607--610},
	Title = {The identification of liquid ethane in {Titan}'s {O}ntario {L}acus},
	Url = {http://dx.doi.org/10.1038/nature07100},
	Volume = {454},
	Year = {2008},
	Bdsk-Url-1 = {http://dx.doi.org/10.1038/nature07100}}

@article{Teixeira08d,
	Author = {J. Teixeira and P. May and M. Flatau and T. F. Hogan},
	Date-Added = {2010-06-13 14:31:11 -0700},
	Date-Modified = {2010-06-13 14:33:53 -0700},
	Journal = {J. Marine Sys.},
	Pages = {29--36},
	Title = {{SST} sensitivity of a global ocean-atmosphere coupled system to the parameterization of boundary layer clouds},
	Volume = {69},
	Year = {2008}}

@book{Stull88,
	Author = {R. B. Stull},
	Date-Added = {2010-06-13 14:14:42 -0700},
	Date-Modified = {2010-06-13 14:17:48 -0700},
	Pages = {666},
	Publisher = {Springer},
	Title = {An Introduction to Boundary Layer Meteorology},
	Year = {1988}}

@article{Teixeira08c,
	Author = {J. Teixeira and C. A. Reynolds},
	Date-Added = {2010-06-13 14:02:31 -0700},
	Date-Modified = {2010-06-13 14:04:20 -0700},
	Journal = {Mon. Wea. Rev.},
	Pages = {483--496},
	Title = {Stochastic Nature of Physical Parameterizations in Ensemble Prediction: A Stochastic Convection Approach},
	Volume = {136},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg90ZWl4ZWlyYTA4Yy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRP5yDZmmQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDbJCQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGVpeGVpcmEwOGMucGRmAA4AIAAPAHQAZQBpAHgAZQBpAHIAYQAwADgAYwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdGVpeGVpcmEwOGMucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdGVpeGVpcmEwOGMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Teixeira08b,
	Author = {J. Teixeira and Y-J. Kim},
	Date-Added = {2010-06-13 14:00:44 -0700},
	Date-Modified = {2010-06-13 14:01:55 -0700},
	Journal = {Asia-Pacific J. Atmos. Sci.},
	Pages = {191--199},
	Title = {On a simple parameterization of convective cloud fraction},
	Volume = {44},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg90ZWl4ZWlyYTA4Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRP4x1uS+gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx1wDegAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGVpeGVpcmEwOGIucGRmAA4AIAAPAHQAZQBpAHgAZQBpAHIAYQAwADgAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdGVpeGVpcmEwOGIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdGVpeGVpcmEwOGIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Teixeira08a,
	Author = {Teixeira, J. and B. Stevens and C. S. Bretherton and R. Cederwall and J. D. Doyle and J. C. Golaz and A. A. M. Holtslag and S. A. Klein and J. K. Lundquist and D. A. Randall and A. P. Siebesma and P. M. M. Soares},
	Date-Added = {2010-06-13 13:50:39 -0700},
	Date-Modified = {2010-06-13 13:58:37 -0700},
	Journal = {Bull. Am. Meteor. Soc.},
	Pages = {453--458},
	Title = {Parameterization of the Atmospheric Boundary Layer: A View from Just Above the Inversion},
	Volume = {89},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg90ZWl4ZWlyYTA4YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRP3yDqUNgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDr2pgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGVpeGVpcmEwOGEucGRmAA4AIAAPAHQAZQBpAHgAZQBpAHIAYQAwADgAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdGVpeGVpcmEwOGEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdGVpeGVpcmEwOGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Kohler05a,
	Author = {M. K{\"o}hler},
	Date-Added = {2010-06-12 09:22:56 -0700},
	Date-Modified = {2010-06-12 09:25:31 -0700},
	Journal = {ECMWF Newsletter},
	Pages = {18--22},
	Title = {Improved prediction of boundary layer clouds},
	Volume = {104},
	Year = {2005},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWwAAAAAAWwAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1rmmhsZXIwNWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGXyDkOWwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDlwywAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a5pobGVyMDVhLnBkZgAOAB4ADgBrAG8DCABoAGwAZQByADAANQBhAC4AcABkAGYADwAYAAsATQBhAGMAQgBvAG8AawAgAFAAcgBvABIAIlVzZXJzL3RhcGlvL1BhcGVycy9rb8yIaGxlcjA1YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdG8QGwAuAC4ALwAuAC4ALwBQAGEAcABlAHIAcwAvAGsAbwMIAGgAbABlAHIAMAA1AGEALgBwAGQAZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIQAhICFwIgAisCLwI9AkQCTQKGAosCjgKbAqAAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACsg==}}

@article{Lunine09a,
	Author = {J. I. Lunine and R. D. Lorenz},
	Date-Added = {2010-06-11 15:52:48 -0700},
	Date-Modified = {2010-06-11 15:54:48 -0700},
	Journal = {Ann. Rev. Earth Planet Sci.},
	Pages = {299--320},
	Title = {Rivers, Lakes, Dunes, and Rain: Crustal Processes in Titan's Methane Cycle g Rivers, Lakes, Dunes, and Rain: Crustal Processes in Titan's Methane Cycle g Rivers, Lakes, Dunes, and Rain: Crustal Processes in Titan's Methane Cycle g Rivers, Lakes, Dunes, and Rain: Crustal Processes in Titan's Methane Cycle g Rivers, Lakes, Dunes, and Rain: Crustal Processes in Titan's Methane Cycle},
	Volume = {37},
	Year = {2009},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1sdW5pbmUwOWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRH2yDaT8gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDb2YgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bHVuaW5lMDlhLnBkZgAOABwADQBsAHUAbgBpAG4AZQAwADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbHVuaW5lMDlhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2x1bmluZTA5YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Abramov03,
	Annote = {Filed under Majda. Conservation of third moment of
                  quasigeostrophic pv relevant for statistical mechanics.},
	Author = {R. V. Abramov and A. J Majda},
	Journal = {Proc. Nat. Acad. Sci.},
	Pages = {3841--3846},
	Title = {Statistically relevant conserved quantities for truncated quasigeostrophic flow},
	Volume = 100,
	Year = 2003}

@article{Achterberg94,
	Annote = {Filed under Ingersoll.},
	Author = {R. K. Achterberg and A. P. Ingersoll},
	Journal = {J. Atmos. Sci.},
	Pages = {541--562},
	Title = {Numerical Simulation of Baroclinic Jovian Vortices},
	Volume = 51,
	Year = 1994}

@article{Adkins01,
	Author = {J. F. Adkins and D. P. Schrag},
	Journal = {Geophys. Res. Lett.},
	Pages = {771--774},
	Title = {Pore fluid constraints on deep ocean temperature and salinity during the last glacial maximum},
	Volume = 28,
	Year = 2001}

@article{Adkins02,
	Author = {J. F. Adkins and K. McIntyre and D. P. Schrag},
	File = {../../Papers/adkins02.pdf},
	Journal = {Science},
	Pages = {1769--1773},
	Title = {The salinity, temperature, and $\delta^{18}\mathrm{O}$ of the glacial deep ocean},
	Volume = 298,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxhZGtpbnMwMi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyIvodu9AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvofRZAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YWRraW5zMDIucGRmAAAOABoADABhAGQAawBpAG4AcwAwADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2Fka2luczAyLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9hZGtpbnMwMi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Adkins97,
	Author = {J. F. Adkins and E. A. Boyle and L. Keigwin and E. Cortijo},
	Journal = {Nature},
	Pages = {154--156},
	Title = {Variability of the {N}orth {A}tlantic Thermohaline circulation during the last interglacial period},
	Volume = 390,
	Year = 1997}

@article{Adkins98,
	Author = {J. F. Adkins and H. Cheng and E. A. Boyle and E. R. M. Druffel and R. L. Edwards},
	Journal = {Science},
	Pages = {725--728},
	Title = {Deep-Sea Coral Evidence for Rapid Change in Ventilation of the Deep North Atlantic 15,400 Years Ago},
	Volume = 280,
	Year = 1998}

@article{Adler08,
	Author = {Adler, R. F. and Gu, G. and Wang, J. J. and Huffman, G. J. and Curtis, S. and Bolvin, D.},
	File = {../../Papers/adler08.pdf},
	Journal = {J. Geophys. Res},
	Note = {doi:10.1029/2008JD010536},
	Pages = {D22104},
	Title = {Relationships between global precipitation and surface temperature on interannual and longer timescales (1979--2006)},
	Volume = {113},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgthZGxlcjA4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyLxec2aAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxeeY2AAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YWRsZXIwOC5wZGYADgAYAAsAYQBkAGwAZQByADAAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYWRsZXIwOC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9hZGxlcjA4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Aharonson09,
	Author = {O. Aharonson and A. G. Hayes and J. I. Lunine and R. D. Lorenz and M. D. Allison and C. Elachi},
	File = {../../Papers/aharonson09.pdf},
	Journal = {Nat. Geosci.},
	Note = {Submitted},
	Pages = {??},
	Title = {Titan's Asymmetric Lake Distribution and its Astronomical Evolution},
	Volume = {??},
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9haGFyb25zb24wOS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyNxzmcsQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxzoNMQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YWhhcm9uc29uMDkucGRmAA4AIAAPAGEAaABhAHIAbwBuAHMAbwBuADAAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvYWhhcm9uc29uMDkucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvYWhhcm9uc29uMDkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Ahmad76,
	Annote = {Filed under Entropy Estimation.},
	Author = {I. A. Ahmad and P.-E. Lin},
	Journal = {IEEE Trans. Inf. Theory},
	Pages = {372--375},
	Title = {A Nonparametric Estimation of the Entropy for Absolutely Continuous Distributions},
	Volume = 22,
	Year = 1976}

@article{Akaike71,
	Annote = {Multivariate final prediction error.},
	Author = {H. Akaike},
	Journal = {Ann. Inst. Statist. Math.},
	Pages = {163--180},
	Title = {Autoregressive Model Fitting for Control},
	Volume = 23,
	Year = 1971}

@article{Alexeev99,
	Annote = {Not on file. Follow-up on Bates99.},
	Author = {V. A. Alexeev and J. R. Bates},
	Journal = {Tellus},
	Pages = {630--651},
	Title = {{GCM} experiments to test a proposed dynamical stabilizing mechanism in the climate system},
	Volume = {51A},
	Year = 1999}

@article{Allan07,
	Author = {R. P. Allan and B. J. Soden},
	File = {../../Papers/allan07.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2007GL031460},
	Pages = {L18705},
	Title = {Large discrepancy between observed and simulated precipitation trends in the ascending and descending branches of the tropical circulation},
	Volume = 34,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgthbGxhbjA3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyPwyhrs1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwyjOIwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YWxsYW4wNy5wZGYADgAYAAsAYQBsAGwAYQBuADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYWxsYW4wNy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9hbGxhbjA3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Allen01,
	Annote = {Filed under Nakamura.},
	Author = {D. R. Allen and N. Nakamura},
	Journal = {J. Geophys. Res.},
	Pages = {7917--7935},
	Title = {A seasonal climatology of effective diffusivity in the stratosphere},
	Volume = {106D},
	Year = 2001}

@article{Allen02,
	Author = {M. R. Allen and W. J. Ingram},
	File = {../../Papers/allen02.pdf},
	Journal = {Nature},
	Pages = {224--232},
	Title = {Constraints on future changes in climate and the hydrologic cycle},
	Volume = 419,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgthbGxlbjAyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyRwp68dgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwp8e5gAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YWxsZW4wMi5wZGYADgAYAAsAYQBsAGwAZQBuADAAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYWxsZW4wMi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9hbGxlbjAyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Allen97,
	Annote = {Filed under Smith.},
	Author = {M. R. Allen and L. A. Smith},
	Journal = {Phys. Lett. A},
	Pages = {419--428},
	Title = {Optimal Filtering in Singular Spectrum Analysis},
	Volume = 234,
	Year = 1997}

@article{Allen99,
	Annote = {Filed under Climate Change Detection. Shows
                  explicitly how fingerprinting can be viewed as
                  regression analysis. Reviews concepts from
                  regression analysis. Shows how consistency of
                  regression model with both simulated and observed
                  data can be checked.},
	Author = {M. R. Allen and S. F. B. Tett},
	Journal = {Climate Dyn.},
	Pages = {419--434},
	Title = {Checking for model consistency in optimal fingerprinting},
	Volume = 15,
	Year = 1999}

@article{Alley03,
	Annote = {Filed under Paleo-Climate Reviews.},
	Author = {R. B. Alley and J. Marotzke and W. D. Nordhaus and J. T. Overpeck and D. M. Peteet and R. A. Pielke Jr. and R. T. Pierrehumbert and P. B. Rhines and T. F. Stocker and L. D. Talley and J. M. Wallace},
	Journal = {Science},
	Pages = {2005--2010},
	Title = {Abrupt Climate Change},
	Volume = 299,
	Year = 2003}

@article{Allison00,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {M. Allison},
	File = {../../Papers/allison00.pdf},
	Journal = {Planet. Space. Sci.},
	Pages = {753--774},
	Title = {A similarity model for the windy jovian thermocline},
	Volume = 48,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1hbGxpc29uMDAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyTvRQuSQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRSQuQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YWxsaXNvbjAwLnBkZgAOABwADQBhAGwAbABpAHMAbwBuADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvYWxsaXNvbjAwLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2FsbGlzb24wMC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Allison90,
	Author = {M. Allison and D. A. Godfrey and R. F. Beebe},
	File = {../../Papers/allison90.pdf},
	Journal = {Science},
	Pages = {1061--1063},
	Title = {A wave dynamical interpretation of {Saturn's} polar hexagon},
	Volume = {247},
	Year = {1990},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1hbGxpc29uOTAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyUxzVLFwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxzW7lwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YWxsaXNvbjkwLnBkZgAOABwADQBhAGwAbABpAHMAbwBuADkAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvYWxsaXNvbjkwLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2FsbGlzb245MC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Allison94,
	Author = {M. Allison and A. D. DelGenio and W. Zhou},
	Journal = {J. Atmos. Sci.},
	Pages = {694--702},
	Title = {Zero Potential Vorticity Envelopes for the Zonal-Mean Velocity of the Venus/Titan Atmospheres},
	Volume = 51,
	Year = 1994}

@article{Ambaum02,
	Annote = {Filed under Hoskins.},
	Author = {M. H. P. Ambaum and B. J. Hoskins},
	Journal = {J. Climate},
	Pages = {1969--1978},
	Title = {The {NAO} Troposphere-Stratosphere Connection},
	Volume = 15,
	Year = 2002}

@article{Ambrizzi97,
	Author = {T. Ambrizzi and B. J. Hoskins},
	File = {../../Papers/ambrizzi97.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {919--928},
	Title = {Stationary {Rossby} wave propagation in a baroclinic atmosphere},
	Volume = 123,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5hbWJyaXp6aTk3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyYwO0FggAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwO1n8gAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YW1icml6emk5Ny5wZGYAAA4AHgAOAGEAbQBiAHIAaQB6AHoAaQA5ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2FtYnJpenppOTcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2FtYnJpenppOTcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@book{Ames77,
	Address = {San Diego},
	Author = {W. F. Ames},
	Edition = {2nd},
	Publisher = {Academic Press},
	Title = {Numerical Methods for Partial Differential Equations},
	Year = 1977}

@article{Anderson01,
	Annote = {Filed under Data Assimilation.},
	Author = {J. L. Anderson},
	Journal = {Mon. Wea. Rev.},
	Note = {submitted},
	Pages = {??},
	Title = {An Ensemble Adjustment Filter for Data Assimilation},
	Volume = {??},
	Year = 2001}

@article{Anderson03,
	Annote = {Filed under GFDL Climate Model.},
	Author = {J. L. Anderson and Collaborators},
	Journal = {J. Climate},
	Pages = {????-????},
	Title = {The new {GFDL} Global Atmosphere and Land Model {AM2/LM2}: Evaluation with prescribed {SST} Simulations},
	Volume = 16,
	Year = 2003}

@book{Anderson84,
	Address = {New York},
	Author = {T. W. Anderson},
	Edition = {2nd},
	File = {../../Papers/anderson84.pdf},
	Pages = 675,
	Publisher = {Wiley},
	Series = {Series in Probability and Mathematical Statistics},
	Title = {An Introduction to Multivariate Statistical Analysis},
	Year = 1984,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5hbmRlcnNvbjg0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyZwI4u7AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwI6RXAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YW5kZXJzb244NC5wZGYAAA4AHgAOAGEAbgBkAGUAcgBzAG8AbgA4ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2FuZGVyc29uODQucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2FuZGVyc29uODQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Anderson91,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {J. G. Anderson and D. W. Toohey and W. H. Brune},
	Journal = {Science},
	Pages = {39--46},
	Title = {Free Radicals Within the {A}ntarctic Vortex: The Role of {CFCs} in {A}ntarctic Ozone Loss},
	Volume = 251,
	Year = 1991}

@article{Anderson92,
	Author = {D. L. T. Anderson and J. Willebrandt},
	Journal = {Rep. Prog. Phys.},
	Pages = {1--37},
	Title = {Recent Advances in Modelling the Ocean Circulation and its Effects on Climate},
	Volume = 55,
	Year = 1992}

@article{Anderson96,
	Annote = {Filed under Data Assimilation.},
	Author = {D. L. T. Anderson and J. Sheinbaum and K. Haines},
	Journal = {Rep. Prog. Phys.},
	Pages = {1209--1266},
	Title = {Data assimilation in ocean models},
	Year = 1996}

@article{Anderson96a,
	Annote = {Filed under Predictability. Compares various methods
                  (SVD, breeding, normal modes) for initialization in
                  3-variable Lorenz model.},
	Author = {J. L. Anderson},
	Journal = {J. Atmos. Sci.},
	Pages = {22--36},
	Title = {Selection of Initial Conditions for Ensemble Forecasts in a Simple Perfect Model Framework},
	Volume = {53},
	Year = {1996}}

@article{Anderson96b,
	Annote = {Filed under Predictability. Assesses usefulness of
                  ensemble forecasts; not distribution based;
                  essentially tests whether the distribution of the
                  prediction error is significantly different from the
                  climatological distribution or not.},
	Author = {J. L. Anderson and W. F. Stern},
	Journal = {J. Climate},
	Pages = {260--269},
	Title = {Evaluating the Potential Predictive Utility of Ensemble Forecasts},
	Volume = 9,
	Year = 1996}

@article{Anderson96c,
	Annote = {Filed under Predictability.},
	Author = {J. L. Anderson},
	Journal = {J. Climate},
	Pages = {1518--1530},
	Title = {A Method for Producing and Evaluating Probabilistic Forecasts from Ensemble Model Integrations},
	Volume = 9,
	Year = 1996}

@article{Anderssen81,
	Annote = {Not on file. Comparison of regularization methods by
                  characterization in terms of Fourier analysis.},
	Author = {R. S. Anderssen and P. M. Prenter},
	Journal = {J. Austral. Math. Soc. B},
	Pages = {488-500},
	Title = {A formal comparison of methods proposed for the numerical solution of first kind integral equations},
	Volume = 22,
	Year = 1981}

@article{Andersson05,
	Author = {Andersson, E. and Bauer, P. and Beljaars, A. and Chevallier, F. and H{\'o}lm, E. and Janiskov{\'a}, M. and K{\aa}llberg, P. and Kelly, G. and Lopez, P. and Mcnally, A. and others},
	File = {../../Papers/andersson05.pdf},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {387--402},
	Title = {Assimilation and Modeling of the Atmospheric Hydrological Cycle in the {ECMWF} Forecasting System},
	Volume = {86},
	Year = {2005},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9hbmRlcnNzb24wNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQybxRjhqAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxRlEGAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YW5kZXJzc29uMDUucGRmAA4AIAAPAGEAbgBkAGUAcgBzAHMAbwBuADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvYW5kZXJzc29uMDUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvYW5kZXJzc29uMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Andersson07,
	Author = {E. Andersson and E. H{\'o}lm and P. Bauer and A. Beljaars and G. A. Kelly and A. P. McNally and A. J. Simmons and J.-N. Th{\'e}paut and A. M. Tompkins},
	File = {../../Papers/andersson07.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1473--1485},
	Title = {Analysis and forecast impact of the main humidity observing systems},
	Volume = 133,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9hbmRlcnNzb24wNy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQycxRjkHQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxRlGjQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YW5kZXJzc29uMDcucGRmAA4AIAAPAGEAbgBkAGUAcgBzAHMAbwBuADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvYW5kZXJzc29uMDcucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvYW5kZXJzc29uMDcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Andrews01,
	Annote = {Not on file.},
	Author = {A. E. Andrews and K. A. Boering and B. C. Daube and S. C. Wofsy and M. Loewenstein and H. Jost and J. R. Podolske and C. R. Webster and R. L. Herman and D. C. Scott and G. J. Flesch and E. J. Moyer and J. W. Elkins and G. S. Dutton and D. F. Hurst and F. L. Moore and E. A. Ray and P. A. Romashkin and S. E. Strahan},
	Journal = {J. Geophys. Res.},
	Pages = {32295--32314},
	Title = {Mean ages of stratospheric air derived from in situ observations of $\mathrm{CO}_2$, $\mathrm{CH_4}$ and $\mathrm{N_2O}$},
	Volume = {106D},
	Year = 2001}

@article{Andrews76,
	Annote = {Transformed Eulerian mean, residual circulation.},
	Author = {D. G. Andrews and M. E. McIntyre},
	Journal = {J. Atmos. Sci.},
	Pages = {2031--2048},
	Title = {Planetary Waves in Horizontal and Vertical Shear: The Generalized {E}liassen-{P}alm Relation and the Mean Zonal Acceleration},
	Volume = 33,
	Year = 1976}

@article{Andrews78a,
	Annote = {EP Theorems in arbitrary coordinate systems},
	Author = {D. G. Andrews and M. E. McIntyre},
	File = {../../Papers/andrews78a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {175--185},
	Title = {Generalized {E}liassen-{P}alm and {C}harney-{D}razin Theorems for Waves on Axisymmetric Mean Flows in Compressible Atmospheres},
	Volume = 35,
	Year = 1978,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5hbmRyZXdzNzhhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQygxGc9p1BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxGegFwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YW5kcmV3czc4YS5wZGYAAA4AHgAOAGEAbgBkAHIAZQB3AHMANwA4AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2FuZHJld3M3OGEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2FuZHJld3M3OGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Andrews78c,
	Annote = {Generalized Lagrangian Mean.},
	Author = {D. G. Andrews and M. E. McIntyre},
	File = {../../Papers/andrews78c.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {609--646},
	Title = {An exact theory of nonlinear waves on a {L}agrangian-mean flow},
	Volume = 89,
	Year = 1978,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5hbmRyZXdzNzhjLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyixGeO4VBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxGfxUQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YW5kcmV3czc4Yy5wZGYAAA4AHgAOAGEAbgBkAHIAZQB3AHMANwA4AGMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2FuZHJld3M3OGMucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2FuZHJld3M3OGMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Andrews83,
	Annote = {EP flux for primitive equations in isentropic
                  coordinates.},
	Author = {D. G. Andrews},
	File = {../../Papers/andrews83.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1877--1883},
	Title = {A Finite-Amplitude {E}liassen-{P}alm Theorem in Isentropic Coordinates},
	Volume = 40,
	Year = 1983,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1hbmRyZXdzODMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyjvt8wPgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvt+SrgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YW5kcmV3czgzLnBkZgAOABwADQBhAG4AZAByAGUAdwBzADgAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvYW5kcmV3czgzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2FuZHJld3M4My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@incollection{Andrews85,
	Author = {D. G. Andrews},
	Booktitle = {Advances in Geophysics},
	Editor = {S. Manabe},
	Pages = {249--275},
	Publisher = {Academic Press},
	Title = {Wave--Mean--Flow Interaction in the Middle Atmosphere},
	Volume = {28A},
	Year = 1985}

@article{Andrews87a,
	Annote = {EP flux for primitive equations in log-pressure
                  coordinates.},
	Author = {D. G. Andrews},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {323--338},
	Title = {On the Interpretation of the {E}liassen-{P}alm flux divergence},
	Volume = 113,
	Year = 1987}

@book{Andrews87b,
	Author = {D. G. Andrews and J. R. Holton and C. B. Leovy},
	Pages = 489,
	Publisher = {Academic Press},
	Series = {International Geophysics Series},
	Title = {Middle Atmosphere Dynamics},
	Volume = 40,
	Year = 1987}

@article{Ansley83,
	Annote = {Not on file.},
	Author = {C. F. Ansley and R. Kohn},
	Journal = {Biometrika},
	Pages = {275--278},
	Title = {Exact Likelihood of a Vector Autoregressive Moving Average Process with Missing or Aggregated Data},
	Volume = 70,
	Year = 1983}

@article{Ansley86,
	Annote = {Filed under AR Modeling.},
	Author = {C. F. Ansley and R. Kohn},
	Journal = {J. Stat. Comp. Sim.},
	Pages = {99--106},
	Title = {A Note on Reparameterising a Vector Autoregressive Moving Average Model to Enforce Stationarity},
	Volume = {24},
	Year = 1986}

@article{Arakawa74,
	Author = {A. Arakawa and W. H. Schubert},
	File = {../../Papers/arakawa74.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {674--701},
	Title = {Interaction of a Cumulus Cloud Ensemble with the Large-Scale Environment. {Part~I}},
	Volume = 31,
	Year = 1974,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1hcmFrYXdhNzQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQylvzKL6wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzLuWwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YXJha2F3YTc0LnBkZgAOABwADQBhAHIAYQBrAGEAdwBhADcANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvYXJha2F3YTc0LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2FyYWthd2E3NC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Archer00,
	Annote = {Filed under Paleo-Climate Reviews.},
	Author = {D. Archer and A. Winguth and D. Lea and N. Mahowald},
	Journal = {Rev. Geophys.},
	Pages = {159--189},
	Title = {What caused the glacial/interglacial atmospheric $p\mathrm{CO}_2$ cycles?},
	Volume = 38,
	Year = 2000}

@book{Arfken85,
	Address = {San Diego, CA},
	Author = {G. Arfken},
	Edition = {3d},
	Pages = 985,
	Publisher = {Academic Press},
	Title = {Mathematical Methods for Physicists},
	Year = 1985}

@article{Atkinson97,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {D. H. Atkinson and A. P. Ingersoll and A. Seiff},
	File = {../../Papers/atkinson97.pdf},
	Journal = {Nature},
	Pages = {649--650},
	Title = {Deep winds on {J}upiter as measured by the {Galileo} probe},
	Volume = 388,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5hdGtpbnNvbjk3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQypw7U/oQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7WwIQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YXRraW5zb245Ny5wZGYAAA4AHgAOAGEAdABrAGkAbgBzAG8AbgA5ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2F0a2luc29uOTcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2F0a2luc29uOTcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Atkinson98,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {D. H. Atkinson and J. B. Pollack and A. Seiff},
	File = {../../Papers/atkinson98.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {22911--22928},
	Title = {The {Galileo} probe {Doppler} wind experiment: Measurement of the deep zonal winds on {J}upiter},
	Volume = 103,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5hdGtpbnNvbjk4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQyqw7VADwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7WwjwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YXRraW5zb245OC5wZGYAAA4AHgAOAGEAdABrAGkAbgBzAG8AbgA5ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2F0a2luc29uOTgucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2F0a2luc29uOTgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Baer81,
	Annote = {Filed under Atmospheric Turbulence Spectra.},
	Author = {F. Baer},
	File = {../../Papers/baer81.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {52--68},
	Title = {Three-Dimensional Scaling and Structure of Atmospheric Energetics},
	Volume = 38,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpiYWVyODEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQy0v1iv0FBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv1kSQAAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmFlcjgxLnBkZgAADgAWAAoAYgBhAGUAcgA4ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2JhZXI4MS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvYmFlcjgxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Baker94,
	Author = {M. B. Baker and J. G. Dash},
	Journal = {J. Geophys. Res.},
	Pages = {10621--10626},
	Title = {Mechanism of charge transfer between colliding ice particles in thunderstorms},
	Volume = {99D},
	Year = 1994}

@article{Balasubramanian97,
	Annote = {Not on file.},
	Author = {G. Balasubramanian and S. T. Garner},
	File = {../../Papers/balasubramanian97.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2850--2871},
	Title = {The equilibration of short baroclinic waves},
	Volume = 54,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYgAAAAAAYgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhViYWxhc3VicmFtYW5pYW45Ny5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQy1wg0DJlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwg1zpgAAAAEADAAJDH4ACE6zAACS8wACADRNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmFsYXN1YnJhbWFuaWFuOTcucGRmAA4ALAAVAGIAYQBsAGEAcwB1AGIAcgBhAG0AYQBuAGkAYQBuADkANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAChVc2Vycy90YXBpby9QYXBlcnMvYmFsYXN1YnJhbWFuaWFuOTcucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfECIuLi8uLi9QYXBlcnMvYmFsYXN1YnJhbWFuaWFuOTcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAiwCLgIzAjwCRwJLAlkCYAJpAo4CkwKWAqMCqAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAK6}}

@article{Baldwin01,
	Author = {M. P. Baldwin and T. J. Dunkerton},
	File = {../../Papers/baldwin01.pdf},
	Journal = {Science},
	Pages = {581--584},
	Title = {Stratospheric Harbingers of Anomalous Weather Regimes},
	Volume = 294,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1iYWxkd2luMDEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQy2wH4qTwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwH6MvwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmFsZHdpbjAxLnBkZgAOABwADQBiAGEAbABkAHcAaQBuADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvYmFsZHdpbjAxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2JhbGR3aW4wMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Balk91,
	Annote = {Filed under Wave Turbulence.},
	Author = {A. M. Balk},
	Journal = {Phys. Lett.},
	Pages = {20--24},
	Title = {A new invariant for {Rossby} wave systems},
	Volume = 155,
	Year = 1991}

@article{Bannon02,
	Annote = {Equations of motion for multiple-phase flow (air
                  with hydrometeors).},
	Author = {P. R. Bannon},
	Journal = {J. Atmos. Sci.},
	Pages = {1967--1982},
	Title = {Theoretical Foundations for Models of Moist Convection},
	Volume = 59,
	Year = 2002}

@article{Bannon86,
	Author = {P. R. Bannon},
	File = {../../Papers/bannon86.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2261--2274},
	Title = {Linear Development of Quasi-Geostrophic Baroclinic Disturbances with Condensational Heating},
	Volume = 43,
	Year = 1986,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxiYW5ub244Ni5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQy5vrdbAwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvre9cwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmFubm9uODYucGRmAAAOABoADABiAGEAbgBuAG8AbgA4ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2Jhbm5vbjg2LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9iYW5ub244Ni5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Barkmeijer95,
	Annote = {Filed under Predictability.},
	Author = {J. Barkmeijer},
	Journal = {Tellus},
	Pages = {495--501},
	Title = {Approximating dominant eigenvalues and eigenvectors of the local forecast error covariance matrix},
	Volume = {47A},
	Year = 1995}

@unpublished{Barkmeijer98,
	Annote = {Filed under Predictability. Uses Hessian of 3D-Var
                  data assimilation cost function to approximate
                  inverse of analysis error covariance matrix.},
	Author = {J. Barkmeijer and M. {van Gijzen} and F. Bouttier},
	Note = {Submitted to {\em Quart. J. Roy. Meteor. Soc.}},
	Title = {Singular Vectors and the Analysis Error Covariance Metric},
	Year = 1997}

@article{Barnes93,
	Annote = {Filed under Mars Dynamics. Sequel to Haberle93.},
	Author = {J. R. Barnes and J. B. Pollack and R. M. Haberle and C. B. Leovy and R. W. Zurek and H. Lee and J. Schaeffer},
	File = {../../Papers/barnes93.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {3125--3148},
	Title = {Mars Atmospheric Dynamics as Simulated by the {NASA} {Ames} General Circulation Model. 2. {T}ransient Baroclinic Eddies},
	Volume = {98E},
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxiYXJuZXM5My5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQy7v3k4iQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3ma+QAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmFybmVzOTMucGRmAAAOABoADABiAGEAcgBuAGUAcwA5ADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2Jhcm5lczkzLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9iYXJuZXM5My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Barnett01,
	Annote = {Filed under Climate Change Detection.},
	Author = {T. P. Barnett and D. W. Pierce and R. Schnur},
	Journal = {Science},
	Pages = {270--274},
	Title = {Detection of Anthropogenic Climate Change in the World's Oceans},
	Volume = 292,
	Year = 2001}

@article{Barnett87,
	Annote = {Filed under Climate Change Detection. Compare 2xC02
                  equilibrium simulation with control simulation of a
                  AGCM coupled to mixed-layer ocean model. Use
                  normalized scalar product of "signal" (=difference
                  between equilibrium climate at 2xCO2 and control)
                  with observations as measure of similarity between
                  model-projected and observed change. Call this
                  scalarproduct fingerprint (?). Find no significant
                  global warming signal in observations. Claim that
                  SST is better suited to detect climate change than
                  SAT because the natural SAT variability resembles
                  GHG-changed SAT. Low signal-to-noise ratio in SLP
                  field.},
	Author = {T. P. Barnett and M. E. Schlesinger},
	Journal = {J. Geophys. Res.},
	Pages = {147772--14780},
	Title = {Detecting Changes in Global Climate Induced by Greenhouse Gases},
	Volume = {92D},
	Year = 1987}

@article{Barnett95,
	Annote = {Filed under Predictability.},
	Author = {T. P. Barnett},
	Journal = {J. Climate},
	Pages = {1005--1022},
	Title = {Monte {C}arlo Climate Forecasting},
	Volume = 8,
	Year = 1995}

@article{Barnett98,
	Annote = {Filed under Climate Change Detection. The impact of
                  model errors on estimates of rates of anthropogenic
                  climate change diminishes as the time scale over
                  which trends are computed increases. Simulated
                  trends over more than 10--20 years are robust.},
	Author = {T. P. Barnett and G. C. Hegerl and B. Santer and K. Taylor},
	Journal = {J. Climate},
	Pages = {659--675},
	Title = {The Potential Effect of {GCM} Uncertainties and Internal Atmospheric Variability on Anthropogenic Signal Detection},
	Volume = 11,
	Year = 1998}

@article{Barone87,
	Annote = {Not on file. Presents method to compute state
                  covariance matrix of AR models without explicitly
                  inverting matrix.},
	Author = {P. Barone},
	Journal = {J. Time Series Anal.},
	Pages = {125--130},
	Title = {A Method for Generating Independent Realizations of a Multivariate Normal Stationary and Invertible {ARMA}($p$,$q$) Process},
	Volume = 8,
	Year = 1987}

@article{Barry00,
	Annote = {Filed under Thuburn.},
	Author = {L. Barry and G. C. Craig and J. Thuburn},
	File = {../../Papers/barry00.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1141--1155},
	Title = {A {GCM} Investigation into the Nature of Baroclinic Adjustment},
	Volume = 57,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtiYXJyeTAwLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQy9wYUPXFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwYV/3AAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmFycnkwMC5wZGYADgAYAAsAYgBhAHIAcgB5ADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYmFycnkwMC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9iYXJyeTAwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Barry02,
	Annote = {Filed under Baroclinic Eddy Flux
                  Parameterizations. Parameterization of bulk heat
                  flux integrated over entire extratropical
                  troposphere. Parameterization depends on rate of
                  'radiative cooling'.},
	Author = {L. Barry and G. C. Craig and J. Thuburn},
	Journal = {Nature},
	Pages = {774--777},
	Title = {Poleward heat transport by the atmospheric heat engine},
	Volume = 415,
	Year = 2002}

@article{Bartello88,
	Author = {Bartello, P. and Warn, T.},
	File = {../../Papers/bartello88.pdf},
	Journal = {Geophys. Astrophys. Fluid Dyn.},
	Pages = {239--259},
	Title = {A one-dimensional turbulence model; Enstrophy cascades and small-scale intermittency in decaying turbulence},
	Volume = 40,
	Year = 1988,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5iYXJ0ZWxsbzg4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQy+wygqPgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwyiMrgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmFydGVsbG84OC5wZGYAAA4AHgAOAGIAYQByAHQAZQBsAGwAbwA4ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2JhcnRlbGxvODgucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2JhcnRlbGxvODgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Bartello93,
	Author = {P. Bartello},
	File = {../../Papers/bartello93.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2542--2546},
	Title = {Inertial ranges and small-scale intermittency in one-dimensional turbulence models},
	Volume = 50,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5iYXJ0ZWxsbzkzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQy/wygqxwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwyiNNwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmFydGVsbG85My5wZGYAAA4AHgAOAGIAYQByAHQAZQBsAGwAbwA5ADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2JhcnRlbGxvOTMucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2JhcnRlbGxvOTMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Bartels98,
	Annote = {Filed under Isentropic Observations.},
	Author = {J. Bartels and D. Peters and G. Schmitz},
	File = {../../Papers/bartels98.pdf},
	Journal = {Ann. Geophysicae},
	Pages = {250--265},
	Title = {Climatological {Ertel}'s potential-vorticity flux and mean meridional circulation in the extratropical troposphere -- lower stratosphere},
	Volume = 16,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1iYXJ0ZWxzOTgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzAv1GLb1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv1Ht3wAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmFydGVsczk4LnBkZgAOABwADQBiAGEAcgB0AGUAbABzADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvYmFydGVsczk4LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2JhcnRlbHM5OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@book{Batchelor67,
	Address = {Cambridge, UK},
	Author = {G. K. Batchelor},
	Pages = 615,
	Publisher = {Cambridge University Press},
	Title = {An Introduction to Fluid Dynamics},
	Year = 1967}

@article{Bates99,
	Annote = {Not on file. Feedback between angular momentum
                  fluxes and evaporation is supposed to stabilize
                  surface temperature perturbation. But feedback rests
                  on questionable parameterization.},
	Author = {J.\ R.\ Bates},
	Journal = {Tellus},
	Pages = {349--372},
	Title = {A dynamical stabilizer in the climate system: A mechanism suggested by a simple model},
	Volume = {51A},
	Year = 1999}

@article{Battisti99,
	Annote = {Filed under ITCZ Dynamics.},
	Author = {D. S. Battisti and E. S. Sarachik and A. C. Hirst},
	File = {../../Papers/battisti99.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2956--2964},
	Title = {A Consistent Model for the Large-Scale Steady Surface Atmospheric Circulation in the {T}ropics},
	Volume = 12,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5iYXR0aXN0aTk5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzBwZDk8wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwZFVcwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmF0dGlzdGk5OS5wZGYAAA4AHgAOAGIAYQB0AHQAaQBzAHQAaQA5ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2JhdHRpc3RpOTkucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2JhdHRpc3RpOTkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Beale75,
	Annote = {Not on file.},
	Author = {E. M. L. Beale and R. J. A. Little},
	Journal = {J. Roy. Stat. Soc. B},
	Pages = {129--146},
	Title = {Missing values in multivariate analysis},
	Volume = 37,
	Year = 1975}

@article{Becker01,
	Author = {E. Becker and G. Schmitz},
	File = {../../Papers/becker01.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {462--480},
	Title = {Interaction between Extratropical Stationary Waves and the Zonal Mean Circulation},
	Volume = {58},
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxiZWNrZXIwMS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzCxbXrpAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxbZcJAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmVja2VyMDEucGRmAAAOABoADABiAGUAYwBrAGUAcgAwADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2JlY2tlcjAxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9iZWNrZXIwMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Becker97,
	Annote = {Filed under Hadley Cell Dynamics. Comparison of 2D
                  and 3D circulations. Strengthening of Hadley cell in
                  non-axisymmetric (3D) case.},
	Author = {E. Becker and G. Schmitz and R. Gepr{\"a}gs},
	Journal = {Tellus},
	Pages = {182--199},
	Title = {The feedback of midlatitude waves onto the {H}adley cell in a simple general circulation model},
	Volume = {49A},
	Year = 1997}

@article{Beckers03,
	Author = {J. M. Beckers and M. Rixen},
	File = {../../Papers/beckers03.pdf},
	Journal = {J. Atmos. Oceanic Technol.},
	Pages = {1839--1856},
	Title = {{EOF} Calculations and Data Filling from Incomplete Oceanographic Datasets},
	Volume = 20,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1iZWNrZXJzMDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzDv+1xPgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv+3hvgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmVja2VyczAzLnBkZgAOABwADQBiAGUAYwBrAGUAcgBzADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvYmVja2VyczAzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2JlY2tlcnMwMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Bell80,
	Annote = {Uses the method of Leith75 to determine response of
                  climate system to changes in external forcing
                  parameters. Employs 20-variable truncation of
                  barotropic vorticity equations. Finds that the
                  fluctuation-dissipation theorem still leads to good
                  estimates of climate sensitivity even when the
                  system under consideration is dissipative.},
	Author = {T. L. Bell},
	Journal = {J. Atmos. Sci.},
	Pages = {1700--1707},
	Title = {Climate Sensitivity from Fluctuation Dissipation: Some Simple Model Tests},
	Volume = 37,
	Year = 1980}

@article{Bell82,
	Annote = {Not on file. Theory reviewed in Bell86.},
	Author = {T. L. Bell},
	Journal = {J. Geophys. Res.},
	Pages = {11161--11170},
	Title = {Optimal Weighting of Data to Detect Climatic Change: Application to the Carbon Dioxide Problem},
	Volume = 87,
	Year = 1982}

@article{Bell86,
	Annote = {Uses discriminant analysis to classify whether
                  climate has changed or not.},
	Author = {T. L. Bell},
	Journal = {J. Atmos. Sci.},
	Pages = {1694--1710},
	Title = {Theory of Optimal Weighting of Data to Detect Climatic Change},
	Volume = 43,
	Year = 1986}

@article{Bello93,
	Annote = {Filed under Imputation of Missing Values.},
	Author = {A. L. Bello},
	Journal = {J. Stat. Comp. Sim.},
	Pages = {167--180},
	Title = {A simulation study of imputation techniques in linear, quadratic and kernel discriminant analyses},
	Volume = 48,
	Year = 1993}

@article{Bengtsson04,
	Annote = {Influence of various kinds of observations on ERA-40
                  reanalysis.},
	Author = {L. Bengtsson and K. I. Hodges and S. Hagemann},
	File = {../../Papers/bengtsson04.pdf},
	Journal = {Tellus},
	Pages = {456--471},
	Title = {Sensitivity of the {ERA40} reanalysis to the observing system: determination of the global atmospheric circulation from reduced observations},
	Volume = {56A},
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9iZW5ndHNzb24wNC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzJvuLSuwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvuM1KwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmVuZ3Rzc29uMDQucGRmAA4AIAAPAGIAZQBuAGcAdABzAHMAbwBuADAANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvYmVuZ3Rzc29uMDQucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvYmVuZ3Rzc29uMDQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Bengtsson06,
	Annote = {Filed under Climate Change Projections.},
	Author = {L. Bengtsson and K. I. Hodges and E. Roeckner},
	File = {../../Papers/bengtsson06.pdf},
	Journal = {J. Climate},
	Pages = {3518--3543},
	Title = {Storm Tracks and Climate Change},
	Volume = 19,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9iZW5ndHNzb24wNi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzKwcK2vAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwcMnPAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmVuZ3Rzc29uMDYucGRmAA4AIAAPAGIAZQBuAGcAdABzAHMAbwBuADAANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvYmVuZ3Rzc29uMDYucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvYmVuZ3Rzc29uMDYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Bengtsson09,
	Author = {L. Bengtsson and K. I. Hodges and N. Keenlyside},
	File = {../../Papers/bengtsson09.pdf},
	Journal = {J. Climate},
	Pages = {2276--2301},
	Title = {Will Extratropical Storms Intensify in a Warmer Climate?},
	Volume = 22,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9iZW5ndHNzb24wOS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzLxjBDpgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxjCmFgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmVuZ3Rzc29uMDkucGRmAA4AIAAPAGIAZQBuAGcAdABzAHMAbwBuADAAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvYmVuZ3Rzc29uMDkucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvYmVuZ3Rzc29uMDkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Bennetts79,
	Annote = {Filed under Hoskins.},
	Author = {D. A. Bennetts and B. J. Hoskins},
	File = {../../Papers/bennetts79.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {945--962},
	Title = {Conditional Symmetric Instability --- A Possible Explanation for Frontal Rainbands},
	Volume = 105,
	Year = 1979,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5iZW5uZXR0czc5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzMvzNdIQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzO/kQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmVubmV0dHM3OS5wZGYAAA4AHgAOAGIAZQBuAG4AZQB0AHQAcwA3ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2Jlbm5ldHRzNzkucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2Jlbm5ldHRzNzkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Benzi89,
	Annote = {Filed under Predictability. Use ratio of average
                  growth rate to most probable growth rate as measure
                  of local predictability.},
	Author = {R. Benzi and G. F. Carnevale},
	Journal = {J. Atmos. Sci.},
	Pages = {3595--3598},
	Title = {A Possible Measure of Local Predictability},
	Volume = 46,
	Year = 1989}

@article{Berger88,
	Annote = {Filed under Climate Stability/Energy Balance Models.},
	Author = {A. Berger},
	File = {../../Papers/berger88.pdf},
	Journal = {Rev. Geophys.},
	Pages = {624--657},
	Title = {Milankovitch theory and climate},
	Volume = 26,
	Year = 1988,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxiZXJnZXI4OC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzOvhavSAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvhcfyAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmVyZ2VyODgucGRmAAAOABoADABiAGUAcgBnAGUAcgA4ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2Jlcmdlcjg4LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9iZXJnZXI4OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Berrisford93,
	Annote = {Filed under John Marshall.},
	Author = {P. Berrisford and J. C. Marshall and A. A. White},
	File = {../../Papers/berrisford93.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {778--782},
	Title = {Quasigeostrophic potential vorticity in isentropic coordinates},
	Volume = 50,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBiZXJyaXNmb3JkOTMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzQvXJEIwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvXKmkwAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmVycmlzZm9yZDkzLnBkZgAADgAiABAAYgBlAHIAcgBpAHMAZgBvAHIAZAA5ADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL2JlcnJpc2ZvcmQ5My5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvYmVycmlzZm9yZDkzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Betts82,
	Author = {A. K. Betts},
	File = {../../Papers/betts82.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1484--1505},
	Title = {Saturation point analysis of moist convective overturning},
	Volume = 39,
	Year = 1982,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtiZXR0czgyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzRxRNIcAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxROq4AAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmV0dHM4Mi5wZGYADgAYAAsAYgBlAHQAdABzADgAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYmV0dHM4Mi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9iZXR0czgyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Betts86a,
	Author = {A. K. Betts},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {677--691},
	Title = {A New Convective Adjustment Scheme. \uppercase{P}art \uppercase{I}: \uppercase{O}bservational and theoretical basis},
	Volume = 112,
	Year = 1986}

@article{Betts86b,
	Author = {A. K. Betts and M. J. Miller},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {693--709},
	Title = {A New Convective Adjustment Scheme. \uppercase{P}art \uppercase{II}: Single column tests using \uppercase{GATE} wave, \uppercase{BOMEX}, \uppercase{ATEX} and arctic air-mass data sets},
	Volume = 112,
	Year = 1986}

@article{Betts87,
	Author = {A. K. Betts and Harshvardhan},
	File = {../../Papers/betts87.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {8483--8485},
	Title = {Thermodynamic constraint on the cloud liquid water feedback in climate models},
	Volume = 92,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtiZXR0czg3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzSxdaWQwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxdcGwwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmV0dHM4Ny5wZGYADgAYAAsAYgBlAHQAdABzADgANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYmV0dHM4Ny5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9iZXR0czg3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Betts89,
	Author = {A. K. Betts and W. L. Ridgway},
	File = {../../Papers/betts89.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2621--2641},
	Title = {Climatic equilibrium of the atmospheric convective boundary layer over a tropical ocean},
	Volume = 46,
	Year = 1989,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtiZXR0czg5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzTxOHqegAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxOJM6gAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmV0dHM4OS5wZGYADgAYAAsAYgBlAHQAdABzADgAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYmV0dHM4OS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9iZXR0czg5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@incollection{Betts93,
	Author = {A. K. Betts and M. J. Miller},
	Booktitle = {The Representation of Cumulus Convection in Numerical Models},
	Editor = {K. A. Emanuel and D. J. Raymond},
	Pages = {107--121},
	Publisher = {Am. Meteor. Soc.},
	Series = {Meteorological Monographs},
	Title = {The {B}etts--{M}iller Scheme},
	Volume = 24,
	Year = 1993}

@incollection{Betts97,
	Author = {A. K. Betts},
	Booktitle = {The Physics and Parameterization of Moist Atmospheric Convection},
	Editor = {R. K. Smith},
	Pages = {255--279},
	Publisher = {Kluwer},
	Title = {The Parameterization of Deep Convection},
	Year = 1997}

@article{Betts98,
	Author = {A. K. Betts},
	File = {../../Papers/betts98.pdf},
	Journal = {Climatic Change},
	Pages = {35--38},
	Title = {Climate-convection feedbacks: Some further issues},
	Volume = 39,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtiZXR0czk4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzUxOAp/gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxOCMbgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmV0dHM5OC5wZGYADgAYAAsAYgBlAHQAdABzADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYmV0dHM5OC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9iZXR0czk4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Bialek01,
	Annote = {Filed under Predictability},
	Author = {W. Bialek and I. Nemenman and N. Tishby},
	File = {../../Papers/bialek01.pdf},
	Journal = {Neural Comp.},
	Pages = {2409--2463},
	Title = {Predictability, Complexity, and Learning},
	Volume = 13,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxiaWFsZWswMS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzVvAI1RwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvAKlxwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmlhbGVrMDEucGRmAAAOABoADABiAGkAYQBsAGUAawAwADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2JpYWxlazAxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9iaWFsZWswMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Birner02,
	Annote = {Filed under Tropopause Dynamics. Claim that there is
                  sharp temperature inversion (and hence jump in
                  static stability) at tropopause. Analysis based on
                  averages of radiosonde soundings, with the averages
                  computed relative to an instantaneous tropopause
                  height diagnosed according to WMO diagnostic. Effect
                  of relative averaging on mean vertical temperature
                  gradient?},
	Author = {T. Birner and A. D{\"o}rnbrack and U. Schumann},
	File = {../../Papers/birner02.pdf},
	Journal = {Geophys. Res. Lett.},
	Pages = {????},
	Title = {How sharp is the tropopause at midlatitudes?},
	Volume = {??},
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxiaXJuZXIwMi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzcvUuVTQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvUv3vQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmlybmVyMDIucGRmAAAOABoADABiAGkAcgBuAGUAcgAwADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2Jpcm5lcjAyLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9iaXJuZXIwMi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@phdthesis{Birner03,
	Annote = {Filed under Tropopause Dynamics.},
	Author = {T. Birner},
	School = {Ludwig-Maximilians-Universit{\"a}t M{\"u}nchen},
	Title = {Die extratropische Tropopausenregion},
	Year = 2003}

@article{Bjerknes38,
	Author = {Bjerknes, J.},
	Journal = {Quart. J. Roy. Meteor. Soc},
	Pages = {325--330},
	Title = {Saturated-adiabatic ascent of air through dry-adiabatically descending environment},
	Volume = {64},
	Year = {1938}}

@article{Bjerknes69,
	Annote = {Not on file. Bjerknes postulate on ENSO: Anomalies
                  in sea surface temperature (SST) in the Pacific
                  cause the trade winds to strengthen or slacken, and
                  these wind anomalies in turn drive the changes in
                  ocean circulation that produce anomalous SST.},
	Author = {J. Bjerknes},
	Journal = {Mon. Wea. Rev.},
	Pages = {163--172},
	Title = {Atmospheric Teleconnections from the Equatorial {P}acific},
	Volume = 97,
	Year = 1969}

@book{Bjorck96,
	Address = {Philadelphia, PA},
	Author = {{\AA}. Bj{\"o}rck},
	Pages = 408,
	Publisher = {Society for Industrial and Applied Mathematics},
	Title = {Numerical Methods for Least Squares Problems},
	Year = 1996}

@article{Black02,
	Annote = {Separate inversion of stratospheric and tropospheric
                  pv anomalies suggests that stratospheric pv
                  anomalies can have significant influence on
                  troposphere.},
	Author = {R. X. Black},
	Journal = {J. Atmos. Sci.},
	Pages = {268--277},
	Title = {Stratospheric Forcing of Surface Climate in the {A}rctic {O}scillation},
	Volume = 15,
	Year = 2002}

@incollection{Bliesner05,
	Address = {Netherlands},
	Author = {B. L. Otto-Bliesner and A. Clement},
	Booktitle = {The {Hadley} Circulation: Present, Past and Future},
	Editor = {H. F. Diaz and R. S. Bradley},
	File = {../../Papers/bliesner05.pdf},
	Pages = {437--464},
	Publisher = {Kluwer Academic Publishers},
	Title = {The Sensitivity of the {Hadley} circulation to past and future forcings in two climate models},
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5ibGllc25lcjA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzhxLP+2QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxLRhSQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YmxpZXNuZXIwNS5wZGYAAA4AHgAOAGIAbABpAGUAcwBuAGUAcgAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2JsaWVzbmVyMDUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2JsaWVzbmVyMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Blumenthal91,
	Annote = {Uses POPs to determine predictability of Cane-Zebiak
                  model. Criticism: is the first order model really a
                  good one?},
	Author = {M. B. Blumenthal},
	Journal = {J. Climate},
	Pages = {766--784},
	Title = {Predictability of a Coupled Ocean-Atmosphere Model},
	Volume = 4,
	Year = 1991}

@article{Boer83a,
	Annote = {Filed under Atmospheric Turbulence Spectra.},
	Author = {G. J. Boer},
	File = {../../Papers/boer83a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {154--163},
	Title = {Homogeneous and Isotropic Turbulence on the Sphere},
	Volume = 40,
	Year = 1983,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtib2VyODNhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzlvgIemAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvgKPGAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9lcjgzYS5wZGYADgAYAAsAYgBvAGUAcgA4ADMAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYm9lcjgzYS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9ib2VyODNhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Boer83b,
	Annote = {Filed under Atmospheric Turbulence Spectra.},
	Author = {G. J. Boer and T. G. Shepherd},
	File = {../../Papers/boer83b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {164--184},
	Title = {Large-Scale Two-Dimensional Turbulence in the Atmosphere},
	Volume = 40,
	Year = 1983,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtib2VyODNiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzmvgIf2gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvgKQWgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9lcjgzYi5wZGYADgAYAAsAYgBvAGUAcgA4ADMAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYm9lcjgzYi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9ib2VyODNiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Boer93,
	Author = {G. J. Boer},
	File = {../../Papers/boer93.pdf},
	Journal = {Clim. Dyn.},
	Pages = {225--239},
	Title = {Climate change and the regulation of the surface moisture and energy budgets},
	Volume = 8,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpib2VyOTMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQznxOLalgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxOM9BgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9lcjkzLnBkZgAADgAWAAoAYgBvAGUAcgA5ADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2JvZXI5My5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvYm9lcjkzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Bokhove00,
	Annote = {Filed under Hamiltonian Balanced Dynamics.},
	Author = {O. Bokhove},
	Journal = {J. Fluid Mech.},
	Pages = {291--310},
	Title = {On hydrostatic flows in isentropic coordinates},
	Volume = 402,
	Year = 2000}

@article{Bolton80,
	Author = {D. Bolton},
	File = {../../Papers/bolton80.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {1046--1053},
	Title = {The Computation of Equivalent Potential Temperature},
	Volume = 108,
	Year = 1980,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxib2x0b244MC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzswzRfrVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwzTCHQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9sdG9uODAucGRmAAAOABoADABiAG8AbAB0AG8AbgA4ADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2JvbHRvbjgwLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9ib2x0b244MC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Bonan97,
	Annote = {Filed under Climate Change Detection.},
	Author = {G. B. Bonan},
	Journal = {Climatic Change},
	Pages = {449--486},
	Title = {Effects of Land Use on the Climate of the {U}nited {S}tates},
	Volume = 37,
	Year = 1997}

@article{Bony06,
	Annote = {Filed under Climate Change Projections.},
	Author = {S. Bony and R. Colman and V. M. Kattsov and R. P. Allan and C. S. Bretherton and J.-L. Dufresne and A. Hall and S. Hallegatte and M. M. Holland and W. Ingram and D. A. Randall and B. J. Soden and G. Tselioudis and M. J. Webb},
	File = {../../Papers/bony06.pdf},
	Journal = {J. Climate},
	Pages = {3445--3482},
	Title = {How well do we understand and evaluate climate change feedback processes},
	Volume = 19,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpib255MDYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQzuwaSlxAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwaUWRAAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9ueTA2LnBkZgAADgAWAAoAYgBvAG4AeQAwADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2JvbnkwNi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvYm9ueTA2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Bordoni04,
	Author = {S. Bordoni and P. E. Ciesielski and R. H. Johnson and B. D. McNoldy and B. Stevens},
	File = {../../Papers/bordoni04.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2004GL020009},
	Pages = {L10109},
	Title = {The low-level circulation of the {N}orth {A}merican {M}onsoon as revealed by {QuikSCAT}},
	Volume = 31,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ib3Jkb25pMDQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQz1wjWdLwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwjX/nwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9yZG9uaTA0LnBkZgAOABwADQBiAG8AcgBkAG8AbgBpADAANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvYm9yZG9uaTA0LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2JvcmRvbmkwNC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Bordoni06,
	Author = {S. Bordoni and B. Stevens},
	File = {../../Papers/bordoni06.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {3395--3414},
	Title = {Principal component analysis of the summertime winds over the {G}ulf of {C}alifornia: a gulf surge index},
	Volume = {134},
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ib3Jkb25pMDYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQz2wjWd3AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwjYATAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9yZG9uaTA2LnBkZgAOABwADQBiAG8AcgBkAG8AbgBpADAANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvYm9yZG9uaTA2LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2JvcmRvbmkwNi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@phdthesis{Bordoni07a,
	Address = {Los Angeles, CA},
	Author = {S. Bordoni},
	School = {University of California},
	Title = {On the Role of Eddies in Monsoonal Circulations: Observations and Theory},
	Year = 2007}

@article{Bordoni08a,
	Author = {S. Bordoni and T. Schneider},
	Date-Modified = {2010-06-11 12:20:39 -0700},
	Journal = {Nature Geosci.},
	Pages = {515--519},
	Title = {Monsoons as eddy-mediated regime transitions of the tropical overturning circulation},
	Volume = 1,
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5ib3Jkb25pMDhhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQz3x6g4qgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx6ipKgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9yZG9uaTA4YS5wZGYAAA4AHgAOAGIAbwByAGQAbwBuAGkAMAA4AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2JvcmRvbmkwOGEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2JvcmRvbmkwOGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Bordoni10a,
	Author = {S. Bordoni and T. Schneider},
	Date-Modified = {2010-06-11 12:21:16 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {1643--1654},
	Title = {Regime Transitions of Steady and Time-Dependent Hadley Circulations: Comparison of Axisymmetric and Eddy-Permitting Simulations},
	Volume = 67,
	Year = 2010,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5ib3Jkb25pMTBhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQz4yC6zegAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyC8V6gAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9yZG9uaTEwYS5wZGYAAA4AHgAOAGIAbwByAGQAbwBuAGkAMQAwAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2JvcmRvbmkxMGEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2JvcmRvbmkxMGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Bosilovich05,
	Annote = {Filed under Water Vapor (Feedback and Kinematics).},
	Author = {M. G. Bosilovich and S. D. Schubert and G. K. Walker},
	File = {../../Papers/bosilovich05.pdf},
	Journal = {J. Climate},
	Pages = {1591--1608},
	Title = {Global Changes of the Water Cycle Intensity},
	Volume = 18,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBib3NpbG92aWNoMDUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQz8v5Gc9FBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5INdAAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9zaWxvdmljaDA1LnBkZgAADgAiABAAYgBvAHMAaQBsAG8AdgBpAGMAaAAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL2Jvc2lsb3ZpY2gwNS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvYm9zaWxvdmljaDA1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Bouchet02,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {F. Bouchet and J. Sommeria},
	Journal = {J. Fluid Mech.},
	Pages = {165--207},
	Title = {Emergence of intense jets and {J}upiter's {G}reat {R}ed {S}pot as maximum-entropy structures},
	Volume = 464,
	Year = 2002}

@article{Bourke74,
	Annote = {Not of file. Vorticity-divergence form of primitive
                  equations.},
	Author = {W. Bourke},
	File = {../../Papers/bourke74.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {687--701},
	Title = {A multilevel spectral model. {I}. {F}ormulation and hemispheric integrations},
	Volume = 102,
	Year = 1974,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxib3Vya2U3NC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQz+xIhUgAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxIi28AAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym91cmtlNzQucGRmAAAOABoADABiAG8AdQByAGsAZQA3ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2JvdXJrZTc0LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9ib3Vya2U3NC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Bourlioux02,
	Annote = {Filed under Majda. Minimum ingredients for
                  intermittency in passive-scalar turbulence.},
	Author = {A. Bourlioux and A. J. Majda},
	Journal = {Phys. Fluids},
	Pages = {881--897},
	Title = {Elementary models with probability distribution function intermittency for passive scalars with a mean gradient},
	Volume = 14,
	Year = 2002}

@article{Bousquet00,
	Annote = {Filed under Carbon Flux Estimates. Consider
                  time-dependence of carbon uptake by
                  biosphere. Enhanced update over North America in
                  1992--93 compared with previous years, suggesting
                  that the analysis of Fan98 covers a time of
                  unusually large update over North America.},
	Author = {P. Bousquet and P. Peylin and P. Ciais and C. {Le Qu{\'e}r{\'e}} and P. Friedlingstein and P. P. Tans},
	Journal = {Science},
	Pages = {1342--1346},
	Title = {Regional Changes in Carbon Dioxide Fluxes of Land and Oceans since 1980},
	Volume = 290,
	Year = 2000}

@article{Bowman02,
	Annote = {Particle-release experiments with statistically
                  axisymmetric GCM (NCAR). Find what they call
                  'transport barrier' between tropics and extratropics
                  (that is, a certain degree of recirculation of air
                  masses within Hadley cell). Do not quantify amount
                  of recirculation.},
	Author = {K. P. Bowman and G. D. Carrie},
	Journal = {J. Atmos. Sci.},
	Pages = {1502--1514},
	Title = {The Mean-Meridional Transport Circulation of the Troposphere in an Idealized {GCM}},
	Volume = 59,
	Year = 2002}

@book{Box70a,
	Address = {San Francisco},
	Author = {G. E. P. Box and G. M. Jenkins},
	Publisher = {Holden-Day},
	Title = {Time Series Analysis: Forecasting and Control},
	Year = {1970}}

@article{Box70b,
	Annote = {Not on file. Classic paper on univariate portmanteau
                  test.},
	Author = {G. E. P. Box and D. A. Pierce},
	Journal = {J. Amer. Statist. Assoc.},
	Pages = {1509--1526},
	Title = {Distribution of the residual autocorrelations in autoregressive-integrated moving average time series models},
	Volume = 65,
	Year = 1970}

@article{Box77,
	Annote = {Filed under AR Modeling. Transformation of
                  multivariate AR process to process with components
                  ordered according to their predictability.},
	Author = {G. E. P. Box and G. C. Tiao},
	Journal = {Biometrika},
	Pages = {355-365},
	Title = {A canonical analysis of multiple time series},
	Volume = 64,
	Year = 1977}

@book{Box78,
	Address = {New York},
	Author = {G. E. P. Box and W. G. Hunter and J. S. Hunter},
	Publisher = {Wiley},
	Series = {Series in Probability and Mathematical Statistics},
	Title = {Statistics for Experimenters: An Introduction to Design, Data Analysis, and Model Building},
	Year = 1978}

@article{Brands99a,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {H. Brands and S. R. Maassen and H. J. J. Clercx},
	Journal = {Phys. Rev. E},
	Pages = {2864--2874},
	Title = {Statistical-mechanical predictions and {N}avier-{S}tokes dynamics of two-dimensional flows on a bounded domain},
	Volume = 60,
	Year = 1999}

@article{Brands99b,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {H. Brands and P.-H. Chavanis and R. Pasmanter and J. Sommeria},
	Journal = {Phys. Fluids},
	Pages = {3465--3477},
	Title = {Maximum entropy versus minimum enstrophy vortices},
	Volume = 11,
	Year = 1999}

@article{Branscome83,
	Annote = {Filed under Surface Heat Flux
                  Parameterizations. Review of Stone's and Green's
                  eddy heat flux parameterizations. Review of
                  Held78. Vertical structure of heat flux given by
                  structure of Charney mode. Test with seasonal
                  observational data.},
	Author = {L. E. Branscome},
	Journal = {J. Atmos. Sci.},
	Pages = {2508--2521},
	Title = {A Parameterization of Transient Eddy Heat Flux on a Beta-Plane},
	Volume = 40,
	Year = 1983}

@article{Branscome88,
	Annote = {Filed under Surface Heat Flux Parameterizations.},
	Author = {L. E. Branscome and E. O'Brien},
	Journal = {J. Atmos. Sci.},
	Pages = {645--656},
	Title = {Feedbacks between Eddy Heat Fluxes and Radiative Heating in an Energy-Balance Model},
	Volume = 45,
	Year = 1988}

@article{Branstator03,
	Annote = {Seasonally varying mean state organizes
                  variability. Use stochastically forced barotropic
                  model linearized about mean state to demonstrate
                  that much of the variability of the mean state can
                  be understood as organized by mean state itself.},
	Author = {G. Branstator and J. Frederiksen},
	Journal = {J. Atmos. Sci.},
	Pages = {1577--1592},
	Title = {The Seasonal Cycle of Interannual Variability and the Dynamical Imprint of the Seasonally Varying Mean State},
	Volume = 60,
	Year = 2003}

@article{Branstator95,
	Author = {G. Branstator and I. Held},
	Journal = {J. Atmos. Sci.},
	Pages = {247--262},
	Title = {Westward Propagating Normal Modes in the Presence of Stationary Background Waves},
	Volume = 52,
	Year = 1995}

@article{Brayshaw08,
	Author = {D. J. Brayshaw and B. Hoskins and M. Blackburn},
	File = {../../Papers/brayshaw08.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2842--2860},
	Title = {The Storm-Track Response to Idealized {SST} Perturbations in an Aquaplanet {GCM}},
	Volume = 65,
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5icmF5c2hhdzA4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0BxP2DbAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxP3l3AAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnJheXNoYXcwOC5wZGYAAA4AHgAOAGIAcgBhAHkAcwBoAGEAdwAwADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2JyYXlzaGF3MDgucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2JyYXlzaGF3MDgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Breiman97,
	Annote = {Filed under Regression Analysis. Exploits the
                  correlations of dependent variables in regression to
                  improve predictions. "Curds & Whey" procedure,
                  multivariate flattening.},
	Author = {L. Breiman and J. H. Friedman},
	File = {../../Papers/breiman97.pdf},
	Journal = {J. Roy. Stat. Soc. B},
	Pages = {3--54},
	Title = {Predicting multivariate responses in multiple linear regression},
	Volume = 59,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1icmVpbWFuOTcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0DxrNCtgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxrOlJgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnJlaW1hbjk3LnBkZgAOABwADQBiAHIAZQBpAG0AYQBuADkANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvYnJlaW1hbjk3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2JyZWltYW45Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Bretherton66a,
	Annote = {Surface temperature anomaly corresponds to anomaly
                  in potential vorticity sheet.},
	Author = {F. P. Bretherton},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {325--334},
	Title = {Critical layer instability in baroclinic flows},
	Volume = 92,
	Year = 1966}

@article{Bretherton66b,
	Annote = {Interpretation of correspondence between Eady model
                  and two-layer model. Shortwave cut-off consequence
                  of zero pv gradient in Eady model, lack of critical
                  layer instability in two-layer model. Interpretation
                  of edge waves in Eady model in terms of pv sheets on
                  boundary.},
	Author = {F. P. Bretherton},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {335--345},
	Title = {Baroclinic instability and the short wavelength cut-off in terms of potential vorticity},
	Volume = 92,
	Year = 1966}

@article{Bretherton89,
	Author = {C. S. Bretherton and P. K. Smolarkiewicz},
	File = {../../Papers/bretherton89.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {740--759},
	Title = {Gravity waves, compensating subsidence and detrainment around cumulus clouds},
	Volume = 46,
	Year = 1989,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBicmV0aGVydG9uODkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0IxRNIygAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxROrOgAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnJldGhlcnRvbjg5LnBkZgAADgAiABAAYgByAGUAdABoAGUAcgB0AG8AbgA4ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL2JyZXRoZXJ0b244OS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvYnJldGhlcnRvbjg5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Bretherton92,
	Annote = {Compares SVD, principal component analysis,
                  canonical correlation analysis.},
	Author = {C. S. Bretherton and C. Smith and J. M. Wallace},
	Journal = {J. Climate},
	Pages = {541--560},
	Title = {An Intercomparison of Methods for Finding Coupled Patterns in Climate Data},
	Volume = 5,
	Year = 1992}

@article{Bretherton93,
	Author = {C. S. Bretherton and C. Sch{\"a}r},
	Journal = {J. Atmos. Sci.},
	Pages = {1834--1836},
	Title = {Flux of Potential Vorticity Substance: A Simple Derivation and a Uniqueness Property},
	Volume = 50,
	Year = 1993}

@article{Breuer93a,
	Annote = {Filed under Petruccione.},
	Author = {H. P. Breuer and F. Petruccione},
	Journal = {Physica A},
	Pages = {569--588},
	Title = {A master equation description of fluctuating hydrodynamics},
	Volume = 192,
	Year = 1993}

@article{Breuer93b,
	Annote = {Filed under Petruccione.},
	Author = {H. P. Breuer and F. Petruccione},
	Journal = {Phyica A},
	Pages = {83--95},
	Title = {Thermostochastics: {H}eat conduction and temperature fluctuations},
	Volume = 209,
	Year = 1994}

@article{Breuer93c,
	Annote = {Filed under Petruccione.},
	Author = {H. P. Breuer and F. Petruccione},
	Journal = {J. Phys. A: Math. Gen.},
	Pages = {7563--7582},
	Title = {A master equation representation of two-dimensional turbulence},
	Volume = 26,
	Year = 1993}

@unpublished{Breuer94,
	Annote = {Filed under Petruccione.},
	Author = {H. P. Breuer and F. Petruccione},
	Note = {Preprint},
	Title = {Stochastic simulations of high-{R}eynolds-number turbulence in two dimensions},
	Year = 1994}

@unpublished{Breuer95,
	Annote = {Filed under Petruccione.},
	Author = {H. P. Breuer and F. Petruccione},
	Note = {Preprint},
	Title = {Mesoscopic Modeling and stochastic simulations of turbulent flows},
	Year = 1995}

@book{Brillouin56,
	Address = {New York},
	Annote = {Excellent book on information theory. B. takes great
                  care to distinguish between entropy, information,
                  the value of information to human beings, etc.},
	Author = {L. Brillouin},
	Pages = {320},
	Publisher = {Academic Press},
	Title = {Science and Information Theory},
	Year = 1956}

@article{Broccoli90,
	Annote = {Filed under Manabe.},
	Author = {A. J. Broccoli and S. Manabe},
	Journal = {Geophys. Res. Lett.},
	Pages = {1917--1920},
	Title = {Can Existing Climate Models be Used to Study Anthropogenic Changes in Tropical Cyclone Climate?},
	Volume = 17,
	Year = 1990}

@article{Broccoli98,
	Annote = {Filed under Wallace. R15 model simulates COWL
                  pattern of Wallace95, Wallace96. Contrast in heat
                  capacity is responsible for COWL pattern.},
	Author = {A. J. Broccoli and N.-C. Lau and M. J. Nath},
	Journal = {J. Climate},
	Pages = {2743--2763},
	Title = {The cold ocean warm land pattern: Model simulation and relevance to climate change detection},
	Volume = 11,
	Year = 1998}

@book{Brockwell91,
	Address = {New York},
	Author = {P. J. Brockwell and A. Davis},
	Edition = {2nd},
	Pages = 577,
	Publisher = {Springer},
	Title = {Time Series: Theory and Methods},
	Year = 1991}

@article{Broecker97,
	Annote = {Not on file.},
	Author = {W. S. Broecker},
	Journal = {Global Biogeochem. Cycles},
	Number = 11,
	Pages = {589--597},
	Title = {Mountain glaciers: {R}ecorders of atmospheric water vapor content?},
	Year = 1997}

@article{Broeker97,
	Annote = {Review of actual and possible thermohaline
                  circulation changes and connected climate
                  changes. Some remarks on atmospheric water vapor
                  transport and its effect on deep water formation.},
	Author = {W. S. Broecker},
	Journal = {Science},
	Pages = {1582--1588},
	Title = {Thermohaline Circulation, the {A}chilles Heel of Our Climate System: Will Man-Made $Co_2$ Upset the Current Balance?},
	Volume = 278,
	Year = 1997}

@article{Broomhead86,
	Annote = {Filed under Singular Spectrum Analysis.},
	Author = {D. S. Broomhead and G. P. King},
	Journal = {Physica D},
	Pages = {217--236},
	Title = {Extracting qualitative dynamics from experimental data},
	Volume = 20,
	Year = 1986}

@article{Brown97,
	Author = {R. G. Brown and C. S. Bretherton},
	Journal = {J. Atmos. Sci.},
	Pages = {624--638},
	Title = {A test of the strict quasi-equilibrium theory on long time and space scales},
	Volume = 54,
	Year = 1997}

@article{Brunet95,
	Annote = {Filed under Isentropic Observations. PV on 315 K
                  isentrope.},
	Author = {G. Brunet and R. Vautard and B. Legras and S. Edouard},
	Journal = {Mon. Wea. Rev.},
	Pages = {1037--1058},
	Title = {Potential Vorticity on Isentropic Surfaces: Climatology and Diagnostics},
	Volume = 123,
	Year = 1995}

@article{Brunt33,
	Annote = {Filed under General Circulation History.},
	Author = {D. Brunt},
	File = {../../Papers/brunt33.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {351--360},
	Title = {The adiabatic lapse-rate for dry and saturated air},
	Volume = {???},
	Year = 1933,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgticnVudDMzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0UvztYIgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzu6kgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnJ1bnQzMy5wZGYADgAYAAsAYgByAHUAbgB0ADMAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYnJ1bnQzMy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9icnVudDMzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Bryan69,
	Annote = {Classic paper on numerical ocean models.},
	Author = {K. Bryan},
	Journal = {J. Comp. Phys.},
	Pages = {347--376},
	Title = {A Numerical Method for the Study of the Circulation of the World Ocean},
	Volume = 4,
	Year = 1969}

@article{Bryan87,
	Author = {F. Bryan},
	Journal = {J. Phys. Oceanogr.},
	Pages = {970--985},
	Title = {Parameter Sensitivity of Primitive Equation Ocean General Circulation Models},
	Volume = {17},
	Year = {1987}}

@article{Bryan99,
	Author = {K. Bryan and J. K. Dukowicz and R. D. Smith},
	Journal = {J. Phys. Oceanogr.},
	Pages = {2442--2456},
	Title = {On the Mixing Coefficient in the Parameterization of Bolus Velocity},
	Volume = 29,
	Year = 1999}

@article{Buck60,
	Annote = {Not on file. Imputation of conditional means.},
	Author = {S. F. Buck},
	Journal = {J. Roy. Stat. Soc. B},
	Pages = {302--306},
	Title = {A method of estimation of missing values in multivariate data suitable for use with an electronic computer},
	Volume = 22,
	Year = 1960}

@article{Buckingham14,
	Annote = {Classic paper on dimensional analysis.},
	Author = {E. Buckingham},
	Journal = {Pys. Rev.},
	Pages = {345--376},
	Title = {On Physically Similar Systems; {I}llustrations of the Use of Dimensional Equations},
	Volume = 4,
	Year = 1914}

@article{Buehler00,
	Author = {O. B{\"u}hler},
	Journal = {J. Fluid Mech.},
	Pages = {235--263},
	Title = {On the vorticity transport due to dissipating or breaking waves in shallow-water flow},
	Volume = 407,
	Year = 2000}

@article{Buehler98,
	Annote = {Overview of GLM theory.},
	Author = {O. B{\"u}hler and M. E. McIntyre},
	Journal = {J. Fluid Mech.},
	Pages = {301--343},
	Title = {On non-dissipative wave-mean interactions in the atmosphere or oceans},
	Volume = 354,
	Year = 1998}

@article{Buehler99,
	Author = {O. B{\"u}hler and P. H. Haynes},
	Journal = {J. Atmos. Sci.},
	Pages = {942--947},
	Title = {Constraints on the Mean Mass Transport Across Potential Vorticity Contours},
	Volume = 56,
	Year = 1999}

@incollection{Burg68a,
	Address = {New York},
	Annote = {Filed under AR Modeling.},
	Author = {J. P. Burg},
	Booktitle = {Modern Spectrum Analysis},
	Editor = {D. G. Childers},
	Pages = {34--41},
	Publisher = {{IEEE} Press},
	Title = {Maximum Entropy Spectral Analysis},
	Year = 1978}

@incollection{Burg68b,
	Address = {New York},
	Annote = {Filed under AR Modeling.},
	Author = {J. P. Burg},
	Booktitle = {Modern Spectrum Analysis},
	Editor = {D. G. Childers},
	Pages = {42--48},
	Publisher = {{IEEE} Press},
	Title = {A New Analysis Technique for Time Series Data},
	Year = 1978}

@article{Busse76,
	Author = {F. H. Busse},
	File = {../../Papers/busse76.pdf},
	Journal = {Icarus},
	Pages = {255--260},
	Title = {A simple model of convection in the {Jovian} atmosphere},
	Volume = 29,
	Year = 1976,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtidXNzZTc2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0Zw7uMJAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7v8pAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnVzc2U3Ni5wZGYADgAYAAsAYgB1AHMAcwBlADcANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYnVzc2U3Ni5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9idXNzZTc2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Busse78,
	Annote = {Filed under Rayleigh-Benard Convection. Review of
                  theory and experiments.},
	Author = {F. H. Busse},
	Journal = {Rep. Prog. Phys.},
	Pages = {1930--1967},
	Title = {Non-linear properties of thermal convection},
	Volume = 41,
	Year = 1978}

@article{Busse94,
	Annote = {Review of convection-driven zonal flows.},
	Author = {F. H. Busse},
	File = {../../Papers/busse94.pdf},
	Journal = {Chaos},
	Pages = {123--134},
	Title = {Convection driven zonal flows and vortices in the major planets},
	Volume = 4,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtidXNzZTk0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0bwtAc/1BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwtB/bwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6YnVzc2U5NC5wZGYADgAYAAsAYgB1AHMAcwBlADkANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvYnVzc2U5NC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9idXNzZTk0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Caballero05,
	Author = {R. Caballero and P. L. Langen},
	File = {../../Papers/caballero05.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2004GL021581},
	Pages = {L02705},
	Title = {The dynamic range of poleward energy transport in an atmospheric general circulation model},
	Volume = 32,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9jYWJhbGxlcm8wNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0cvkYPRgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvkZ/xgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2FiYWxsZXJvMDUucGRmAA4AIAAPAGMAYQBiAGEAbABsAGUAcgBvADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvY2FiYWxsZXJvMDUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvY2FiYWxsZXJvMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Caballero07,
	Author = {R. Caballero},
	File = {../../Papers/caballero07.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2008GL035084},
	Pages = {L18709},
	Title = {Role of eddies in the interannual variability of {H}adley cell strength},
	Volume = 34,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9jYWJhbGxlcm8wNy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0dw3WPRwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw3X/xwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2FiYWxsZXJvMDcucGRmAA4AIAAPAGMAYQBiAGEAbABsAGUAcgBvADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvY2FiYWxsZXJvMDcucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvY2FiYWxsZXJvMDcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Caballero08,
	Author = {R. Caballero},
	File = {../../Papers/caballero08.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2007GL030971},
	Pages = {L22705},
	Title = {Hadley cell bias in climate models linked to extratropical eddy stress},
	Volume = 34,
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9jYWJhbGxlcm8wOC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0exSamggAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxScI8gAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2FiYWxsZXJvMDgucGRmAA4AIAAPAGMAYQBiAGEAbABsAGUAcgBvADAAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvY2FiYWxsZXJvMDgucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvY2FiYWxsZXJvMDgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Caballero08b,
	Author = {R. Caballero and R.T. Pierrehumbert and J.L. Mitchell},
	File = {../../Papers/caballero08b.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1269--1285},
	Title = {Axisymmetric, nearly inviscid circulations in non-condensing radiative-convective atmospheres},
	Volume = 134,
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBjYWJhbGxlcm8wOGIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0fxfgvkQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxfiSAQAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2FiYWxsZXJvMDhiLnBkZgAADgAiABAAYwBhAGIAYQBsAGwAZQByAG8AMAA4AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL2NhYmFsbGVybzA4Yi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvY2FiYWxsZXJvMDhiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Caldeira92,
	Annote = {Filed under Snowball Earth.},
	Author = {K. Caldeira and J. F. Kasting},
	Journal = {Nature},
	Pages = {226--228},
	Title = {Susceptibility of the early {E}arth to irreversible glaciation caused by carbon dioxide clouds},
	Volume = 359,
	Year = 1992}

@article{Callis86,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {L. B. Callis and M. Natarajan},
	Journal = {J. Geophys. Res.},
	Pages = {10771--10796},
	Title = {The {A}ntarctic Ozone Minimum: {R}elationship to odd nitrogen, odd chlorine, the final warming, and the 11-year solar cycle},
	Volume = {91D},
	Year = 1986}

@article{Cambon97,
	Annote = {Filed under Turbulence Closure Theories.},
	Author = {C. Cambon and N. N. Mansour and F. S. Godeferd},
	Journal = {J. Fluid. Mech.},
	Pages = {303--332},
	Title = {Energy transfer in rotating turbulence},
	Volume = 337,
	Year = 1997}

@article{Cane81,
	Annote = {Not on file. Discusses eigenmodes of zonally
                  bounded, equatorial ocean basin.},
	Author = {M. A. Cane and D. W. Moore},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1578--1584},
	Title = {A Note on Low-Frequency Equatorial Basin Modes},
	Volume = 11,
	Year = 1981}

@article{Cane85,
	Annote = {Not on file. On the CZ intermediate coupled model.},
	Author = {M. A. Cane and S. E. Zebiak},
	Journal = {Science},
	Pages = {1084--1087},
	Title = {A Theory for {E}l {N}i{\~n}o and the {S}outhern {O}scillation},
	Volume = 228,
	Year = 1985}

@article{Cao95,
	Annote = {Conservation law for pv with equivalent potential
                  temperature. Used to diagnose cyclogenesis.},
	Author = {Z. Cao and H.-R Cho},
	File = {../../Papers/cao95.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3263--3281},
	Title = {Generation of Moist Potential Vorticity in Extratropical Cyclones},
	Volume = 52,
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgljYW85NS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0svEWTxAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvEYERAAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2FvOTUucGRmAA4AFAAJAGMAYQBvADkANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvY2FvOTUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvY2FvOTUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Carnevale01,
	Annote = {Large-eddy simulations of buoyancy-range
                  turbulence.},
	Author = {G. F. Carnevale and M. Briscolini and P. Orlandi},
	Journal = {J. Fluid Mech.},
	Pages = {205--239},
	Title = {Buoyancy- to inertial-range transition in forced stratified turbulence},
	Volume = 427,
	Year = 2001}

@article{Cash02,
	Annote = {Annular mode represents zonally homogeneous
                  distribution of localized events with a similar
                  meridional structure, rather than a zonally
                  symmetric mode of variability per se.},
	Author = {B. A. Cash and P. J. Kushner and G. K. Vallis},
	Journal = {J. Atmos. Sci.},
	Pages = {3399--3414},
	Title = {The structure and composition of the annular modes in an aquaplanet general circulation model},
	Volume = {59},
	Year = 2002}

@article{Cau05,
	Annote = {Filed under Water Vapor (Feedback and
                  Kinematics). Analysis of dry intrusions in Tropics,
                  including their radiative impact. Some dry
                  intrusions come from extratropics.},
	Author = {P. Cau and J. Methven and B. Hoskins},
	File = {../../Papers/cau05.pdf},
	Journal = {J. Geophys. Res.},
	Note = {doi:10.1029/2004JD004928},
	Pages = {D06110},
	Title = {Representation of dry tropical layers and their origins in {ERA-40} data},
	Volume = {110D},
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgljYXUwNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0wv3VOMQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3WwoQAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2F1MDUucGRmAA4AFAAJAGMAYQB1ADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvY2F1MDUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvY2F1MDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Chang02,
	Annote = {Review.},
	Author = {E. K. M. Chang and S. Lee and K. L. Swanson},
	File = {../../Papers/chang02.pdf},
	Journal = {J. Climate},
	Pages = {2163--2183},
	Title = {Storm Track Dynamics},
	Volume = 15,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtjaGFuZzAyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ06v+gdZQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv+iN5QAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhbmcwMi5wZGYADgAYAAsAYwBoAGEAbgBnADAAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvY2hhbmcwMi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9jaGFuZzAyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Chang07a,
	Author = {E. K. M. Chang and P. Zurita-Gotor},
	File = {../../Papers/chang07a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2309--2331},
	Title = {Simulating the Seasonal Cycle of the Northern Hemisphere Storm Tracks Using Idealized Nonlinear Storm-Track Models},
	Volume = 64,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxjaGFuZzA3YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ07wwTbDFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwwU9fAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhbmcwN2EucGRmAAAOABoADABjAGgAYQBuAGcAMAA3AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2NoYW5nMDdhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9jaGFuZzA3YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Chang95,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {E. K. M. Chang},
	Journal = {J. Atmos. Sci.},
	Pages = {2006--2024},
	Title = {The Influence of {H}adley Circulation Intensity Changes on Extratropical Climate in an Idealized Model},
	Volume = 52,
	Year = 1995}

@article{Chang96,
	Annote = {Doesn't discuss mass transport; doesn't use TEM.},
	Author = {E. K. M. Chang},
	Journal = {J. Atmos. Sci.},
	Pages = {113--125},
	Title = {Mean Meridional Circulation Driven by Eddy Forcings of Different Timescales},
	Volume = {53},
	Year = {1996}}

@article{Chao00,
	Annote = {Filed under Monsoon Dynamics. Interprets abrupt
                  transition to monsoon flow regime (abrupt shift of
                  ITCZ in response to gradual shift in SST maximum) in
                  terms of "forces" that pull the ITCZ toward the
                  equator (due to Coriolis forces) or toward the SST
                  maximum. (Interpretation and "forces" are very
                  vague, essentially diagnostic.) Shows transition in
                  GCM experiments. Transition depends on convection
                  scheme (see also Numaguti95).},
	Author = {W. C. Chao},
	File = {../../Papers/chao00.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {641--651},
	Title = {Multiple Quasi Equilibria of the {ITCZ} and the Origin of Monsoon Onset},
	Volume = 57,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpjaGFvMDAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ0/wAGfaFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwAIP6AAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhbzAwLnBkZgAADgAWAAoAYwBoAGEAbwAwADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2NoYW8wMC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvY2hhbzAwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Chao01,
	Annote = {Filed under Monsoon Dynamics. GCM experiments in
                  which selected continents are replaced by ocean or
                  in which topography in continental areas is
                  removed. Experiments show that land-sea contrast is
                  not necessary for existence of monsoons (loosely
                  defined, it appears, as precipitation region with
                  summer westerly component equatorward of it), but it
                  modifies the precipitation zones. Likewise,
                  topography is not essential for Indian monsoon, but
                  modifies it strongly (without topography and/or
                  land-sea contrast, however, the distribution of
                  Indian monsoon precipitation looks quite
                  different). Both topography and land-sea contrast
                  appear to be important for N. American monsoon.},
	Author = {W. C. Chao and B. Chen},
	File = {../../Papers/chao01.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3497--3507},
	Title = {The Origin of Monsoons},
	Volume = 58,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpjaGFvMDEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1Av/6qSQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv/8ayQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhbzAxLnBkZgAADgAWAAoAYwBoAGEAbwAwADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2NoYW8wMS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvY2hhbzAxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Charlson87,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {R. J. Charlson and J.E. Lovelock and M.O. Andreae and S.G. Warren},
	Journal = {Nature},
	Pages = {655--661},
	Title = {Oceanic phytoplankton, atmospheric sulphur, cloud albedo and climate},
	Volume = 326,
	Year = 1987}

@article{Charlson94,
	Author = {R. J. Charlson and T. M. L. Wigley},
	Journal = {Scientific American},
	Pages = {48--57},
	Title = {Sulfate Aerosol and Climatic Change},
	Volume = 270,
	Year = 1994}

@article{Charney47,
	Annote = {Charney's stability problem.},
	Author = {J. G. Charney},
	Journal = {J. Meteor.},
	Pages = {135--163},
	Title = {The dynamics of long waves in a baroclinic westerly current},
	Volume = 4,
	Year = 1947}

@article{Charney48,
	Annote = {??},
	Author = {J. G. Charney},
	Journal = {Geofys. Publ},
	Pages = {1--17},
	Title = {On the scale of atmospheric motions},
	Volume = 17,
	Year = 1948}

@incollection{Charney59a,
	Address = {New York},
	Author = {J. Charney},
	Booktitle = {The Atmosphere and the Sea in Motion},
	Editor = {B. Bolin},
	File = {../../Papers/charney59a.pdf},
	Pages = {178--193},
	Publisher = {Rockefeller Inst. Press},
	Title = {On the General Circulation of the Atmosphere},
	Year = 1959,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5jaGFybmV5NTlhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1DwpgghVBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwpiC9QAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhcm5leTU5YS5wZGYAAA4AHgAOAGMAaABhAHIAbgBlAHkANQA5AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2NoYXJuZXk1OWEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2NoYXJuZXk1OWEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Charney61,
	Author = {J. G. Charney and P. G. Drazin},
	File = {../../Papers/charney61.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {83--109},
	Title = {Propagation of Planetary-Scale Disturbances from the Lower into the Upper Atmosphere},
	Volume = 66,
	Year = 1961,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1jaGFybmV5NjEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1FxqGfbQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxqIB3QAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhcm5leTYxLnBkZgAOABwADQBjAGgAYQByAG4AZQB5ADYAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvY2hhcm5leTYxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2NoYXJuZXk2MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Charney62,
	Author = {J. G. Charney and M. E. Stern},
	File = {../../Papers/charney62.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {159--172},
	Title = {On the stability of internal baroclinic jets in a rotating atmosphere},
	Volume = 19,
	Year = 1962,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1jaGFybmV5NjIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1Gvk1qdgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvk3a9gAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhcm5leTYyLnBkZgAOABwADQBjAGgAYQByAG4AZQB5ADYAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvY2hhcm5leTYyLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2NoYXJuZXk2Mi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Charney63,
	Annote = {Proposes possible forcing of tropical atmosphere
                  from higher latitudes.},
	Author = {J. G. Charney},
	File = {../../Papers/charney63.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {607--609},
	Title = {A Note on Large-Scale Motions in the {T}ropics},
	Volume = 20,
	Year = 1963,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1jaGFybmV5NjMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1HwOz7VQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwO1dxQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhcm5leTYzLnBkZgAOABwADQBjAGgAYQByAG4AZQB5ADYAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvY2hhcm5leTYzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2NoYXJuZXk2My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Charney69,
	Annote = {Sequel to Charney63. Only Rossby waves with westward
                  phase speed greater than the zonal mean easterly
                  flow can propogate in Tropics.},
	Author = {J. G. Charney},
	File = {../../Papers/charney69.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {182--185},
	Title = {A Further Note on Large-Scale Motions in the {T}ropics},
	Volume = 26,
	Year = 1969,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1jaGFybmV5NjkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1IwOz72gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwO1eSgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhcm5leTY5LnBkZgAOABwADQBjAGgAYQByAG4AZQB5ADYAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvY2hhcm5leTY5LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2NoYXJuZXk2OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Charney71,
	Annote = {Arguments for energy and enstrophy cascades in
                  geostrophic turbulence.},
	Author = {J. G. Charney},
	File = {../../Papers/charney71.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1087--1095},
	Title = {Geostrophic turbulence},
	Volume = 28,
	Year = 1971,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1jaGFybmV5NzEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1JwZG4blBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwZIo7gAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhcm5leTcxLnBkZgAOABwADQBjAGgAYQByAG4AZQB5ADcAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvY2hhcm5leTcxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2NoYXJuZXk3MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@incollection{Charney71b,
	Address = {Providence, RI},
	Annote = {Filed under ITCZ Dynamics.},
	Author = {J. Charney},
	Booktitle = {Mathematical Problems in the Geophysical Sciences. 1. Geophysical Fluid Dynamics},
	Editor = {W. H. Reid},
	Pages = {355--368},
	Publisher = {American Math. Soc.},
	Series = {Lectures in Applied Mathematics},
	Title = {Tropical Cyclogenesis and the Formation of the Intertropical Convergence Zone},
	Volume = 13,
	Year = 1971}

@article{Charney79,
	Author = {J. G. Charney and J. G. DeVore},
	File = {../../Papers/charney79.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1205--1216},
	Title = {Multiple flow equilibria in the atmosphere and blocking},
	Volume = 36,
	Year = 1979,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1jaGFybmV5NzkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1Kwf65alBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwf8p6gAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hhcm5leTc5LnBkZgAOABwADQBjAGgAYQByAG4AZQB5ADcAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvY2hhcm5leTc5LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2NoYXJuZXk3OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Chavanis02,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {P.-H. Chavanis and J. Sommeria},
	Journal = {Phys. Rev. E},
	Pages = 026302,
	Title = {Statistical mechanics of the shallow water system},
	Volume = 65,
	Year = 2002}

@article{Chavanis03,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {P.-H. Chavanis},
	Journal = {Phys. Rev. E},
	Pages = 036108,
	Title = {Generalized thermodynamics and {Fokker}-{Planck} equations: {A}pplications to stellar dynamics and two-dimensional turbulence},
	Volume = 68,
	Year = 2003}

@article{Chavanis97,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {P.-H. Chavanis and J. Sommeria},
	Journal = {Phys. Rev. Lett.},
	Pages = {3302--3305},
	Title = {Thermodynamical Approach for Small-Scale Parameterization in 2D Turbulence},
	Volume = 78,
	Year = 1997}

@article{Cheinet03,
	Author = {Cheinet, S. and Teixeira, J.},
	File = {../../Papers/cheinet03.pdf},
	Journal = {Geophys. Rese. Lett.},
	Note = {doi:10.1029/2003GL017377},
	Pages = {1930},
	Title = {A simple formulation for the eddy-diffusivity parameterization of cloud-topped boundary layers},
	Volume = {30},
	Year = {2003},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1jaGVpbmV0MDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1Lx0gnugAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx0iYOgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hlaW5ldDAzLnBkZgAOABwADQBjAGgAZQBpAG4AZQB0ADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvY2hlaW5ldDAzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2NoZWluZXQwMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Chelton98,
	Annote = {First baroclinic Rossby radius computed from
                  stratification only is of order of energy-containing
                  eddy scale, sometimes smaller.},
	Author = {D. B. Chelton and R. A. deSzoeke and M. G. Schlax and K. El Naggar and N. Siwertz},
	File = {../../Papers/chelton98.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {433--460},
	Title = {Geographical variability of the first baroclinic {Rossby} radius of deformation},
	Volume = 28,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1jaGVsdG9uOTgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1MvcOzUwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvcQj0wAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hlbHRvbjk4LnBkZgAOABwADQBjAGgAZQBsAHQAbwBuADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvY2hlbHRvbjk4LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2NoZWx0b245OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Chen02,
	Annote = {Filed under Hadley Cell Dynamics. Based on satellite
                  radiation data, authors claim that Hadley cell has
                  strenghtened in the 1990s, with increase of
                  upper-tropospheric relative humidity in deep tropics
                  and decrease in subtropics.},
	Author = {J. Chen and B. E. Carlson and A. D. {Del Genio}},
	Journal = {Science},
	Pages = {838--841},
	Title = {Evidence for Strengthening of the Tropical General Circulation in the 1990s},
	Volume = 295,
	Year = 2002}

@article{Chen07b,
	Author = {Chen, G. and Held, I. M.},
	File = {../../Papers/chen07b.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2007GL031200},
	Pages = {{L}21805},
	Title = {Phase speed spectra and the recent poleward shift of {S}outhern {H}emisphere surface westerlies},
	Volume = {34},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtjaGVuMDdiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1Ow2ntKgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw2pdqgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hlbjA3Yi5wZGYADgAYAAsAYwBoAGUAbgAwADcAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvY2hlbjA3Yi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9jaGVuMDdiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Chen98,
	Annote = {Filed under Holm.},
	Author = {S. Chen and C. Foias and D. D. Holm and E. Olson and E. S. Titi and S. Wynne},
	Journal = {Phys. Rev. Lett.},
	Pages = {5338--5341},
	Title = {The Camassa--Holm equations as a clusure model for turbulent channel flow},
	Volume = 81,
	Year = 1998}

@article{Cheng92,
	Annote = {Filed under Discriminant Analysis. Considers rank
                  deficient scatter matrices.},
	Author = {Y.-Q. Cheng and Y.-M. Zhuang and J.-Y. Yang},
	Journal = {Pattern Recognition},
	Pages = {101--111},
	Title = {Optimal {F}isher Discriminant Analysis Using the Rank Decomposition},
	Volume = 25,
	Year = 1992}

@article{Chiang05,
	Author = {J. C. H. Chiang and C. M. Bitz},
	File = {../../Papers/chiang05.pdf},
	Journal = {Clim. Dyn.},
	Pages = {477--496},
	Title = {Influence of high latitude ice cover on the marine Intertropical Convergence Zone},
	Volume = {25},
	Year = {2005},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxjaGlhbmcwNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1TxgFE/gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxgGnbgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hpYW5nMDUucGRmAAAOABoADABjAGgAaQBhAG4AZwAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2NoaWFuZzA1LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9jaGlhbmcwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Cho96b,
	Annote = {Filed under Polvani.},
	Author = {J. Y.-K. Cho and L. M. Polvani},
	Journal = {Science},
	Pages = {335--337},
	Title = {The Morphogenesis of Bands and Zonal Winds in the Atmospheres on the Giant Outer Planets},
	Volume = 273,
	Year = 1996}

@article{Chorin78,
	Author = {A. J. Chorin},
	Journal = {J. Comp. Phys.},
	Pages = {428--442},
	Title = {Vortex Sheet Approximation of Boundary Layers},
	Volume = 27,
	Year = 1978}

@article{Chou01,
	Author = {Chou, C. and Neelin, J. D. and Su, H.},
	File = {../../Papers/chou01.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1869--1892},
	Title = {Ocean-atmosphere-land feedbacks in an idealized monsoon},
	Volume = 127,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpjaG91MDEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1XvVumEgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvVwIggAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hvdTAxLnBkZgAADgAWAAoAYwBoAG8AdQAwADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2Nob3UwMS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvY2hvdTAxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Chou01b,
	Author = {Chou, C. and Neelin, J. D.},
	Journal = {Geophys. Res. Lett.},
	Pages = {2433--2436},
	Title = {Mechanisms limiting the southward extent of the {S}outh {A}merican summer monsoon},
	Volume = 28,
	Year = 2001}

@article{Chou03,
	Author = {Chou, C. and Neelin, J. D.},
	File = {../../Papers/chou03.pdf},
	Journal = {J. Climate},
	Pages = {406--425},
	Title = {Mechanisms limiting the northward extent of the northern summer monsoons over {N}orth {A}merica, {A}sia, and {A}frica},
	Volume = 16,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpjaG91MDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1YvWXxigAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvWZT+gAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hvdTAzLnBkZgAADgAWAAoAYwBoAG8AdQAwADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2Nob3UwMy5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvY2hvdTAzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Chou04,
	Annote = {Filed under Neelin.},
	Author = {C. Chou and J. D. Neelin},
	File = {../../Papers/chou04.pdf},
	Journal = {J. Climate},
	Pages = {2688--2701},
	Title = {Mechanisms of Global Warming Impacts on Regional Tropical Precipitation},
	Volume = 17,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpjaG91MDQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1axXPd0AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxXROUAAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hvdTA0LnBkZgAADgAWAAoAYwBoAG8AdQAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2Nob3UwNC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvY2hvdTA0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Chou09,
	Annote = {Filed under Neelin.},
	Author = {C. Chou and J. D. Neelin and C.-A. Chen and J.-Y. Tu},
	File = {../../Papers/chou09.pdf},
	Journal = {J. Climate},
	Pages = {1982--2005},
	Title = {Evaluating the ``Rich-Get-Richer'' Mechanism in Tropical Precipitation Change under Global Warming},
	Volume = 22,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpjaG91MDkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1cxi4TYgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxi510gAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2hvdTA5LnBkZgAADgAWAAoAYwBoAG8AdQAwADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2Nob3UwOS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvY2hvdTA5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Chu95,
	Annote = {Filed under Predictability.},
	Author = {P.-S. Chu and R. W. Katz and P. Ding},
	Journal = {Int. J. Climatology},
	Pages = {53--64},
	Title = {Modelling and Forecasting Seasonal Precipitation in {F}lorida: A Vector Time-domain Approach},
	Volume = 15,
	Year = 1995}

@article{Chuang97,
	Annote = {Filed under Climate Change Detection.},
	Author = {C. C. Chuang and J. E. Penner and K. E. Taylor and A. S. Grossman and J. J. Walton},
	Journal = {J. Geophys. Res.},
	Pages = {3761--3778},
	Title = {An assessment of the radiative effects of anthropogenic sulfate},
	Volume = {102D},
	Year = 1997}

@inproceedings{Chubachi85,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {S. Chubachi},
	Booktitle = {Atmospheric Ozone},
	Editor = {C. S. Zerefos and A. M. Ghazi},
	Note = {Proceedings of the Quadrennial Ozone Symposium held in Halkidiki, Greece, 3--7 September 1984.},
	Pages = {285--289},
	Title = {A special ozone observation at {S}yowa {S}tation, {A}ntarctica from {F}ebruary 1982 to {J}anuary 1983},
	Year = 1985}

@article{Clement01,
	Annote = {Abrupt phase locking between ENSO and seasonal cycle
                  can change tropical SST and global climate. In
                  Cane-Zebiak model of ENSO, phase locking to seasonal
                  cycle likely with orbital parameters corresponding
                  to Younger Dryas conditions. Speculate that shutdown
                  in ENSO is responsible for Younger Dryas cooling.},
	Author = {A. C. Clement and M. A. Cane and R. Seager},
	Journal = {J. Climate},
	Pages = {2369--2375},
	Title = {An orbitally driven Tropical Source for Abrupt Climate Change},
	Volume = 14,
	Year = 2001}

@article{Clement06,
	Annote = {Filed under Hadley Cell Dynamics. In simulation
                  without ocean heat transport, main
                  ascent of Hadley cell remains closer to
                  equator than in simulation with OHT. However, this
                  result may be an artifact: the Tropics in a
                  simulation without OHT are *cooler* than in a
                  simulation with ocean heat transport (apparently due
                  to change in stratus cloud cover) and do not develop
                  off-equatorial surface temperature maximum (i.e.,
                  weaker or no monsoons).},
	Author = {A. C. Clement},
	File = {../../Papers/clement06.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3351--3365},
	Title = {The Role of the Ocean in the Seasonal Cycle of the {H}adley Circulation},
	Volume = 63,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1jbGVtZW50MDYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1fwbqsv1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwbsdPwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2xlbWVudDA2LnBkZgAOABwADQBjAGwAZQBtAGUAbgB0ADAANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvY2xlbWVudDA2LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2NsZW1lbnQwNi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Clement99,
	Author = {A. C. Clement and R. Seager and M. A. Cane},
	File = {../../Papers/clement99.pdf},
	Journal = {Paleoceanogr.},
	Pages = {441--456},
	Title = {Orbital controls on the {El~Ni{\~n}o}/{S}outhern {O}scillation and tropical climate},
	Volume = 14,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1jbGVtZW50OTkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1jxUC/2gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxUEwWgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y2xlbWVudDk5LnBkZgAOABwADQBjAGwAZQBtAGUAbgB0ADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvY2xlbWVudDk5LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2NsZW1lbnQ5OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Clerc01,
	Annote = {Filed under Marsden.},
	Author = {M. G. Clerc and J. E. Marsden},
	Journal = {Phys. Rev. E},
	Pages = 067603,
	Title = {Dissipation-induced instabilities in an optical cavity laser: A mechanical analog near the 1:1 resonance},
	Volume = 64,
	Year = 2001}

@article{Codoban03,
	Annote = {Filed under Shepherd and Hamiltonian Balanced
                  Dynamics. Extension of available potential energy
                  concept to include momentum constraints.},
	Author = {S. Codoban and T. G. Shepherd},
	Journal = {J. Atmos. Sci.},
	Pages = {2019--2028},
	Title = {Energetics of a Symmetric Circulation Including Momentum Constraints},
	Volume = 60,
	Year = 2003}

@article{Cohen00,
	Annote = {Not on file.},
	Author = {J. L. Cohen and D. A. Salstein and R. D. Rosen},
	Journal = {J. Hydrometeor.},
	Pages = {547--553},
	Title = {Interannual variability in the meridional transport of water vapor},
	Volume = 6,
	Year = 2000}

@article{Cohen96,
	Annote = {Filed under Wavelets.},
	Author = {A. Cohen and J. Kova\v{c}evi\'c},
	Journal = {Proc. IEEE},
	Pages = {514--522},
	Title = {Wavelets: {T}he Mathematical Background},
	Volume = {84},
	Year = {1996}}

@article{Conrath98,
	Author = {Conrath, B.J. and Gierasch, P.J. and Ustinov, E.A.},
	File = {../../Papers/conrath98.pdf},
	Journal = {Icarus},
	Number = {2},
	Pages = {501--517},
	Title = {Thermal Structure and Para Hydrogen Fraction on the Outer Planets from {Voyager} {IRIS} Measurements},
	Volume = {135},
	Year = {1998},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1jb25yYXRoOTgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1nxFhkFAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxFjGhAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y29ucmF0aDk4LnBkZgAOABwADQBjAG8AbgByAGEAdABoADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvY29ucmF0aDk4LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2NvbnJhdGg5OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Cook03a,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {K. H. Cook},
	Date-Modified = {2010-06-23 00:22:19 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {957--976},
	Title = {Role of Continents in Driving the Hadley Cells},
	Volume = 60,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtjb29rMDNhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1oyEcEFgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEdmhgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y29vazAzYS5wZGYADgAYAAsAYwBvAG8AawAwADMAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvY29vazAzYS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9jb29rMDNhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Cook92,
	Annote = {Filed under Held.},
	Author = {K. H. Cook and I. M. Held},
	Journal = {J. Atmos. Sci.},
	Pages = {525--539},
	Title = {The Stationary Response to Large-Scale Orography in a General Circulation Model and a Linear Model},
	Volume = 49,
	Year = 1992}

@article{Corbeil76,
	Annote = {Filed under Parameter Estimation.},
	Author = {R.~R. Corbeil and S.~R. Searle},
	Journal = {Technometrics},
	Key = {parameter estimation},
	Pages = {31--38},
	Title = {Restricted Maximum Lielihood Estimation of Variance Components in the Mixed Model},
	Volume = 18,
	Year = 1976}

@incollection{Corrsin74,
	Annote = {Conditions on mean-flow fields when diffusive
                  turbulence closure might be appropriate},
	Author = {S. Corrsin},
	Booktitle = {Advances in Geophysics},
	Pages = {25--60},
	Publisher = {Academic Press},
	Title = {Limitations of Gradient Transport Models in Random Walks and in Turbulence},
	Volume = {18A},
	Year = 1974}

@article{Corti99,
	Annote = {Not on file.},
	Author = {S. Corti and F. Molteni and T. N. Palmer},
	Journal = {Nature},
	Pages = {799-802},
	Title = {Signature of recent climate change in frequencies of natural atmospheric circulation regimes},
	Volume = 398,
	Year = 1999}

@article{Couhert10a,
	Author = {A. Couhert and T. Schneider and J. Li and D. E. Waliser and A. M. Tompkins},
	Date-Modified = {2010-06-18 16:06:51 -0700},
	Journal = {J. Climate},
	Pages = {390--403},
	Title = {The Maintenance of the Relative Humidity of the Subtropical Free Troposphere},
	Volume = 23,
	Year = 2010,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5jb3VoZXJ0MTBhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1qx2eZdgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx2gJ9gAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y291aGVydDEwYS5wZGYAAA4AHgAOAGMAbwB1AGgAZQByAHQAMQAwAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2NvdWhlcnQxMGEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2NvdWhlcnQxMGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Courtier94,
	Author = {P. Courtier and J.-N. Th{\'e}paut and A. Hollingsworth},
	File = {../../Papers/courtier94.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1367--1387},
	Title = {A strategy for operational implementation of {4D-Var}, using an incremental approach},
	Volume = {120},
	Year = {1994},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5jb3VydGllcjk0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1rxoC62wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxoEdSwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Y291cnRpZXI5NC5wZGYAAA4AHgAOAGMAbwB1AHIAdABpAGUAcgA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2NvdXJ0aWVyOTQucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2NvdXJ0aWVyOTQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Cressie93,
	Annote = {Filed under REML Asymptotics.},
	Author = {N. Cressie and S. N. Lahiri},
	Journal = {J. Multivariate Anal.},
	Pages = {217--233},
	Title = {The Asymptotic Distribution of {REML} Estimators},
	Volume = 45,
	Year = 1993}

@article{Crutzen70,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {P. J. Crutzen},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {320--325},
	Title = {The influence of nitrogen oxides on the atmospheric ozone content},
	Volume = 96,
	Year = 1970}

@article{Cuffey00a,
	Author = {K. M. Cuffey and H. Conway and A. M. Gades and B. Hallet and R. Lorrain and J. P. Severinghaus and E. J. Steig and B. Vaughn and J. W. C. White},
	Journal = {Geology},
	Pages = {351--354},
	Title = {Entrainment of cold glacier beds},
	Volume = 28,
	Year = 2000}

@article{Cuffey00b,
	Author = {K. M. Cuffey and S. J. Marshall},
	Journal = {Nature},
	Pages = {591--594},
	Title = {Substantial contribution to sea-level rise during the last interglacial from the Greenland ice sheet},
	Volume = 404,
	Year = 2000}

@article{Cuffey00c,
	Author = {K. M. Cuffey},
	Journal = {Geophys. Res. Lett.},
	Pages = {3065--3068},
	Title = {Methodology for Use of Isotopic Climate Forcings in Ice Sheet Models},
	Volume = 27,
	Year = 2000}

@article{Cuffey00d,
	Author = {K. M. Cuffey and H. Conway and A. Gades and B. Hallet and C. F. Raymond and S. Whitlow},
	Journal = {J. Geophys. Res.},
	Pages = {27895--27915},
	Title = {Deformation properties of subfreezing glacier ice: Role of crystal size, chemical impurities, and rock particles inferred from in situ measurements},
	Volume = {105B},
	Year = 2000}

@article{Cuffey01,
	Author = {K. M. Cuffey and F. Vimeux},
	Journal = {Nature},
	Pages = {523--527},
	Title = {Covariation of carbon dioxide and temperature from the {Vostok} ice core after deuterium-excess correction},
	Volume = 412,
	Year = 2001}

@article{Cuffey95,
	Author = {K. M. Cuffey and G. D. Clow and R. B. Alley and M. Stuiver and E. D. Waddington and R. W. Saltus},
	Journal = {Science},
	Pages = {455--458},
	Title = {Large {Arctic} Temperature Change at the {Wisconsin}-{Holocene} Glacial Transition},
	Volume = 270,
	Year = 1995}

@article{Cuffey97,
	Author = {K. M. Cuffey and G. D. Clow},
	Journal = {J. Geophys. Res.},
	Pages = {26383--26396},
	Title = {Temperature, accumulation, and ice sheet elevation in central {Greenland} through the last deglacial transition},
	Volume = {102C},
	Year = 1997}

@article{Cullen02,
	Author = {M. J. P. Cullen},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1623--2639},
	Title = {Large scale non-turbulent dynamics in the atmosphere},
	Volume = 128,
	Year = 2002}

@article{Czaja01,
	Author = {A. Czaja and J. Marshall},
	Journal = {Quart. J. Roy. Meteor. Soc},
	Pages = {1893--1916},
	Title = {Observations of atmosphere--ocean coupling in the {N}orth {A}tlantic},
	Volume = 127,
	Year = 2001}

@article{Dai01,
	Annote = {Filed under Climate Change Projections. Strength of
                  Hadley cell decreases in 21th century, along with
                  decrease in extratropical eddy activity.},
	Author = {A. Dai and T. M. L. Wigley and B. A. Boville and J. T. Kiehl and L. E. Buja},
	File = {../../Papers/dai01.pdf},
	Journal = {J. Climate},
	Pages = {485--519},
	Title = {Climates of the Twentieth and Twenty-First Centuries Simulated by the {NCAR} Climate System Model},
	Volume = 14,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglkYWkwMS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1xv9syDAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv9uijAAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGFpMDEucGRmAA4AFAAJAGQAYQBpADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvZGFpMDEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvZGFpMDEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Dai99,
	Author = {A. Dai and F. Giorgi and K. E. Trenberth},
	File = {../../Papers/dai99.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {6377--6402},
	Title = {Observed and model-simulated diurnal cycles of precipitation over the contiguous {U}nited {S}tates},
	Volume = 104,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglkYWk5OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1ywqAxTAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwqCTvAAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGFpOTkucGRmAA4AFAAJAGQAYQBpADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvZGFpOTkucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvZGFpOTkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@book{Daley91,
	Author = {R. Daley},
	Pages = 457,
	Publisher = {Cambridge University Press},
	Series = {Cambridge Atmospheric and Space Science Series},
	Title = {Atmospheric Data Analysis},
	Volume = 2,
	Year = 1991}

@article{Danielsen82,
	Annote = {Not on file. Tropical tropopause determined by
                  cumolonimbus convection.},
	Author = {E. F. Danielsen},
	Journal = {Geophys. Res. Lett.},
	Pages = {605--608},
	Title = {A dehydration mechanism for the stratosphere},
	Volume = 9,
	Year = 1982}

@article{Danilov01,
	Annote = {Filed under Gryanik.},
	Author = {S. D. Danilov and V. M. Gryanik and D. J. Olbers},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1075--1087},
	Title = {Equilibration and Lateral Spreading of a Strip-Shaped Convective Region},
	Volume = 31,
	Year = 2001}

@article{Danilov02,
	Annote = {Similar to Smith et al. 2002.},
	Author = {S. Danilov and D. Gurarie},
	File = {../../Papers/danilov02.pdf},
	Journal = {Phys. Rev. E},
	Note = {art.\ no.\ 067301},
	Title = {Rhines scale and spectra of the $\beta$-plane turbulence with bottom drag},
	Volume = 65,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1kYW5pbG92MDIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ1zxAhJygAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxAisOgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGFuaWxvdjAyLnBkZgAOABwADQBkAGEAbgBpAGwAbwB2ADAAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZGFuaWxvdjAyLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2Rhbmlsb3YwMi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Danilov04,
	Annote = {Filed under 2D Turbulence.},
	Author = {S. D. Danilov and V. M. Gryanik},
	Journal = {J. Atmos. Sci.},
	Pages = {2283--2295},
	Title = {Barotropic beta-plane turbulence in a regime with strong zonal jets revisited},
	Volume = 61,
	Year = 2004}

@article{Das05,
	Annote = {Filed under Stochastic Lagrangian Models of Turbulence.},
	Author = {S. K. Das and P. A. Durbin},
	File = {../../Papers/das05.pdf},
	Journal = {Phys. Fluids},
	Pages = {025109-1--10},
	Title = {A {L}agrangian stochastic model for dispersion in stratified turbulence},
	Volume = 17,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglkYXMwNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ10v5GYglBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5IJAgAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGFzMDUucGRmAA4AFAAJAGQAYQBzADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvZGFzMDUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvZGFzMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Daubechies88,
	Annote = {Classic paper on wavelet bases.},
	Author = {I. Daubechies},
	Journal = {Comm. Pure. Appl. Math.},
	Pages = {909-996},
	Title = {Orthonormal Bases of Compactly Supported Wavelets},
	Volume = 41,
	Year = 1988}

@unpublished{Daubechies96,
	Annote = {Additional material filed under Wavelets. Her SIAM
                  1992 book is good reference for course material.},
	Author = {I. Daubechies},
	Note = {Lecture Notes},
	Title = {Wavelet Analysis},
	Year = {Spring 1996}}

@article{Defant21,
	Annote = {Filed under General Circulation History. Eddies
                  transport heat to higher latitudes.},
	Author = {A. Defant},
	File = {../../Papers/defant21.pdf},
	Journal = {Geograf. Ann.},
	Pages = {209--266},
	Title = {Die {Z}irkulation der {A}tmosph{\"a}re in den gem{\"a}ssigten {B}reiten der {E}rde: Grundz{\"u}ge einer {T}heorie der {K}limaschwankungen},
	Volume = 3,
	Year = 1921,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxkZWZhbnQyMS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ12vuXknwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvuZHDwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGVmYW50MjEucGRmAAAOABoADABkAGUAZgBhAG4AdAAyADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2RlZmFudDIxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9kZWZhbnQyMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{DelGenio07,
	Author = {A. D. {Del Genio} and J. M. Barbara and J. Ferrier and A. P. Ingersoll and R. A. West and A. R. Vasavada and J. Spitale and C. C. Porco},
	File = {../../Papers/delgenio07.pdf},
	Journal = {Icarus},
	Pages = {479--492},
	Title = {Saturn eddy momentum fluxes and convection: First estimates from {Cassini} images},
	Volume = {189},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5kZWxnZW5pbzA3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ13xHior1BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxHkLHwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGVsZ2VuaW8wNy5wZGYAAA4AHgAOAGQAZQBsAGcAZQBuAGkAbwAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2RlbGdlbmlvMDcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2RlbGdlbmlvMDcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{DelGenio94,
	Annote = {Eddies dominate water vapor transport into
                  extratropics in GCM.},
	Author = {A. D. {DelGenio}},
	Journal = {Geophys. Res. Lett.},
	Pages = {2701--2704},
	Title = {Climatic implications of the seasonal variation of upper troposphere water vapor},
	Volume = 21,
	Year = 1994}

@article{DelSole01a,
	Author = {T. {DelSole}},
	Journal = {J. Atmos. Sci.},
	Pages = {3762--3775},
	Title = {A theory for the forcing and dissipation in stochastic turbulence models},
	Volume = 58,
	Year = 2001}

@article{DelSole01b,
	Author = {T. {DelSole}},
	Journal = {J. Atmos. Sci.},
	Pages = {3019--3035},
	Title = {A Simple Model for the Transient Eddy Momentum Fluxes in the Upper Troposphere},
	Volume = 58,
	Year = 2001}

@article{DelSole03a,
	Annote = {See also Reviews.},
	Author = {T. {DelSole} and P. Chang},
	Journal = {J. Atmos. Sci.},
	Pages = {409--416},
	Title = {Predictable Component Analysis, Canonical Correlation Analysis, and Autoregressive Models},
	Volume = 60,
	Year = 2003}

@article{DelSole03b,
	Annote = {Review of linear stochastic models of QG turbulence:
                  stochastic optimals, non-normals growth, etc.},
	Author = {T. {DelSole}},
	Journal = {Surveys Geophys.},
	Pages = {??},
	Title = {Stochastic Models of Quasigeostrophic Turbulence},
	Volume = {??},
	Year = 2003}

@article{DelSole95,
	Author = {T. {DelSole} and B. F. Farrell},
	Journal = {J. Atmos. Sci.},
	Pages = {2531--2547},
	Title = {A stochastically excited linear system as a model for {QG} turbulence: Analytical results for one and two-layer fluids},
	Volume = 52,
	Year = 1995}

@article{DelSole96a,
	Annote = {Filed under Stochastic Dynamics of Storm Tracks.},
	Author = {T. {DelSole} and B. F. Farrell},
	Journal = {J. Atmos. Sci.},
	Pages = {1781--1797},
	Title = {The Quasi-Linear Equilibration of a Thermally Maintained, Stochastically Excited Jet in a Quasigeostrophic Model},
	Volume = 53,
	Year = 1996}

@article{DelSole96b,
	Annote = {Tries to fit continuous analog of {ARMA} model to
                  turbulent jet.},
	Author = {T. {DelSole}},
	Journal = {J. Atmos. Sci.},
	Pages = {1617--1633},
	Title = {Can Quasigeostrophic Turbulence be Modeled Stochastically?},
	Volume = 53,
	Year = 1996}

@article{Delworth00a,
	Annote = {Not on file. Comparison between observations and
                  simulations of oscillation in North
                  Atlantic. Cf. Delworth93, Kushnir94.},
	Author = {T. L. Delworth and M. E. Mann},
	Journal = {Climate Dyn.},
	Pages = {661--676},
	Title = {Observed and simulated multidecadal variability in the {N}orthern {H}emisphere},
	Volume = {16},
	Year = 2000}

@article{Delworth00b,
	Annote = {Filed under Climate Change Detection.},
	Author = {T. L. Delworth and T. R. Knutson},
	Journal = {Science},
	Pages = {2246--2250},
	Title = {Simulation of Early 20th Century Global Warming},
	Volume = 287,
	Year = 2000}

@article{Delworth93,
	Annote = {Filed under Manabe.},
	Author = {T. Delworth and S. Manabe and R. J. Stouffer},
	Journal = {J. Climate},
	Pages = {1993--2011},
	Title = {Interdecadal Variations of the Thermohaline Circulation in a Coupled Ocean-Atmosphere Model},
	Volume = {6},
	Year = {1993}}

@article{Delworth97,
	Annote = {Not on file.},
	Author = {T. L. Delworth and S. Manabe and R. J. Stouffer},
	Journal = {Geophys. Res. Lett.},
	Pages = {257--260},
	Title = {Multidecadal Climate Variability in the {G}reenland {S}eas and Surrounding Regions: A Coupled Model Simulation},
	Volume = 24,
	Year = 1997}

@article{Deming97,
	Author = {Deming, D. and Reuter, D. and Jennings, D. and Bjoraker, G. and McCabe, G. and Fast, K. and Wiedemann, G.},
	File = {../../Papers/deming97.pdf},
	Journal = {Icarus},
	Pages = {301--312},
	Title = {Observations and Analysis of Longitudinal Thermal Waves on {Jupiter}},
	Volume = {126},
	Year = {1997},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxkZW1pbmc5Ny5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2FxJlhcQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxJnD4QAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGVtaW5nOTcucGRmAAAOABoADABkAGUAbQBpAG4AZwA5ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2RlbWluZzk3LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9kZW1pbmc5Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Dempster77,
	Annote = {Not on File.},
	Author = {A. P. Dempster and N. M. Laird and D. B. Rubin},
	Journal = {J. Roy. Stat. Soc. B},
	Pages = {1--38},
	Title = {Maximum likelihood estimation from incomplete data via the {EM} algorithm (with discussion)},
	Volume = 39,
	Year = 1977}

@article{Dempster84,
	Annote = {Filed under Parameter Estimation},
	Author = {A. P. Dempster and C.~M. Patel and M.~R. Selwyn and A.~J. Roth},
	Journal = {Appl. Statist.},
	Pages = {203--214},
	Title = {Statistical and Computational Aspects of Mixed Model Analysis},
	Volume = 33,
	Year = 1984}

@article{Dempster98,
	Annote = {Filed under Climate Change Detection. Argues from a
                  logicist point of view for subjectivity in applied
                  statistics. Discussion and critique of work in
                  climate change detection literature. Considers
                  distinction between signal and noise
                  misleading. Finds the use of GCM-inferred natural
                  variability statistics in regression model
                  troubling.},
	Author = {A. P. Dempster},
	File = {../../Papers/dempster98.pdf},
	Journal = {Statist. Sci.},
	Pages = {248--276},
	Title = {Logicist Statistics {I}. {M}odels and Modeling},
	Volume = 13,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5kZW1wc3Rlcjk4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2GwTsU0AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwTt3QAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGVtcHN0ZXI5OC5wZGYAAA4AHgAOAGQAZQBtAHAAcwB0AGUAcgA5ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2RlbXBzdGVyOTgucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2RlbXBzdGVyOTgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Deser96,
	Annote = {Not on file.},
	Author = {C. Deser and M. A. Alexander and M. S. Timlin},
	Journal = {J. Climate},
	Pages = {1840--1855},
	Title = {Upper-ocean thermal variations in the {N}orth {P}acific during 1970--1991},
	Volume = 9,
	Year = 1996}

@article{Dessler00,
	Author = {A. E. Dessler and S. C. Sherwood},
	Journal = {J. Geophys. Res.},
	Pages = {20155--20163},
	Title = {Simulations of Tropical Upper Tropospheric Humidity},
	Volume = {105D},
	Year = 2000}

@article{Dessler07,
	Annote = {Filed under Water Vapor (Feedback and Kinematics).},
	Author = {A. E. Dessler and K. Minschwaner},
	File = {../../Papers/dessler07.pdf},
	Journal = {J. Geophys. Res.},
	Note = {doi:10.1029/2006JD007683},
	Pages = {D10120},
	Title = {An analysis of the regulation of tropical tropospheric water vapor},
	Volume = {112},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1kZXNzbGVyMDcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2KwsEi9gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsGFZgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGVzc2xlcjA3LnBkZgAOABwADQBkAGUAcwBzAGwAZQByADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZGVzc2xlcjA3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2Rlc3NsZXIwNy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Dewar03,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {R. Dewar},
	File = {../../Papers/dewar03.pdf},
	Journal = {J. Phys. A},
	Pages = {631--641},
	Title = {Information Theory Explanation of the Fluctuation Theorem, Maximum Entropy Production and Self-Organized Criticality in Non-Equilibrium Stationary States},
	Volume = 36,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtkZXdhcjAzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2MvzlVIAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzm3kAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGV3YXIwMy5wZGYADgAYAAsAZABlAHcAYQByADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvZGV3YXIwMy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9kZXdhcjAzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{DiBattista00,
	Annote = {Filed under Majda.},
	Author = {M. T. DiBattista and A. J. Majda},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1325--1353},
	Title = {An Equilibrium Statistical Theory for Large-Scale Features of Open-Ocean Convection},
	Volume = 30,
	Year = 2000}

@article{DiBattista98,
	Annote = {Filed under Majda.},
	Author = {M. T. DiBattista and A. J. Majda and B. Turkington},
	Journal = {Geophys. Astrophys. Fluid Dynamics},
	Pages = {235--283},
	Title = {Prototype Geophysical Vortex Structures Via Large-Scale Statistical Theory},
	Volume = 89,
	Year = 1998}

@article{Dickinson71,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {R. E. Dickinson},
	File = {../../Papers/dickinson71.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {501--510},
	Title = {Analytic Model for Zonal Winds in the {T}ropics: {I.} {D}etails of the Model and Simulation of Gross Features of the Zonal Mean Troposphere},
	Volume = 99,
	Year = 1971,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9kaWNraW5zb243MS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2Pvwrq4gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvwtNUgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGlja2luc29uNzEucGRmAA4AIAAPAGQAaQBjAGsAaQBuAHMAbwBuADcAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZGlja2luc29uNzEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZGlja2luc29uNzEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@incollection{Dickinson96,
	Address = {Cambridge, UK},
	Author = {R. E. Dickinson and V. Meleshko and D. Randall and E. Sarachik and P. Silva-Dias},
	Booktitle = {Climate Change 1995: The Science of Climate Change},
	Editor = {J. T. Houghton and L. G. {Meira Filho} and B. A. Callander and N. Harris and A. Kattenberg and K. Maskell},
	Pages = {193--227},
	Publisher = {Intergovernmental Panel on Climate Change, Cambridge University Press},
	Title = {Climate Processes},
	Year = 1996}

@article{Dijkstra95,
	Annote = {Not on file.},
	Author = {H. A. Dijkstra and J. D. Neelin},
	Journal = {J. Climate},
	Pages = {1343--1359},
	Title = {Ocean-Atmosphere Interaction and the Tropical Climatology. {P}art {II}: {W}hy the {P}acific Cold Tongue is in the east},
	Volume = 8,
	Year = 1995}

@article{Dijkstra99,
	Annote = {Filed under Neelin. Flux correction can force the
                  existence of spurious multiple equilibria.},
	Author = {H. A. Dijkstra and J. D. Neelin},
	Journal = {J. Climate},
	Pages = {1382--1392},
	Title = {Imperfections of the Thermohaline Circulation: {M}ultiple Equilibria and Flux Correction},
	Volume = 12,
	Year = 1999}

@article{Dima03,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {I. M. Dima and J. M. Wallace},
	File = {../../Papers/dima03.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1522--1527},
	Title = {On the seasonality of the {H}adley cell},
	Volume = 60,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpkaW1hMDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2RvQiFIAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvQjnkAAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGltYTAzLnBkZgAADgAWAAoAZABpAG0AYQAwADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2RpbWEwMy5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvZGltYTAzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Dima05,
	Author = {I. M. Dima and J. W. Wallace and I. Kraucunas},
	File = {../../Papers/dima05.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2499--2513},
	Title = {Tropical Zonal Momentum Balance in the {NCEP} Reanalyses},
	Volume = 62,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpkaW1hMDUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2TxbXr5AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxbZcZAAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZGltYTA1LnBkZgAADgAWAAoAZABpAG0AYQAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2RpbWEwNS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvZGltYTA1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Dimotakis00,
	Author = {P. E. Dimotakis},
	Journal = {J. Fluid Mech.},
	Pages = {69--98},
	Title = {The mixing transition in turbulent flows},
	Volume = 409,
	Year = 2000}

@article{Dimotakis86,
	Author = {P. E. Dimotakis},
	Journal = {AIAA Journal},
	Pages = {1791--1796},
	Title = {Two-dimensional shear-layer entrainment},
	Volume = 24,
	Year = 1986}

@incollection{Dimotakis91,
	Address = {Washington, DC},
	Author = {P. E. Dimotakis},
	Booktitle = {High-Speed Flight Propulsion Systems},
	Editor = {S. N. B. Murthy and E. T. Curran},
	Publisher = {AIAA},
	Series = {Progress in Astronautics and Aeronautics},
	Title = {Turbulent free shear layer mixing and combustion},
	Volume = 137,
	Year = 1991}

@article{Ding03,
	Annote = {Filed under Lee Vortex Generation.},
	Author = {L. Ding and R. L. Street},
	Journal = {J. Atmos. Sci.},
	Pages = {1678--1690},
	Title = {Numerical Study of the Wake Structure behind a Three-Dimensional Hill},
	Volume = 60,
	Year = 2003}

@article{Dixon99,
	Annote = {Filed under Climate Change Detection.},
	Author = {K. W. Dixon and J. R. Lanzante},
	Journal = {Geophys. Res. Lett.},
	Pages = {1885--1888},
	Title = {Global mean surface air temperature and {N}orth {A}tlantic overturning in a suite of coupled {GCM} climate change experiments},
	Volume = 26,
	Year = 1999}

@article{Dmitriev73,
	Annote = {Filed under Entropy Estimation. Entropy estimation
                  using kernel estimators},
	Author = {Y. G. Dmitriev and F. P. Tarasenko},
	Journal = {Theory Probab. Appl.},
	Pages = {628--633},
	Title = {On the Estimation of Functionals of the Probability Density and its Derivatives},
	Volume = 18,
	Year = 1973}

@article{Dodd97,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {J. P. Dodd and I. N. James},
	File = {../../Papers/dodd97.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1763--1770},
	Title = {The impact of latent-heat release on the {H}adley circulation},
	Volume = 123,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpkb2RkOTcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2XvwF8/gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvwHfbgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZG9kZDk3LnBkZgAADgAWAAoAZABvAGQAZAA5ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2RvZGQ5Ny5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvZG9kZDk3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Donahue98,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {N. M. Donahue and J. G. Anderson and K. L. Demerjian},
	Journal = {J. Phys. Chem. A},
	Pages = {3121--3126},
	Title = {New rate constants for ten {OH} alkane reactions from 300 to 400~K: {A}n assessment of accuracy},
	Volume = 102,
	Year = 1998}

@article{Donivan69,
	Author = {F. F. Donivan and T. D. Carr},
	Journal = {Astrophys. J.},
	Pages = {L65--L68},
	Title = {Jupiter's decametric rotation period},
	Volume = {157},
	Year = {1969}}

@unpublished{Donner97,
	Annote = {Mostly following the
                  books by Iribane & Godson and Emanuel.},
	Author = {L. Donner},
	Note = {Class notes},
	Title = {Thermodynamics and Convection},
	Year = 1997}

@article{Dowling89,
	Annote = {Filed under Ingersoll.},
	Author = {T. E. Dowling and A. P. Ingersoll},
	File = {../../Papers/dowling89.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3256--3278},
	Title = {Jupiter's {G}reat {R}ed {S}pot as a Shallow Water System},
	Volume = 46,
	Year = 1989,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1kb3dsaW5nODkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2Zw1OT0VBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw1QEUQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZG93bGluZzg5LnBkZgAOABwADQBkAG8AdwBsAGkAbgBnADgAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZG93bGluZzg5LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2Rvd2xpbmc4OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Dowling95,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {T. E. Dowling},
	File = {../../Papers/dowling95.pdf},
	Journal = {Annu. Rev. Fluid Mech.},
	Pages = {293--334},
	Title = {Dynamics of {J}ovian Atmospheres},
	Volume = 27,
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1kb3dsaW5nOTUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2avxkfVgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvxmBxgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZG93bGluZzk1LnBkZgAOABwADQBkAG8AdwBsAGkAbgBnADkANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZG93bGluZzk1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2Rvd2xpbmc5NS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Draper79,
	Annote = {Filed under Regression Analysis.},
	Author = {N. R. Draper and R. C. {Van Nostrand}},
	Journal = {Technometrics},
	Pages = {451--466},
	Title = {Ridge Regression and {J}ames-{S}tein Estimation: Review and Comments},
	Volume = 21,
	Year = 1979}

@book{Draper81,
	Address = {New York},
	Author = {N. Draper and H. Smith},
	Edition = {2nd},
	Pages = 709,
	Publisher = {Wiley},
	Series = {Series in Probability and Mathematical Statistics},
	Title = {Applied Regression Analysis},
	Year = 1981}

@article{Draper95,
	Annote = {Filed under Predictability. Classical paper on
                  assessment of structural uncertainties in model
                  fitting. Examples from econometrics.},
	Author = {D. Draper},
	Journal = {J. Roy. Statist. Soc. B},
	Pages = {45--97},
	Title = {Assessment and Propagation of Model Uncertainty},
	Volume = 57,
	Year = 1995}

@book{Drazin81,
	Author = {P. G. Drazin and W. H. Reid},
	Pages = 527,
	Publisher = {Cambridge University Press},
	Title = {Hydrodynamic Stability},
	Year = 1981}

@article{Dritschel08,
	Author = {D. G. Dritschel and M. E. McIntyre},
	File = {../../Papers/dritschel08.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {855--874},
	Title = {Multiple Jets as {PV} Staircases: The {Phillips} Effect and the Resilience of Eddy-Transport Barriers},
	Volume = 65,
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9kcml0c2NoZWwwOC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2bxBMWX1BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxBN4zwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZHJpdHNjaGVsMDgucGRmAA4AIAAPAGQAcgBpAHQAcwBjAGgAZQBsADAAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZHJpdHNjaGVsMDgucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZHJpdHNjaGVsMDgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Dritschel93,
	Author = {D. G. Dritschel and B. Legras},
	Journal = {Physics Today},
	Month = {March},
	Title = {Modeling Oceanic and Atmospheric Vortices},
	Year = 1993}

@article{Dunbar94,
	Author = {R. B. Dunbar and G. M. Wellington and M. W. Colgan and P. W. Glynn},
	Journal = {Paleoceanography},
	Pages = {291--315},
	Title = {Eastern {P}acific sea surface temperature since {1600 A.D.}: {T}he $\delta^{18}\mathrm{O}$ record of climate variability in {G}alapagos corals},
	Volume = 9,
	Year = 1994}

@article{Duncan44,
	Author = {W. J. Duncan},
	Journal = {Philos. Mag. (7)},
	Pages = {660--670},
	Title = {Some devices for the solution of large sets of simultaneous linear equations},
	Volume = 35,
	Year = 1944}

@article{Dunkerton89,
	Annote = {Filed under Hadley Cell Dynamics. Stratospheric Hadley cell.},
	Author = {T. J. Dunkerton},
	File = {../../Papers/dunkerton89.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {956--974},
	Title = {Nonlinear {H}adley circulation driven by asymmetric heating},
	Volume = 46,
	Year = 1989,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9kdW5rZXJ0b244OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2fvwF7XAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvwHdzAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZHVua2VydG9uODkucGRmAA4AIAAPAGQAdQBuAGsAZQByAHQAbwBuADgAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZHVua2VydG9uODkucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZHVua2VydG9uODkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Durran91,
	Annote = {Third-order Adams-Bashcroft time differencing
                  requires only 3/2 the storage of leap-frog time
                  differencing, but is more accurate, stable, and
                  efficient.},
	Author = {D. R. Durran},
	Journal = {Mon. Wea. Rev.},
	Pages = {702--720},
	Title = {The Third-Order Adams-Bashforth Method: An Attractive Alternative to Leapfrog Time Differencing},
	Volume = 119,
	Year = 1991}

@book{Durran99,
	Address = {New York},
	Author = {D. R. Durran},
	Pages = 483,
	Publisher = {Springer},
	Series = {Texts in Applied Mathematics},
	Title = {Numerical Methods for Wave Equations in Geophysical Fluid Dynamics},
	Volume = 32,
	Year = 1999}

@article{Eady49,
	Author = {E. T. Eady},
	Journal = {Tellus},
	Pages = {33--52},
	Title = {Long Waves and Cyclone Waves},
	Volume = 1,
	Year = 1949}

@article{Edmon80,
	Annote = {EP fluxes and their divergences from observations
                  and implications for planetary-wave
                  propagation. Transient eddies more reliably
                  determined by nonlinear baroclinic instability,
                  linear theory inadequate. Residual meridional
                  circulation examined.},
	Author = {H. J. Edmon and B. J. Hoskins and M. E. Mc{I}ntyre},
	File = {../../Papers/edmon80.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2600--2616},
	Title = {{E}liassen-{P}alm Cross Sections for the Troposphere},
	Volume = 37,
	Year = 1980,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtlZG1vbjgwLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2nv04zGlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv06VigAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZWRtb244MC5wZGYADgAYAAsAZQBkAG0AbwBuADgAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvZWRtb244MC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9lZG1vbjgwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Edouard97,
	Annote = {Filed under Isentropic Observations. Observational
                  study of distribution of IPV and IPV fluxes;
                  consider various source terms and redistribution
                  mechanisms.},
	Author = {S. Edouard and R. Vautard and G. Brunet},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {2069--2094},
	Title = {On the Maintenance of Potential Vorticity in Isentropic Coordinates},
	Volume = 123,
	Year = 1997}

@article{Elden77,
	Annote = {Not on File. Classical algorithm for Tikhonov
                  regularization.},
	Author = {L. Eld{\'e}n},
	Journal = {BIT},
	Pages = {134--145},
	Title = {Algorithms for the regularization of ill-conditioned least squares problems},
	Volume = 17,
	Year = 1977}

@article{Elliott97,
	Annote = {Filed under Stochastic Turbulence Closures.},
	Author = {F. W. Elliott Jr. and D. J. Horntrop and A. J. Majda},
	Journal = {J. Comp. Phys.},
	Pages = {384--408},
	Title = {A {F}ourier-Wavelet {M}onte {C}arlo Method for Fractal Random Fields},
	Volume = 132,
	Year = 1997}

@article{Elsner93,
	Annote = {Filed under Predictability. Uses long precipitation
                  record to estimate complexity (information entropy)
                  of time series. Concludes that precipitation time
                  series is more complex than a purely random
                  sequence.},
	Author = {J. B. Elsner and A. A. Tsonis},
	Journal = {J. Atmos. Sci.},
	Pages = {400--405},
	Title = {Complexity and Predictability of Hourly Precipitation},
	Volume = 50,
	Year = 1993}

@article{Eluszkiewicz96,
	Author = {J. Eluszkiewicz and D. Crisp and R. Zurek and L. Elson and E. Fishbein and L. Froidevaux and J. Waters and R. G. Grainger and A. Lambert and R. Harwood and G. Peckham},
	Journal = {J. Atmos. Sci.},
	Pages = {217--240},
	Title = {Residual Circulation in the Stratosphere and Lower Mesosphere as Diagnosed from {M}icrowave {L}imb {S}ounder Data},
	Volume = 53,
	Year = 1996}

@article{Emanuel01,
	Annote = {Tropical cyclones stir ocean and, by mechanical
                  mixing, allow for horizontal heat
                  transport. Meridional heat transport "due" to
                  tropical cyclones may be substantial fraction of
                  total heat transport out of tropics.},
	Author = {K. Emanuel},
	Journal = {J. Geophys. Res.},
	Pages = {14771--14781},
	Title = {Contribution of tropical cyclones to meridional heat transport by the oceans},
	Volume = {106D},
	Year = 2001}

@article{Emanuel02a,
	Annote = {Multiple equilibria by feedbacks by stirring of
                  ocean by tropical cyclones, ocean heat transport,
                  and atmosphere circulation.},
	Author = {K. Emanuel},
	Journal = {J. Geophys. Res.},
	Pages = {10.129/2001/JD001002},
	Title = {A simple model of multiple climate regimes},
	Volume = {107},
	Year = 2002}

@incollection{Emanuel02b,
	Author = {K. Emanuel},
	Booktitle = {Meteorology at the Millennium},
	Editor = {R. P. Pearce},
	Pages = {62--71},
	Publisher = {Academic Press},
	Series = {International Geophysics Series},
	Title = {The Role of Water in Atmospheric Dynamics and Climate},
	Volume = 83,
	Year = 2002}

@article{Emanuel03,
	Author = {K. Emanuel},
	File = {../../Papers/emanuel03.pdf},
	Journal = {Annu. Rev. Earth. Planet. Sci.},
	Pages = {75--104},
	Title = {Tropical Cyclones},
	Volume = 31,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1lbWFudWVsMDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2vv6iR6wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv6kCawAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZW1hbnVlbDAzLnBkZgAOABwADQBlAG0AYQBuAHUAZQBsADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZW1hbnVlbDAzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2VtYW51ZWwwMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Emanuel04,
	Author = {K. Emanuel and C. DesAutels and C. Holloway and R. Korty},
	Journal = {J. Atmos. Sci.},
	Pages = {843--858},
	Title = {Environmental Control of Tropical Cyclone Intensity},
	Volume = 61,
	Year = 2004}

@article{Emanuel05,
	Author = {K. Emanuel},
	File = {../../Papers/emanuel05.pdf},
	Journal = {Nature},
	Pages = {686--688},
	Title = {Increasing destructiveness of tropical cyclones over the past 30 years},
	Volume = 436,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1lbWFudWVsMDUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2wv1eIHlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv1fqjgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZW1hbnVlbDA1LnBkZgAOABwADQBlAG0AYQBuAHUAZQBsADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZW1hbnVlbDA1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2VtYW51ZWwwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@incollection{Emanuel07,
	Address = {Princeton, NJ},
	Author = {K. Emanuel},
	Booktitle = {The Global Circulation of the Atmosphere},
	Editor = {T. Schneider and A. H. Sobel},
	Pages = {186--218},
	Publisher = {Princeton University Press},
	Title = {Quasi-Equilibrium Dynamics of the Tropical Atmosphere},
	Year = 2007}

@article{Emanuel83a,
	Annote = {Slantwise convection.},
	Author = {K. A. Emanuel},
	File = {../../Papers/emanuel83a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2368--2376},
	Title = {The {L}agrangian Parcel Dynamics of Moist Symmetric Instability},
	Volume = 40,
	Year = 1983,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5lbWFudWVsODNhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ21voXJYQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvoYr0QAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZW1hbnVlbDgzYS5wZGYAAA4AHgAOAGUAbQBhAG4AdQBlAGwAOAAzAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2VtYW51ZWw4M2EucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2VtYW51ZWw4M2EucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Emanuel83b,
	Annote = {Slantwise convection.},
	Author = {K. A. Emanuel},
	File = {../../Papers/emanuel83b.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {2016--2033},
	Title = {On assessing local conditional symmetric instability from atmospheric soundings},
	Volume = 111,
	Year = 1983,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5lbWFudWVsODNiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ22vo2dmgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvo4ACgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZW1hbnVlbDgzYi5wZGYAAA4AHgAOAGUAbQBhAG4AdQBlAGwAOAAzAGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2VtYW51ZWw4M2IucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2VtYW51ZWw4M2IucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Emanuel86,
	Author = {K. A. Emanuel},
	Journal = {J. Atmos. Sci.},
	Pages = {585--604},
	Title = {An Air-Sea Interaction Theory for Tropical Cyclones. {P}art {I}: Steady-State Maintenance},
	Volume = 43,
	Year = 1986}

@article{Emanuel87a,
	Author = {K. A. Emanuel},
	File = {../../Papers/emanuel87a.pdf},
	Journal = {Nature},
	Pages = {483--485},
	Title = {The dependence of hurricane intensity on climate},
	Volume = 326,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5lbWFudWVsODdhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ23vzqkN1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzsGpwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZW1hbnVlbDg3YS5wZGYAAA4AHgAOAGUAbQBhAG4AdQBlAGwAOAA3AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2VtYW51ZWw4N2EucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2VtYW51ZWw4N2EucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Emanuel87b,
	Annote = {.},
	Author = {K. A. Emanuel and M. Fantini and A. J. Thorpe},
	File = {../../Papers/emanuel87b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1559--1573},
	Title = {Baroclinic instability in an environment of small stability to slantwise moist convection. {P}art~{I}: {T}wo-dimensional models},
	Volume = 44,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5lbWFudWVsODdiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ24vrcbOQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvrd9qQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZW1hbnVlbDg3Yi5wZGYAAA4AHgAOAGUAbQBhAG4AdQBlAGwAOAA3AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2VtYW51ZWw4N2IucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2VtYW51ZWw4N2IucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Emanuel87c,
	Author = {K. A. Emanuel},
	File = {../../Papers/emanuel87c.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2324--2340},
	Title = {An air-sea interaction model of intraseasonal oscillations in the {T}ropics},
	Volume = 44,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5lbWFudWVsODdjLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ25wS3wb1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwS5S3wAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZW1hbnVlbDg3Yy5wZGYAAA4AHgAOAGUAbQBhAG4AdQBlAGwAOAA3AGMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2VtYW51ZWw4N2MucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2VtYW51ZWw4N2MucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Emanuel88a,
	Annote = {Atmosphere slantwise neutral in ascending regions.},
	Author = {K. A. Emanuel},
	File = {../../Papers/emanuel88a.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {1805--1816},
	Title = {Observational Evidence of Slantwise Convective Adjustment},
	Volume = 116,
	Year = 1988,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5lbWFudWVsODhhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ26wYUQklBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwYWBEgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZW1hbnVlbDg4YS5wZGYAAA4AHgAOAGUAbQBhAG4AdQBlAGwAOAA4AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2VtYW51ZWw4OGEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2VtYW51ZWw4OGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Emanuel88b,
	Annote = {Hypercanes. Uses thermodynamic cycle model to derive
                  maximum pressure drop at hurricane center.},
	Author = {K. A. Emanuel},
	Journal = {J. Atmos. Sci.},
	Pages = {1143--1155},
	Title = {The Maximum Intensity of Hurricanes},
	Volume = 45,
	Year = 1988}

@book{Emanuel94,
	Address = {New York},
	Author = {K. A. Emanuel},
	Pages = 580,
	Publisher = {Oxford University Press},
	Title = {Atmospheric Convection},
	Year = 1994}

@article{Emanuel94b,
	Author = {K. A. Emanuel and J. D. Neelin and C. S. Bretherton},
	File = {../../Papers/emanuel94b.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1111--1143},
	Title = {On large-scale circulations in convecting atmospheres},
	Volume = 120,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5lbWFudWVsOTRiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ28w9CYcQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw9EI8QAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZW1hbnVlbDk0Yi5wZGYAAA4AHgAOAGUAbQBhAG4AdQBlAGwAOQA0AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2VtYW51ZWw5NGIucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2VtYW51ZWw5NGIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@inproceedings{Emanuel95a,
	Author = {K. A. Emanuel and R. T. Pierrehumbert},
	Booktitle = {Clouds, Chemistry, and Climate},
	Editor = {P. J. Crutzen and V. Ramanathan},
	File = {../../Papers/emanuel95a.pdf},
	Pages = {17--28},
	Publisher = {Springer},
	Series = {{NATO} {ASI} Series {I}},
	Title = {Microphysical and Dynamical Control of Tropospheric Water Vapor},
	Volume = {35},
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5lbWFudWVsOTVhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ29wCOJ7gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwCP6bgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZW1hbnVlbDk1YS5wZGYAAA4AHgAOAGUAbQBhAG4AdQBlAGwAOQA1AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2VtYW51ZWw5NWEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2VtYW51ZWw5NWEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Emanuel95b,
	Author = {K. A. Emanuel and K. Speer and R. Rotunno and R. Srivastava and M. Molina},
	Journal = {J. Geophys. Res.},
	Pages = {13755--13765},
	Title = {Hypercanes: {A} Possible Link in Global Extinction Scenarios},
	Volume = {100D},
	Year = 1995}

@article{Emanuel95c,
	Annote = {Filed under Hadley Cell Dynamics. Constraints on
                  subcloud-layer moist entropy gradient from angular
                  momentum conservation in upper branch of Hadley cell.},
	Author = {K. A. Emanuel},
	File = {../../Papers/emanuel95c.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1529--1534},
	Title = {On Thermally Direct Circulations in Moist Atmospheres},
	Volume = 52,
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5lbWFudWVsOTVjLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ2+v00QGlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv01yigAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZW1hbnVlbDk1Yy5wZGYAAA4AHgAOAGUAbQBhAG4AdQBlAGwAOQA1AGMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2VtYW51ZWw5NWMucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2VtYW51ZWw5NWMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@incollection{Emanuel97,
	Address = {Netherlands},
	Annote = {Filed under Moist Convection. Sensitivity of
                  parameterized convective moistening to vertical
                  resolution. Test ability of convection schemes to
                  reproduce relative humidity (sensitive field).},
	Author = {K. A. Emanuel},
	Booktitle = {The Physics and Parameterization of Moist Atmospheric Convection},
	Editor = {R. K. Smith},
	Pages = {447--461},
	Publisher = {Kluwer Academic Publishers},
	Title = {The Problem of Convective Moistening},
	Year = 1997}

@article{Engl93,
	Annote = {Not on file.},
	Author = {H. W. Engl},
	Journal = {Surveys Math. Indust.},
	Pages = {71--143},
	Title = {Regularization Methods for the Stable Solution of Inverse Problems},
	Volume = 3,
	Year = 1993}

@book{Engl96,
	Address = {Dordrecht},
	Author = {H. W. Engl and M. Hanke and A. Neubauer},
	Pages = 321,
	Publisher = {Kluwer},
	Title = {Regularization of Inverse Problems},
	Year = 1996}

@article{Epifanio02b,
	Annote = {Filed under Lee Vortex Generation.},
	Author = {C. C. Epifanio and D. R. Durran},
	Journal = {J. Atmos. Sci.},
	Pages = {1166--1181},
	Title = {Lee-vortex formation in free-slip stratified flow over ridges. {P}art {II}: {M}echanisms of vorticity and {PV} production in nonlinear viscous wakes},
	Volume = 59,
	Year = 2002}

@article{Epifanio05,
	Annote = {Filed under Lee Vortex Generation.},
	Author = {C. C. Epifanio and R. Rotunno},
	File = {../../Papers/epifanio05.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3127--3150},
	Title = {The Dynamics of Orographic Wake Formation in Flows with Upstream Blocking},
	Volume = 62,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5lcGlmYW5pbzA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3Dv2/t2gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3BQSgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZXBpZmFuaW8wNS5wZGYAAA4AHgAOAGUAcABpAGYAYQBuAGkAbwAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2VwaWZhbmlvMDUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2VwaWZhbmlvMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Ertel49,
	Annote = {Ertel PV conservation.},
	Author = {H. Ertel and C.-G. Rossby},
	Journal = {Geofisica Pura E Applicata},
	Pages = {189--193},
	Title = {A New Conservation-Theorem of Hydrodynamics},
	Volume = 14,
	Year = 1949}

@article{Esler99,
	Annote = {Filed under Haynes. Breaking of baroclinic waves on
                  isentropes in zonally symmetric idealized
                  model. Waves near the tropopause break predominantly
                  equatorward; mean flux of wave activity is directed
                  equatorward. Equatorward breaking occurs when the
                  jet is broad and weak and when there are strong
                  isentropic PV gradients on the equatorward flank of
                  the jet. Poleward breaking occurs when the jet is
                  narrow and strong and when there are weak positive
                  or negative gradients of isentropic PV on the
                  equatorward flank of the jet. They argue that the
                  region of weak or negative PV gradients reflects
                  waves poleward. Jet moves poleward when radiative
                  heating is weakened. Jet moves poleward when surface
                  drag is weakened.},
	Author = {J. G. Esler and P. H Haynes},
	Journal = {J. Atmos. Sci.},
	Pages = {4014--4031},
	Title = {Baroclinic Wave Breaking and the Internal Variability of the Tropospheric Ciculation},
	Volume = 56,
	Year = 1999}

@article{Esper02,
	Annote = {Filed under Paleo-Climate
                  Reviews. Mann-Briffa-Hughes reconstruction of
                  climate post 1000 A.D. underestimates centenntial
                  variability, and in particular the 'Little Ice Age',
                  but long-term variability can be inferred from
                  tree-ring chronologies.},
	Author = {J. Esper and E. R. Cook and F. H. Schweingruber},
	Journal = {Science},
	Pages = {2250--2253},
	Title = {Low-Frequency Signals in Long Tree-Ring Chronologies for Reconstructing Past Temperature Variability},
	Volume = 295,
	Year = 2002}

@article{Everson95,
	Author = {R. Everson and L. Sirovich},
	File = {../../Papers/everson95.pdf},
	Journal = {J. Opt. Soc. Am. A},
	Pages = {1657--1664},
	Title = {Karhunen-Lo{\`e}ve procedure for gappy data},
	Volume = {12},
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ldmVyc29uOTUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3EwRC/GQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwREhiQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZXZlcnNvbjk1LnBkZgAOABwADQBlAHYAZQByAHMAbwBuADkANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZXZlcnNvbjk1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2V2ZXJzb245NS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Fahrmeier92,
	Annote = {Filed under Regression Analysis.},
	Author = {L. Fahrmeier and H. Frost},
	Journal = {Comp. Statist.},
	Pages = {137--164},
	Title = {On Stepwise Variable Selection in Generalized Linear Regression and Time Series Models},
	Volume = 7,
	Year = 1992}

@article{Falkovich01,
	Annote = {Review of particle (path-integral) methods in
                  turbulence, especially passive-scalar turbulence.},
	Author = {G. Falkovich and K. Gawedzki and M. Vergassola},
	Journal = {Rev. Mod. Phys.},
	Pages = {913--973},
	Title = {Particles and Fields in Fluid Turbulence},
	Year = 2001}

@article{Falkovich02,
	Annote = {Droplets advected as passive scalar. Effects on
                  concentration distribution and rain formation.},
	Author = {G. Falkovich and A. Fouxon and M. G. Stepanov},
	Journal = {Nature},
	Pages = {151--154},
	Title = {Acceleration of rain initiation by cloud turbulence},
	Volume = 419,
	Year = 2002}

@article{Fan98,
	Annote = {Filed under Carbon Flux Estimates. Poorly
                  constrained estimate of large sink over North
                  America. Errors almost certainly underestimated
                  (because of regularization). Questionable
                  methodology: division of globe into regions
                  (division seems at least partially politically
                  motivated).},
	Author = {S. Fan and M. Gloor and J. Mahlman and S. Pacala and J. Sarmiento and T. Takahashi and P. Tans},
	Journal = {Science},
	Pages = {442--446},
	Title = {A large terrestrial carbon sink in {N}orth {A}merica implied by atmospheric and oceanic carbon dioxide data and models},
	Volume = 282,
	Year = 1998}

@article{Fan99,
	Annote = {Filed under Carbon Flux Estimates.},
	Author = {S.-M. Fan and J. L. Sarmiento and M. Gloor and S. W. Pacala},
	Journal = {J. Geophys. Res.},
	Pages = {21503--21512},
	Title = {On the use of regularization techniques in the inverse modeling of atmospheric carbon dioxide},
	Volume = {104D},
	Year = 1999}

@article{Fang94,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {M. Fang and K. K. Tung},
	File = {../../Papers/fang94.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1261--1272},
	Title = {Solution to the {C}harney Problem of Viscous Symmetric Circulation},
	Volume = 51,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpmYW5nOTQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3Gvd3woQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvd5hIQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZmFuZzk0LnBkZgAADgAWAAoAZgBhAG4AZwA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2Zhbmc5NC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvZmFuZzk0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Fang96,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {M. Fang and K. K. Tung},
	Journal = {J. Atmos. Sci.},
	Pages = {1241--1261},
	Title = {A simple model of nonlinear {H}adley circulation with an {ITCZ}: {A}nalytic and Numerical Solutions},
	Volume = 53,
	Year = 1996}

@article{Fang97,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {M. Fang and K. K. Tung},
	Journal = {J. Atmos. Sci.},
	Pages = {1379--1384},
	Title = {The Dependence of the {H}adley Circulation on the Thermal Relaxation Time},
	Volume = 54,
	Year = 1997}

@article{Fang99,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {M. Fang and K. K. Tung},
	File = {../../Papers/fang99.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1797--1807},
	Title = {Time-Dependent Nonlinear {H}adley Circulation},
	Volume = 56,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpmYW5nOTkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3HvdzqEAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvd1akAAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZmFuZzk5LnBkZgAADgAWAAoAZgBhAG4AZwA5ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2Zhbmc5OS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvZmFuZzk5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Fantini90,
	Annote = {Not on file.},
	Author = {M. Fantini},
	Journal = {J. Atmos. Sci.},
	Pages = {1277--1287},
	Title = {Nongeostrophic corrections to the eigensolutions of a moist baroclinic instability problem},
	Volume = 47,
	Year = 1990}

@article{Fantini93,
	Author = {M. Fantini},
	File = {../../Papers/fantini93.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1199--1210},
	Title = {A Numerical Study of Two-Dimensional Moist Baroclinic Instability},
	Volume = 50,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1mYW50aW5pOTMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3JvrcbGgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvrd9igAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZmFudGluaTkzLnBkZgAOABwADQBmAGEAbgB0AGkAbgBpADkAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZmFudGluaTkzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2ZhbnRpbmk5My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Farge96,
	Annote = {Filed under Wavelets.},
	Author = {M. Farge and N. Kevlahan and V. Perrier and E. Goirand},
	Journal = {Proc. IEEE},
	Pages = {639--669},
	Title = {Wavelets and Turbulence},
	Volume = {84},
	Year = {1996}}

@article{Farman85,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {J. C. Farman and B. G. Gardiner and J. D. Shanklin},
	Journal = {Nature},
	Pages = {207--210},
	Title = {Large losses of total ozone in {A}ntarctica reveal seasonal $\mathrm{CLO}_x/\mathrm{NO}_x$ interaction},
	Volume = 315,
	Year = 1985}

@article{Farrell07,
	Annote = {Filed under Turbulence Closure Theories.},
	Author = {B. F. Farrell and P. J. Ioannou},
	File = {../../Papers/farrell07.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3652--3665},
	Title = {Structure and Spacing of Jets in Barotropic Turbulence},
	Volume = 64,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1mYXJyZWxsMDcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3Nwz5ubgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwz7Q3gAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZmFycmVsbDA3LnBkZgAOABwADQBmAGEAcgByAGUAbABsADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZmFycmVsbDA3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2ZhcnJlbGwwNy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Farrell92,
	Annote = {Filed under Adjoint Method.},
	Author = {B. F. Farrell and A. M. Moore},
	Journal = {J. Phys. Oceanogr.},
	Pages = {338--349},
	Title = {An Adjoint Method for Obtaining the Most Rapidly Growing Perturbation to Oceanic Flows},
	Volume = 22,
	Year = 1992}

@article{Farrell93a,
	Annote = {Filed under Stochastic Dynamics of Storm Tracks.},
	Author = {B. F. Farrell and P. J. Ioannou},
	Journal = {J. Atmos. Sci.},
	Pages = {4044--4057},
	Title = {Stochastic Dynamics of Baroclinic Waves},
	Volume = 50,
	Year = 1993}

@article{Farrell93b,
	Annote = {Filed under Stochastic Dynamics of Storm Tracks.},
	Author = {B. F. Farrell and P. J. Ioannou},
	Journal = {J. Atmos. Sci.},
	Pages = {200--211},
	Title = {Stochastic Forcing of Perturbation Variance in Unbounded Shear and Deformation Flows},
	Volume = 50,
	Year = 1993}

@article{Fedorov00,
	Annote = {Filed under Philander. Review of ENSO mechanisms and
                  of impacts of changes in background state on El
                  Nino.},
	Author = {A. V. Fedorov and S. G. Philander},
	Journal = {Science},
	Pages = {1997--2002},
	Title = {Is {E}l {N}i{\~n}o Changing?},
	Volume = 288,
	Year = 2000}

@article{Fennessy94,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {Fennessy, M. J. and Kinter III, J. L. and Kirtman, B. and Marx, L. and Nigam, S. and Schneider, E. and Shukla, J. and Straus, D. and Vernekar, A. and Xue, Y. and Zhou, J.},
	Date-Modified = {2010-06-22 14:33:45 -0700},
	Journal = {J. Climate},
	Pages = {33--43},
	Title = {The Simulated {I}ndian Monsoon: A {GCM} Sensitivity Study},
	Volume = {7},
	Year = 1994}

@article{Ferrel1859,
	Annote = {Filed under General Circulation History.},
	Author = {W. Ferrel},
	File = {../../Papers/ferrel1859.pdf},
	Journal = {Math. Mon.},
	Pages = {140--148, 210--216, 300--307, 366--372, 397--406},
	Title = {The motion of fluids and solids relative to the {E}arth's surface},
	Volume = 1,
	Year = 1859,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5mZXJyZWwxODU5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3bvvP7QQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvvRdsQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZmVycmVsMTg1OS5wZGYAAA4AHgAOAGYAZQByAHIAZQBsADEAOAA1ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2ZlcnJlbDE4NTkucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2ZlcnJlbDE4NTkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Fierro97,
	Annote = {Filed under Regularization.},
	Author = {R. D. Fierro and G. H. Golub and P. C. Hansen and D. P. O'Leary},
	File = {../../Papers/fierro97.pdf},
	Journal = {SIAM J. Sci. Comput.},
	Pages = {1223-1241},
	Title = {Regularization by truncated total least squares},
	Volume = 18,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxmaWVycm85Ny5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3dwHGyrgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwHIVHgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZmllcnJvOTcucGRmAAAOABoADABmAGkAZQByAHIAbwA5ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2ZpZXJybzk3LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9maWVycm85Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Flasar98b,
	Author = {F. M. Flasar},
	File = {../../Papers/flasar98b.pdf},
	Journal = {Icarus},
	Pages = {1125--1147},
	Title = {The dynamic meteorology of {Titan}},
	Volume = 46,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1mbGFzYXI5OGIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3jxgPm1gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxgRJRgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Zmxhc2FyOThiLnBkZgAOABwADQBmAGwAYQBzAGEAcgA5ADgAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZmxhc2FyOThiLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2ZsYXNhcjk4Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Foias01,
	Annote = {Filed under Holm.},
	Author = {C. Foias and D. D. Holm and E. S. Titi},
	Journal = {Physica D},
	Pages = {505--519},
	Title = {The {N}avier-{S}tokes-alpha model of fluid turbulence},
	Volume = 152,
	Year = 2001}

@article{Folkins03,
	Author = {I. Folkins and C. Braun},
	File = {../../Papers/folkins03.pdf},
	Journal = {J. Climate},
	Pages = {1807--1820},
	Title = {Tropical Rainfall and Boundary Layer Moist Entropy},
	Volume = 16,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1mb2xraW5zMDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3pxgIodwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxgKK5wAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Zm9sa2luczAzLnBkZgAOABwADQBmAG8AbABrAGkAbgBzADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZm9sa2luczAzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2ZvbGtpbnMwMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Forest02,
	Annote = {Estimate pdfs of climate sensitivity, aerosol
                  radiative forcing, and oceanic heat uptake by
                  regression of simulations with MIT GCM (simple GCM)
                  onto 20th-century surface temperature, upper-air
                  temperature, and global-average ocean temperatures
                  (linear trends and zonal mean for air
                  temperatures).},
	Author = {C. E. Forest and P. H. Stone and A. P. Sokolov and M. R. Allen and M. D. Webster},
	File = {../../Papers/forest02.pdf},
	Journal = {Science},
	Pages = {113--117},
	Title = {Quantifying Uncertainties in Climate System Properties with the Use of Recent Climate Observations},
	Volume = 295,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxmb3Jlc3QwMi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3rwIVuHlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwIXQjgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Zm9yZXN0MDIucGRmAAAOABoADABmAG8AcgBlAHMAdAAwADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2ZvcmVzdDAyLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9mb3Jlc3QwMi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Forster97,
	Annote = {Filed under Tropopause Dynamics. Need to define
                  tropopause in tropics dynamically to obtain
                  meaningful definition of the concept of radiative
                  forcing by stratospheric processes.},
	Author = {{P. M. de F.} Forster and R. S. Freckleton and K. P. Shine},
	Journal = {Climate Dyn.},
	Pages = {547--560},
	Title = {On aspects of the concept of radiative forcing},
	Volume = 13,
	Year = 1997}

@article{Frank93,
	Annote = {Filed under Regression Analysis.},
	Author = {I. E. Frank and J. H. Friedman},
	Journal = {Technometrics},
	Pages = {109--135},
	Title = {A statistical view of some chemometrics regression tools},
	Volume = 35,
	Year = 1993}

@article{Frederiksen83,
	Annote = {Filed under Baroclinic Instability. 3D eddy fluxes
                  resemble in structure those of linearly most
                  unstable waves.},
	Author = {J. S. Frederiksen},
	File = {../../Papers/frederiksen83.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {836--855},
	Title = {Disturbances and Eddy Fluxes in Northern Hemisphere Flows: Instability of Three-Dimensional {J}anuary and {J}uly Flows},
	Volume = 40,
	Year = 1983,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXgAAAAAAXgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhFmcmVkZXJpa3NlbjgzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3wvz4YTAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvz56vAAAAAEADAAJDH4ACE6zAACS8wACADBNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnJlZGVyaWtzZW44My5wZGYADgAkABEAZgByAGUAZABlAHIAaQBrAHMAZQBuADgAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACRVc2Vycy90YXBpby9QYXBlcnMvZnJlZGVyaWtzZW44My5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHi4uLy4uL1BhcGVycy9mcmVkZXJpa3NlbjgzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIcAh4CIwIsAjcCOwJJAlACWQJ6An8CggKPApQAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACpg==}}

@article{Friedman89,
	Annote = {Filed under Discriminant Analysis.},
	Author = {J. H. Friedman},
	Journal = {J. Amer. Statist. Assoc.},
	Pages = {165--175},
	Title = {Regularized Discriminant Analysis},
	Volume = 84,
	Year = 1989}

@article{Frierson04,
	Author = {D. M. W. Frierson and A. J. Majda and O. M. Pauluis},
	File = {../../Papers/frierson04.pdf},
	Journal = {Comm. Math. Sci.},
	Pages = {591--626},
	Title = {Large Scale Dynamics of Precipitation Fronts in the Tropical Atmosphere: A Novel Relaxation Limit},
	Volume = 2,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5mcmllcnNvbjA0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3xvp7M5wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvp8vVwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnJpZXJzb24wNC5wZGYAAA4AHgAOAGYAcgBpAGUAcgBzAG8AbgAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2ZyaWVyc29uMDQucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2ZyaWVyc29uMDQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Frierson06a,
	Author = {Frierson, D. M. W. and Held, I. M. and Zurita-Gotor, P.},
	File = {../../Papers/frierson06a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2548--2566},
	Title = {A gray-radiation aquaplanet moist {GCM}. {Part~I}: Static stability and eddy scale},
	Volume = 63,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9mcmllcnNvbjA2YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3zwYfWvAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwYhHPAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnJpZXJzb24wNmEucGRmAA4AIAAPAGYAcgBpAGUAcgBzAG8AbgAwADYAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZnJpZXJzb24wNmEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZnJpZXJzb24wNmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Frierson06b,
	Author = {D. M. W. Frierson},
	File = {../../Papers/frierson06b.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2006GL027504},
	Pages = {L24816},
	Title = {Robust increases in midlatitude static stability in simulations of global warming},
	Volume = 33,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9mcmllcnNvbjA2Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ30wx2o4QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwx4LUQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnJpZXJzb24wNmIucGRmAA4AIAAPAGYAcgBpAGUAcgBzAG8AbgAwADYAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZnJpZXJzb24wNmIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZnJpZXJzb24wNmIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Frierson07a,
	Author = {Frierson, D. M. W. and Held, I. M. and Zurita-Gotor, P.},
	File = {../../Papers/frierson07a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1680--1693},
	Title = {A gray-radiation aquaplanet moist {GCM}. {Part~II}: {E}nergy transports in altered climates},
	Volume = {64},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9mcmllcnNvbjA3YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ31ww7QtAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAww8zJAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnJpZXJzb24wN2EucGRmAA4AIAAPAGYAcgBpAGUAcgBzAG8AbgAwADcAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZnJpZXJzb24wN2EucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZnJpZXJzb24wN2EucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Frierson07b,
	Author = {D. M. W. Frierson},
	File = {../../Papers/frierson07b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1959--1976},
	Title = {The dynamics of idealized convection schemes and their effect on the zonally averaged tropical circulation},
	Volume = {64},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9mcmllcnNvbjA3Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ32ww7Q2QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAww8zSQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnJpZXJzb24wN2IucGRmAA4AIAAPAGYAcgBpAGUAcgBzAG8AbgAwADcAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZnJpZXJzb24wN2IucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZnJpZXJzb24wN2IucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Frierson07c,
	Author = {D. M. W. Frierson},
	File = {../../Papers/frierson07c.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2076--2090},
	Title = {Convectively Coupled {Kelvin} Waves in an Idealized Moist General Circulation Model},
	Volume = {64},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9mcmllcnNvbjA3Yy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ33ww7Q9gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAww8zZgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnJpZXJzb24wN2MucGRmAA4AIAAPAGYAcgBpAGUAcgBzAG8AbgAwADcAYwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZnJpZXJzb24wN2MucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZnJpZXJzb24wN2MucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Frierson07d,
	Author = {D. M. W. Frierson and J. Lu and G. Chen},
	File = {../../Papers/frierson07d.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2007GL031115},
	Pages = {L18804},
	Title = {Width of the {Hadley} cell in simple and comprehensive general circulation models},
	Volume = {34},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9mcmllcnNvbjA3ZC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ34xMcHulBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxMdqKgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnJpZXJzb24wN2QucGRmAA4AIAAPAGYAcgBpAGUAcgBzAG8AbgAwADcAZAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZnJpZXJzb24wN2QucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZnJpZXJzb24wN2QucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Frierson08a,
	Author = {D. M. W. Frierson},
	File = {../../Papers/frierson08a.pdf},
	Journal = {J. Atmos. Sci},
	Pages = {1049--1062},
	Title = {Midlatitude static stability in simple and comprehensive general circulation models},
	Volume = {65},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9mcmllcnNvbjA4YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ35xBMXAFBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxBN5cAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnJpZXJzb24wOGEucGRmAA4AIAAPAGYAcgBpAGUAcgBzAG8AbgAwADgAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZnJpZXJzb24wOGEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZnJpZXJzb24wOGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Frisch90,
	Annote = {Filed under Orszag.},
	Author = {U. Frisch and S. A. Orszag},
	Journal = {Physics Today},
	Month = {January},
	Title = {Turbulence: {C}hallenges for theory and experiment},
	Year = 1990}

@article{Fritsch84,
	Annote = {Not on file. Monotonicity-preserving piecewise cubic
                  Hermite interpolants. Algorithm implemented in NAG
                  Library E01BEF.},
	Author = {F. N. Fritsch and J. Butland},
	Journal = {SIAM J. Sci. Stat. Comput.},
	Pages = {300-304},
	Title = {A method for constructing local monotone piecewise cubic interpolants},
	Volume = 5,
	Year = 1984}

@article{Fu06,
	Author = {Q. Fu and C. M. Johanson and J. M. Wallace and T. Reichler},
	File = {../../Papers/fu06.pdf},
	Journal = {Science},
	Pages = {1179},
	Title = {Enhanced mid-latitude tropospheric warming in satellite measurements},
	Volume = 312,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfghmdTA2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ36w67KHlBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw686ngAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnUwNi5wZGYAAA4AEgAIAGYAdQAwADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL2Z1MDYucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL2Z1MDYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@book{Fukunaga90,
	Address = {San Diego, CA},
	Author = {K. Fukunaga},
	Edition = {2nd},
	Pages = 591,
	Publisher = {Academic Press},
	Title = {Introduction to Statistical Pattern Recognition},
	Year = 1990}

@book{Fuller87,
	Address = {New York},
	Annote = {QA275.F85 Fine Hall},
	Author = {W. A. Fuller},
	Pages = 440,
	Publisher = {Wiley},
	Series = {Series in Probability and Mathematical Statistics},
	Title = {Measurement Error Models},
	Year = 1987}

@article{Fyfe03,
	Author = {Fyfe, J.C.},
	File = {../../Papers/fyfe03.pdf},
	Journal = {J. Climate},
	Pages = {2802--2805},
	Title = {Extratropical Southern Hemisphere Cyclones: Harbingers of Climate Change?},
	Volume = {16},
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpmeWZlMDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ37xAbb4gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxAc+UgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6ZnlmZTAzLnBkZgAADgAWAAoAZgB5AGYAZQAwADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2Z5ZmUwMy5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvZnlmZTAzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Gabriel99,
	Annote = {Filed under Tropopause Dynamics.},
	Author = {A. Gabriel and G. Schmitz and R. Gepr{\"a}gs},
	Journal = {J. Atmos. Sci.},
	Pages = {4059--4068},
	Title = {The Tropopause in a {2D} Circulation Model},
	Volume = 56,
	Year = 1999}

@article{Gadgil03,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {S. Gadgil},
	File = {../../Papers/gadgil03.pdf},
	Journal = {Ann. Rev. Earth Planet Sci.},
	Pages = {429--467},
	Title = {The {I}ndian Monsoon and its Variability},
	Volume = 31,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxnYWRnaWwwMy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ38v/6q2QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv/8bWQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2FkZ2lsMDMucGRmAAAOABoADABnAGEAZABnAGkAbAAwADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2dhZGdpbDAzLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9nYWRnaWwwMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Galewsky05,
	Author = {J. Galewsky and A. Sobel and I. Held},
	File = {../../Papers/galewsky05.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3353--3367},
	Title = {Diagnosis of subtropical humidity dynamics using tracers of last saturation},
	Volume = 62,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5nYWxld3NreTA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ3+v2/rXAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3BNzAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2FsZXdza3kwNS5wZGYAAA4AHgAOAGcAYQBsAGUAdwBzAGsAeQAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2dhbGV3c2t5MDUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2dhbGV3c2t5MDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Gallego01,
	Annote = {Energy-balance atmosphere coupled to two ocean
                  basins. Sustains decadal oscillations (because of
                  decadal time scale of Rossby wave propagation in
                  ocean). Phase-locking, steady solution, and chaos
                  regimes.},
	Author = {B. Gallego and P. Cessi},
	Journal = {J. Climate},
	Pages = {2815--2832},
	Title = {Decadal Variability of Two Oceans and an Atmosphere},
	Volume = 14,
	Year = 2001}

@article{Gallimore81a,
	Author = {R. G. Gallimore and D. R. Johnson},
	File = {../../Papers/gallimore81a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {583--599},
	Title = {The forcing of the meridional circulation of the isentropic zonally averaged circumpolar vortex},
	Volume = 38,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBnYWxsaW1vcmU4MWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4Gvt8wxQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvt+TNQAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2FsbGltb3JlODFhLnBkZgAADgAiABAAZwBhAGwAbABpAG0AbwByAGUAOAAxAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL2dhbGxpbW9yZTgxYS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvZ2FsbGltb3JlODFhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Gallimore81b,
	Author = {R. G. Gallimore and D. R. Johnson},
	File = {../../Papers/gallimore81b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1870--1890},
	Title = {A numerical diagnostic model of the zonally averaged circulation in isentropic coordinates},
	Volume = 38,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBnYWxsaW1vcmU4MWIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4Hvt8w+QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvt+TaQAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2FsbGltb3JlODFiLnBkZgAADgAiABAAZwBhAGwAbABpAG0AbwByAGUAOAAxAGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL2dhbGxpbW9yZTgxYi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvZ2FsbGltb3JlODFiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Galperin01,
	Annote = {Filed under Geostrophic Turbulence.},
	Author = {B. Galperin and S. Sukoriansky and H.-P. Huang},
	File = {../../Papers/galperin01.pdf},
	Journal = {Phys. Fluids},
	Pages = {1545--1548},
	Title = {Universal $n^{-5}$ spectrum of zonal flows on giant planets},
	Volume = 13,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5nYWxwZXJpbjAxLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4Iwm4vPAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwm6RrAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2FscGVyaW4wMS5wZGYAAA4AHgAOAGcAYQBsAHAAZQByAGkAbgAwADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2dhbHBlcmluMDEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2dhbHBlcmluMDEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Ganopolski01,
	Annote = {Filed under Rahmstorf.},
	Author = {A. Ganopolski and S. Rahmstorf},
	Journal = {Nature},
	Pages = {153--158},
	Title = {Rapid changes of glacial climate simulated in a coupled climate model},
	Volume = 409,
	Year = 2001}

@article{Ganopolski98,
	Annote = {Filed under Rahmstorf. Simulation of equilibrium
                  climate of today and the Last Glacial Maximum
                  without flux adjustments.},
	Author = {A. Ganopolski and S. Rahmstorf and V. Petoukhov and M. Claussen},
	Journal = {Nature},
	Pages = {351--356},
	Title = {Simulation of Modern and Glacial Climates with a Coupled Global Model of Intermediate Complexity},
	Volume = 391,
	Year = 1998}

@book{Gardiner04,
	Address = {Berlin, Heidelberg},
	Author = {C. W. Gardiner},
	Edition = {3rd},
	Pages = 415,
	Publisher = {Springer},
	Series = {Series in Synergetics},
	Title = {Handbook of Stochastic Methods},
	Year = 2004}

@article{Garner92,
	Annote = {Follow-up on Nakamura89. Equlibration by
                  vortex-rollup. Eady problem in isentropic
                  coordinates and similarity to barotropic shear layer
                  instability.},
	Author = {S. T. Garner and N. Nakamura and I. M. Held},
	Journal = {J. Atmos. Sci.},
	Pages = {1984--1996},
	Title = {Nonlinear Equilibration of Two-Dimensional {E}ady Waves: A New Perspective},
	Volume = 49,
	Year = 1992}

@article{Garrat93,
	Author = {J. R. Garrat},
	Journal = {J. Climate},
	Pages = {419--449},
	Title = {Sensitivity of Climate Simulations to Land-Surface and Atmospheric Boundary-Layer Treatments --- {A} Review},
	Volume = 6,
	Year = 1993}

@article{Gates92,
	Annote = {Not on file.},
	Author = {W. L. Gates},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {1962--1970},
	Title = {{AMIP}: {T}he Atmospheric Model Intercomparison Project},
	Volume = 73,
	Year = 1992}

@article{Gauthier86,
	Annote = {Filed under Adjoint Methods.},
	Author = {O. Gauthier and J. Virieux and A. Tarantola},
	Journal = {Geophys.},
	Pages = {1387--1403},
	Title = {Two-dimensional nonlinear inversion of seismic waveforms: {N}umerical results},
	Volume = 51,
	Year = 1986}

@article{Geng03a,
	Author = {Geng, Q. and Sugi, M.},
	Date-Modified = {2010-06-12 10:03:10 -0700},
	Journal = {J. Climate},
	Pages = {2262--2274},
	Title = {Possible Change of Extratropical Cyclone Activity due to Enhanced Greenhouse Gases and Sulfate Aerosols---{S}tudy with a High-Resolution {AGCM}},
	Volume = {16},
	Year = {2003},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtnZW5nMDNhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4PxYuvvAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxYwgPAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2VuZzAzYS5wZGYADgAYAAsAZwBlAG4AZwAwADMAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvZ2VuZzAzYS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9nZW5nMDNhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Gent90,
	Annote = {Filed under Baroclinic Eddy Parameterizations.},
	Author = {P. R. Gent and J. C. {McWilliams}},
	Journal = {J. Phys. Oceanogr.},
	Pages = {150--155},
	Title = {Isopycnal Mixing in Ocean Circulation Models},
	Volume = 20,
	Year = 1990}

@article{Gent95,
	Annote = {Filed under Baroclinic Eddy Parameterizations.},
	Author = {P. R. Gent and J. Willebrand and T. J. {McDougall} and J. C. {McWilliams}},
	Journal = {J. Phys. Oceanogr.},
	Pages = {463--474},
	Title = {Parameterizing Eddy-Induced Transports in Ocean Circulation Models},
	Volume = 25,
	Year = 1995}

@article{Gierasch00,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {P. J. Gierasch and A. P. Ingersoll and D. Banfield and S. P. Ewald and P. Helfenstein and A. Simon-Miller and A. R. Vasavada and H. H. Breneman and D. A. Senske and {the Galileo Imaging Team}},
	File = {../../Papers/gierasch00.pdf},
	Journal = {Nature},
	Pages = {628--630},
	Title = {Observation of moist convection in {J}upiter's atmosphere},
	Volume = 403,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5naWVyYXNjaDAwLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4SwxtdflBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwxu/7gAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2llcmFzY2gwMC5wZGYAAA4AHgAOAGcAaQBlAHIAYQBzAGMAaAAwADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2dpZXJhc2NoMDAucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2dpZXJhc2NoMDAucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Gierasch04,
	Author = {P. J. Gierasch and B. J. Conrath and P. L. Read},
	File = {../../Papers/gierasch04.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1953--1965},
	Title = {Nonconservation of {Ertel} potential vorticity in hydrogen atmospheres},
	Volume = {61},
	Year = {2004},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5naWVyYXNjaDA0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4Twst5mlBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsvcCgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2llcmFzY2gwNC5wZGYAAA4AHgAOAGcAaQBlAHIAYQBzAGMAaAAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2dpZXJhc2NoMDQucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2dpZXJhc2NoMDQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Gierasch75,
	Author = {P. J. Gierasch},
	File = {../../Papers/gierasch75.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1038--1044},
	Title = {Meridional circulation and the maintenance of the {Venus} atmospheric rotation},
	Volume = 32,
	Year = 1975,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5naWVyYXNjaDc1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4UwTYkIlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwTaGkgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2llcmFzY2g3NS5wZGYAAA4AHgAOAGcAaQBlAHIAYQBzAGMAaAA3ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2dpZXJhc2NoNzUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2dpZXJhc2NoNzUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Gierasch93,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {P. J. Gierasch and B. J. Conrath},
	File = {../../Papers/gierasch93.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {5459--5469},
	Title = {Dynamics of the Atmospheres of the Outer Planets: {P}ost-{V}oyager Measurement Objectives},
	Volume = 98,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5naWVyYXNjaDkzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4VvRg9gQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRif8QAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2llcmFzY2g5My5wZGYAAA4AHgAOAGcAaQBlAHIAYQBzAGMAaAA5ADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2dpZXJhc2NoOTMucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2dpZXJhc2NoOTMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Gilchrist88,
	Author = {A. Gilchrist},
	Journal = {Rep. Prog. Phys.},
	Pages = {1205--1226},
	Title = {Numerical Weather Prediction and Climate Simulation},
	Volume = 51,
	Year = 1988}

@article{Gildor00,
	Annote = {Filed under Tziperman.},
	Author = {H. Gildor and E. Tziperman},
	Journal = {Paleoceanogr.},
	Pages = {605--615},
	Title = {Sea ice as the glacial cycles' climate switch: {R}ole of seasonal and orbital forcing},
	Volume = 15,
	Year = 2000}

@article{Gill72,
	Annote = {Not on file.},
	Author = {P. E. Gill and W. Murray},
	Journal = {J. Inst. Maths. Applics.},
	Pages = {91--108},
	Title = {Quasi-{N}ewton Methods for Unconstrained Optimization},
	Volume = 9,
	Year = 1972}

@article{Gill80,
	Author = {A. E. Gill},
	File = {../../Papers/gill80.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {447--462},
	Title = {Some Simple Solutions for Heat Induced Tropical Circulation},
	Volume = 106,
	Year = 1980,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpnaWxsODAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4WwZOv6VBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwZQgaQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2lsbDgwLnBkZgAADgAWAAoAZwBpAGwAbAA4ADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2dpbGw4MC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvZ2lsbDgwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@book{Gill82,
	Author = {A. E. Gill},
	Pages = 662,
	Publisher = {Academic Press},
	Series = {International Geophysics Series},
	Title = {Atmosphere-Ocean Dynamics},
	Volume = 30,
	Year = 1982}

@article{Gillett03,
	Annote = {Filed under Climate Change Detection. Flawed. See
                  correspondence with Paul Kushner.},
	Author = {N. P. Gillett and F. W. Zwiers and A. J. Weaver and P. A. Stott},
	File = {../../Papers/gillett03.pdf},
	Journal = {Nature},
	Pages = {292--294},
	Title = {Detection of human influence on sea-level pressure},
	Volume = 422,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1naWxsZXR0MDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4XwKuSaVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwKv02QAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z2lsbGV0dDAzLnBkZgAOABwADQBnAGkAbABsAGUAdAB0ADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZ2lsbGV0dDAzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2dpbGxldHQwMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Giorgi91,
	Author = {F. Giorgi and L. O. Mearns},
	Journal = {Rev. Geophys.},
	Pages = {191--216},
	Title = {Approaches to the Simulation of Regional Climate Change: A Review},
	Volume = {29},
	Year = {1991}}

@article{Gold1909,
	Annote = {Filed under General Circulation History.},
	Author = {E. Gold},
	File = {../../Papers/gold1909.pdf},
	Journal = {Proc. Roy. Soc. Lond. A},
	Pages = {43--70},
	Title = {The Isothermal Layer of the Atmosphere and Atmospheric Radiation},
	Volume = {82},
	Year = 1909,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxnb2xkMTkwOS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4hvzDzqAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzFWGAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z29sZDE5MDkucGRmAAAOABoADABnAG8AbABkADEAOQAwADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2dvbGQxOTA5LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9nb2xkMTkwOS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Golub79,
	Annote = {Not on file.},
	Author = {G. H. Golub and M. T. Heath and G. Wahba},
	Journal = {Technometrics},
	Pages = {215--223},
	Title = {Generalized cross-validation as a method for choosing a good ridge parameter},
	Volume = 21,
	Year = 1979}

@book{Golub93,
	Address = {Baltimore},
	Author = {G. H. Golub and C. F. {van Loan}},
	Edition = {2nd},
	Pages = 642,
	Publisher = {Johns Hopkins University Press},
	Title = {Matrix Computations},
	Year = 1993}

@article{Golub99,
	Annote = {Filed under Regularization.},
	Author = {G. H. Golub and P. C. Hansen and D. P. O'Leary},
	File = {../../Papers/golub99.pdf},
	Journal = {SIAM J. Matrix Anal. Appl.},
	Pages = {185--194},
	Title = {Tikhonov regularization and total least squares},
	Volume = {21},
	Year = {1999},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtnb2x1Yjk5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4jwHGxXwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwHITzwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z29sdWI5OS5wZGYADgAYAAsAZwBvAGwAdQBiADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvZ29sdWI5OS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9nb2x1Yjk5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@book{Goody89,
	Address = {New York},
	Author = {R. M. Goody and Y. L. Yung},
	Edition = {2nd},
	Pages = 519,
	Publisher = {Oxford University Press},
	Title = {Atmospheric Radiation: Theoretical Basis},
	Year = 1989}

@article{Graham87,
	Author = {N. E. Graham and T. P. Barnett},
	File = {../../Papers/graham87.pdf},
	Journal = {Science},
	Pages = {657--659},
	Title = {Sea surface temperature, surface wind divergence, and convection over tropical oceans},
	Volume = 238,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxncmFoYW04Ny5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4oxgIn8QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxgKKYQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3JhaGFtODcucGRmAAAOABoADABnAHIAYQBoAGEAbQA4ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2dyYWhhbTg3LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9ncmFoYW04Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Graham94,
	Annote = {Not on file.},
	Author = {N. E. Graham},
	Journal = {Climate Dyn.},
	Pages = {135--162},
	Title = {Decadal-scale climate variability in the tropical and {N}orth {P}acific during the 1970s and 1980s: Observations and model results},
	Volume = 10,
	Year = 1994}

@article{Greatbatch98,
	Annote = {Filed under Baroclinic Eddy Parameterizations.},
	Author = {R. J. Greatbatch},
	Journal = {J. Phys. Oceanogr.},
	Pages = {422--432},
	Title = {Exploring the Relationship between Eddy-Induced Transport Velocity, Vertical Momentum Transfer, and the Isopycnal Flux of Potential Vorticity},
	Volume = 28,
	Year = 1998}

@article{Green60,
	Annote = {Filed under Baroclinic Instability. Unification of
                  Charney and Eady models.},
	Author = {J. S. A. Green},
	File = {../../Papers/green60.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {237--251},
	Title = {A problem in baroclinic instability},
	Volume = 86,
	Year = 1960,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtncmVlbjYwLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4qviO6gAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAviQrAAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3JlZW42MC5wZGYADgAYAAsAZwByAGUAZQBuADYAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvZ3JlZW42MC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9ncmVlbjYwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Green70,
	Annote = {Baroclinic eddy flux parameterization.},
	Author = {J. S. A. Green},
	File = {../../Papers/green70.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {157--185},
	Title = {Transfer Properties of the Large-Scale Eddies and the General Circulation of the Atmosphere},
	Volume = 96,
	Year = 1970,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtncmVlbjcwLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4rwsZDOgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsalqgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3JlZW43MC5wZGYADgAYAAsAZwByAGUAZQBuADcAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvZ3JlZW43MC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9ncmVlbjcwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Grenier01,
	Author = {H. Grenier and C. S. Bretherton},
	Journal = {Mon. Wea. Rev.},
	Pages = {357--377},
	Title = {A Moist {PBL} Parameterization for Large-Scale Models and Its Application to Subtropical Cloud-Topped Marine Boudary Layers},
	Volume = 129,
	Year = 2001}

@book{Griewank91,
	Author = {A. Griewank and G. F. Corliss},
	Publisher = {Society for Industrial and Applied Mathematics},
	Title = {Automatic Differentiation of Algorithms: Theory, Implementation, and Application},
	Year = {1991}}

@article{Griffies95,
	Author = {S. M. Griffies and E. Tziperman},
	Journal = {J. Climate},
	Pages = {2440--2453},
	Title = {A linear thermohaline oscillator driven by stochastic atmospheric forcing},
	Volume = 8,
	Year = 1995}

@article{Griffies97a,
	Annote = {Short version of Griffies97b.},
	Author = {S. M. Griffies and K. Bryan},
	Journal = {Science},
	Pages = {181--184},
	Title = {Predictability of {N}orth {A}tlantic Multidecadal Climate Variability},
	Volume = 275,
	Year = 1997}

@article{Griffies97b,
	Author = {S. M. Griffies and K. Bryan},
	Journal = {Climate Dyn.},
	Pages = {459--488},
	Title = {A Predictability Study of Simulated {N}orth {A}tlantic Multidecadal Variability},
	Volume = 8,
	Year = 1997}

@article{Groisman05,
	Annote = {Filed uner Precipitation Statistics.},
	Author = {P. Ya. Groisman and R. W. Knight and D. R. Easterling and T. R. Karl and G. C. Hegerl and V. N. Razuvaev},
	File = {../../Papers/groisman05.pdf},
	Journal = {J. Climate},
	Pages = {1326--1350},
	Title = {Trends in intense precipitation in the climate record},
	Volume = 18,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5ncm9pc21hbjA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4xwdLRrQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwdNCLQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3JvaXNtYW4wNS5wZGYAAA4AHgAOAGcAcgBvAGkAcwBtAGEAbgAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2dyb2lzbWFuMDUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2dyb2lzbWFuMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Groisman99,
	Annote = {Filed uner Precipitation Statistics. Introduces to use
                  of gamma function to characterize precip pdf.},
	Author = {P. Ya. Groisman and T. R. Karl and D. R. Easterling and R. W. Knight and P. F. Jamason and K. J. Hennessy and R. Suppiah and C. M. Page and J. Wibig and K. Fortuniak and V. N. Razuvaev and A. Douglas and E. F{\o}rland and P.-M. Zhai},
	File = {../../Papers/groisman99.pdf},
	Journal = {Climatic Change},
	Pages = {243--283},
	Title = {Changes in the probability of heavy precipitation: Important indicators of climatic change},
	Volume = 42,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5ncm9pc21hbjk5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4ywdLRCwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwdNBiwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3JvaXNtYW45OS5wZGYAAA4AHgAOAGcAcgBvAGkAcwBtAGEAbgA5ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2dyb2lzbWFuOTkucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2dyb2lzbWFuOTkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Grossmann00,
	Annote = {Filed under Rayleigh-Benard Convection. Uses
                  expression of total kinetic and thermal dissipation
                  rates as functions of Rayleigh and Prandtl number
                  and scaling estimates of dissipation rates in bulk
                  and boundary layers to obtain scaling theories in
                  different regimes.},
	Author = {S. Grossmann and D. Lohse},
	File = {../../Papers/grossmann00.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {27--56},
	Title = {Scaling in thermal convection: a unifying theory},
	Volume = 407,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9ncm9zc21hbm4wMC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4zvFek4gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvFgVYgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3Jvc3NtYW5uMDAucGRmAA4AIAAPAGcAcgBvAHMAcwBtAGEAbgBuADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZ3Jvc3NtYW5uMDAucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZ3Jvc3NtYW5uMDAucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Grossmann01,
	Annote = {Filed under Rayleigh-Benard Convection.},
	Author = {S. Grossmann and D. Lohse},
	File = {../../Papers/grossmann01.pdf},
	Journal = {Phys. Rev. Lett.},
	Pages = {3316--3319},
	Title = {Thermal Convection for Large {P}randtl Numbers},
	Volume = 86,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9ncm9zc21hbm4wMS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ40vFej0AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvFgUUAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3Jvc3NtYW5uMDEucGRmAA4AIAAPAGcAcgBvAHMAcwBtAGEAbgBuADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvZ3Jvc3NtYW5uMDEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvZ3Jvc3NtYW5uMDEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Grote01,
	Author = {E. Grote and F. H. Busse},
	File = {../../Papers/grote01.pdf},
	Journal = {Fluid Dyn. Res.},
	Pages = {349--368},
	Title = {Dynamics of convection and dynamos in rotating spherical fluid shells},
	Volume = 28,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtncm90ZTAxLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ41xGsG6gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxGtpWgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3JvdGUwMS5wZGYADgAYAAsAZwByAG8AdABlADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvZ3JvdGUwMS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9ncm90ZTAxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Grote97,
	Annote = {Filed under Stochastic Turbulence Closures.},
	Author = {M. J. Grote and A. J. Majda},
	Journal = {Phys. Fluids},
	Pages = {3431--3442},
	Title = {Crude Closure Dynamics through Large Scale Statistical Theories},
	Volume = 9,
	Year = 1997}

@article{Grotjahn99,
	Author = {R. Grotjahn and D. Hodyss and C. Castello},
	Journal = {Mon. Wea. Rev.},
	Pages = {1089--1095},
	Title = {Do Frontal Cyclones Change Size? Observed Widths of {N}orth {P}acific Lows},
	Volume = 127,
	Year = 1999}

@article{Gryanik00,
	Author = {V. M. Gryanik and T. N. Doronina and D. J. Olbers and T. H. Warncke},
	Journal = {J. Fluid Mech.},
	Pages = {71--125},
	Title = {The theory of three-dimensional hetons and vortex-dominated spreading in localized turbulent convection in a fast rotating stratified fluid},
	Volume = 423,
	Year = 2000}

@article{Gryanik88,
	Annote = {Introduces hetons.},
	Author = {V. M. Gryanik},
	Journal = {Izv. Atmos. Ocean. Physics},
	Pages = {919--926},
	Title = {Localized Vortical Disturbances, "Vortex Charges" and "Vortex Filaments," in a Baroclinic, Differentially Rotating Fluid},
	Volume = 24,
	Year = 1988}

@article{Gu01,
	Annote = {Filed under ITCZ Dynamics.},
	Author = {G. Gu and C. Zhang},
	Journal = {J. Climate},
	Pages = {2725--2739},
	Title = {A Spectrum Analysis of Synoptic-Scale Disturbances in the {ITCZ}},
	Volume = 14,
	Year = 2001}

@article{Gu07,
	Author = {G. Gu and R. F. Adler and G. J. Huffman and S. Curtis},
	File = {../../Papers/gu07.pdf},
	Journal = {J. Climate},
	Pages = {4033--4046},
	Title = {Tropical Rainfall Variability on Interannual-to-Interdecadal and Longer Time Scales Derived from the {GPCP} Monthly Product},
	Volume = 20,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfghndTA3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ43w2dSjgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw2fDDgAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3UwNy5wZGYAAA4AEgAIAGcAdQAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL2d1MDcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL2d1MDcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@article{Gu97,
	Annote = {Filed under Philander. Subduction of water parcels
                  in extratropics and upwelling in tropics.},
	Author = {D. Gu and S. G. Philander},
	File = {../../Papers/gu97.pdf},
	Journal = {Science},
	Pages = {805--807},
	Title = {Interdecadal Climate Fluctuations That Depend on Exchanges Between the Tropics and Extratropics},
	Volume = 275,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfghndTk3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ44xUdEJQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxUe0pQAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3U5Ny5wZGYAAA4AEgAIAGcAdQA5ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL2d1OTcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL2d1OTcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@book{Guckenheimer83,
	Address = {New York},
	Author = {J. Guckenheimer and P. Holmes},
	Pages = 459,
	Publisher = {Springer},
	Title = {Nonlinear Oscillations, Dynamical Systems, and Bifurcations of Vector Fields},
	Year = 1983}

@incollection{Guillot04,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {T. Guillot and D. J. Stevenson and W. B. Hubbard and D. Saumon},
	Booktitle = {Jupiter: The Planet, Satellites and Magnetosphere},
	Editor = {F. Bagenal and T. E. Dowling and W. B. McKinnon},
	Pages = {35--57},
	Publisher = {Cambridge University Press},
	Title = {The Interior of {J}upiter},
	Year = 2004}

@article{Guillot05,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {T. Guillot},
	File = {../../Papers/guillot05.pdf},
	Journal = {Ann. Rev. Earth Planet. Sci.},
	Pages = {493--530},
	Title = {The Interiors of Giant Planets: Models and Outstanding Questions},
	Volume = 33,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ndWlsbG90MDUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ45w7Zi9QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7bTdQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3VpbGxvdDA1LnBkZgAOABwADQBnAHUAaQBsAGwAbwB0ADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZ3VpbGxvdDA1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2d1aWxsb3QwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Guillot99,
	Author = {T. Guillot},
	File = {../../Papers/guillot99.pdf},
	Journal = {Planet. Space Sci.},
	Pages = {1183--1200},
	Title = {A comparison of the interiors of {J}upiter and {S}aturn},
	Volume = {47},
	Year = {1999},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ndWlsbG90OTkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ46xJ2OLwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxJ3wnwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3VpbGxvdDk5LnBkZgAOABwADQBnAHUAaQBsAGwAbwB0ADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvZ3VpbGxvdDk5LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2d1aWxsb3Q5OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Gurney02,
	Annote = {Filed under Carbon Flux Estimates. Comparison of
                  models in inversion of regional-average carbon
                  fluxes.},
	Author = {K. R. Gurney and R. M. Law and A. S. Denning and P. J. Rayner and D. Baker and P. Bousquet and L. Bruhwiler and Y.-H. Chen and P. Clais and S. Fan and I. Y. Fung and M. Gloor and M. Heimann and K. Higuchi and J. John and T. Maki and S. Maksyutov and K. Masarie and P. Peylin and M. Prather and B. C. Pak and J. Randerson and J. Sarmiento and S. Taguchi and Taro Takahashi and C.-W. Yuen},
	Journal = {Nature},
	Pages = {626--630},
	Title = {Towards robust regional estimates of {$\mathrm{CO}_2$} sources and sinks using atmospheric transport models},
	Volume = 415,
	Year = 2002}

@article{Gutowski92,
	Author = {Gutowski, Jr., W. J. and L. E. Branscome and D. A. Stewart},
	File = {../../Papers/gutowski92.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {306--319},
	Title = {Life Cycles of Moist Baroclinic Eddies},
	Volume = 49,
	Year = 1992,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5ndXRvd3NraTkyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ49vrcb/QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvrd+bQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Z3V0b3dza2k5Mi5wZGYAAA4AHgAOAGcAdQB0AG8AdwBzAGsAaQA5ADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2d1dG93c2tpOTIucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2d1dG93c2tpOTIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Gutowski97,
	Annote = {Not on file.},
	Author = {W. J. Gutowski and Y. B. Chen Z. Otles},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {1957--1969},
	Title = {Atmospheric water vapor transport in NCEP-NCAR reanalyses: Comparison with river discharge in the central United States},
	Volume = 78,
	Year = 1997}

@article{Haberle93,
	Annote = {Filed under Mars Dynamics.},
	Author = {R. M. Haberle and J. B. Pollack and J. R. Barnes and R. W. Zurek and C. B. Leovy and J. R. Murphy and H. Lee and J. Schaeffer},
	File = {../../Papers/haberle93.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {3093--3123},
	Title = {Mars Atmospheric Dynamics as Simulated by the {NASA} {Ames} General Circulation Model. 1. {T}he Zonal-Mean Circulation},
	Volume = {98E},
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1oYWJlcmxlOTMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ4+v3k4SQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3mauQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGFiZXJsZTkzLnBkZgAOABwADQBoAGEAYgBlAHIAbABlADkAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaGFiZXJsZTkzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hhYmVybGU5My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Hadley1735,
	Author = {G. Hadley},
	File = {../../Papers/hadley1735.pdf},
	Journal = {Phil. Trans.},
	Pages = {58--62},
	Title = {Concerning the Cause of the General Trade-Winds},
	Volume = 39,
	Year = 1735,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5oYWRsZXkxNzM1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5BvXCDxQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvXDmNQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGFkbGV5MTczNS5wZGYAAA4AHgAOAGgAYQBkAGwAZQB5ADEANwAzADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2hhZGxleTE3MzUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2hhZGxleTE3MzUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Hagan05,
	Annote = {Filed under Ornstein-Uhlenbeck
                  Processes. First-passage times.},
	Author = {P. S. Hagan and C. R. Doering and C. D. Levermore},
	Journal = {SIAM J. App. Math.},
	Pages = {1480--1513},
	Title = {Mean Exit Times for Particles Driven by Weakly Colored Noise},
	Volume = 49,
	Year = 1989}

@article{Haidvogel80,
	Annote = {Filed under Geostrophic Turbulence.},
	Author = {D. B. Haidvogel and I. M. Held},
	File = {../../Papers/haidvogel80.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2644-2660},
	Title = {Homogeneous quasi-geostrophic turbulence driven by a uniform temperature gradient},
	Volume = 37,
	Year = 1980,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9oYWlkdm9nZWw4MC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5CvRcnKgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvReJmgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGFpZHZvZ2VsODAucGRmAA4AIAAPAGgAYQBpAGQAdgBvAGcAZQBsADgAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvaGFpZHZvZ2VsODAucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvaGFpZHZvZ2VsODAucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@book{Haken83,
	Author = {H. Haken},
	Edition = {2nd},
	Publisher = {Springer},
	Title = {Synergetics --- {A}n Introduction},
	Year = {1983}}

@article{Hall01,
	Author = {A. Hall and R. J. Stouffer},
	Journal = {Nature},
	Pages = {171--174},
	Title = {An abrupt climate event in a coupled ocean-atmosphere simulation without external forcing},
	Volume = 409,
	Year = 2001}

@article{Hall93,
	Annote = {Filed under Entropy Estimation. Expand work of
                  Joe89.},
	Author = {P. Hall and S. C. Morton},
	Journal = {Ann. Inst. Stat. Math.},
	Pages = {69--88},
	Title = {On the Estimation of Entropy},
	Volume = 45,
	Year = 1993}

@article{Hall94,
	Author = {T. M. Hall and R. A. Plumb},
	File = {../../Papers/hall94.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {1059--1070},
	Title = {Age as a diagnostic of stratospheric transport},
	Volume = {99D},
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoYWxsOTQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5Dw7ESQFBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7GCwAAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGFsbDk0LnBkZgAADgAWAAoAaABhAGwAbAA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hhbGw5NC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGFsbDk0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Hall95,
	Annote = {Not on file.},
	Author = {N. M. J. Hall and B. J. Hoskins and P. J. Valdes and C. A. Senior},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1209--1230},
	Title = {Storm tracks in a high-resolution {GCM} with doubled carbon dioxide},
	Volume = 120,
	Year = 1995}

@article{Hall99a,
	Annote = {Filed under Water Vapor Feedback (Feedback and
                  Kinematics).},
	Author = {A. Hall and S. Manabe},
	Date-Modified = {2010-06-22 12:55:28 -0700},
	Journal = {J. Climate},
	Pages = {2327--2346},
	Title = {The role of water vapor feedback in unperturbed climate variability and global warming},
	Volume = 12,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoYWxsOTlhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5FyEZiggAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEbE8gAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGFsbDk5YS5wZGYADgAYAAsAaABhAGwAbAA5ADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGFsbDk5YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oYWxsOTlhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{HallNMJ94,
	Author = {Hall N. M. J. and Hoskins B. J. and Valdes P. J., Senior C. A.},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1209--1230},
	Title = {Storm Tracks in a High-Resolution {GCM} with Doubled Carbon-Dioxide},
	Volume = 120,
	Year = 1994}

@incollection{Hallberg00,
	Author = {R. Hallberg and P. B. Rhines},
	Booktitle = {Developments in Geophysical Turbulence},
	Editor = {R. M. Kerr and Y. Kimura},
	Pages = {51--65},
	Publisher = {Kluwer Acad. Publishers},
	Title = {Boundary sources of potential vorticity in geophysical circulations},
	Year = 2000}

@article{Hallberg96,
	Author = {R. Hallberg and P. Rhines},
	Journal = {J. Phys. Oceanogr.},
	Pages = {913--940},
	Title = {Buoyancy-driven circulation in an ocean basin with isopycnals intersecting the sloping boundary},
	Volume = 26,
	Year = 1996}

@article{Hallberg97,
	Author = {R. Hallberg},
	Journal = {J. Phys. Oceanogr.},
	Pages = {977--998},
	Title = {Localized coupling between surface and bottom-intensified flow over topography},
	Volume = 26,
	Year = 1997}

@article{Halley1686,
	Author = {E. Halley},
	File = {../../Papers/halley1686.pdf},
	Journal = {Phil. Trans.},
	Pages = {153--168},
	Title = {An Historical Account of the Trade Winds, and Monsoons, observable in the Seas between and near the Tropicks, with an attempt to assign the Phisical cause of the said Winds},
	Volume = 16,
	Year = 1686,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5oYWxsZXkxNjg2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5Gxxb9sAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxxduMAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGFsbGV5MTY4Ni5wZGYAAA4AHgAOAGgAYQBsAGwAZQB5ADEANgA4ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2hhbGxleTE2ODYucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2hhbGxleTE2ODYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Halliwell97,
	Annote = {Not on file.},
	Author = {G. R. Halliwell},
	Journal = {J. Climate},
	Pages = {2405--2411},
	Title = {Decadal and Multidecadal {N}orth {A}tlantic {SST} Anomalies Driven by Standing and Propagating Basin-Scale Atmospheric Anomalies},
	Volume = {10},
	Year = 1997}

@article{Halliwell98,
	Annote = {Not on file.},
	Author = {G. R. Halliwell},
	Journal = {J. Phys. Oceanogr.},
	Pages = {5--21},
	Title = {Simulation of {N}orth {A}tlantic decadal/multidecadal winter {SST} anomalies driven by basin-scale atmospheric circulation anomalies},
	Volume = {28},
	Year = 1998}

@book{Haltiner80,
	Address = {New York},
	Author = {G. J. Haltiner and R. T. Williams},
	Edition = {2nd},
	Pages = 477,
	Publisher = {Wiley},
	Title = {Numerical Prediction and Dynamic Meteorology},
	Year = 1980}

@article{Hamilton01,
	Author = {K. Hamilton and R. J. Wilson and R. S Hemler},
	Journal = {J. Atmos. Sci.},
	Pages = {3271--3292},
	Title = {Spontaneous Stratospheric {QBO}-like Oscillations Simulated by the {GFDL} {SKYHI} General Circulation Model},
	Volume = 58,
	Year = 2001}

@incollection{Hamilton87,
	Annote = {Nice review of observations: only sparse data for
                  SAO so that its meridional/azimuthal structure
                  cannot be determined reliably; better data for QBO},
	Author = {K. P. Hamilton},
	Booktitle = {Transport Processes in the Middle Atmosphere},
	Editor = {G. Visconti and R. Garcia},
	Pages = {19--29},
	Publisher = {D. Reidel Publishing Company},
	Title = {A Review of Observations of the {Q}uasi-biennial and {S}emiannual {O}scillations of Wind and Temperature in the Tropical Middle Atmosphere},
	Year = {1987}}

@article{Hamilton89,
	Author = {K. Hamilton},
	Journal = {J. Atmos. Sci.},
	Pages = {1019--1025},
	Title = {Interhemispheric Asymmetry and Annual Synchronization of the Ozone {Q}uasi-biennial {O}scillation},
	Volume = 46,
	Year = 1989}

@incollection{Hamilton94,
	Author = {K. P. Hamilton},
	Booktitle = {Encyclopedia of Applied Physics},
	Pages = {215--237},
	Publisher = {VCH Publishers},
	Title = {Meteorology and Climatology},
	Volume = {10},
	Year = {1994}}

@article{Hamilton95,
	Author = {K. P. Hamilton},
	Journal = {J. Atmos. Terr. Phys.},
	Note = {In press},
	Title = {Comprehensive Meteorological Modeling of the Middle Atmosphere: {A} Tutorial Review},
	Volume = {?},
	Year = {1996}}

@unpublished{Hamilton96,
	Annote = {Shallow water waves; internal inertia-gravity waves;
                  3D separable problems, normal modes; QG waves and
                  instabilities. Computer programs for simple QBO
                  model, linear gravity waves.},
	Author = {K. P. Hamilton},
	Note = {Lecture notes},
	Title = {Geophysical Wave Dynamics},
	Year = {Spring 1996}}

@article{Hammel05,
	Author = {Hammel, H. B. and de Pater, I. and Gibbard, S. and Lockwood, G. W. and Rages, K.},
	File = {../../Papers/hammel05.pdf},
	Journal = {Icarus},
	Pages = {534--545},
	Title = {{Uranus} in 2003: {Z}onal winds, banded structure, and discrete features},
	Volume = {175},
	Year = {2005},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxoYW1tZWwwNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5JyCvhbAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyCxD3AAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGFtbWVsMDUucGRmAAAOABoADABoAGEAbQBtAGUAbAAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2hhbW1lbDA1LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9oYW1tZWwwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@book{Hand81,
	Address = {Chichester},
	Author = {D. J. Hand},
	Pages = 218,
	Publisher = {Wiley},
	Series = {Series in Probability and Mathematical Statistics},
	Title = {Discrimination and Classification},
	Year = 1981}

@article{Hanel81,
	Author = {R. A. Hanel and B. J. Conrath and L. W. Herath and V. G. Kunde and J. A. Pirraglia},
	File = {../../Papers/hanel81.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {8705--8712},
	Title = {Albedo, internal heat, and energy balance of {J}upiter---preliminary results of the {V}oyager infrared investigation},
	Volume = 86,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoYW5lbDgxLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5KxFmp7AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxFoMXAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGFuZWw4MS5wZGYADgAYAAsAaABhAG4AZQBsADgAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGFuZWw4MS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oYW5lbDgxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Hanke93,
	Annote = {Not on file.},
	Author = {M. Hanke and P. C. Hansen},
	Journal = {Surveys Math. Indust.},
	Pages = {253--315},
	Title = {Regularization Methods for Large-Scale Problems},
	Volume = 3,
	Year = 1993}

@article{Hansen92,
	Annote = {Not on file.},
	Author = {P. C. Hansen},
	Journal = {SIAM Review},
	Pages = {561--580},
	Title = {Analysis of Discrete Ill-Posed Problems by Means of the {L}-Curve},
	Volume = 34,
	Year = 1992}

@article{Hansen94,
	Annote = {Not on File. Available at
                  serv1.imm.dtu.dk/~pch/Regutools/regutools.html},
	Author = {P. C. Hansen},
	Journal = {Numer. Algorithms},
	Pages = {1--35},
	Title = {Regularization Tools: A {M}atlab package for analysis and solution of discrete ill-posed problems},
	Volume = 6,
	Year = 1994}

@book{Hansen98,
	Address = {Philadelphia, PA},
	Author = {P. C. Hansen},
	Pages = 247,
	Publisher = {Society for Industrial and Applied Mathematics},
	Series = {SIAM Monogr. on Mathematical Modeling and Computation},
	Title = {Rank-Deficient and Discrete Ill-Posed Problems: Numerical Aspects of Linear Inversion},
	Year = 1998}

@article{Hao93,
	Annote = {Not on file.},
	Author = {Z. Hao and J. D. Neelin and F.-F. Jin},
	Journal = {J. Climate},
	Pages = {1523--1544},
	Title = {Nonlinear Tropical Air-Sea Interaction in the Fast-Wave Limit},
	Volume = 6,
	Year = 1993}

@article{Harnik98,
	Annote = {Filed under Tropopause Dynamics. Elaborate on
                  Lindzen93 model.},
	Author = {N. Harnik and R. S. Lindzen},
	Journal = {J. Atmos. Sci.},
	Pages = {344-360},
	Title = {The Effect of Basic-State Potential Vorticity Gradients on the Growth of Baroclinic Waves and the Height of the Tropopause},
	Volume = 55,
	Year = 1998}

@article{Hartley98,
	Annote = {Use pv inversion to determine influence of pv
                  anomalies on geopotential height. Find that
                  disturbances at polar vortex edge significantly
                  influence tropopause height anomalies.},
	Author = {D. E. Hartley and J. T. Villarin and R. X. Black and C. A. Davis},
	Journal = {Nature},
	Pages = {471--474},
	Title = {A new perspective on the dynamical link between the stratosphere and troposphere},
	Volume = 391,
	Year = 1998}

@article{Hartmann00,
	Annote = {Overview over possible stratosphere-troposphere
                  interactions, annular modes, NAO, etc. Possible
                  interactions between ozone depletion and global
                  warming.},
	Author = {D. L. Hartmann and J. M. Wallace and V. Limpasuvan and D. W. J. Thompson and J. R. Holton},
	Journal = {Proc. Nat. Acad. Sci.},
	Pages = {1412--1417},
	Title = {Can ozone depletion and glovbal warming interact to produce rapid climate change?},
	Volume = 97,
	Year = 2000}

@article{Hartmann01,
	Annote = {Use ERBE and ISCCP data to estimate effect of
                  various cloud types on radiation budget. Propose
                  feedback mechanism that lead to cancelation of
                  positive and negative effects on radiation balance.},
	Author = {D. L. Hartmann and L. A. Moy and Q. Fu},
	Journal = {J. Climate},
	Pages = {4495--4511},
	Title = {Tropical Convection and the Energy Balance at the Top of the Atmosphere},
	Volume = 14,
	Year = 2001}

@article{Hartmann07,
	Author = {D. L. Hartmann},
	Journal = {J. Meteor. Soc. Japan},
	Pages = {123--143},
	Title = {The Atmospheric General Circulation and its Variability},
	Volume = {85B},
	Year = 2007}

@unpublished{Hartmann94,
	Author = {D. L. Hartmann},
	Note = {submitted to {\em J. Atmos. Sci.}},
	Title = {A {PV} View of Zonal Mean Flow Vacillation},
	Year = 1994}

@article{Harville74,
	Annote = {Filed under Parameter Estimation.},
	Author = {D.~A. Harville},
	Journal = {Biometrika},
	Key = {parameter estimation, restricted maximum likelihood},
	Pages = {383--385},
	Title = {Bayesian inference for variance components using only error contrasts},
	Volume = {61},
	Year = 1974}

@article{Harville77,
	Annote = {Filed under Parameter Estimation.},
	Author = {D.~A. Harville},
	Journal = {J. Amer. Statist. Assoc.},
	Key = {parameter estimation, restricted maximum likelihood},
	Pages = {320--341},
	Title = {Maximum likelihood approaches to variance component estimation and to related problems},
	Volume = {72},
	Year = 1977}

@article{Harzallah95,
	Annote = {Filed under Predictability.},
	Author = {A. Harzallah and R. Sadourny},
	Journal = {J. Climate},
	Pages = {474--495},
	Title = {Internal Versus {SST}-Forced Atmospheric Variability as Simulated by an Atmospheric Circulation Model},
	Volume = 8,
	Year = 1995}

@article{Hasselmann76,
	Author = {K. Hasselmann},
	Journal = {Tellus},
	Pages = {473--485},
	Title = {Stochastic Climate Models. {P}art {I}: {T}heory},
	Volume = 28,
	Year = 1976}

@article{Hasselmann88,
	Author = {K. Hasselmann},
	Journal = {J. Geophys. Res.},
	Pages = {11015--11021},
	Title = {{PIP}s and {POP}s: The Reduction of Complex Dynamical Systems using {P}rincipal {I}nteraction and {O}scillation {P}atterns},
	Volume = {93D},
	Year = 1988}

@article{Hasselmann93,
	Annote = {Filed under Climate Change Detection. Uses
                  discriminant analysis to find the linear combination
                  of data that discriminates best between control and
                  climate change populations.},
	Author = {K. Hasselmann},
	Journal = {J. Climate},
	Pages = {1957--1971},
	Title = {Optimal Fingerprints for the Detection of Time-dependent Climate Change},
	Volume = 6,
	Year = 1993}

@article{Hasselmann97,
	Annote = {Filed under Climate Change Detection. Claims that
                  dimension reduction always improves tests of climate
                  change detection. Gives an example using Gaussian
                  distribution (instead of the correct t-or
                  F-distribution) to substantiate his claim. Arguments
                  appears to be wrong because they suggest that ANOVA
                  is always preferable to MANOVA, which is not
                  true. Probably he should have considered the power
                  of the test as a function of dimension and "signal
                  strength," holding the significance level
                  fixed. This would give some optimum dimension that
                  depends on the exact characteristics of signal and
                  noise. The optimum dimension need not be
                  one. Additional informative components can increase
                  the power of the test (as in the $T^2$-statistic,
                  for example; see Johnson82, chap.~5B). Another
                  important distinction that is lacking in his
                  argument: that between simultaneous confidence
                  intervals (from F-statistic) and Bonferroni
                  confidence intervals (from t-statistic). His use of
                  Gaussian statistics is wrong. (Asymptotically,
                  chi-squared would be justified.)},
	Author = {K. Hasselmann},
	Journal = {Climate Dyn.},
	Pages = {601--611},
	Title = {Multi-pattern fingerprint method for detection and attribution of climate change},
	Volume = 13,
	Year = 1997}

@article{Hayashi81,
	Annote = {Not on file.},
	Author = {Y. Hayashi and D. G. Golder},
	Journal = {J. Atmos. Sci.},
	Pages = {2532--2539},
	Title = {The effects of condensational heating on midlatitude transient waves in their mature stage: {C}ontrol experiments with a {GFDL} general circulation model},
	Volume = 38,
	Year = 1981}

@article{Hayashi85,
	Annote = {Apparent nonaccleration theorem violations in
                  standard EP diagnostics because of lower boundary
                  conditions. },
	Author = {Y. Hayashi},
	File = {../../Papers/hayashi85.pdf},
	Journal = {J. Meteor. Soc. Japan},
	Pages = {497--512},
	Title = {Theoretical Interpretation of the {E}liassen-{P}alm Diagnostics of Wave-Mean Flow Interaction. {Part}~I: Effects of the Lower Boundary},
	Volume = 63,
	Year = 1985,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1oYXlhc2hpODUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5SvMFTFAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvMG1hAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGF5YXNoaTg1LnBkZgAOABwADQBoAGEAeQBhAHMAaABpADgANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaGF5YXNoaTg1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hheWFzaGk4NS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Hayashi86,
	Annote = {Filed under Predictability.},
	Author = {Y. Hayashi},
	Journal = {J. Meteor. Soc. Japan},
	Pages = {167--181},
	Title = {Statistical Interpretation of Ensemble-Time Mean Predictability},
	Volume = 64,
	Year = 1986}

@article{Hayes77,
	Author = {M. Hayes},
	File = {../../Papers/hayes77.pdf},
	Journal = {Proc. Roy. Soc. London A},
	Pages = {533--535},
	Title = {A note on group velocity},
	Volume = 354,
	Year = 1977,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoYXllczc3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5TxGc9M1BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxGefowAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGF5ZXM3Ny5wZGYADgAYAAsAaABhAHkAZQBzADcANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGF5ZXM3Ny5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oYXllczc3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Haynes00a,
	Author = {P. Haynes and E. Shuckburgh},
	File = {../../Papers/haynes00a.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {22777--22794},
	Title = {Effective diffusivity as a diagnostic of atmospheric transport. 1. {Stratosphere}},
	Volume = {105D},
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1oYXluZXMwMGEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5Uvt+fLAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvuABnAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGF5bmVzMDBhLnBkZgAOABwADQBoAGEAeQBuAGUAcwAwADAAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaGF5bmVzMDBhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hheW5lczAwYS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Haynes00b,
	Author = {P. Haynes and E. Shuckburgh},
	File = {../../Papers/haynes00b.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {22795--22810},
	Title = {Effective diffusivity as a diagnostic of atmospheric transport. 2. {Troposphere} and lower stratosphere},
	Volume = {105D},
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1oYXluZXMwMGIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5Vvt+fTgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvuABvgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGF5bmVzMDBiLnBkZgAOABwADQBoAGEAeQBuAGUAcwAwADAAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaGF5bmVzMDBiLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hheW5lczAwYi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Haynes01,
	Annote = {Filed under Tropopause Dynamics. Simulations with
                  primitive equation model show that tropopause can
                  form by interaction of baroclinic eddies with
                  large-scale dissipation (thermal relaxation towards
                  smooth equilibrium state).},
	Author = {P. Haynes and J. Scinocca and M. Greenslade},
	File = {../../Papers/haynes01.pdf},
	Journal = {Geophys. Res. Lett.},
	Pages = {4179--4182},
	Title = {Formation and maintenance of the extratropical tropopause by baroclinic eddies},
	Volume = {28},
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxoYXluZXMwMS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5Wvt+dvAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvuAALAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGF5bmVzMDEucGRmAAAOABoADABoAGEAeQBuAGUAcwAwADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2hheW5lczAxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9oYXluZXMwMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Haynes87,
	Annote = {Filed under Haynes. Regard PV as
                  tracer. Impermeability theorem.},
	Author = {P. H. Haynes and M. E. {McIntyre}},
	Journal = {J. Atmos. Sci.},
	Pages = {828--841},
	Title = {On the Evolution of Vorticity and Potential Vorticity in the Presence of Diabatic Heating and Frictional or Other Forces},
	Volume = 44,
	Year = 1987}

@article{Haynes87b,
	Annote = {Filed under Haynes. Weakly nonlinear models (taken
                  only interaction between one wave and mean flow into
                  account) represent gross features of critical layer
                  dynamics qualitatively, despite lack of wave-wave
                  interactions that lead to the generation of small
                  scales.},
	Author = {P. H. Haynes and M. E. {McIntyre}},
	File = {../../Papers/haynes87b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2359--2382},
	Title = {On the reprensentation of {Rossby} wave critical layers and wave breaking in zonally truncated models},
	Volume = 44,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1oYXluZXM4N2IucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5bwq3kz1BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwq5HPwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGF5bmVzODdiLnBkZgAOABwADQBoAGEAeQBuAGUAcwA4ADcAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaGF5bmVzODdiLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hheW5lczg3Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Haynes88,
	Author = {P. H. Haynes},
	Journal = {J. Atmos. Sci.},
	Pages = {2352--2362},
	Title = {Forced, Dissipative Generalizations of Finite-Amplitude Wave-Activity Conservation Relations for Zonal and Nonzonal Basic Flows},
	Volume = 45,
	Year = 1988}

@article{Haynes90,
	Annote = {Filed under Haynes. Sequel to Haynes and McIntyre
                  (1987).},
	Author = {P. H. Haynes and M. E. {McIntyre}},
	Journal = {J. Atmos. Sci.},
	Pages = {2021--2031},
	Title = {On the Conservation and Impermeability Theorems for Potential Vorticity},
	Volume = 47,
	Year = 1990}

@article{Haynes91,
	Annote = {Downward control principle. Stratospheric influence
                  on tropopause height.},
	Author = {P. H. Haynes and C. J. Marks and M. E. McIntyre and T. G. Shepherd and K. P. Shine},
	File = {../../Papers/haynes91.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {651--679},
	Title = {On the downward control of extratropical diabatic circulations by eddy-induced mean zonal forces},
	Volume = 48,
	Year = 1991,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxoYXluZXM5MS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5cw8KQmQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw8MBGQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGF5bmVzOTEucGRmAAAOABoADABoAGEAeQBuAGUAcwA5ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2hheW5lczkxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9oYXluZXM5MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Haywood95,
	Annote = {Filed under Climate Change Detection.},
	Author = {J. M. Haywood and K. P. Shine},
	Journal = {Geophys. Res. Lett.},
	Pages = {603--606},
	Title = {The effect of anthropogenic sulfate and soot aerosol on the clear sky planetary radiation budget},
	Volume = 22,
	Year = 1995}

@article{Hegerl06a,
	Author = {G. C. Hegerl and T. J. Crowley and W. T. Hyde and D. J. Frame},
	Journal = {Nature},
	Pages = {1029--1032},
	Title = {Climate sensitivity constrained by temperature reconstructions over the past seven centuries},
	Volume = 440,
	Year = 2006}

@article{Hegerl06b,
	Author = {G. C. Hegerl and T. J. Crowley and M. Allen and W. T. Hyde and H. N. Pollack and J. Smerdon and E. Zorita},
	File = {../../Papers/hegerl06b.pdf},
	Journal = {J. Climate},
	Note = {Submitted},
	Title = {Detection of human influence on a new, validated 1500~year temperature reconstruction},
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1oZWdlcmwwNmIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5dwYE49VBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwYGpdQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVnZXJsMDZiLnBkZgAOABwADQBoAGUAZwBlAHIAbAAwADYAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaGVnZXJsMDZiLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hlZ2VybDA2Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@incollection{Hegerl07,
	Address = {Cambridge, UK, and New York, NY, USA},
	Author = {G. C. Hegerl and F. W. Zwiers and P. Braconnot and N. P. Gillett and Y. Luo and J. A. Marengo Orsini and N. Nicholls and J. E. Penner and P.A. Stott},
	Booktitle = {Climate Change 2007: The Physical Science Basis. Contribution of Working Group I to the Fourth Assessment Report of the Intergovernmental Panel on Climate Change},
	Editor = {S. Solomon and D. Qin and M. Manning and Z. Chen and M. Marquis and K.B. Averyt and M. Tignor and H.L. Miller},
	Pages = {664--745},
	Publisher = {Cambridge Univ. Press},
	Title = {Understanding and Attributing Climate Change},
	Year = 2007}

@article{Hegerl96,
	Annote = {Filed under Climate Change Detection. Assess
                  significance of 15, 20, and 30 year trends in
                  observed SAT over the decades prior to 1994. Use
                  pattern correlation statistic and `detection
                  variable', which is the projection of the
                  temperature trends on the fingerprint $f=C^{-1}g$,
                  where $g$ is the `guess pattern' of climate
                  change. The guess pattern of climate change is the
                  difference between the simulated climate 1986--1995
                  and 2076--2085. (`Static view' of climate change:
                  pattern `emerging' from background of natural
                  variability.) There is confusion about basic linear
                  algebra concepts: non-orthogonal transformations are
                  called `rotation', mixing up of dual vectors with
                  coordinate vectors, etc.},
	Author = {G. C. Hegerl and H. {von Storch} and K. Hasselmann and B. D. Santer and U. Cubasch and P. D. Jones},
	Journal = {J. Climate},
	Pages = {2281--2306},
	Title = {Detecting Greenhouse-Gas-Induced Climate Change with an Optimal Fingerprint Method},
	Volume = 9,
	Year = 1996}

@article{Hegerl97a,
	Annote = {Filed under Climate Change Detection. Reviews
                  Hasselmann79, Hasselmann93, Bell82, North95. Shows
                  that all approaches to climate change detection are
                  essentially the same. Seem to think that a
                  ``detection variable'' leads to ``clearer detection
                  of [climate change] signal'' in observational
                  record; but a detection variable can only indicate
                  what climate characteristic changes most drastically
                  when the climate changes.},
	Author = {G. C. Hegerl and G. R. North},
	Journal = {J. Climate},
	Pages = {1125--1133},
	Title = {Comparison of Statistically Optimal Approaches to Detecting Anthropogenic Climate Change},
	Volume = 10,
	Year = 1997}

@article{Hegerl97b,
	Annote = {Filed under Climate Change Detection. Define climate
                  change signal as EOF of model simulation and try to
                  ``detect'' signal in observed record using the
                  methodology of Hasselmann97.},
	Author = {G. C. Hegerl and K. Hasselmann and U. Cubasch and J. F. B. Mitchell and E. Roeckner and R. Voss and J. Waszkewitz},
	Journal = {Climate Dyn.},
	Pages = {613--634},
	Title = {Multi-fingerprint detection and attribution analysis of greenhouse gas, greenhouse gas-plus-aerosol and solar forced climate change},
	Volume = 13,
	Year = 1997}

@article{Heimpel05,
	Author = {M. Heimpel and J. Aurnou and J. Wicht},
	File = {../../Papers/heimpel05.pdf},
	Journal = {Nature},
	Pages = {193--196},
	Title = {Simulation of equatorial and high-latitude jets on {J}upiter in a deep convection model},
	Volume = 438,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1oZWltcGVsMDUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5ewfjdgwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwflOAwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVpbXBlbDA1LnBkZgAOABwADQBoAGUAaQBtAHAAZQBsADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaGVpbXBlbDA1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hlaW1wZWwwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Heimpel07,
	Author = {Heimpel, M. and Aurnou, J.},
	File = {../../Papers/heimpel07.pdf},
	Journal = {Icarus},
	Pages = {540--557},
	Title = {Turbulent convection in rapidly rotating spherical shells: A model for equatorial and high latitude jets on {Jupiter} and {Saturn}},
	Volume = {187},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1oZWltcGVsMDcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5fw47HKlBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw483qgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVpbXBlbDA3LnBkZgAOABwADQBoAGUAaQBtAHAAZQBsADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaGVpbXBlbDA3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hlaW1wZWwwNy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Held00a,
	Annote = {Filed under Water Vapor (Feedback and
                  Kinematics). Review of water vapor feedback.},
	Author = {I. M. Held and B. J. Soden},
	File = {../../Papers/held00a.pdf},
	Journal = {Annu. Rev. Energy Environ.},
	Pages = {441-475},
	Title = {Water Vapor Feedback and Global Warming},
	Volume = 25,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkMDBhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5gv7uL7AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv7v8bAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDAwYS5wZGYADgAYAAsAaABlAGwAZAAwADAAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDAwYS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkMDBhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@inproceedings{Held00b,
	Address = {Woods Hole, MA},
	Author = {I. M. Held},
	Booktitle = {Proc. Program in Geophysical Fluid Dynamics},
	File = {../../Papers/held00b.pdf},
	Organization = {Woods Hole Oceanographic Institution},
	Title = {The General Circulation of the Atmosphere},
	Url = {https://darchive.mblwhoilibrary.org/handle/1912/15},
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkMDBiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5hv+MtogAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv+OeIgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDAwYi5wZGYADgAYAAsAaABlAGwAZAAwADAAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDAwYi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkMDBiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==},
	Bdsk-Url-1 = {https://darchive.mblwhoilibrary.org/handle/1912/15}}

@article{Held01,
	Author = {I. M. Held},
	File = {../../Papers/held01.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {943--948},
	Title = {The Partitioning of the Poleward Energy Transport between the Tropical Ocean and Atmosphere},
	Volume = 58,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoZWxkMDEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5jwMIV0VBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwMJ4QQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDAxLnBkZgAADgAWAAoAaABlAGwAZAAwADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hlbGQwMS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGVsZDAxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Held02,
	Annote = {Review of stationary wave theory and modeling.},
	Author = {I. M. Held and M. Ting and H. Wang},
	File = {../../Papers/held02.pdf},
	Journal = {J. Climate},
	Pages = {2125--2144},
	Title = {Northern Winter Stationary Waves: {T}heory and Modeling},
	Volume = 15,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoZWxkMDIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5kx1fjTgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx1hTzgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDAyLnBkZgAADgAWAAoAaABlAGwAZAAwADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hlbGQwMi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGVsZDAyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Held06,
	Annote = {Filed under Water Vapor (Feedback and
                  Kinematics).},
	Author = {I. M. Held and B. J. Soden},
	File = {../../Papers/held06.pdf},
	Journal = {J. Climate},
	Pages = {5686--5699},
	Title = {Robust responses of the hydrological cycle to global warming},
	Volume = 19,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoZWxkMDYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5nwYfUfFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwYhE/AAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDA2LnBkZgAADgAWAAoAaABlAGwAZAAwADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hlbGQwNi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGVsZDA2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Held07a,
	Author = {I. M. Held and M. Zhao and B. Wyman},
	File = {../../Papers/held07a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {228--238},
	Title = {Dynamic radiative-convective equilibria using {GCM} column physics},
	Volume = 64,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkMDdhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5oweer0wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwegcUwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDA3YS5wZGYADgAYAAsAaABlAGwAZAAwADcAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDA3YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkMDdhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@incollection{Held07b,
	Address = {Princeton, NJ},
	Author = {I. M. Held},
	Booktitle = {The Global Circulation of the Atmosphere},
	Editor = {T. Schneider and A. H. Sobel},
	Pages = {1--21},
	Publisher = {Princeton University Press},
	Title = {Progress and Problems in Large-Scale Atmospheric Dynamics},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkMDdiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5pwoPHIgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwoQpkgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDA3Yi5wZGYADgAYAAsAaABlAGwAZAAwADcAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDA3Yi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkMDdiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Held74,
	Annote = {Filed under Climate Stability/Energy Balance Models.},
	Author = {I. M. Held and M. J. Suarez},
	File = {../../Papers/held74.pdf},
	Journal = {Tellus},
	Pages = {613--629},
	Title = {Simple albedo feedback models of the icecaps},
	Volume = 26,
	Year = 1974,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoZWxkNzQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5svhaJKgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvhb5qgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDc0LnBkZgAADgAWAAoAaABlAGwAZAA3ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hlbGQ3NC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGVsZDc0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Held75,
	Author = {I. M. Held},
	File = {../../Papers/held75.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1494--1497},
	Title = {Momentum Transport by Quasi-Geostrophic Eddies},
	Volume = 32,
	Year = 1975,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoZWxkNzUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5tvvfvYgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvvhR0gAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDc1LnBkZgAADgAWAAoAaABlAGwAZAA3ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hlbGQ3NS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGVsZDc1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Held78a,
	Author = {I. M. Held and M. J. Suarez},
	File = {../../Papers/held78a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {206--229},
	Title = {A Two-Level Primitive Equation Atmospheric Model Designed for Climatic Sensitivity Experiments},
	Volume = 35,
	Year = 1978,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkNzhhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5uwcGaaQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwcIK6QAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDc4YS5wZGYADgAYAAsAaABlAGwAZAA3ADgAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDc4YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkNzhhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Held78b,
	Author = {I. M. Held},
	File = {../../Papers/held78b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {572--576},
	Title = {The Vertical Scale of an Unstable Baroclinic Wave and Its Importance for Eddy Heat Flux Parameterizations},
	Volume = 35,
	Year = 1978,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkNzhiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5vvRhlNwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRjHpwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDc4Yi5wZGYADgAYAAsAaABlAGwAZAA3ADgAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDc4Yi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkNzhiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Held78c,
	Author = {I. M. Held},
	File = {../../Papers/held78c.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2083--2098},
	Title = {The Tropospheric Lapse Rate and Climatic Sensitivity: Experiments with a Two-Level Atmospheric Model},
	Volume = 35,
	Year = 1978,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkNzhjLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5wwCtbfQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwCvL/QAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDc4Yy5wZGYADgAYAAsAaABlAGwAZAA3ADgAYwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDc4Yy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkNzhjLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Held80,
	Annote = {Filed under Hadley Cell Dynamics. Dynamics of
                  axisymmetric Hadley cell. Scaling theory for extent
                  and width of Hadley cell.},
	Author = {I. M. Held and A. Y. Hou},
	File = {../../Papers/held80.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {515--533},
	Title = {Nonlinear Axially Symmetric Circulations in a Nearly Inviscid Atmosphere},
	Volume = 37,
	Year = 1980,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoZWxkODAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5xvRhllQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRjIBQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDgwLnBkZgAADgAWAAoAaABlAGwAZAA4ADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hlbGQ4MC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGVsZDgwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Held81,
	Annote = {Filed under Climate Stability/Energy Balance Models.},
	Author = {I. M. Held and D. I. Linder and M. J. Suarez},
	File = {../../Papers/held81.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1911--1927},
	Title = {Albedo Feedback, the Meridional Structure of the Effective Heat Diffusivity, and Climate Sensitivity: Results from Dynamic and Diffusive Models},
	Volume = 38,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoZWxkODEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5yvhWW1wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvhYHVwAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDgxLnBkZgAADgAWAAoAaABlAGwAZAA4ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hlbGQ4MS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGVsZDgxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Held82,
	Annote = {Filed under Tropopause Dynamics.},
	Author = {I. M. Held},
	File = {../../Papers/held82.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {412--417},
	Title = {On the Height of the Tropopause and the Static Stability of the Troposphere},
	Volume = 39,
	Year = 1982,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoZWxkODIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ5zvMA2UgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvMCYwgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDgyLnBkZgAADgAWAAoAaABlAGwAZAA4ADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hlbGQ4Mi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGVsZDgyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Held83a,
	Author = {I. M. Held and D. G. Andrews},
	Journal = {J. Atmos. Sci.},
	Pages = {2220--2231},
	Title = {On the direction of the eddy momentum flux in baroclinic instability},
	Volume = 40,
	Year = 1983}

@incollection{Held83b,
	Address = {London},
	Author = {I. M. Held},
	Booktitle = {Large-Scale Dynamical Processes in the Atmosphere},
	Editor = {B. Hoskins and R. P. Pearce},
	Pages = {127--168},
	Publisher = {Academic Press},
	Title = {Stationary and Quasi-Stationary Eddies in the Extratropical Troposphere: Theory},
	Year = 1983}

@incollection{Held85,
	Author = {I. M. Held and B. J. Hoskins},
	Booktitle = {Advances in Geophysics},
	Editor = {S. Manabe},
	File = {../../Papers/held85.pdf},
	Pages = {3--31},
	Publisher = {Academic Press},
	Title = {Large-scale Eddies and the General Circulation of the Troposphere},
	Volume = {28A},
	Year = 1985,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoZWxkODUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ51wpAr91BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwpCOZwAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDg1LnBkZgAADgAWAAoAaABlAGwAZAA4ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hlbGQ4NS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGVsZDg1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Held90b,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {I. M. Held and P. J. Phillips},
	File = {../../Papers/held90b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {856--869},
	Title = {A Barotropic Model of the Interaction between the {H}adley Cell and a {R}ossby Wave},
	Volume = 47,
	Year = 1990,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkOTBiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ52vwy4xgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvw0bNgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDkwYi5wZGYADgAYAAsAaABlAGwAZAA5ADAAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDkwYi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkOTBiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Held92,
	Author = {I. M. Held and E. {O'Brien}},
	Journal = {J. Atmos. Sci.},
	Pages = {1861--1870},
	Title = {Quasigeostrophic Turbulence in a Three-Layer Model: Effects of Vertical Structure in the Mean Shear},
	Volume = 49,
	Year = 1992}

@article{Held93a,
	Author = {I. M. Held},
	Date-Modified = {2010-06-21 10:18:30 -0700},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {228--241},
	Title = {Large-Scale Dynamics and Global Warming},
	Volume = 74,
	Year = {1993},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkOTNhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ53wd0UlgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwd2FFgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDkzYS5wZGYADgAYAAsAaABlAGwAZAA5ADMAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDkzYS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkOTNhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Held93b,
	Annote = {Shear in mean flow organizes convection.},
	Author = {I. M. Held and R. S. Hemler and V. Ramaswamy},
	Journal = {J. Atmos. Sci.},
	Pages = {3909--3927},
	Title = {Radiative-Convective Equilibrium with Explicit Two-Dimensional Moist Convection},
	Volume = 50,
	Year = 1993}

@article{Held94,
	Annote = {Benchmark calculations with Rayleigh friction in
                  boundary layer and Newtonian cooling in interior.},
	Author = {I. M. Held and M. J. Suarez},
	File = {../../Papers/held94.pdf},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {1825--1830},
	Title = {A Proposal for the Intercomparison of the Dynamical Cores of Atmospheric General Circulation Models},
	Volume = 75,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoZWxkOTQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ54xIiODVBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxIjwfQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDk0LnBkZgAADgAWAAoAaABlAGwAZAA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hlbGQ5NC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGVsZDk0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Held95a,
	Author = {I. M. Held and R. T. Pierrehumbert and S. T. Garner and K. L. Swanson},
	Journal = {J. Fluid. Mech.},
	Key = {turbulence},
	Pages = {1--20},
	Title = {Surface quasi-geostrophic dynamics},
	Volume = 282,
	Year = 1995}

@article{Held96,
	Annote = {Filed under Held. Based on Larichev95.},
	Author = {I. M. Held and V. D. Larichev},
	File = {../../Papers/held96.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {946--952},
	Title = {A Scaling Theory for Horizontally Homogeneous, Baroclinically Unstable Flow on a Beta-Plane},
	Volume = 53,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoZWxkOTYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ55vRiHhQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRjp9QAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDk2LnBkZgAADgAWAAoAaABlAGwAZAA5ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hlbGQ5Ni5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGVsZDk2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@unpublished{Held97,
	Author = {I. M. Held},
	Note = {Class notes},
	Title = {Geophysical Fluid Dynamics},
	Year = 1997}

@article{Held99a,
	Author = {I. M. Held and T. Schneider},
	Journal = {J. Atmos. Sci.},
	Pages = {1688--1697},
	Title = {The Surface Branch of the Zonally Averaged Mass Transport Circulation in the Troposphere},
	Volume = 56,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkOTlhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ56ubdjfAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAubfF7AAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDk5YS5wZGYADgAYAAsAaABlAGwAZAA5ADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDk5YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkOTlhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Held99b,
	Author = {I. M. Held},
	File = {../../Papers/held99b.pdf},
	Journal = {Tellus},
	Pages = {59--70},
	Title = {The Macroturbulence of the Troposphere},
	Volume = {51A-B},
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkOTliLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ57wimMVAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwinuxAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDk5Yi5wZGYADgAYAAsAaABlAGwAZAA5ADkAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDk5Yi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkOTliLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@unpublished{Held99c,
	Author = {I. M. Held},
	File = {../../Papers/held99c.pdf},
	Note = {Bernhard Haurwitz Memorial Lecture, American Meteorological Society. Available at www.gfdl.noaa.gov/\~{}ih.},
	Title = {Equatorial Superrotation in {Earth}-like Atmospheric Models},
	Year = {1999},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtoZWxkOTljLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ58wTYwgAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwTaS8AAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVsZDk5Yy5wZGYADgAYAAsAaABlAGwAZAA5ADkAYwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaGVsZDk5Yy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9oZWxkOTljLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Herweijer05,
	Author = {C. Herweijer and R. Seager and M. Winton and A. Clement},
	File = {../../Papers/herweijer05.pdf},
	Journal = {Tellus},
	Pages = {662--675},
	Title = {Why ocean heat transport warms the global mean climate},
	Volume = {57A},
	Year = {2005},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9oZXJ3ZWlqZXIwNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6BxkivKAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxkkRmAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGVyd2VpamVyMDUucGRmAA4AIAAPAGgAZQByAHcAZQBpAGoAZQByADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvaGVyd2VpamVyMDUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvaGVyd2VpamVyMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Herzel94,
	Annote = {Filed under Entropy Estimation. Recommended by Jens
                  Timmer.},
	Author = {H. Herzel and A. O. Schmitt and W. Ebeling},
	Journal = {Chaos, Solitons \& Fractals},
	Pages = {97--113},
	Title = {Finite Sample Effects in Sequence Analysis},
	Volume = 4,
	Year = 1994}

@article{Hide69,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {R. Hide},
	File = {../../Papers/hide69.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {841--853},
	Title = {Dynamics of the Atmospheres of the Major Planets with an Appendix on the Viscous Boundary Layer at the Rigid Bounding Surface of an Electrically-Conducting Rotating Fluid in the Presence of a Magnetic Field},
	Volume = 26,
	Year = 1969,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoaWRlNjkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6CvvmhVAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvvoDxAAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGlkZTY5LnBkZgAADgAWAAoAaABpAGQAZQA2ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hpZGU2OS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGlkZTY5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Hide70,
	Author = {R. Hide},
	File = {../../Papers/hide70.pdf},
	Journal = {Nature},
	Pages = {254--255},
	Title = {Equatorial jets in planetary atmospheres},
	Volume = 225,
	Year = 1970,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpoaWRlNzAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6Dwst7k1BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsveAwAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aGlkZTcwLnBkZgAADgAWAAoAaABpAGQAZQA3ADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hpZGU3MC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaGlkZTcwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@book{Higham96,
	Address = {Philadelphia, PA},
	Author = {N. J. Higham},
	Pages = {688},
	Publisher = {Society for Industrial and Applied Mathematics},
	Title = {Accuracy and Stability of Numerical Algorithms},
	Year = 1996}

@article{Highwood98,
	Annote = {Filed under Hoskins.},
	Author = {E. J. Highwood and B. J. Hoskins},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1579--1604},
	Title = {The Tropical Tropopause},
	Volume = 124,
	Year = 1998}

@article{Hocking76,
	Annote = {Filed under Regression Analysis.},
	Author = {R. R. Hocking},
	Journal = {Biometrics},
	Pages = {1--49},
	Title = {The Analysis and Selection of Variables in Linear Regression},
	Volume = 32,
	Year = 1976}

@article{Hocking83,
	Annote = {Filed under Regression Analysis.},
	Author = {R. R. Hocking},
	Journal = {Technometrics},
	Pages = {219--249 (including discussion)},
	Title = {Developments in Linear Regression Methodology: 1959--1982},
	Volume = 25,
	Year = 1983}

@article{Hodyss01,
	Author = {D. Hodyss and R. Grotjahn},
	Journal = {Tellus},
	Pages = {567--577},
	Title = {Diagnosing cyclogenesis by partitioning energy and potential enstrophy in a linear quasi-geostrophic model},
	Volume = {53A},
	Year = 2001}

@article{Hodyss02,
	Author = {D. Hodyss and T. R. Nathan},
	Journal = {Geophys. Astrophys. Fluid Dynamics},
	Pages = {239--262},
	Title = {Solitary {R}ossby Waves in Zonally Varying Jet Flows},
	Volume = 96,
	Year = 2002}

@article{Hodyss03,
	Author = {D. Hodyss and R. Grotjahn},
	Journal = {Dyn. Atmos. Oceans},
	Pages = {??--??},
	Title = {Nonmodal and unstable normal mode barolcinic growth as a function of horizontal scale},
	Volume = 666,
	Year = 2003}

@article{Hoerl70a,
	Annote = {Not on file. Classic paper on ridge regression.},
	Author = {A. E. Hoerl and R. W. Kennard},
	Journal = {Technometrics},
	Pages = {55--67},
	Title = {Ridge regression: {B}iased estimation for non-orthogonal problems},
	Volume = 12,
	Year = 1970}

@article{Hoerl70b,
	Annote = {Not on file. Classic paper on ridge regression.},
	Author = {A. E. Hoerl and R. W. Kennard},
	Journal = {Technometrics},
	Note = {Correction, {\bf 12}, 723},
	Pages = {69--82},
	Title = {Ridge regression: {A}pplications to non-orthogonal problems},
	Volume = 12,
	Year = 1970}

@article{Hoerling01,
	Author = {M. P. Hoerling and J. W. Hurrell and T. Xu},
	Journal = {Science},
	Pages = {90--92},
	Title = {Tropical Origins for Recent {N}orth {A}tlantic Climate Change},
	Volume = 292,
	Year = 2001}

@article{Hoerling91,
	Annote = {Filed under Isentropic Observations. Finds that
                  3.5-PVU potential vorticity surface is good
                  approximation to tropopause outside tropics.},
	Author = {M. P. Hoerling and T. K. Schaak and A. J. Lenzen},
	Journal = {Mon. Wea. Rev.},
	Pages = {1816--1831},
	Title = {Global Objective Tropopause Analysis},
	Volume = 119,
	Year = 1991}

@article{Hoerling92,
	Annote = {Filed under Isentropic Observations.},
	Author = {M. P. Hoerling},
	Journal = {J. Atmos. Sci.},
	Pages = {2282--2292},
	Title = {Diabatic Sources of Potential Vorticity in the General Circulation},
	Volume = 49,
	Year = 1992}

@article{Hoffman98,
	Annote = {Filed under Snowball Earth.},
	Author = {P. F. Hoffman and A. J. Kaufman and G. P. Halverson and D. P. Schrag},
	Journal = {Science},
	Pages = {1342--1346},
	Title = {A {N}eoproterozoic Snowball {E}arth},
	Volume = 281,
	Year = 1998}

@article{Holland01a,
	Author = {D. M. Holland},
	Journal = {J. Climate},
	Pages = {1585--1601},
	Title = {An Impact of Subgrid-Scale Ice-Ocean Dynamics on Sea-Ice Cover},
	Volume = 14,
	Year = 2001}

@article{Holland01b,
	Author = {D. M. Holland},
	Journal = {Science},
	Pages = {1697--1700},
	Title = {Explaining the Weddell Polynya --- a Large Ocean Eddy Shed at {M}aud {R}ise},
	Volume = 292,
	Year = 2001}

@article{Holland01c,
	Author = {D. M. Holland},
	Journal = {Prog. Oceanogr.},
	Pages = {403--460},
	Title = {Transient sea-ice polynya forced by oceanic flow variability},
	Volume = 48,
	Year = 2001}

@article{Holland01d,
	Author = {D. M. Holland and A. Jenkins},
	Journal = {Mon. Wea. Rev.},
	Pages = {1905--1927},
	Title = {Adaptation of an isopycninc coordinate ocean model for the study of circulation beneath ice shelves},
	Volume = 129,
	Year = 2001}

@article{Holloway77,
	Annote = {Filder under Wave Turbulence.},
	Author = {G. Holloway and M. C. Hendershott},
	File = {../../Papers/holloway77.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {747--765},
	Title = {Stochastic closure for nonlinear {Rossby} waves},
	Volume = 82,
	Year = 1977,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5ob2xsb3dheTc3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6Hwr1xrQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwr3UHQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9sbG93YXk3Ny5wZGYAAA4AHgAOAGgAbwBsAGwAbwB3AGEAeQA3ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2hvbGxvd2F5NzcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2hvbGxvd2F5NzcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Holloway84,
	Annote = {Filed under Geostrophic Turbulence. Tracer transport by geostrophic
                  turbulence. Scalar more easily diffused than
                  vorticity.},
	Author = {G. Holloway and S. Kristmannsson},
	File = {../../Papers/holloway84.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {27--50},
	Title = {Stirring and transport of tracer fields by geostrophic turbulence},
	Volume = 141,
	Year = 1984,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5ob2xsb3dheTg0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6Ivzts6QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzvPWQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9sbG93YXk4NC5wZGYAAA4AHgAOAGgAbwBsAGwAbwB3AGEAeQA4ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2hvbGxvd2F5ODQucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2hvbGxvd2F5ODQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Holloway86a,
	Annote = {Filed under Geostrophic Turbulence.},
	Author = {G. Holloway},
	Date-Modified = {2010-06-11 10:51:50 -0700},
	File = {../../Papers/holloway86a.pdf},
	Journal = {Ann. Rev. Fluid Mech.},
	Pages = {91--147},
	Title = {Eddies, Waves, Circulation, and Mixing: Statistical Geofluid Mechanics},
	Volume = 18,
	Year = 1986,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9ob2xsb3dheTg2YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6Jwtj9vVBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwtlgLQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9sbG93YXk4NmEucGRmAA4AIAAPAGgAbwBsAGwAbwB3AGEAeQA4ADYAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvaG9sbG93YXk4NmEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvaG9sbG93YXk4NmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Holloway86b,
	Annote = {Not on file.},
	Author = {G. Holloway},
	File = {../../Papers/holloway86b.pdf},
	Journal = {Nature},
	Pages = {243--244},
	Title = {Estimation of oceanic eddy transports from satellite altimetry},
	Volume = 323,
	Year = 1986,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9ob2xsb3dheTg2Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6KvztYRwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzu6twAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9sbG93YXk4NmIucGRmAA4AIAAPAGgAbwBsAGwAbwB3AGEAeQA4ADYAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvaG9sbG93YXk4NmIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvaG9sbG93YXk4NmIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Holloway92,
	Author = {G. Holloway},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1033--1046},
	Title = {Representing Topographic Stress for Large-Scale Ocean Models},
	Volume = 22,
	Year = 1992}

@techreport{Holm02,
	Address = {[Available at http://www.ecmwf.int/publications/.]},
	Author = {H{\'o}lm, E. and Andersson, E. and Beljaars, A. and Lopez, P. and Mahfouf, J.-F. and Simmons, A. and Th{\'e}paut, J.-N.},
	File = {../../Papers/holm02.pdf},
	Institution = {European Centre for Medium-Range Weather Forecasts},
	Pages = {55},
	Series = {ECMWF Technical Memorandum},
	Title = {Assimilation and Modelling of the Hydrological Cycle: {ECMWF's} Status and Plans},
	Volume = {383},
	Year = {2002},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpob2xtMDIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6LxRji0wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxRlFQwAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9sbTAyLnBkZgAADgAWAAoAaABvAGwAbQAwADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2hvbG0wMi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvaG9sbTAyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Holm96,
	Annote = {Filed under Hamiltonian Balanced Dynamics.},
	Author = {D. D. Holm},
	Journal = {Physica D},
	Pages = {379--414},
	Title = {Hamiltonian Balance Equations},
	Volume = 98,
	Year = 1996}

@article{Holm98,
	Author = {D. D. Holm and J. E. Marsden and T. S. Ratiu},
	Journal = {Adv. Math.},
	Pages = {1--81},
	Title = {The {E}uler-{P}oincar{\'e} equations and Semidirect Products with Applications to Continuum Theories},
	Volume = 137,
	Year = 1998}

@article{Holm99,
	Author = {D. D. Holm},
	Journal = {Physica D},
	Pages = {215--269},
	Title = {Fluctuation effects on 3d {L}agrangian mean and {E}ulerian mean fluid motion},
	Volume = 133,
	Year = 1999}

@article{Holopainen91,
	Annote = {Uses invertibility principle (QG) to assess
                  influences of pv anomalies on atmospheric flow at
                  various levels.},
	Author = {E. Holopainen and J. Kaurola},
	Journal = {J. Atmos. Sci.},
	Pages = {2614--2625},
	Title = {Decomposing the Atmospheric Flow Using Potential Vorticity Framework},
	Volume = 48,
	Year = 1991}

@book{Holton04,
	Author = {J. R. Holton},
	Edition = {4th},
	Pages = {547},
	Publisher = {Elsevier},
	Series = {International Geophysics Series},
	Title = {An Introduction to Dynamic Meteorology},
	Volume = 88,
	Year = 2004}

@article{Holton72a,
	Author = {J. R. Holton},
	Journal = {J. Atmos. Sci.},
	Pages = {368--375},
	Title = {Waves in the Equatorial Stratosphere Generated by Tropospheric Heat Sources},
	Volume = {29},
	Year = {1972}}

@article{Holton72b,
	Author = {J. R. Holton and R. S. Lindzen},
	Journal = {J. Atmos. Sci.},
	Pages = {1076--1080},
	Title = {An updated theory for the {Q}uasi-{B}iennial Cycle of the Tropical Stratosphere},
	Volume = 29,
	Year = 1972}

@article{Holton76,
	Annote = {Vacillations of mean zonal wind in stratosphere by
                  interaction of upward-propagating planetary waves
                  with mean zonal flow and radiative
                  processes. Wave-mean flow interaction similar to QBO
                  models.},
	Author = {J. R. Holton and C. Mass},
	File = {../../Papers/holton76.pdf},
	Journal = {J. Atmos. Sci.},
	Title = {Stratospheric Vacillation Cycles},
	Year = 1976,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxob2x0b243Ni5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6NveHjwQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAveJUQQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9sdG9uNzYucGRmAAAOABoADABoAG8AbAB0AG8AbgA3ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2hvbHRvbjc2LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9ob2x0b243Ni5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Holton80,
	Author = {J. R. Holton},
	File = {../../Papers/holton80.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2200--2208},
	Title = {The Influence of the Equatorial {Q}uasi-{B}iennial Oscillation on the Global Circulation at 50~mb},
	Volume = 37,
	Year = 1980,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxob2x0b244MC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6OveHjcQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAveJT8QAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9sdG9uODAucGRmAAAOABoADABoAG8AbAB0AG8AbgA4ADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2hvbHRvbjgwLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9ob2x0b244MC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Holton82,
	Author = {J. R. Holton},
	File = {../../Papers/holton82.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {791--799},
	Title = {The Role of Gravity Wave Induced Drag and Diffusion in the Momentum Budget of the Mesosphere},
	Volume = 39,
	Year = 1982,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxob2x0b244Mi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6PveHi1gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAveJTVgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9sdG9uODIucGRmAAAOABoADABoAG8AbAB0AG8AbgA4ADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2hvbHRvbjgyLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9ob2x0b244Mi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Holton83,
	Author = {J. R. Holton},
	File = {../../Papers/holton83.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2497--2507},
	Title = {The Influence of Gravity Wave Breaking on the General Circulation of the Middle Atmosphere},
	Volume = 40,
	Year = 1983,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxob2x0b244My5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6QveHjHAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAveJTnAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9sdG9uODMucGRmAAAOABoADABoAG8AbAB0AG8AbgA4ADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2hvbHRvbjgzLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9ob2x0b244My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Holton90,
	Author = {J. R. Holton},
	File = {../../Papers/holton90.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {392--395},
	Title = {On the Global Exchange of Mass between the Stratosphere and Troposphere},
	Volume = 47,
	Year = 1990,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxob2x0b245MC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6RveHj/wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAveJUfwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9sdG9uOTAucGRmAAAOABoADABoAG8AbAB0AG8AbgA5ADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2hvbHRvbjkwLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9ob2x0b245MC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@book{Holton92,
	Address = {San Diego},
	Author = {J. R. Holton},
	Edition = {3rd},
	Pages = 507,
	Publisher = {Academic Press},
	Title = {An Introduction to Dynamic Meteorology},
	Year = 1992}

@article{Holton95,
	Annote = {Filed under Tropopause
                  Dynamics. Stratosphere-troposphere exchange as large
                  scale process. Refers to Hoskins' underworld
                  etc. picture.},
	Author = {J. R. Holton and P. H. Haynes and M. E. Mc{I}ntyre and A. R. Douglass and R. B. Rood and L. Pfister},
	Journal = {Rev. Geophys.},
	Pages = {403--439},
	Title = {Stratosphere-Troposphere Exchange},
	Volume = {33},
	Year = {1995}}

@book{Honerkamp94,
	Address = {New York},
	Author = {J. Honerkamp},
	Pages = 535,
	Publisher = {{VCH}},
	Title = {Stochastic Dynamical Systems: Concepts, Numerical Methods, Data Analysis},
	Year = 1994}

@book{Horn85,
	Author = {R. A. Horn and C. R. Johnson},
	Pages = 561,
	Publisher = {Cambridge University Press},
	Title = {Matrix Analysis},
	Year = 1985}

@book{Horn94,
	Author = {R. A. Horn and C. R. Johnson},
	Pages = 607,
	Publisher = {Cambridge University Press},
	Title = {Topics in Matrix Analysis},
	Year = 1994}

@article{Hoskins00,
	Annote = {"Higher-latitude forcing can project directly onto
                  equatorial waves and give a significant tropical
                  response in both easterly and westerly tropical
                  flow." Response can be significant because of
                  near-resonance between forcing and
                  equatorially-trapped wave frequencies. Forcing can
                  be particularly effective at triggering equatorial
                  Kelvin wave response (MJO implications).},
	Author = {B. J. Hoskins and G.-Y. Yang},
	File = {../../Papers/hoskins00.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1197--1213},
	Title = {The Equatorial Response to Higher-Latitude Forcing},
	Volume = 57,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ob3NraW5zMDAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6SwOz3swAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwO1aIwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9za2luczAwLnBkZgAOABwADQBoAG8AcwBrAGkAbgBzADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaG9za2luczAwLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hvc2tpbnMwMC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Hoskins03,
	Author = {B. J. Hoskins},
	File = {../../Papers/hoskins03.pdf},
	Journal = {Phil. Trans. R. Soc. Lond. A},
	Pages = {1945--1960},
	Title = {Atmospheric processes and observations},
	Volume = 361,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ob3NraW5zMDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6TvT/KCQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvUAseQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9za2luczAzLnBkZgAOABwADQBoAG8AcwBrAGkAbgBzADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaG9za2luczAzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hvc2tpbnMwMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Hoskins05,
	Author = {B. J. Hoskins and K. I. Hodges},
	File = {../../Papers/hoskins05.pdf},
	Journal = {J. Climate},
	Pages = {4108--4129},
	Title = {A New Perspective on {S}outhern {H}emisphere Storm Tracks},
	Volume = 18,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ob3NraW5zMDUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6Uv6o7pgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv6qsJgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9za2luczA1LnBkZgAOABwADQBoAG8AcwBrAGkAbgBzADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaG9za2luczA1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hvc2tpbnMwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Hoskins81,
	Author = {Hoskins, B. J. and Karoly, D. J.},
	File = {../../Papers/hoskins81.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1179--1196},
	Title = {The steady linear response of a spherical atmosphere to thermal and orographic forcing},
	Volume = {38},
	Year = {1981},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ob3NraW5zODEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6WwOMdP1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwON/rwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9za2luczgxLnBkZgAOABwADQBoAG8AcwBrAGkAbgBzADgAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaG9za2luczgxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hvc2tpbnM4MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@incollection{Hoskins83,
	Address = {London},
	Author = {B. J. Hoskins},
	Booktitle = {Large-Scale Dynamical Processes in the Atmosphere},
	Editor = {B. J. Hoskins and R. P. Pearce},
	File = {../../Papers/hoskins83.pdf},
	Pages = {169--199},
	Publisher = {Academic Press},
	Title = {Modelling of the transient eddies and their feedback on the mean flow},
	Year = 1983,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ob3NraW5zODMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6XvzNenwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzPBDwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9za2luczgzLnBkZgAOABwADQBoAG8AcwBrAGkAbgBzADgAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaG9za2luczgzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hvc2tpbnM4My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Hoskins85,
	Annote = {Review article on isentropic potential
                  vorticity. Conservation and invertibility
                  principle.},
	Author = {B. J. Hoskins and M. E. McIntyre and A. W. Robertson},
	File = {../../Papers/hoskins85.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {877--946},
	Title = {On the use and significance of isentropic potential vorticity maps},
	Volume = 111,
	Year = 1985,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ob3NraW5zODUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6ZwO2vE1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwO4RgwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9za2luczg1LnBkZgAOABwADQBoAG8AcwBrAGkAbgBzADgANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaG9za2luczg1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hvc2tpbnM4NS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Hoskins90,
	Annote = {What maintains storm tracks against action of
                  eddies? It may be the mean diabatic heating
                  associated with eddy fluxes.},
	Author = {B. J. Hoskins and P. J. Valdes},
	File = {../../Papers/hoskins90.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1854--1864},
	Title = {On the Existence of Storm Tracks},
	Volume = 47,
	Year = 1990,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ob3NraW5zOTAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6ax1FG2gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx1G3WgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9za2luczkwLnBkZgAOABwADQBoAG8AcwBrAGkAbgBzADkAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaG9za2luczkwLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hvc2tpbnM5MC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Hoskins91,
	Author = {B. J. Hoskins},
	File = {../../Papers/hoskins91.pdf},
	Journal = {Tellus},
	Pages = {27--35},
	Title = {Towards a {PV}-$\theta$ View of the General Circulation},
	Volume = {43 AB},
	Year = 1991,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ob3NraW5zOTEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6bv+Z5cVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv+bp8QAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9za2luczkxLnBkZgAOABwADQBoAG8AcwBrAGkAbgBzADkAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaG9za2luczkxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hvc2tpbnM5MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Hoskins95,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {B. J. Hoskins and M. J. Rodwell},
	File = {../../Papers/hoskins95.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1329--1340},
	Title = {A Model of the {A}sian Summer Monsoons. {P}art~I: {T}he Global Scale},
	Volume = 52,
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ob3NraW5zOTUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6dwjXYVgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwjY6xgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aG9za2luczk1LnBkZgAOABwADQBoAG8AcwBrAGkAbgBzADkANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaG9za2luczk1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2hvc2tpbnM5NS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Hou92,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {A. Y. Hou and R. S. Lindzen},
	Journal = {J. Atmos. Sci.},
	Pages = {1233--1241},
	Title = {The Influence of Concentrated Heating on the {H}adley Circulation},
	Volume = 49,
	Year = 1992}

@article{Hou93,
	Annote = {Not on file. Shows by an idealized GCM study that
                  shift of tropical convective heating away from the
                  equator induces changes in extratropical
                  temperatures: shift of heating toward summer pole
                  leads to a more intense cross-equatorial Hadley
                  circulation, enhanced upper-level tropical
                  easterlies, and a stronger subtropical winter jet,
                  accompanied by dynamic warming at the winter middle
                  and high latitudes.},
	Author = {A. Y. Hou},
	Journal = {J. Atmos. Sci.},
	Pages = {3553--3570},
	Title = {The Influence of Tropical Heating Displacements on the Extratropical Climate},
	Volume = 50,
	Year = 1993}

@article{Hou95,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {A. Y. Hou and A. Molod},
	Journal = {J. Atmos. Sci.},
	Pages = {2609--2626},
	Title = {Modulation of Dynamic Heating in the Winter Extratropics Associated with the Cross-Equatorial {H}adley Circulation},
	Volume = 52,
	Year = 1995}

@article{Hou98,
	Annote = {Filed under Hadley Cell Dynamics. Intensification of
                  Hadley circulation leads to acceleration of
                  subtropical jet, increased baroclinicity, hence
                  increased eddy heat flux in subtropics, hence
                  midlatitude cooling and high-latitude warming.},
	Author = {A. Y. Hou},
	Journal = {J. Atmos. Sci.},
	Pages = {2437--2457},
	Title = {Hadley Circulation as a Modulator of the Extratropical Climate},
	Volume = 55,
	Year = 1998}

@book{Houghton86,
	Author = {J. T. Houghton},
	Edition = {2nd},
	Publisher = {Cambridge University Press},
	Title = {The Physics of Atmospheres},
	Year = 1986}

@article{Houtekamer95,
	Annote = {Compares breeding, optimal perturbation and a
                  Monte-Carlo method for ensemble prediction.},
	Author = {P. L. Houtekamer and J. Derome},
	Journal = {Mon. Wea. Rev.},
	Pages = {2181--2196},
	Title = {Methods for Ensemble Prediction},
	Volume = {123},
	Year = {1995}}

@article{Hsu00,
	Annote = {Show angular-momentum conserving circulation
                  corresponding to localized heating. Stability of
                  circulation. Eddy-shedding by monsoon.},
	Author = {C. J. Hsu and R. A. Plumb},
	File = {../../Papers/hsu00.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1255--1276},
	Title = {Nonaxisymmetric thermally driven circulations and upper-tropospheric monsoon dynamics},
	Volume = 57,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgloc3UwMC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6gvGyyBAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvG0ihAAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aHN1MDAucGRmAA4AFAAJAGgAcwB1ADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvaHN1MDAucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvaHN1MDAucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Hsu01,
	Author = {C. J. Hsu and F. Zwiers},
	Journal = {J. Geophys. Res.},
	Pages = {20145--20159},
	Title = {Climate change in recurrent regimes and modes of {N}orthern {H}emisphere atmospheric variability},
	Volume = {106D},
	Year = 2001}

@article{Hsu99,
	Author = {H.-H. Hsu and C.-T. Terng and C.-T. Chen},
	File = {../../Papers/hsu99.pdf},
	Journal = {J. Climate},
	Pages = {793--810},
	Title = {Evolution of Large-Scale Circulation and Heating during the First Transition of {A}sian Summer Monsoon},
	Volume = 12,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgloc3U5OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6hwbnpaVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwbpZ6QAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aHN1OTkucGRmAA4AFAAJAGgAcwB1ADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvaHN1OTkucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvaHN1OTkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Hu01a,
	Annote = {Filed under Newell.},
	Author = {Y. Hu and R. E. Newell and Y. Zhu},
	Journal = {J. Geophys. Res.},
	Pages = {32445--32467},
	Title = {Mean moist circulation for {PEM}-{Tropics} missions},
	Volume = {106D},
	Year = 2001}

@article{Hu01b,
	Annote = {Filed under Pierrehumbert.},
	Author = {Y. Hu and R. T. Pierrehumbert},
	Journal = {J. Atmos. Sci.},
	Pages = {1493--1510},
	Title = {The Advection-Diffusion Problem for Stratospheric Flow. Part {I}: {C}oncentration Probability Distribution Functions},
	Volume = 58,
	Year = 2001}

@article{Hu02,
	Annote = {Filed under Pierrehumbert.},
	Author = {Y. Hu and R. T. Pierrehumbert},
	Journal = {J. Atmos. Sci.},
	Pages = {2830--2845},
	Title = {The Advection-Diffusion Problem for Stratospheric Flow. Part {II}: {P}robability Distribution Function of Tracer Gradients},
	Volume = 59,
	Year = 2002}

@article{Hu07,
	Annote = {Filed under ITCZ dynamics},
	Author = {Y. Hu and D. Li and J. Liu},
	File = {../../Papers/hu07.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2007GL030950},
	Pages = {L18814},
	Title = {Abrupt seasonal variation of the {ITCZ} and the {Hadley} circulation},
	Volume = 34,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfghodTA3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6iw0f5ZAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw0hb1AAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aHUwNy5wZGYAAA4AEgAIAGgAdQAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL2h1MDcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL2h1MDcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@article{HuFu07,
	Author = {Hu, Y. and Fu, Q.},
	Date-Modified = {2010-06-11 10:52:54 -0700},
	File = {../../Papers/HuFu07.pdf},
	Journal = {Atmos. Chem. Phys.},
	Pages = {5229--5236},
	Title = {Observed poleward expansion of the {Hadley} circulation since 1979},
	Volume = {7},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpIdUZ1MDcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6txNPn4gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxNRKUgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6SHVGdTA3LnBkZgAADgAWAAoASAB1AEYAdQAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL0h1RnUwNy5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvSHVGdTA3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Hu98,
	Annote = {Filed under Water Vapor (Feedback and Kinetmatics).},
	Author = {H. Hu and T. Liu},
	File = {../../Papers/hu98.pdf},
	Journal = {Geophys. Res. Lett.},
	Pages = {3151--3154},
	Title = {The impact of upper tropospheric humidity from {M}icrowave {L}imb {S}ounder on the midlatitude greenhouse effect},
	Volume = 25,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfghodTk4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6jv3AZLwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3B7nwAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aHU5OC5wZGYAAA4AEgAIAGgAdQA5ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL2h1OTgucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL2h1OTgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@article{Hua86,
	Annote = {Filed under Baroclinic Eddy Parameterizations.},
	Author = {B. L. Hua and D. B. Haidvogel},
	File = {../../Papers/hua86.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2923--2936},
	Title = {Numerical Simulations of the Vertical Structure of Quasi-Geostrophic Turbulence},
	Volume = 43,
	Year = 1986,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglodWE4Ni5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6kwsUnEwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsWJgwAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aHVhODYucGRmAA4AFAAJAGgAdQBhADgANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvaHVhODYucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvaHVhODYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Huang01b,
	Annote = {Filed under 2D Turbulence and Atmospheric Turbulence Spectra.},
	Author = {H.-P. Huang and B. Galperin and S. Sukoriansky},
	Date-Modified = {2010-06-11 10:53:45 -0700},
	File = {../../Papers/huang01b.pdf},
	Journal = {Phys. Fluids},
	Pages = {225--240},
	Title = {Anisotropic spectra in two-dimensional turbulence on the surface of a rotating sphere},
	Volume = 13,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxodWFuZzAxYi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6mwr1xMwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwr3TowAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aHVhbmcwMWIucGRmAAAOABoADABoAHUAYQBuAGcAMAAxAGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2h1YW5nMDFiLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9odWFuZzAxYi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Huang97,
	Annote = {Not on file.},
	Author = {B. H. Huang and J. Shukla},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1693--1712},
	Title = {Characteristics of the interannual and decadal variability in a general circulation model of the tropical {A}tlantic {O}cean},
	Volume = 27,
	Year = 1997}

@article{Huang98,
	Author = {N. E. Huang and Z. Shen and S. R. Long and M. C. Wu and H. H. Shih and Q. Zheng and N.-C. Yen and C. C. Tung and H. H. Liu},
	File = {../../Papers/huang98.pdf},
	Journal = {Proc. Roy. Soc. Lond. A},
	Pages = {903--995},
	Title = {The empirical mode decomposition and the {H}ilbert spectrum for nonlinear and non-stationary time series analysis},
	Volume = 454,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtodWFuZzk4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6nvW9p6wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvW/MWwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aHVhbmc5OC5wZGYADgAYAAsAaAB1AGEAbgBnADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvaHVhbmc5OC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9odWFuZzk4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{HuangHP98,
	Annote = {Filed under 2D Turbulence. Discuss spectral energy
                  transfer by shearing (can be as large as the
                  nonlinear eddy-eddy interactions) and demonstrate
                  spectrally nonlocal transfer from small eddies to
                  mean flow.},
	Author = {H.-P. Huang and W. A. Robinson},
	Journal = {J. Atmos. Sci.},
	Pages = {611--632},
	Title = {Two-dimensional turbulence and persistent zonal jets in a global barotropic model},
	Volume = 55,
	Year = 1998}

@article{Hubbard91,
	Author = {W. B. Hubbard and W. J. Nellis and A. C. Mitchell and N. C. Holmes and S. S. Limaye and P. C. McCandless},
	File = {../../Papers/hubbard91.pdf},
	Journal = {Science},
	Pages = {648--651},
	Title = {Interior structure of {Neptune}: {C}omparison with {Uranus}},
	Volume = 253,
	Year = 1991,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1odWJiYXJkOTEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6oxrwX+gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxrx6agAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aHViYmFyZDkxLnBkZgAOABwADQBoAHUAYgBiAGEAcgBkADkAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaHViYmFyZDkxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2h1YmJhcmQ5MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Huber01,
	Annote = {Filed under Chaotic Advection.},
	Author = {M. Huber and J. C. McWilliams and M. Ghil},
	Journal = {J. Atmos. Sci.},
	Pages = {2377--2394},
	Title = {A Climatology of Turbulent Dispersion in the Troposphere},
	Volume = 58,
	Year = 2001}

@article{Huck01,
	Author = {T. Huck and G. V. Vallis},
	Journal = {Tellus},
	Pages = {???--???},
	Title = {Linear stability analysis of the three-dimensional thermally-driven ocean circulation: application to interdecadal oscillations},
	Volume = {53A},
	Year = 2001}

@article{Hulburt31,
	Annote = {Filed under General Circulation History},
	Author = {E. O. Hulburt},
	File = {../../Papers/hulburt31.pdf},
	Journal = {Phys. Rev.},
	Pages = {1876--1890},
	Title = {The Temperature of the Lower Atmosphere of the {Earth}},
	Volume = 38,
	Year = 1931,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1odWxidXJ0MzEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6uvzC/egAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzEh6gAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aHVsYnVydDMxLnBkZgAOABwADQBoAHUAbABiAHUAcgB0ADMAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaHVsYnVydDMxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2h1bGJ1cnQzMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Hyvarinen99,
	Annote = {Not on file.},
	Author = {Aapo Hyv{\"a}rinen},
	Journal = {Neural Computing Surveys},
	Pages = {94--128},
	Title = {Survey on Independent Component Analysis},
	Volume = 2,
	Year = 1999}

@proceedings{IPCC90,
	Editor = {J. T. Houghton and G. J. Jenkins and J. J. Ephraums},
	Organization = {Intergovernmental Panel on Climate Change},
	Publisher = {Cambridge University Press},
	Title = {Climate Change: The {IPCC} Scientific Assessment},
	Year = 1990}

@article{Imbrie80,
	Annote = {Filed under Climate Stability/Energy Balance Models.},
	Author = {J. Imbrie and J. Z. Imbrie},
	File = {../../Papers/imbrie80.pdf},
	Journal = {Science},
	Pages = {943--953},
	Title = {Modeling the climatic response to orbital variations},
	Volume = 207,
	Year = 1980,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxpbWJyaWU4MC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ69vhWVhQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvhYGBQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aW1icmllODAucGRmAAAOABoADABpAG0AYgByAGkAZQA4ADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2ltYnJpZTgwLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9pbWJyaWU4MC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Ingersoll00,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {A. P. Ingersoll and P. J. Gierasch and D. Banfield and A. R. Vasavada and {the Galileo Imaging Team}},
	File = {../../Papers/ingersoll00.pdf},
	Journal = {Nature},
	Pages = {630--632},
	Title = {Moist convection as an energy source for the large-scale motions in {J}upiter's atmosphere},
	Volume = 403,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9pbmdlcnNvbGwwMC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6+wxteKlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwxvAmgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aW5nZXJzb2xsMDAucGRmAA4AIAAPAGkAbgBnAGUAcgBzAG8AbABsADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvaW5nZXJzb2xsMDAucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvaW5nZXJzb2xsMDAucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@incollection{Ingersoll04,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {A. P. Ingersoll and T. E. Dowling and P. J. Gierasch and G. S. Orton and P. L. Read and A. S{\'a}nchez-Lavega and A. P. Showman and A. A. Simon-Miller and A. R. Vasavada},
	Booktitle = {Jupiter: The Planet, Satellites and Magnetosphere},
	Editor = {F. Bagenal and T. E. Dowling and W. B. McKinnon},
	File = {../../Papers/ingersoll04.pdf},
	Pages = {105--128},
	Publisher = {Cambridge University Press},
	Title = {Dynamics of {J}upiter's Atmosphere},
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9pbmdlcnNvbGwwNC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ6/vHNMJgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvHO8pgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aW5nZXJzb2xsMDQucGRmAA4AIAAPAGkAbgBnAGUAcgBzAG8AbABsADAANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvaW5nZXJzb2xsMDQucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvaW5nZXJzb2xsMDQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Ingersoll76b,
	Author = {A. P. Ingersoll},
	Journal = {Icarus},
	Pages = {245--253},
	Title = {{Pioneer}~10 and 11 observations and the dynamics of {Jupiter's} atmosphere},
	Volume = {29},
	Year = {1976}}

@article{Ingersoll78,
	Author = {A. P. Ingersoll and C. C. Porco},
	File = {../../Papers/ingersoll78.pdf},
	Journal = {Icarus},
	Pages = {27--43},
	Title = {Solar heating and internal heat flow on {Jupiter}},
	Volume = {35},
	Year = {1978},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9pbmdlcnNvbGw3OC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ7Cw7uMMQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7v8sQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aW5nZXJzb2xsNzgucGRmAA4AIAAPAGkAbgBnAGUAcgBzAG8AbABsADcAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvaW5nZXJzb2xsNzgucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvaW5nZXJzb2xsNzgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Ingersoll81,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {A. P. Ingersoll and R. F. Beebe and J. L. Mitchell and G. W. Garneau and G. M. Yagi and J.-P. M{\"u}ller},
	File = {../../Papers/ingersoll81.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {8733--8743},
	Title = {Interaction of eddies and mean zonal flow on {J}upiter as inferred from {Voyager} 1 and 2 images},
	Volume = 86,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9pbmdlcnNvbGw4MS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ7Dw8UpwQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw8WaQQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aW5nZXJzb2xsODEucGRmAA4AIAAPAGkAbgBnAGUAcgBzAG8AbABsADgAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvaW5nZXJzb2xsODEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvaW5nZXJzb2xsODEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Ingersoll82,
	Author = {A. P. Ingersoll and D. Pollard},
	Journal = {Icarus},
	Pages = {62--80},
	Title = {Motion in the interiors and atmospheres of {Jupiter} and {Saturn}: Scale analysis, anelastic equations, barotropic stability criterion},
	Volume = {52},
	Year = {1982}}

@article{Ingersoll90,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {A. P. Ingersoll},
	File = {../../Papers/ingersoll90.pdf},
	Journal = {Science},
	Pages = {308--315},
	Title = {Atmospheric Dynamics of the Outer Planets},
	Volume = 248,
	Year = 1990,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9pbmdlcnNvbGw5MC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ7EvRhLPAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRitrAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aW5nZXJzb2xsOTAucGRmAA4AIAAPAGkAbgBnAGUAcgBzAG8AbABsADkAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvaW5nZXJzb2xsOTAucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvaW5nZXJzb2xsOTAucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Ingersoll95,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {A. P. Ingersoll and H. Kanamori},
	File = {../../Papers/ingersoll95.pdf},
	Journal = {Nature},
	Pages = {706--708},
	Title = {Waves from the collisions of comet {S}hoemaker-{L}evy~9 with {J}upiter},
	Volume = 374,
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9pbmdlcnNvbGw5NS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ7FvRYBvAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRZkLAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aW5nZXJzb2xsOTUucGRmAA4AIAAPAGkAbgBnAGUAcgBzAG8AbABsADkANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvaW5nZXJzb2xsOTUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvaW5nZXJzb2xsOTUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Ioannou86,
	Annote = {Filed under Lindzen.},
	Author = {P. Ioannou and R. S. Lindzen},
	File = {../../Papers/ioannou86.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2999--3014},
	Title = {Baroclinic Instability in the Presence of Barotropic Jets},
	Volume = 43,
	Year = 1986,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1pb2Fubm91ODYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQ7Gv9h/+QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv9jweQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aW9hbm5vdTg2LnBkZgAOABwADQBpAG8AYQBuAG4AbwB1ADgANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaW9hbm5vdTg2LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2lvYW5ub3U4Ni5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@book{Iribarne81,
	Address = {Dordrecht, Holland},
	Author = {J. V. Iribarne and W. L. Godson},
	Edition = {2nd},
	Pages = 275,
	Publisher = {D. Reidel},
	Series = {Geophysics and Astrophysics Monographs},
	Title = {Atmospheric Thermodynamics},
	Year = 1981}

@article{Iwasaki01,
	Author = {T. Iwasaki},
	File = {../../Papers/iwasaki01.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3036--3052},
	Title = {Atmospheric energy cycle viewed from wave--mean flow interaction and {L}agrangian mean circulation},
	Volume = 58,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1pd2FzYWtpMDEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFTvq/nrgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvrBKHgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aXdhc2FraTAxLnBkZgAOABwADQBpAHcAYQBzAGEAawBpADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaXdhc2FraTAxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2l3YXNha2kwMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Iwasaki90,
	Author = {T. Iwasaki},
	File = {../../Papers/iwasaki90.pdf},
	Journal = {J. Meteor. Soc. Japan},
	Pages = {347--356},
	Title = {Lagrangian-mean circulation and wave--mean flow interactions of {Eady}'s Baroclinic Instability Waves},
	Volume = 68,
	Year = 1990,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1pd2FzYWtpOTAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFUvMV5hQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvMXb9QAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6aXdhc2FraTkwLnBkZgAOABwADQBpAHcAYQBzAGEAawBpADkAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvaXdhc2FraTkwLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2l3YXNha2k5MC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Iwasaki98,
	Author = {T. Iwasaki},
	Journal = {J. Atmos. Sci.},
	Pages = {3000--3002},
	Title = {A set of zonal mean equations in a pressure-isentrope hybrid vertical coordinate},
	Volume = 55,
	Year = 1998}

@book{Jackson75,
	Address = {New York},
	Author = {J. D. Jackson},
	Edition = {2nd},
	Pages = 848,
	Publisher = {Wiley},
	Title = {Classical Electrodynamics},
	Year = 1975}

@article{James86,
	Annote = {Reducing surface drag results in reduced
                  baroclinicity and increased barotropic flow. Strong
                  horizontal shears in barotropic flow inhibit
                  baroclinic instability. Find that scales of
                  baroclinic eddies are determined by Rossby radius
                  and Rhines scale, drag scale is very large and hence
                  unimportant.},
	Author = {I. N. James and L. J. Gray},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1231--1250},
	Title = {Concerning the Effect of Surface Drag on the Circulation of a Baroclinic Planetary Atmosphere},
	Volume = 112,
	Year = 1986}

@article{James89,
	Author = {I. N. James and P. M. James},
	Journal = {Nature},
	Pages = {53--55},
	Title = {Ultra-low-frequency variability in a simple atmospheric circulation model},
	Volume = 342,
	Year = 1989}

@book{James94,
	Author = {I. N. James},
	Pages = 422,
	Publisher = {Cambridge University Press},
	Series = {Cambridge Atmospheric and Space Science Series},
	Title = {An Introduction to Circulating Atmospheres},
	Year = 1994}

@article{Jayne01,
	Annote = {Filed under Ocean Heat Transport.},
	Author = {S. R. Jayne and J. Marotzke},
	File = {../../Papers/jayne01.pdf},
	Journal = {Rev. Geophys.},
	Pages = {385--411},
	Title = {The Dynamics of Ocean Heat Transport Variability},
	Volume = 39,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtqYXluZTAxLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFWwMLCo1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwMMlEwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6amF5bmUwMS5wZGYADgAYAAsAagBhAHkAbgBlADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvamF5bmUwMS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9qYXluZTAxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Jeffreys26,
	Annote = {Filed under General Circulation History. Eddies
                  transport angular momentum.},
	Author = {H. Jeffreys},
	File = {../../Papers/jeffreys26.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {85--104},
	Title = {On the Dynamics of Geostrophic Winds},
	Volume = 52,
	Year = 1926,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5qZWZmcmV5czI2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFYvucpkQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvueMAQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6amVmZnJleXMyNi5wZGYAAA4AHgAOAGoAZQBmAGYAcgBlAHkAcwAyADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2plZmZyZXlzMjYucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2plZmZyZXlzMjYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Jenkins01,
	Annote = {Filed under Holland.},
	Author = {A. Jenkins and H. H. Hellmer and D. M. Holland},
	Journal = {J. Phys. Oceanogr.},
	Pages = {285--296},
	Title = {The Role of Meltwater Advection in the Formulation of Conservative Boundary Conditions at an Ice-Ocean Interface},
	Volume = 31,
	Year = 2001}

@article{Jiang96,
	Annote = {Filed under REML Asymptotics.},
	Author = {J. Jiang},
	Journal = {Ann. Statistics},
	Pages = {255--286},
	Title = {{REML} Estimation: Asymptotic Behavior and Related Topics},
	Volume = 24,
	Year = 1996}

@article{Jin93a,
	Annote = {Filed under Neelin. Second of a series of three
                  papers by these authors. Gave presentation based on
                  this paper in spring 1996. My comments plus a few
                  transparancies in folder. Interannual variability in
                  tropics generated by first Hopf bifurcation from
                  climatology. Analyzes coupled modes in parameter
                  space of dimension 3: coupling strength, time scale
                  of ocean dynamics, surface layer feedback. Numerical
                  exploration of parameter space. Open issues: What
                  generates irregularity? What physical mechanisms do
                  parameters represent?},
	Author = {F.-F. Jin and J. D. Neelin},
	Journal = {J. Atmos. Sci.},
	Pages = {3477--3503},
	Title = {Modes of Interannual Tropical Ocean-Atmosphere Interaction --- a Unified View. {P}art {I}: {N}umerical Results},
	Volume = {50},
	Year = {1993}}

@article{Jin93b,
	Annote = {Filed under Neelin. Third of a series of three
                  papers by these authors.},
	Author = {F.-F. Jin and J. D. Neelin},
	Journal = {J. Atmos. Sci.},
	Pages = {3523--3540},
	Title = {Modes of Interannual Tropical Ocean-Atmosphere Interaction --- a Unified View. {P}art {III}: {A}nalytical results in fully coupled cases},
	Volume = {50},
	Year = {1993}}

@book{Jobson92,
	Address = {New York},
	Author = {J. D. Jobson},
	Pages = {731},
	Publisher = {Springer},
	Title = {Applied Multivariate Data Analysis. Volume {II}: Categorical and Multivariate Methods},
	Year = 1992}

@article{Joe89,
	Annote = {Filed under Entropy Estimation. Derives bias
                  correction and (non-unimodal) density estimation
                  kernels that lead to low bias in entropy estimate.},
	Author = {H. Joe},
	Journal = {Ann. Inst. Statist. Math.},
	Pages = {683--697},
	Title = {Estimation of Entropy and Other Functionals of a Multivariate Density},
	Volume = 41,
	Year = 1989}

@article{Johanson09,
	Author = {C. M. Johanson and Q. Fu},
	File = {../../Papers/johanson09.pdf},
	Journal = {J. Climate},
	Pages = {2713--2725},
	Title = {Hadley Cell Widening: Model Simulations versus Observations},
	Volume = 22,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5qb2hhbnNvbjA5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFZxjmDlgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxjnmBgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6am9oYW5zb24wOS5wZGYAAA4AHgAOAGoAbwBoAGEAbgBzAG8AbgAwADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2pvaGFuc29uMDkucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2pvaGFuc29uMDkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@book{Johnson02,
	Address = {Englewood Cliffs},
	Author = {R. A. Johnson and D. W. Wichern},
	Edition = {5th},
	Pages = 767,
	Publisher = {Prentice-Hall},
	Title = {Applied Multivariate Statistical Analysis},
	Year = 2002}

@article{Johnson02a,
	Annote = {Variability in the driving of the thermohaline
                  circulation leads to changes only in the hemisphere
                  in which the driving acts. Effects of driving
                  transmitted throughout the hemisphere by coastal
                  Kelvin waves along the western boundary and
                  equatorial waves along the equator. Use
                  reduced-gravity model driven by imposed mass fluxes
                  to test the theory.},
	Author = {H. L. Johnson and D. P. Marshall},
	Journal = {Geophys. Res. Lett.},
	Pages = {????},
	Title = {Localization of abrupt change in the {N}orth {A}tlantic thermohaline circulation},
	Volume = 29,
	Year = 2002}

@article{Johnson02b,
	Annote = {Response of shallow-water ocean to changes in rates
                  of deep water formation at a boundary of
                  basin. Coastal Kelvin waves communicate changes
                  southward towards the equator; there they are
                  transferred along the equator by an equatorial
                  Kelvin wave. Rossby waves spread response into
                  interior ocean. For forcing in northern hemisphere,
                  weak response in southern hemisphere ("equatorial
                  buffer"). },
	Author = {H. L. Johnson and D. P. Marshall},
	Journal = {J. Phys. Oceanogr.},
	Pages = {??},
	Title = {A theory for the surface {A}tlantic response to thermohaline variability},
	Volume = {??},
	Year = 2002}

@article{Johnson80,
	Annote = {Transformation to isentropic coordinates etc.},
	Author = {D. R. Johnson},
	Journal = {Mon. Wea. Rev.},
	Pages = {733--745},
	Title = {A generalized transport equation for use with meteorological coordinate systems},
	Volume = 108,
	Year = 1980}

@book{Johnson82,
	Address = {Englewood Cliffs},
	Annote = {QA273.J63; in GFDL library.},
	Author = {R. A. Johnson and D. W. Wichern},
	Pages = 594,
	Publisher = {Prentice-Hall},
	Title = {Applied Multivariate Statistical Analysis},
	Year = 1982}

@incollection{Johnson89,
	Author = {D. R. Johnson},
	Booktitle = {Advances in Geophysics},
	Editor = {B. Saltzman},
	File = {../../Papers/johnson89.pdf},
	Pages = {43--316},
	Publisher = {Academic Press},
	Title = {The Forcing and Maintenance of Global Monsoonal Circulations: An Isentropic Analysis},
	Volume = {31},
	Year = 1989,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1qb2huc29uODkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFbvt3VtgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvt44JgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6am9obnNvbjg5LnBkZgAOABwADQBqAG8AaABuAHMAbwBuADgAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvam9obnNvbjg5LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2pvaG5zb244OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@book{Jolliffe86,
	Address = {New York},
	Annote = {QA278.5.J65},
	Author = {I. T. Jolliffe},
	Pages = 271,
	Publisher = {Springer},
	Series = {Springer Series in Statistics},
	Title = {Principal Component Analysis},
	Year = 1986}

@article{Joly95,
	Annote = {Filed under Adjoint Method.},
	Author = {A. Joly},
	Journal = {J. Atmos. Sci.},
	Pages = {3082--3108},
	Title = {The Stability of Steady Fronts and the Adjoint Method: {N}onmodal Frontal Waves},
	Volume = 52,
	Year = 1995}

@article{Jones01,
	Annote = {Filed under Paleo-Climate Reviews.},
	Author = {P. D. Jones and T. J. Osborn and K. R. Briffa},
	Journal = {Science},
	Pages = {662--667},
	Title = {The Evolution of Climate Over the Last Millennium},
	Volume = 292,
	Year = 2001}

@article{Jones09,
	Author = {C. A. Jones and K. M. Kuzanyan and R. H. Mitchell},
	File = {../../Papers/jones09.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {291--319},
	Title = {Linear theory of compressible convection in rapidly rotating spherical shells, using the anelastic approximation},
	Volume = 634,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtqb25lczA5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFdxpxzjAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxpzV/AAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6am9uZXMwOS5wZGYADgAYAAsAagBvAG4AZQBzADAAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvam9uZXMwOS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9qb25lczA5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Jones94,
	Annote = {Not on File.},
	Author = {P. D. Jones},
	Journal = {J. Climate},
	Pages = {1794--1802},
	Title = {Hemispheric Surface Air Temperature Variations: {A} Reanalysis and an Update up to 1993},
	Volume = 7,
	Year = 1994}

@article{Joshi97,
	Author = {M. M. Joshi and R. M. Haberle and R. T. Reynolds},
	File = {../../Papers/joshi97.pdf},
	Journal = {Icarus},
	Pages = {450--465},
	Title = {Simulations of the Atmospheres of Synchronously Rotating Terrestrial Planets Orbiting {M Dwarfs}: Conditions for Atmospheric Collapse and the Implications for Habitability},
	Volume = {129},
	Year = {1997},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtqb3NoaTk3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFgxcCJSAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxcD5yAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6am9zaGk5Ny5wZGYADgAYAAsAagBvAHMAaABpADkANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvam9zaGk5Ny5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9qb3NoaTk3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Juckes00,
	Annote = {Filed under Tropopause Dynamics. Convection in
                  mature baroclinic waves determines mean potential
                  temperature difference between tropopause and
                  surface.},
	Author = {M. N. Juckes},
	File = {../../Papers/juckes00.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3050--3057},
	Title = {The Static Stability of the Midlatitude Troposphere: The Relevance of Moisture},
	Volume = {57},
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxqdWNrZXMwMC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFjvaxihQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvazTBQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6anVja2VzMDAucGRmAAAOABoADABqAHUAYwBrAGUAcwAwADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2p1Y2tlczAwLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9qdWNrZXMwMC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Juckes01,
	Annote = {Transformed Eulerian mean circulation in arbitrary
                  coordinate system, in particular in coordinate
                  system with potential vorticity as vertical
                  coordinate. Used to diagnose mass transport near
                  extratropical tropopause.},
	Author = {M. Juckes},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {147--160},
	Title = {A generalization of the tranformed {E}ulerian-mean meridional circulation},
	Volume = 127,
	Year = 2001}

@article{Juckes94,
	Annote = {Use Andrews83 Transformed Eulerian Mean circulation
                  to diagnose eddy fluxes along isentropes near
                  surface.},
	Author = {M. N. Juckes and I. N. James and M. Blackburn},
	File = {../../Papers/juckes94.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1017--1044},
	Title = {The influence of {Antarctica} on the momentum budget of the southern extratropics},
	Volume = 120,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxqdWNrZXM5NC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFlvOXKPgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvOYsrgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6anVja2VzOTQucGRmAAAOABoADABqAHUAYwBrAGUAcwA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2p1Y2tlczk0LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9qdWNrZXM5NC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Juckes97,
	Annote = {Estimates circulation in the vicinity of the
                  tropopause using QG scaling.},
	Author = {M. N. Juckes},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {71--99},
	Title = {The mass flux across the tropopause: Quasi-geostrophic theory},
	Volume = 123,
	Year = 1997}

@article{Juckes98a,
	Author = {M. N. Juckes},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {2227--2257},
	Title = {Baroclinic instability of semi-geostrophic fronts with uniform potential vorticity. {I}: {A}n analystic solution},
	Volume = 124,
	Year = 1998}

@article{Juckes98b,
	Author = {M. N. Juckes},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {2259--2290},
	Title = {Baroclinic instability of semi-geostrophic fronts with uniform potential vorticity. {II}: {C}omparison of analytic and numerical solutions},
	Volume = 124,
	Year = 1998}

@techreport{Kallberg04,
	Address = {Reading, United Kingdom},
	Annote = {Filed under ECMWF Data.},
	Author = {P. K{\aa}llberg and A. Simmons and S. Uppala and M. Fuentes},
	File = {../../Papers/kallberg04.pdf},
	Institution = {European Centre for Medium-Range Weather Forecasts},
	Pages = 31,
	Series = {{ECMWF} {ERA-40} Project Report Series},
	Title = {The {ERA-40} Archive},
	Url = {www.ecmwf.int/publications},
	Volume = 17,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5rYWxsYmVyZzA0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFnv3Kg4gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3MDUgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2FsbGJlcmcwNC5wZGYAAA4AHgAOAGsAYQBsAGwAYgBlAHIAZwAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2thbGxiZXJnMDQucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2thbGxiZXJnMDQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ},
	Bdsk-Url-1 = {www.ecmwf.int/publications}}

@article{Kalnay96,
	Annote = {Not on file.},
	Author = {E. Kalnay and M. Kanamitsu and R. Kistler and W. Collins and D. Deaven and L. Gandin and M. Iredell and S. Saha G. and White and J. Woollen and Y. Zhu and M. Chelliah and W. Ebisuzaki and W. Higgins and J. Janowiak and K. C. Mo and C. Ropelewski and J. Wang and A. Leetmaa and R. Reynolds and R. Jenne and D. Joseph},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {437--471},
	Title = {The {NCEP/NCAR} 40-year reanalysis project},
	Volume = 77,
	Year = 1996}

@article{Kaminski99,
	Annote = {Filed under Adjoint Method.},
	Author = {T. Kaminski and M. Heimann and R. Giering},
	Journal = {J. Geophys. Res.},
	Pages = {18535--18553},
	Title = {A coarse grid three-dimensional global inverse model of the atmospheric transport. 1. {A}djoint model and {J}acobian matrix},
	Volume = {104D},
	Year = 1999}

@article{Kaneda81,
	Annote = {Not on file. Lagrangian Direct Interaction
                  Approximation.},
	Author = {Y. Kaneda},
	File = {../../Papers/kaneda81.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {131--145},
	Title = {Renormalized expansions in the theory of turbulence with the use of the {L}agrangian position function},
	Volume = 107,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxrYW5lZGE4MS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFpwTXlc1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwTZH4wAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2FuZWRhODEucGRmAAAOABoADABrAGEAbgBlAGQAYQA4ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2thbmVkYTgxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9rYW5lZGE4MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Kang09,
	Author = {S. M. Kang and D. M. W. Frierson and I. M. Held},
	File = {../../Papers/kang09.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2812--2827},
	Title = {The Tropical Response to Extratropical Thermal Forcing in an Idealized {GCM}: The Importance of Radiative Feedbacks and Convective Parameterization},
	Volume = 66,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgprYW5nMDkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFrxs7qRQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxs9MtQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2FuZzA5LnBkZgAADgAWAAoAawBhAG4AZwAwADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2thbmcwOS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMva2FuZzA5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Kaplan97,
	Annote = {Filed under Imputation of Missing Values. Fits model
                  of first order in time to data to model temporal
                  transitions.},
	Author = {A. Kaplan and Y. Kushnir and M. A. Cane and M. B. Blumenthal},
	Journal = {J. Geophys. Res.},
	Pages = {27835--27860},
	Title = {Reduced space optimal analysis for historical data sets: 136 years of {A}tlantic sea surface temperatures},
	Volume = {102C},
	Year = 1997}

@article{Kaplan98,
	Annote = {Filed under Imputation of Missing Values. Comparison
                  of imputation techniques. Also including temporal
                  information.},
	Author = {A. Kaplan and M. A. Cane and Y. Kushnir and A. C. Clement and M. B. Blumenthal and B. Rajagopalan},
	Journal = {J. Geophys. Res.},
	Pages = {18567-18589},
	Title = {Analyses of global sea surface temperature 1856-1991},
	Volume = {103C},
	Year = 1998}

@article{Karniadakis93,
	Annote = {Filed under Orszag.},
	Author = {G. E. Karniadakis and S. A. Orszag},
	Journal = {Physics Today},
	Key = {turbulence},
	Month = {March},
	Title = {Nodes, Modes and Flow Codes},
	Year = 1993}

@article{Karoly97,
	Annote = {Not on file.},
	Author = {D. J. Karoly and P. C. McIntosh and P. Berrisford and T. J. McDougall and A. C. Hirst},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {519--526},
	Title = {Similarities of the {D}eacon cell in the {S}outhern {O}cean and {F}errel cells in the atmosphere},
	Volume = 123,
	Year = 1997}

@article{Karsten02,
	Annote = {Filed under Marshall},
	Author = {R. Karsten and H. Jones and J. Marshall},
	Journal = {J. Phys. Oceanogr.},
	Pages = {39--54},
	Title = {The Role of Eddy Transfer in Setting the Stratification and Transport of a Circumpolar Current},
	Volume = 32,
	Year = 2002}

@article{Kaspi07,
	Author = {Y. Kaspi and G. R. Flierl},
	File = {../../Papers/kaspi07.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3177--3194},
	Title = {Formation of Jets by Baroclinic Instability on Gas Planet Atmospheres},
	Volume = 64,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtrYXNwaTA3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFswy8rnFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwy+ODAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2FzcGkwNy5wZGYADgAYAAsAawBhAHMAcABpADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMva2FzcGkwNy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9rYXNwaTA3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@phdthesis{Kaspi_thesis08,
	Address = {Cambridge, MA},
	Author = {Y. Kaspi},
	Date-Modified = {2010-06-11 10:53:45 -0700},
	File = {../../Papers/kaspi_thesis08.pdf},
	School = {Massachusetts Institute of Technology},
	Title = {Turbulent convection in an anelastic rotating sphere: {A} model for the circulation on the giant planets},
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAX4AAAAAAX4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhJrYXNwaV90aGVzaXMwOC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFvxJjRPwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxJkzrwAAAAEADAAJDH4ACE6zAACS8wACADFNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2FzcGlfdGhlc2lzMDgucGRmAAAOACYAEgBrAGEAcwBwAGkAXwB0AGgAZQBzAGkAcwAwADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAlVXNlcnMvdGFwaW8vUGFwZXJzL2thc3BpX3RoZXNpczA4LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHy4uLy4uL1BhcGVycy9rYXNwaV90aGVzaXMwOC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACIgIkAikCMgI9AkECTwJWAl8CgQKGAokClgKbAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAq0=}}

@article{Kaspi09,
	Author = {Y. Kaspi and G. R. Flierl and A.P. Showman},
	File = {../../Papers/kaspi09.pdf},
	Journal = {Icarus},
	Pages = {525--542},
	Title = {The deep wind structure of the giant planets: Results from an anelastic general circulation model},
	Volume = {202},
	Year = {2009},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtrYXNwaTA5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFtxwua8QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxwv9YQAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2FzcGkwOS5wZGYADgAYAAsAawBhAHMAcABpADAAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMva2FzcGkwOS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9rYXNwaTA5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@book{Katsaggelos91,
	Address = {Berlin},
	Author = {A. K. Katsaggelos},
	Publisher = {Springer},
	Title = {Digital Image Restoration},
	Year = 1991}

@incollection{Kattenberg96,
	Address = {Cambridge, UK},
	Author = {A. Kattenberg and Coauthors},
	Booktitle = {Climate Change 1995: The Science of Climate Change},
	Editor = {J. T. Houghton and L. G. {Meira Filho} and B. A. Callander and N. Harris and A. Kattenberg and K. Maskell},
	Pages = {285--357},
	Publisher = {Intergovernmental Panel on Climate Change, Cambridge University Press},
	Title = {Climate Models: Projections of Future Climate},
	Year = 1996}

@article{Kaufman02,
	Annote = {Filed under Atmospheric Chemistry
                  (ESE172-02). Review of aerosol properties and ways
                  of inferring them from satellite measurements.},
	Author = {Y. J. Kaufman and D. Tanr{\'e} and Olivier Boucher},
	Journal = {Nature},
	Pages = {215--223},
	Title = {A satellite view of aerosols in the climate system},
	Volume = 419,
	Year = 2002}

@article{Kavanaugh02,
	Annote = {Filed under Cuffey.},
	Author = {J. L. Kavanaugh and K. M. Cuffey},
	Journal = {Global Biogeochem. Cycles},
	Pages = {in press},
	Title = {Space and time variation of $\delta^{18}\mathrm{O}$ and $\delta \mathrm{D}$ in {Antarctic} Precipitation, Revised},
	Volume = {??},
	Year = 2002}

@article{Kazantsev98,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {E. Kazantsev and J. Sommeria and J. Verron},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1017--1042},
	Title = {Subgrid-scale eddy parameterization by statistical mechanics in a barotropic ocean model},
	Volume = 28,
	Year = 1998}

@article{Kazeminejad07,
	Author = {Kazeminejad, B. and Atkinson, D. H. and P{\'e}rez-Ay{\'u}car, M. and Lebreton, J. P. and Sollazzo, C.},
	File = {../../Papers/kazeminejad07.pdf},
	Journal = {Planet. Space Sci.},
	Pages = {1845--1876},
	Title = {Huygens' entry and descent through {Titan}'s atmosphere---{M}ethodology and results of the trajectory reconstruction},
	Volume = {55},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXgAAAAAAXgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhFrYXplbWluZWphZDA3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFxxgPfhwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxgRB9wAAAAEADAAJDH4ACE6zAACS8wACADBNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2F6ZW1pbmVqYWQwNy5wZGYADgAkABEAawBhAHoAZQBtAGkAbgBlAGoAYQBkADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACRVc2Vycy90YXBpby9QYXBlcnMva2F6ZW1pbmVqYWQwNy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHi4uLy4uL1BhcGVycy9rYXplbWluZWphZDA3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIcAh4CIwIsAjcCOwJJAlACWQJ6An8CggKPApQAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACpg==}}

@techreport{Keller51,
	Annote = {Asymptotics for equations of motion.},
	Author = {J. B. Keller and L. Ting},
	File = {../../Papers/keller51.pdf},
	Institution = {Institute for Mathematics and Mechanics, New York University},
	Title = {Approximate Equations for Large Scale Atmospheric Motions},
	Year = 1951,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxrZWxsZXI1MS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFywMlDmFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwMmmCAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2VsbGVyNTEucGRmAAAOABoADABrAGUAbABsAGUAcgA1ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2tlbGxlcjUxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9rZWxsZXI1MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Kelly91,
	Annote = {Filed under Water Vapor (Feedback and
                  Kinematics).},
	Author = {K. K. Kelly and A. F. Tuck and T. Davies},
	File = {../../Papers/kelly91.pdf},
	Journal = {Nature},
	Pages = {244--247},
	Title = {Wintertime asymmetry of upper tropospheric water between the northern and southern hemispheres},
	Volume = 353,
	Year = 1991,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtrZWxseTkxLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRF0v7mvHVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv7ofnQAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2VsbHk5MS5wZGYADgAYAAsAawBlAGwAbAB5ADkAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMva2VsbHk5MS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9rZWxseTkxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Kerstein94,
	Annote = {Filed under Stochastic Lagrangian Models of Turbulence.},
	Author = {A. R. Kerstein and P. A. McMurty},
	File = {../../Papers/kerstein94.pdf},
	Journal = {Phys. Rev. E},
	Pages = {474--482},
	Title = {Mean-Field Theories of Random Advection},
	Volume = 49,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5rZXJzdGVpbjk0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRF2v5Lc/FBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5NNfAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2Vyc3RlaW45NC5wZGYAAA4AHgAOAGsAZQByAHMAdABlAGkAbgA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2tlcnN0ZWluOTQucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2tlcnN0ZWluOTQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Kharin05,
	Annote = {Filed under Precipitation Statistics. Also consider
                  temperature extremes. Estimate return periods.},
	Author = {V. V. Kharin and F. W. Zwiers},
	File = {../../Papers/kharin05.pdf},
	Journal = {J. Climate},
	Pages = {1156--1173},
	Title = {Estimating Extremes in Transient Climate Change Simulations},
	Volume = 18,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxraGFyaW4wNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRF4wdLTfQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwdND/QAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2hhcmluMDUucGRmAAAOABoADABrAGgAYQByAGkAbgAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2toYXJpbjA1LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9raGFyaW4wNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Kiehl94,
	Author = {J. Kiehl},
	Journal = {Physics Today},
	Month = {November},
	Title = {Clouds and their effects on the climate system},
	Year = 1994}

@techreport{Kiehl96,
	Address = {Boulder, Colorado},
	Author = {J. T. Kiehl and J. J. Hack and G. B. Bonan and B. A. Boville and B. P. Briegleb and D. L. Williamson and P. J. Rasch},
	Institution = {National Center for Atmospheric Research},
	Note = {NCAR Technical Note NCAR/TN-420+STR},
	Title = {Description of the {NCAR} {C}ommunity {C}limate {M}odel ({CCM3})},
	Url = {www.cgd.ucar.edu/cms/ccm3/TN-420/},
	Year = 1996,
	Bdsk-Url-1 = {www.cgd.ucar.edu/cms/ccm3/TN-420/}}

@article{Kiehl97,
	Author = {J. T. Kiehl and K. E. Trenberth},
	File = {../../Papers/kiehl97.pdf},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {197--208},
	Title = {Earth's Annual Global Mean Energy Budget},
	Volume = 78,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtraWVobDk3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRF9wpEKVAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwpFsxAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2llaGw5Ny5wZGYADgAYAAsAawBpAGUAaABsADkANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMva2llaGw5Ny5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9raWVobDk3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Killworth01,
	Annote = {Addresses the question on what kind of
                  density-averages are to be used in transformed mean
                  circulations. See also papers by McDougall and
                  McIntosh.},
	Author = {P. D. Killworth},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1132--1155},
	Title = {Boundary Condition on Quasi-{S}tokes Velocities in Parameterizations},
	Volume = 31,
	Year = 2001}

@article{Killworth97,
	Annote = {Taking zonal flow structure into account improves
                  agreement between phase speeds of linear Rossby
                  waves and observed waves.},
	Author = {P. D. Killworth and D. B. Chelton and R. A. deSzoeke},
	File = {../../Papers/killworth97.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1946--1966},
	Title = {The speed of observed and theoretical long extratropical planetary waves},
	Volume = 27,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9raWxsd29ydGg5Ny5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGAvcOy1gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvcQjVgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2lsbHdvcnRoOTcucGRmAA4AIAAPAGsAaQBsAGwAdwBvAHIAdABoADkANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMva2lsbHdvcnRoOTcucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMva2lsbHdvcnRoOTcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Kim01a,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {H. K. Kim and S. Y. Lee},
	File = {../../Papers/kim01a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2845--2858},
	Title = {Hadley Cell Dynamics in a Primitive Equation Model. {P}art {I}: {A}xisymmetric Flow},
	Volume = 58,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpraW0wMWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGBv+dIV1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv+e41wAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2ltMDFhLnBkZgAADgAWAAoAawBpAG0AMAAxAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2tpbTAxYS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMva2ltMDFhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Kim01b,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {H. K. Kim and S. Y. Lee},
	File = {../../Papers/kim01b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2859--2871},
	Title = {Hadley Cell Dynamics in a Primitive Equation Model. {P}art {II}: {N}onaxisymmetric Flow},
	Volume = 58,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpraW0wMWIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGCv+dIflBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv+e4/gAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2ltMDFiLnBkZgAADgAWAAoAawBpAG0AMAAxAGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2tpbTAxYi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMva2ltMDFiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Kirk_Davidoff00,
	Annote = {Filed under Lindzen.},
	Author = {D. B. Kirk-Davidoff and R. S. Lindzen},
	Journal = {J. Atmos. Sci.},
	Pages = {431--448},
	Title = {An Energy Balance Model Based on Potential Vorticity Homogenization},
	Volume = 13,
	Year = 2000}

@article{Kirtman00,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {B. P. Kirtman and E. K. Schneider},
	File = {../../Papers/kirtman00.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2080--2093},
	Title = {A spontaneously generated tropical atmospheric general circulation},
	Volume = 57,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1raXJ0bWFuMDAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGFv9bdRgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv9dNxgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2lydG1hbjAwLnBkZgAOABwADQBrAGkAcgB0AG0AYQBuADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMva2lydG1hbjAwLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2tpcnRtYW4wMC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Kirtman98,
	Annote = {Dependence of ENSO predictability on background
                  state.},
	Author = {B. P. Kirtman and P. S. Schopf},
	Journal = {J. Climate},
	Pages = {2804--2822},
	Title = {Decadal Variability in {ENSO} Predictability and Prediction},
	Volume = 11,
	Year = 1998}

@article{Kleeman02,
	Annote = {Filed under Majda 2002 review.},
	Author = {R. Kleeman},
	Journal = {J. Atmos. Sci.},
	Pages = {2057--2072},
	Title = {Measuring Dynamical Prediction Utility Using Relative Entropy},
	Volume = 59,
	Year = 2002}

@article{Kleidon03,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {A. Kleidon and K. Fraedrich and T. Kunz and F. Lunkeit},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2003GL018363},
	Pages = {2223},
	Title = {The atmospheric circulation and states of maximum entropy production},
	Volume = 30,
	Year = 2003}

@article{Klein93,
	Author = {S. A. Klein and D. L. Hartmann},
	File = {../../Papers/klein93.pdf},
	Journal = {J. Climate},
	Pages = {1587--1606},
	Title = {The seasonal cycle of low stratiform clouds},
	Volume = {6},
	Year = {1993},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtrbGVpbjkzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGIx7JliwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx7LWCwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2xlaW45My5wZGYADgAYAAsAawBsAGUAaQBuADkAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMva2xlaW45My5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9rbGVpbjkzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Klinger00,
	Annote = {Filed under Ocean Heat Transport.},
	Author = {B. A. Klinger and J. Marotzke},
	File = {../../Papers/klinger00.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {696--705},
	Title = {Meridional Heat Transport by the Subtropical Cell},
	Volume = 30,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1rbGluZ2VyMDAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGJwMIdmlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwMKACgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a2xpbmdlcjAwLnBkZgAOABwADQBrAGwAaQBuAGcAZQByADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMva2xpbmdlcjAwLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2tsaW5nZXIwMC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@book{Kloeden92,
	Address = {Berlin},
	Author = {P.E. Kloeden and E. Platen},
	Publisher = {Springer},
	Title = {Numerical Solution of Stochastic Differential Equations},
	Year = 1992}

@article{Knutson95,
	Annote = {Filed under Manabe.},
	Author = {T. R. Knutson and S. Manabe},
	File = {../../Papers/knutson95.pdf},
	Journal = {J. Climate},
	Pages = {2181--2199},
	Title = {Time-mean response over the tropical {P}acific to increased {CO$_2$} in a coupled ocean-atmosphere model},
	Volume = 8,
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1rbnV0c29uOTUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGOxT35qAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxT5qKAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a251dHNvbjk1LnBkZgAOABwADQBrAG4AdQB0AHMAbwBuADkANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMva251dHNvbjk1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2tudXRzb245NS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Knutson97,
	Annote = {Filed under Manabe. Weak ENSO signal in R15 model.},
	Author = {T. R. Knutson and S. Manabe and D. Gu},
	Journal = {J. Climate},
	Pages = {138--161},
	Title = {Simulated {ENSO} in a Global Coupled Ocean-Atmosphere Model: {M}ultidecadal Amplitude Modulation and {$\mbox{CO}_2$} Sensitivity},
	Volume = 10,
	Year = 1997}

@article{Knutson98,
	Annote = {Filed under Manabe.},
	Author = {T. R. Knutson and S. Manabe},
	Journal = {J. Climate},
	Pages = {2273--2296},
	Title = {Model Assessment of Decadal Variability and Trends in the Tropical Pacific Ocean},
	Volume = 11,
	Year = 1998}

@article{Knutson99,
	Annote = {Filed under Climate Change Detection.},
	Author = {T. R. Knutson and T. L. Delworth and K. W. Dixon and R. J. Stouffer},
	Journal = {J. Geophys. Res.},
	Pages = {30981--30996},
	Title = {Model assessment of regional surface temperature trends (1949--97)},
	Volume = {104D},
	Year = 1999}

@article{Koch02,
	Annote = {Filed under Regularization.},
	Author = {K.-R. Koch and J. Kusche},
	Journal = {J. Geodesy},
	Pages = {259--268},
	Title = {Regularization of geopotential determination from satellite data by variance components},
	Volume = 76,
	Year = 2002}

@article{Koh00,
	Author = {T.-Y. Koh and A. Plumb},
	Journal = {Phys. Fluids},
	Pages = {1518--1528},
	Title = {Lobe dynamics applied to barotropic {R}ossby-wave breaking},
	Volume = 12,
	Year = 2000}

@article{Koh04,
	Author = {T.-Y. Koh and R. A. Plumb},
	File = {../../Papers/koh04.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1631--1654},
	Title = {Isentropic zonal average formulation and the near-surface circulation},
	Volume = 130,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglrb2gwNC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGPvljBRwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvlkxxwAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a29oMDQucGRmAA4AFAAJAGsAbwBoADAANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMva29oMDQucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMva29oMDQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Kondrashov06,
	Annote = {Filed under "Comment on Kondrashov and Ghil (2006) among my ms.},
	Author = {D. Kondrashov and M. Ghil},
	File = {../../Papers/kondrashov06.pdf},
	Journal = {Nonlin. Processes Geophys.},
	Pages = {151--159},
	Title = {Spatio-temporal filling of missing points in geophysical data sets},
	Volume = 13,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBrb25kcmFzaG92MDYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGQwK9FjQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwK+n/QAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a29uZHJhc2hvdjA2LnBkZgAADgAiABAAawBvAG4AZAByAGEAcwBoAG8AdgAwADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL2tvbmRyYXNob3YwNi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMva29uZHJhc2hvdjA2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Korty07b,
	Author = {R. L. Korty and T. Schneider},
	Date-Modified = {2010-06-11 12:17:36 -0700},
	Journal = {J. Climate},
	Pages = {5977--5991},
	Title = {A climatology of the tropospheric thermal stratification using saturation potential vorticity},
	Volume = 20,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxrb3J0eTA3Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGVw6JjWQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw6LT2QAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a29ydHkwN2IucGRmAAAOABoADABrAG8AcgB0AHkAMAA3AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2tvcnR5MDdiLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9rb3J0eTA3Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Korty07a,
	Author = {Korty, R. L. and Emanuel, K. A.},
	File = {../../Papers/korty07a.pdf},
	Journal = {J. Climate},
	Pages = {5213--5228},
	Title = {The dynamic response of the winter stratosphere to an equable climate surface temperature gradient},
	Volume = {20},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxrb3J0eTA3YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGUxizq/AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxi1NbAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a29ydHkwN2EucGRmAAAOABoADABrAG8AcgB0AHkAMAA3AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2tvcnR5MDdhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9rb3J0eTA3YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Korty08a,
	Author = {R. L. Korty and T. Schneider},
	Date-Modified = {2010-06-11 12:18:18 -0700},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2008GL035847},
	Pages = {{L23803}},
	Title = {Extent of {Hadley} circulations in dry atmospheres},
	Volume = {35},
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxrb3J0eTA4YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGWxVldLwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxVnNrwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a29ydHkwOGEucGRmAAAOABoADABrAG8AcgB0AHkAMAA4AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2tvcnR5MDhhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9rb3J0eTA4YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Koshyk01,
	Annote = {Spectral energy budget changes markedly from
                  troposphere to stratosphere. In troposphere, APE-KE
                  conversion large and positive at all scales; in
                  stratosphere, APE-KE conversion much smaller at
                  large scales, negative at small scales. [Consistent
                  with picture of troposphere as thermal boundary
                  layer of the atmosphere.]},
	Author = {J. N. Koshyk and K. Hamilton},
	Journal = {J. Atmos. Sci.},
	Pages = {329--348},
	Title = {The Horizontal Kinetic Energy Spectrum and Spectral Budget Simulated by a High-Resolution Troposphere-Stratosphere-Mesosphere GCM},
	Volume = 58,
	Year = 2001}

@article{Koshyk96,
	Annote = {Comparison of advective flux of PV with
                  non-advective flux components. Non-advective
                  components important in boundary layer, in
                  gravity-wave drag region, and in tropical
                  midtroposphere in regions of latent heat release.},
	Author = {J. N. Koshyk and N. A. McFarlane},
	Journal = {J. Atmos. Sci.},
	Pages = {550--563},
	Title = {The Potential Vorticity Budget of an Atmospheric General Circulation Model},
	Volume = 53,
	Year = 1996}

@article{Koutavas02,
	Annote = {Filed under Paleo-Climate Reviews.},
	Author = {A. Koutavas and J. Lynch-Stieglitz and T. M. Marchitto Jr. and J. P. Sachs},
	Journal = {Science},
	Pages = {226--230},
	Title = {El {N}i{\~n}o-Like Pattern in {I}ce {A}ge Tropical Pacific Sea Surface Temperature},
	Volume = 297,
	Year = 2002}

@article{Kraichnan59,
	Annote = {Direct Interaction Approximation. Not on File.},
	Author = {R. H. Kraichnan},
	Journal = {J. Fluid Mech.},
	Pages = {497--543},
	Title = {The structure of isotropic turbulence at very high {R}eynolds numbers},
	Volume = 5,
	Year = 1959}

@article{Kraichnan77,
	Annote = {Alternative derivation of Direct Interaction
                  Approximation by renormalized perturbation
                  expansion. Not on File.},
	Author = {R. H. Kraichnan},
	Journal = {J. Fluid Mech.},
	Pages = {349--374},
	Title = {Eulerian and {L}agrangian renormalization in turbulence theory},
	Volume = 83,
	Year = 1977}

@article{Krakauer04,
	Author = {N. Y. Krakauer and T. Schneider and J. T. Randerson and S. C. Olsen},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2004GL020323},
	Pages = {L19108},
	Title = {Using generalized cross-validation to select parameters in inversions for regional carbon fluxes},
	Volume = 31,
	Year = 2004}

@article{Kraucunas07,
	Annote = {Filed under Hartmann.},
	Author = {I. Kraucunas and D. L. Hartmann},
	File = {../../Papers/kraucunas07.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2540--2557},
	Title = {Tropical Stationary Waves in a Nonlinear Shallow-Water Model with Realistic Basic States},
	Volume = {64},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9rcmF1Y3VuYXMwNy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGaw8KXjgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw8MIDgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a3JhdWN1bmFzMDcucGRmAA4AIAAPAGsAcgBhAHUAYwB1AG4AYQBzADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMva3JhdWN1bmFzMDcucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMva3JhdWN1bmFzMDcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Kraus67,
	Annote = {Classic paper on seasonal thermocline. See also
                  Turner67},
	Author = {E. B. Kraus and J. S. Turner},
	Journal = {Tellus},
	Pages = {98--105},
	Title = {A one-dimensional model of the seasonal thermocline: {II}. {T}he general theory and its consequences},
	Volume = 19,
	Year = 1967}

@article{Kravtsov03,
	Author = {S. Kravtsov and A. W. Robertson and M. Ghil},
	Journal = {J. Atmos. Sci.},
	Pages = {2267--2286},
	Title = {Low-frequency variability in a baroclinic $\beta$ channel with land--sea contrast},
	Volume = 60,
	Year = 2003}

@article{Krishnamurti81,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {T. N. Krishnamurti and P. Ardanuy and Y. Ramanathan and R. Pasch},
	File = {../../Papers/krishnamurti81.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {344--363},
	Title = {On the onset vortex of the summer monsoons},
	Volume = 109,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAX4AAAAAAX4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhJrcmlzaG5hbXVydGk4MS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGcwah5agAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwajp6gAAAAEADAAJDH4ACE6zAACS8wACADFNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a3Jpc2huYW11cnRpODEucGRmAAAOACYAEgBrAHIAaQBzAGgAbgBhAG0AdQByAHQAaQA4ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAlVXNlcnMvdGFwaW8vUGFwZXJzL2tyaXNobmFtdXJ0aTgxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHy4uLy4uL1BhcGVycy9rcmlzaG5hbXVydGk4MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACIgIkAikCMgI9AkECTwJWAl8CgQKGAokClgKbAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAq0=}}

@article{Krishnamurti82,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {T. N. Krishnamurti and Y. Ramanathan},
	File = {../../Papers/krishnamurti82.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1290--1306},
	Title = {Sensitivity of the monsoon onset to differential heating},
	Volume = {39},
	Year = {1982},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAX4AAAAAAX4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhJrcmlzaG5hbXVydGk4Mi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGdwzj05AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwzlXVAAAAAEADAAJDH4ACE6zAACS8wACADFNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a3Jpc2huYW11cnRpODIucGRmAAAOACYAEgBrAHIAaQBzAGgAbgBhAG0AdQByAHQAaQA4ADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAlVXNlcnMvdGFwaW8vUGFwZXJzL2tyaXNobmFtdXJ0aTgyLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHy4uLy4uL1BhcGVycy9rcmlzaG5hbXVydGk4Mi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACIgIkAikCMgI9AkECTwJWAl8CgQKGAokClgKbAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAq0=}}

@article{Krzanowski95,
	Annote = {Filed under Discriminant Analysis.},
	Author = {W. J. Krzanowski and P. Jonathan and W. V. {McCarthy} and M. R. Thomas},
	Journal = {Appl. Stat.},
	Pages = {101--115},
	Title = {Discriminant Analysis with Singular Covariance Matrices: Methods and Applications to Spectroscopic Data},
	Volume = 44,
	Year = 1995}

@article{Kucharski97,
	Annote = {Filed under Available Potential Energy. Derivation
                  of APE from 'extended exergy.' Local formulation of
                  APE.},
	Author = {F. Kucharski},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {2141--2156},
	Title = {On the concept of exergy and available potential energy},
	Volume = 123,
	Year = 1997}

@article{Kuo04,
	Annote = {Filed under Plumb.},
	Author = {A. Kuo and R. A. Plumb and J. Marshall},
	Journal = {J. Phys. Oceanogr.},
	Note = {submitted},
	Pages = {??},
	Title = {Transformed Eulerian-mean theory. {II}: Potential vorticity homogenization, and the equilibrium of a wind- and buoyancy-driven zonal flow},
	Volume = {??},
	Year = 2004}

@article{Kuo05,
	Annote = {Filed under Plumb. Part II of Plumb05.},
	Author = {A. Kuo and R. A. Plumb and J. Marshall},
	File = {../../Papers/kuo05.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {175--187},
	Title = {Transformed Eulerian-mean theory. {II}: Potential Vorticity Homogenization and the Equilibrium of a Wind- and Buoyancy-Driven Zonal Flow},
	Volume = {35},
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglrdW8wNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGivnyHzAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvnzqPAAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a3VvMDUucGRmAA4AFAAJAGsAdQBvADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMva3VvMDUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMva3VvMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Kuo51,
	Author = {Kuo, H.-L.},
	File = {../../Papers/kuo51.pdf},
	Journal = {J. Meteor.},
	Pages = {307--315},
	Title = {Vorticity transfer as related to the development of the general circulation},
	Volume = 8,
	Year = 1951,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglrdW81MS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGjw7m04VBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7olYQAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a3VvNTEucGRmAA4AFAAJAGsAdQBvADUAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMva3VvNTEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMva3VvNTEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Kusche03,
	Annote = {Filed under Regularization.},
	Author = {J. Kusche},
	Journal = {J. Geodesy},
	Pages = {641--652},
	Title = {A {M}onte-{C}arlo technique for weight estimation in satellite geodesy},
	Volume = 76,
	Year = 2003}

@article{Kushner01,
	Author = {Kushner, P. J. and Held, I. M. and Delworth, T. L.},
	File = {../../Papers/kushner01.pdf},
	Journal = {J. Climate},
	Pages = {2238--2249},
	Title = {Southern {H}emisphere Atmospheric Circulation Response to Global Warming},
	Volume = 14,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1rdXNobmVyMDEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGlv9xyPlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv9zivgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a3VzaG5lcjAxLnBkZgAOABwADQBrAHUAcwBoAG4AZQByADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMva3VzaG5lcjAxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2t1c2huZXIwMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Kushner95a,
	Author = {P. J. Kushner and T. G. Shepherd},
	Journal = {J. Fluid Mech.},
	Pages = {67--104},
	Title = {Wave-activity conservation laws and stability theorems for semi-geostrophic dynamics. {P}art {1}. {P}seudomomentum-based theory},
	Volume = 290,
	Year = 1995}

@article{Kushner95b,
	Author = {P. J. Kushner and T. G. Shepherd},
	Journal = {J. Fluid Mech.},
	Pages = {105--129},
	Title = {Wave-activity conservation laws and stability theorems for semi-geostrophic dynamics. {P}art {2}. {P}seudoenergy-based theory},
	Volume = 290,
	Year = 1995}

@article{Kushner95c,
	Annote = {Not on file.},
	Author = {P. J. Kushner},
	Journal = {Tellus},
	Pages = {541--547},
	Title = {A generalized {C}harney-{S}tern theorem for semi-geostrophic dynamics},
	Volume = {47A},
	Year = 1995}

@article{Kushner98,
	Annote = {Filed under Surface Heat Flux Parameterizations.},
	Author = {P. J. Kushner and I. M. Held},
	File = {../../Papers/kushner98.pdf},
	Journal = {Geophys. Res. Lett.},
	Pages = {4213--4216},
	Title = {A test, using atmospheric data, of a method for estimating oceanic eddy diffusivity},
	Volume = 25,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1rdXNobmVyOTgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGnwsFEzAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsGnPAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a3VzaG5lcjk4LnBkZgAOABwADQBrAHUAcwBoAG4AZQByADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMva3VzaG5lcjk4LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2t1c2huZXI5OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Kushnir94,
	Annote = {Not on file.},
	Author = {Y. Kushnir},
	Journal = {J. Climate},
	Pages = {141--157},
	Title = {Interdecadal variations in {N}orth {A}tlantic sea surface temperature and associated atmospheric condition},
	Volume = 7,
	Year = 1994}

@article{Kushnir96,
	Annote = {Filed under Predictability. Extratropics not well
                  predictable with R15 model; this may be due to model
                  deficiencies in boundary layer.},
	Author = {Y. Kushnir and I. M. Held},
	Journal = {J. Climate},
	Pages = {1208--1220},
	Title = {Equilibrium Atmospheric Response to {N}orth {A}tlantic {SST} Anomalies},
	Volume = 9,
	Year = 1996}

@article{Kutzbach97,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {J. E. Kutzbach and Z. Liu},
	File = {../../Papers/kutzbach97.pdf},
	Journal = {Science},
	Pages = {440--443},
	Title = {Response of the {A}frican monsoon to orbital forcing and ocean feedbacks in the middle {H}olocene},
	Volume = 278,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5rdXR6YmFjaDk3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGqwO/N9wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwPAwZwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6a3V0emJhY2g5Ny5wZGYAAA4AHgAOAGsAdQB0AHoAYgBhAGMAaAA5ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2t1dHpiYWNoOTcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2t1dHpiYWNoOTcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Lambeck01,
	Annote = {Filed under Paleo-Climate Reviews.},
	Author = {K. Lambeck and J. Chappell},
	Journal = {Science},
	Pages = {679--686},
	Title = {Sea Level Change Through the Last Glacial Cycle},
	Volume = 292,
	Year = 2001}

@article{Lambeck02,
	Annote = {Filed under Paleo-Climate Reviews.},
	Author = {K. Lambeck and T. M. Esat and E.-K. Potter},
	Journal = {Nature},
	Pages = {199--206},
	Title = {Links between climate and sea levels for the past three million years},
	Volume = 419,
	Year = 2002}

@article{Lambert84,
	Author = {S. J. Lambert},
	File = {../../Papers/lambert84.pdf},
	Journal = {Atmos.-Ocean},
	Pages = {265--282},
	Title = {A Global Available Potential Energy--Kinetic Energy Budget in Terms of the Two-Dimensional Wavenumber for the {FGGE} Year},
	Volume = 22,
	Year = 1984,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1sYW1iZXJ0ODQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGswVlKI1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwVmskwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGFtYmVydDg0LnBkZgAOABwADQBsAGEAbQBiAGUAcgB0ADgANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbGFtYmVydDg0LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2xhbWJlcnQ4NC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@mastersthesis{Lamquin06,
	Address = {Toulouse, France},
	Author = {N. Lamquin},
	Note = {(Research carried out at California Institute of Technology.)},
	School = {Universit{\'e} Paul Sabatier and Ecole Nationale Superieure de l'A{\'e}ronautique et de l'Espace},
	Title = {Stochastic Models for Moisture Transport in Two-Dimensional Turbulence},
	Year = 2006}

@book{Landau87,
	Address = {Oxford},
	Author = {L. D. Landau and E. M. Lifshitz},
	Edition = {2nd},
	Pages = 539,
	Publisher = {Pergamon Press},
	Title = {Fluid Mechanics},
	Year = 1987}

@article{Lapeyre03,
	Annote = {Filed under Baroclinic Eddy Flux Parameterizations.},
	Author = {G. Lapeyre and I. M. Held},
	File = {../../Papers/lapeyre03.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2907--2916},
	Title = {Diffusivity, Kinetic Energy Dissipation, and Closure Theories for the Poleward Eddy Heat Flux},
	Volume = 60,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1sYXBleXJlMDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGtvrdbiQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvre9+QAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGFwZXlyZTAzLnBkZgAOABwADQBsAGEAcABlAHkAcgBlADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbGFwZXlyZTAzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2xhcGV5cmUwMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Lapeyre04,
	Annote = {Filed under Held.},
	Author = {G. Lapeyre and I. M. Held},
	File = {../../Papers/lapeyre04.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1693--1710},
	Title = {The role of moisture in the dynamics and energetics of turbulent baroclinic eddies},
	Volume = 61,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1sYXBleXJlMDQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGuvT1GoQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvT2pEQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGFwZXlyZTA0LnBkZgAOABwADQBsAGEAcABlAHkAcgBlADAANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbGFwZXlyZTA0LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2xhcGV5cmUwNC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Larichev95,
	Annote = {Filed under Held.},
	Author = {V. D. Larichev and I. M. Held},
	Journal = {J. Phys. Oceanogr.},
	Pages = {2285--2297},
	Title = {Eddy Amplitudes and Fluxes in a Homogeneous Model of Fully Developed Baroclinic Instability},
	Volume = 25,
	Year = 1995}

@article{Latif98,
	Annote = {.},
	Author = {M. Latif},
	Journal = {J. Climate},
	Pages = {602--624},
	Title = {Dynamics of Interdecadal Variability in Coupled Ocean-Atmosphere Models},
	Volume = 11,
	Year = 1998}

@article{Lau78,
	Author = {N.-G. Lau},
	File = {../../Papers/lau78.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1900--1923},
	Title = {On the Three-Dimensional Structure of the Observed Transient Eddy Statistics of the {N}orthern {H}emisphere Wintertime Circulation},
	Volume = 35,
	Year = 1978,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglsYXU3OC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGwvRswqQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRuTGQAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGF1NzgucGRmAA4AFAAJAGwAYQB1ADcAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvbGF1NzgucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvbGF1NzgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Lau85,
	Annote = {Not on file.},
	Author = {N.-C. Lau},
	Journal = {Mon. Wea. Rev.},
	Pages = {19700--1996},
	Title = {Modeling the seasonal dependence of the atmospheric response to observed {E}l {N}i{\~n}os in 1962--1976},
	Volume = 113,
	Year = 1985}

@article{Lau88a,
	Author = {N.-C. Lau},
	File = {../../Papers/lau88a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2718--2743},
	Title = {Variability of the observed midlatitude storm tracks in relation to low-frequency changes in the circulation pattern},
	Volume = 45,
	Year = 1988,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpsYXU4OGEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGxx1U5fgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx1Wp/gAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGF1ODhhLnBkZgAADgAWAAoAbABhAHUAOAA4AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2xhdTg4YS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvbGF1ODhhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Lau88b,
	Author = {N.-C. Lau and I. M. Held and J. D. Neelin},
	Journal = {J. Atmos. Sci.},
	Pages = {3810--3832},
	Title = {The {M}adden-{J}ulian {O}scillation in an idealized general circulation model},
	Volume = 45,
	Year = 1988}

@article{Lau94,
	Annote = {Not on file.},
	Author = {N.-C. Lau and M. J. Nath},
	Journal = {J. Climate},
	Pages = {1184--1207},
	Title = {A Modelling Study of the Relative Roles of Tropical and Extratropical {SST} Anomalies in the Variability of the Global Atmosphere-Ocean System},
	Volume = 7,
	Year = 1994}

@article{Lau96,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {K.-M. Lau and S. Yang},
	File = {../../Papers/lau96.pdf},
	Journal = {J. Climate},
	Pages = {965--985},
	Title = {Seasonal Variation, Abrupt Transition, and Intraseasonal Variability Associated with the {A}sian Summer Monsoon in the {GLA} {GCM}},
	Volume = 9,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglsYXU5Ni5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGywa1nxwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwa3YRwAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGF1OTYucGRmAA4AFAAJAGwAYQB1ADkANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvbGF1OTYucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvbGF1OTYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@unpublished{Lau96b,
	Annote = {Midlatitude circulation systems. Tropical
                  circulation systems. Low-frequency variability. Lab
                  exercises on stationary waves and the Superstorm
                  March 13, 1993},
	Author = {N.-C. Lau},
	Note = {Lecture Notes},
	Title = {Weather Dynamics},
	Year = {Spring 1996}}

@article{Lawley56,
	Annote = {Computes estimate of bias in eigenvalues of
                  covariance and correlation matrices.},
	Author = {D. N. Lawley},
	Journal = {Biometrika},
	Pages = {128--136},
	Title = {Tests of Significance for the Latent Roots of Covariance and Correlation Matrices},
	Volume = 43,
	Year = 1956}

@article{Lawrence03,
	Author = {J. R. Lawrence and S. D. Gedzelman},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2002GL015906},
	Pages = 1072,
	Title = {Tropical ice core isotopes: Do they reflect changes in storm activity?},
	Volume = 30,
	Year = 2003}

@article{Lawrence04,
	Author = {J. R. Lawrence and S. D. Gedzelman and D. Dexheimer and H.-K. Cho and G. D. Carrie and R. Gasparini and C. R. Anderson and K. P. Bowman and M. I. Biggerstaff},
	Journal = {J. Geophys. Res.},
	Note = {doi:10.1029/2003JD004046},
	Pages = {D06115},
	Title = {Stable isotopic composition of water vapor in the tropics},
	Volume = 109,
	Year = 2004}

@article{Lawrence05,
	Annote = {Filed under Moist Convection.},
	Author = {M. G. Lawrence and P. J. Rasch},
	File = {../../Papers/lawrence05.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2880--2894},
	Title = {Tracer Transport in Deep Convective Updrafts: Plume Ensemble versus Bulk Formulations},
	Volume = 62,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5sYXdyZW5jZTA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRGzw3MhqQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw3OSKQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGF3cmVuY2UwNS5wZGYAAA4AHgAOAGwAYQB3AHIAZQBuAGMAZQAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2xhd3JlbmNlMDUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2xhd3JlbmNlMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Lawrence96,
	Author = {J. R. Lawrence and S. D. Gedzelman},
	Journal = {Geophys. Res. Lett.},
	Pages = {527--530},
	Title = {Low stable isotope ratios of tropical cyclone rains},
	Volume = 23,
	Year = 1996}

@book{Lawson74,
	Address = {Englewood Cliffs, NJ},
	Author = {C. L. Lawson and R. J. Hanson},
	Publisher = {Prentice-Hall},
	Title = {Solving Least Squares Problems},
	Year = 1974}

@article{Lee03,
	Annote = {Baroclinic waves grow predominantly along
                  subtropical jet only when jet is sufficiently strong.},
	Author = {S. Lee and H.-Y. Kim},
	File = {../../Papers/lee03.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1490--1503},
	Title = {The Dynamical Relationship between Subtropical and Eddy-driven Jets},
	Volume = 60,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglsZWUwMy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRG2wRztPQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwR1PrQAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGVlMDMucGRmAA4AFAAJAGwAZQBlADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvbGVlMDMucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvbGVlMDMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Lee05,
	Author = {S. Lee},
	File = {../../Papers/lee05.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2484--2498},
	Title = {Baroclinic Multiple Zonal Jets on the Sphere},
	Volume = 62,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglsZWUwNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRG3vyYgqwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvyaDGwAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGVlMDUucGRmAA4AFAAJAGwAZQBlADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvbGVlMDUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvbGVlMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Lee08,
	Author = {Lee, M. I. and Suarez, M. J. and Kang, I. S. and Held, I. M. and Kim, D.},
	File = {../../Papers/lee08.pdf},
	Journal = {J. Climate},
	Pages = {4934--4954},
	Title = {A Moist Benchmark Calculation for Atmospheric General Circulation Models},
	Volume = {21},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglsZWUwOC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRG6xuetlQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxugQBQAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGVlMDgucGRmAA4AFAAJAGwAZQBlADAAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvbGVlMDgucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvbGVlMDgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Lee97,
	Annote = {Inter-jet disturbances maintain separation between
                  jets.},
	Author = {S. Lee},
	File = {../../Papers/lee97.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1726--1738},
	Title = {Maintenance of Multiple Jets in a Baroclinic Flow},
	Volume = 54,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglsZWU5Ny5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRG8wptgllBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwpvDBgAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGVlOTcucGRmAA4AFAAJAGwAZQBlADkANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvbGVlOTcucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvbGVlOTcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Legras80,
	Annote = {Filed under Wave Turbulence.},
	Author = {B. Legras},
	File = {../../Papers/legras80.pdf},
	Journal = {Geophys. Astrophys. Fluid Dyn.},
	Pages = {253--281},
	Title = {Turbulent Phase Shift of Rossby Waves},
	Volume = 15,
	Year = 1980,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxsZWdyYXM4MC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRG/wsEJDlBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsFrfgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGVncmFzODAucGRmAAAOABoADABsAGUAZwByAGEAcwA4ADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2xlZ3JhczgwLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9sZWdyYXM4MC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Leith71,
	Author = {C. E. Leith},
	Journal = {J. Atmos. Sci.},
	Key = {turbulence},
	Pages = {145--161},
	Title = {Atmospheric Predictability and Two-Dimensional Turbulence},
	Volume = 28,
	Year = 1971}

@article{Leith75,
	Annote = {Uses fluctuation-dissipation relation to determine
                  the mean response of the climate system to changes
                  in external forcing.},
	Author = {C. E. Leith},
	Journal = {J. Atmos. Sci.},
	Pages = {2022--2026},
	Title = {Climate Response and Fluctuation Dissipation},
	Volume = 32,
	Year = 1975}

@article{Leith80,
	Annote = {Reviews nonlinear normal mode initialization, which
                  seeks states whose gravity wave compoenent does not
                  change with time. Shows that for an f-plane
                  Boussinesq model, nonlinear normal mode
                  initialization results in QG dynamics as a first
                  approximation.},
	Author = {C. E. Leith},
	Journal = {J. Atmos. Sci.},
	Pages = {958--968},
	Title = {Nonlinear Normal Mode Initialization and Quasi-Geostrophic Theory},
	Volume = 37,
	Year = 1980}

@article{Leith90,
	Author = {C. E. Leith},
	Journal = {Phys. Fluids A},
	Pages = {297--299},
	Title = {Stochastic backscatter in a subrid-scale model: Plane shear mixing layer},
	Volume = 2,
	Year = 1990}

@article{Leith96,
	Annote = {Considers modeling of probabilistic properties of
                  nonlinear deterministic systems by linear stochastic
                  models. Develops stochastic model that simulates the
                  transient energy spectrum of the global atmosphere.},
	Author = {C. E. Leith},
	Journal = {Physica D},
	Pages = {481--491},
	Title = {Stochastic Models of Chaotic Systems},
	Volume = 98,
	Year = 1996}

@article{Lellouch89,
	Author = {Lellouch, E. and Coustenis, A. and Gautier, D. and Raulin, F. and Dubouloz, N. and Fr{\`e}re, C.},
	Journal = {Icarus},
	Pages = {328--349},
	Title = {{Titan}'s atmosphere and hypothesized ocean: A reanalysis of the {Voyager 1} radio-occultation and {IRIS} 7.7-$\mu$m data},
	Volume = {79},
	Year = {1989}}

@article{Leovy01,
	Annote = {Filed under Mars Dynamics. Short review of literature.},
	Author = {C. Leovy},
	File = {../../Papers/leovy01.pdf},
	Journal = {Nature},
	Pages = {245--249},
	Title = {Weather and climate on {M}ars},
	Volume = 412,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtsZW92eTAxLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHDv3fq+AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3hNaAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGVvdnkwMS5wZGYADgAYAAsAbABlAG8AdgB5ADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvbGVvdnkwMS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9sZW92eTAxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Leroy98,
	Annote = {Filed under Climate Change Detection. Much talk
                  about generalities, few specifics to put one's hands
                  on. Claims to use Bayesian methods, but does not, in
                  fact, do it. No actual prior probabilities are being
                  used in practical examples. Obscure talk about
                  penalizing overparameterized models.},
	Author = {S. S. Leroy},
	Journal = {J. Climate},
	Pages = {640--651},
	Title = {Detecting Climate Signals: Some Bayesian Aspects},
	Volume = 11,
	Year = 1998}

@article{Leung90,
	Annote = {Claim that transinformation is superior measure of
                  predictability than signal-to-noise ratio (variance
                  ratio). But in their examples, which are all
                  Gaussian, the two are essentially equivalent: the
                  variance ratio measure is obtained by taking the
                  exponential of the transinformation. Present
                  concepts of information theory in complicated way.},
	Author = {L.-Y. Leung and G. R. North},
	Journal = {J. Climate},
	Pages = {5--14},
	Title = {Information Theory and Climate Prediction},
	Volume = 3,
	Year = 1990}

@article{Levine10,
	Author = {X. J. Levine and T. Schneider},
	Journal = {J. Atmos. Sci.},
	Note = {To be submitted.},
	Pages = {?},
	Title = {Response of the {H}adley Circulation to Climate Change in an Aquaplanet {GCM} Coupled to Ocean Heat Transport},
	Volume = {?},
	Year = 2009}

@article{Levine77,
	Author = {Levine, J.S. and Kraemer, D.R. and Kuhn, W.R.},
	Journal = {Icarus},
	Number = {1},
	Pages = {136--145},
	Title = {Solar radiation incident on {Mars} and the outer planets: Latitudinal, seasonal, and atmospheric effects},
	Volume = {31},
	Year = {1977}}

@article{Levitus01,
	Annote = {Filed under Climate Change Detection.},
	Author = {S. Levitus and J. I. Antonov and J. Wang and T. L. Delworth and K. W. Dixon and A. J. Broccoli},
	Journal = {Science},
	Pages = {267--270},
	Title = {Anthropogenic Warming of Earth's Climate System},
	Volume = 292,
	Year = 2001}

@article{Levy71,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {H. Levy {II}},
	Journal = {Science},
	Pages = {141--143},
	Title = {Normal Atmosphere: Large Radical and Formaldehyde Concentrations Predicted},
	Volume = 173,
	Year = 1971}

@article{Li04,
	Author = {Li, L. and Ingersoll, A.P. and Vasavada, A.R. and Porco, C.C. and Del Genio, A.D. and Ewald, S.P.},
	File = {../../Papers/li04.pdf},
	Journal = {Icarus},
	Pages = {9--23},
	Title = {Life cycles of spots on {Jupiter} from {Cassini} images},
	Volume = {172},
	Year = {2004},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfghsaTA0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHJwst8RVBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsvetQAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGkwNC5wZGYAAA4AEgAIAGwAaQAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL2xpMDQucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL2xpMDQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@article{Li08,
	Author = {C. Li and D. S. Battisti},
	File = {../../Papers/li08.pdf},
	Journal = {J. Climate},
	Pages = {3561--3579},
	Title = {Reduced {A}tlantic Storminess during {L}ast {G}lacial {M}aximum: Evidence from a Coupled Climate Model},
	Volume = 21,
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfghsaTA4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHOxRjovwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxRlLLwAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGkwOC5wZGYAAA4AEgAIAGwAaQAwADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL2xpMDgucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL2xpMDgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@article{Li81,
	Annote = {Filed under AR Modeling. Multivariate portmanteau
                  test},
	Author = {W. K. Li and A. I. {McLeod}},
	Journal = {J. Roy. Stat. Soc. B},
	Pages = {231--239},
	Title = {Distribution of the Residual Autocorrelations in Multivariate {ARMA} Time Series Models},
	Volume = 43,
	Year = 1981}

@article{Li96,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {Li, C. and Yanai, M.},
	File = {../../Papers/li96.pdf},
	Journal = {J. Climate},
	Pages = {358--375},
	Title = {The onset and interannual variability of the {A}sian summer monsoon in relation to land-sea thermal contrast},
	Volume = 9,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfghsaTk2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHPwSQk41BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwSSHUwAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGk5Ni5wZGYAAA4AEgAIAGwAaQA5ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL2xpOTYucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL2xpOTYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@article{Lian08,
	Author = {Y. Lian and A. P. Showman},
	File = {../../Papers/lian08.pdf},
	Journal = {Icarus},
	Pages = {597--616},
	Title = {Deep jets on gas-giant planets},
	Volume = 194,
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpsaWFuMDgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHQxBwNbwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxBxv3wAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGlhbjA4LnBkZgAADgAWAAoAbABpAGEAbgAwADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2xpYW4wOC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvbGlhbjA4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Lian10,
	Author = {Lian, Y. and Showman, A. P.},
	File = {../../Papers/lian10.pdf},
	Journal = {Icarus},
	Pages = {373--393},
	Title = {Generation of equatorial jets by large-scale latent heating on giant planets},
	Volume = 207,
	Year = {2010},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpsaWFuMTAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHRyCyNLQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyCzvnQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGlhbjEwLnBkZgAADgAWAAoAbABpAGEAbgAxADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2xpYW4xMC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvbGlhbjEwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@incollection{Lighthill63,
	Address = {Oxford},
	Author = {M. J. Lighthill},
	Booktitle = {Laminar Boundary Layers},
	Editor = {L. Rosenhead},
	Pages = {46--113},
	Publisher = {Clarendon Press},
	Title = {Boundary Layer Theory},
	Year = 1963}

@article{Lilly96,
	Author = {D. K. Lilly},
	Journal = {Atmos. Res.},
	Pages = {143--151},
	Title = {A comparison of incompressible, anelastic, and {B}oussinesq dynamics},
	Volume = 40,
	Year = 1996}

@article{Lin96,
	Annote = {Generalization of van Leer scheme to higher
                  dimensions. Test as tracer advection scheme in GCM.},
	Author = {S.-J. Lin and R. B. Rood},
	Journal = {Mon. Wea. Rev.},
	Pages = {2046--2070},
	Title = {Multidimensional Flux-Form Semi-Lagrangian Transport Schemes},
	Volume = 124,
	Year = 1996}

@article{Lindstrom88,
	Annote = {Filed under Parameter Estimation.},
	Author = {M.~J. Lindstrom and D.~M. Bates},
	Journal = {J. Amer. Statist. Assoc.},
	Key = {parameter estimation},
	Pages = {1014-1022},
	Title = {Newton-{R}aphson and {EM} algorithms for linear mixed-effects models for repeated-measures data},
	Volume = 83,
	Year = 1988}

@incollection{Lindzen7?,
	Author = {R. Lindzen},
	Booktitle = {???},
	Editor = {???},
	Pages = {293--350},
	Publisher = {??},
	Title = {Atmospheric Tides},
	Year = {197?}}

@article{Lindzen80a,
	Annote = {Maximum growth rate of baroclinic instability is
                  proportional to supercriticality.},
	Author = {R. S. Lindzen and B. Farrell},
	Journal = {J. Atmos. Sci.},
	Pages = {1648--1654},
	Title = {A simple approximate result for the maximum growth rate of baroclinic instabilities},
	Volume = 37,
	Year = 1980}

@article{Lindzen80b,
	Annote = {Not on file. Neutralization of troposphere with zero
                  pseudo-pv gradients.},
	Author = {R. S. Lindzen and B. Farrell},
	Journal = {Mon. Wea. Rev.},
	Pages = {2064--2079},
	Title = {The role of the polar regions in global climate, and a new parameterization of global heat transport},
	Volume = 108,
	Year = 1980}

@article{Lindzen81,
	Author = {R. S. Lindzen},
	Journal = {J. Geophys. Res.},
	Pages = {9707--9714},
	Title = {Turbulence and Stress Owing to Gravity Wave and Tidal Breakdown},
	Volume = {86C},
	Year = {1981}}

@article{Lindzen83,
	Annote = {Filed under Barotropic Point Jet. Linear Charney
                  problem is homomorphic to linear stability problem
                  of barotropic point jet.},
	Author = {R. S. Lindzen and A. J. Rosenthal and B. Farrell},
	Journal = {J. Atmos. Sci.},
	Pages = {1029--1034},
	Title = {Charney's Problem for Baroclinic Instability Applied to Barotropic Instability},
	Volume = 40,
	Year = 1983}

@article{Lindzen87a,
	Annote = {History of QBO theory.},
	Author = {R. S. Lindzen},
	File = {../../Papers/lindzen87a.pdf},
	Journal = {Bull. Am. Meteor. Soc.},
	Pages = {329--337},
	Title = {On the Development of the Theory of the {QBO}},
	Volume = 68,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5saW5kemVuODdhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHXvxax5AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvxcUVAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGluZHplbjg3YS5wZGYAAA4AHgAOAGwAaQBuAGQAegBlAG4AOAA3AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2xpbmR6ZW44N2EucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2xpbmR6ZW44N2EucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Lindzen87b,
	Author = {R. S. Lindzen and S. Nigam},
	File = {../../Papers/lindzen87b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2418--2436},
	Title = {On the Role of Sea Surface Temperature Gradients in Forcing Low-Level Winds and Convergence in the {T}ropics},
	Volume = 44,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5saW5kemVuODdiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHYveJDIgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAveKzogAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGluZHplbjg3Yi5wZGYAAA4AHgAOAGwAaQBuAGQAegBlAG4AOAA3AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL2xpbmR6ZW44N2IucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL2xpbmR6ZW44N2IucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Lindzen88,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {R. S. Lindzen and A. Y. Hou},
	File = {../../Papers/lindzen88.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2416--2427},
	Title = {Hadley Circulations for Zonally Averaged Heating Centered off the Equator},
	Volume = 45,
	Year = 1988,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1saW5kemVuODgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHZvdzrBwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvd1bhwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGluZHplbjg4LnBkZgAOABwADQBsAGkAbgBkAHoAZQBuADgAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbGluZHplbjg4LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2xpbmR6ZW44OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Lindzen93,
	Annote = {Filed under Tropopause Dynamics. Baroclinic
                  neutrality via short-wave cutoff in Eady model.},
	Author = {R. S. Lindzen},
	File = {../../Papers/lindzen93.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1148--1151},
	Title = {Baroclinic Neutrality and the Tropopause},
	Volume = 50,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1saW5kemVuOTMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHav1HVplBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv1I4FgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGluZHplbjkzLnBkZgAOABwADQBsAGkAbgBkAHoAZQBuADkAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbGluZHplbjkzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2xpbmR6ZW45My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Linsley00,
	Annote = {Filed under Paleo-Climate Reviews},
	Author = {B. K. Linsley and G. M. Wellington and D. P. Schrag},
	Journal = {Science},
	Pages = {1145--1148},
	Title = {Decadal Sea Surface Temperature Variability in the Subtropical {S}outh {P}acific from 1726 to 1997 A.D.},
	Volume = 290,
	Year = 2000}

@article{Linz84,
	Annote = {Not on file.},
	Author = {P. Linz},
	Journal = {BIT},
	Pages = {92--101},
	Title = {Uncertainty in the solution of linear operator equations},
	Volume = 24,
	Year = 1984}

@book{Little02,
	Address = {New York},
	Author = {R. J. A. Little and D. B. Rubin},
	Edition = {2nd},
	Pages = 381,
	Publisher = {Wiley},
	Series = {Series in Probability and Mathematical Statistics},
	Title = {Statistical Analysis with Missing Data},
	Year = 2002}

@book{Little87,
	Address = {New York},
	Author = {R. J. A. Little and D. B. Rubin},
	Pages = 278,
	Publisher = {Wiley},
	Series = {Series in Probability and Mathematical Statistics},
	Title = {Statistical Analysis with Missing Data},
	Year = 1987}

@article{Liu03,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {Z. Liu and H. Yang},
	File = {../../Papers/liu03.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2002GL016492},
	Pages = 1230,
	Title = {Extratropical control of tropical climate, the atmospheric bridge and oceanic tunnel},
	Volume = 30,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglsaXUwMy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHewHGwxwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwHITNwAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGl1MDMucGRmAA4AFAAJAGwAaQB1ADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvbGl1MDMucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvbGl1MDMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Liu04,
	Annote = {Demonstrate presence of 41kyr cycle in Pleistocene
                  equatorial temperature proxies and infer
                  high-latitude influence on tropical climate.},
	Author = {Z. Liu and T. D. Herbert},
	Journal = {Nature},
	Pages = {720--723},
	Title = {High-latitude influence on the eastern equatorial {P}acific climate in the early {P}leistocene epoch},
	Volume = 427,
	Year = 2004}

@article{Liu08,
	Author = {J. J. Liu and P. M. Goldreich and D. J. Stevenson},
	File = {../../Papers/liu08.pdf},
	Journal = {Icarus},
	Pages = {653--664},
	Title = {Constraints on deep-seated zonal winds inside {Jupiter} and {Saturn}},
	Volume = {196},
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglsaXUwOC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHfxPRACwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxPSiewAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bGl1MDgucGRmAA4AFAAJAGwAaQB1ADAAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvbGl1MDgucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvbGl1MDgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Llewellyn_Smith02,
	Annote = {Linear theory of scattering of barotropic tide at
                  topography. Asymptotic expressions in limit of small
                  topographic slopes. Various idealized examples.},
	Author = {S. G. Llewellyn~Smith and W. R. Young},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1554--1566},
	Title = {Conversion of the Barotropic Tide},
	Volume = 32,
	Year = 2002}

@book{Lodders98,
	Address = {New York},
	Author = {Lodders, K. and Fegley, Jr., B.},
	Pages = 391,
	Publisher = {Oxford University Press},
	Title = {The Planetary Scientist's Companion},
	Year = 1998}

@article{Longuet-Higgins66,
	Author = {M. S. Longuet-Higgins},
	Journal = {Philos. Trans. Roy. Soc. London},
	Pages = {39--50},
	Title = {Planetary waves on a hemisphere bounded by meridians of longitude},
	Volume = 260,
	Year = 1966}

@article{Lopez01,
	Annote = {Filed under Chaotic Advection.},
	Author = {C. L{\'o}pez and Z. Neufeld and E. Hern{\'a}ndez-Garcia and P. H. Haynes},
	Journal = {Phys. Chem. Earth (B)},
	Pages = {313--317},
	Title = {Chaotic Advection of Reacting Substances: Plankton Dynamics on a Meandering Jet},
	Volume = 26,
	Year = 2001}

@article{Lorenz01,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {R. D. Lorenz and J. I. Lunine and P. G. Withers},
	Journal = {Geophys. Res. Lett.},
	Pages = {415--418},
	Title = {Titan, {Mars} and {Earth}: {E}ntropy Production by Latitudinal Heat Transport},
	Volume = 28,
	Year = 2001}

@article{Lorenz07,
	Author = {D. J. Lorenz and E. T. DeWeaver},
	File = {../../Papers/lorenz07.pdf},
	Journal = {J. Geophys. Res.},
	Note = {doi:10.1029/2006JD008087},
	Pages = {D10119},
	Title = {Tropopause height and zonal wind response to global warming in the {IPCC} scenario integrations},
	Volume = 112,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxsb3JlbnowNy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHjxfmBQAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxfnjsAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bG9yZW56MDcucGRmAAAOABoADABsAG8AcgBlAG4AegAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2xvcmVuejA3LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9sb3JlbnowNy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Lorenz07b,
	Author = {D. J. Lorenz and E. T. DeWeaver},
	File = {../../Papers/lorenz07b.pdf},
	Journal = {J. Climate},
	Pages = {3470--3484},
	Title = {The Response of the Extratropical Hydrological Cycle to Global Warming},
	Volume = 20,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1sb3JlbnowN2IucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHkxMfxKwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxMhTmwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bG9yZW56MDdiLnBkZgAOABwADQBsAG8AcgBlAG4AegAwADcAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbG9yZW56MDdiLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL2xvcmVuejA3Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Lorenz55,
	Annote = {Classic paper on the concept of APE. Discusses
                  approximate form for APE and energy cycle in the
                  atmosphere.},
	Author = {E. N. Lorenz},
	File = {../../Papers/lorenz55.pdf},
	Journal = {Tellus},
	Pages = {157--167},
	Title = {Available Potential Energy and the Maintenance of the General Circulation},
	Volume = 7,
	Year = 1955,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxsb3Jlbno1NS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHnwOVSXwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwOW0zwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bG9yZW56NTUucGRmAAAOABoADABsAG8AcgBlAG4AegA1ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2xvcmVuejU1LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9sb3Jlbno1NS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Lorenz60,
	Annote = {Lorenz's two-level model.},
	Author = {E. N. Lorenz},
	Journal = {Tellus},
	Pages = {364--373},
	Title = {Energy and numerical weather prediction},
	Volume = 12,
	Year = 1960}

@article{Lorenz63,
	Annote = {Classic 3-variable model.},
	Author = {E. N. Lorenz},
	File = {../../Papers/lorenz63.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {130--141},
	Title = {Deterministic Nonperiodic Flow},
	Volume = 20,
	Year = 1963,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxsb3Jlbno2My5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHqvAI1SAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvAKlyAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bG9yZW56NjMucGRmAAAOABoADABsAG8AcgBlAG4AegA2ADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2xvcmVuejYzLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9sb3Jlbno2My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Lorenz65,
	Annote = {Not on file. Classic paper on limits of
                  predictability and chaos.},
	Author = {E. N. Lorenz},
	Journal = {Tellus},
	Pages = {321--333},
	Title = {A Study of the Predictability of a 28-variable Atmospheric Model},
	Volume = 17,
	Year = 1965}

@book{Lorenz67,
	Address = {Geneva},
	Author = {E. N. Lorenz},
	Publisher = {World Meteorological Organization},
	Series = {{WMO} Publications},
	Title = {The Nature and Theory of the General Circulation of the Atmosphere},
	Volume = {218},
	Year = {1967}}

@article{Lorenz69a,
	Annote = {.},
	Author = {E. N. Lorenz},
	Journal = {J. Atmos. Sci.},
	Pages = {636--646},
	Title = {Atmospheric Predictability as Revealed by Naturally Occurring Analogues},
	Volume = 26,
	Year = 1969}

@inproceedings{Lorenz69b,
	Address = {London},
	Author = {E. N. Lorenz},
	Booktitle = {The Global Circulation of the Atmosphere},
	Editor = {G. A. Corby},
	Organization = {Royal Meteorological Society},
	Pages = {3--23},
	Title = {The nature of the global circulation of the atmosphere: a present view},
	Year = 1969}

@incollection{Lorenz75,
	Annote = {Filed under Predictability.},
	Author = {E. N. Lorenz},
	Booktitle = {The Physical Basis of Climate and Climate Modelling},
	Editor = {B. Bolin and Coauthors},
	Pages = {132--136},
	Publisher = {World Meteorological Organization},
	Series = {{GARP} Publication Series},
	Title = {Climatic Predictability},
	Volume = 16,
	Year = 1975}

@article{Lorenz78,
	Author = {Lorenz, E. N.},
	Journal = {Tellus},
	Pages = {15--31},
	Title = {Available energy and the maintenance of a moist circulation},
	Volume = {30},
	Year = {1978}}

@article{Lorenz79,
	Author = {Lorenz, E. N.},
	Journal = {Tellus},
	Pages = {230--235},
	Title = {Numerical evaluation of moist available energy},
	Volume = {31},
	Year = {1979}}

@article{Lorenz80,
	Annote = {Introduces 9-variable primitive equation model to
                  study attractor of simplified atmospheric
                  model. Gravity waves, which are initially present in
                  integrations, are damped out after a few days. Model
                  attractor is approximately
                  quasi-geostrophic. Devises algorithm to find states
                  that are free of gravity waves; these states form a
                  three-dimensional stable invariant manifold.},
	Author = {E. N. Lorenz},
	Journal = {J. Atmos. Sci.},
	Pages = {1685--1699},
	Title = {Attractor Sets and Quasi-Geostrophic Equilibrium},
	Volume = 37,
	Year = 1980}

@article{Lorenz83,
	Annote = {Filed under General Circulation History.},
	Author = {E. N. Lorenz},
	File = {../../Papers/lorenz83.pdf},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {730--734},
	Title = {A History of Prevailing Ideas about the General Circulation of the Atmosphere},
	Volume = 64,
	Year = 1983,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxsb3Jlbno4My5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHuvRhMOgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRiuqgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bG9yZW56ODMucGRmAAAOABoADABsAG8AcgBlAG4AegA4ADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2xvcmVuejgzLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9sb3Jlbno4My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Lorenz86,
	Annote = {Slow manifold consists of states free of gravity
                  wave activity. Schemes designed to determine the
                  slow manifold fail to converge. Questions whether
                  the complete absence of gravity waves can be
                  logically defined.},
	Author = {E. N. Lorenz},
	Journal = {J. Atmos. Sci.},
	Pages = {1547--1557},
	Title = {On the Existence of a Slow Manifold},
	Volume = 43,
	Year = 1986}

@article{Lorenz91,
	Annote = {Short history of general circulation research.},
	Author = {E. N. Lorenz},
	File = {../../Papers/lorenz91.pdf},
	Journal = {Tellus},
	Pages = {8--15},
	Title = {The general circulation of the atmosphere: an evolving problem},
	Volume = {43AB},
	Year = 1991,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxsb3Jlbno5MS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHvvRhGQwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRioswAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bG9yZW56OTEucGRmAAAOABoADABsAG8AcgBlAG4AegA5ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2xvcmVuejkxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9sb3Jlbno5MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Lovelock72,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {J. E. Lovelock and R. J. Maggs and R. A. Rasmussen},
	Journal = {Nature},
	Pages = 452,
	Title = {Atmospheric Dimethyl Sulphide and the Natural Sulphur Cycle},
	Volume = 237,
	Year = 1972}

@article{Lovelock77,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {J. E. Lovelock},
	Journal = {Nature},
	Pages = 32,
	Title = {Methyl chloroform in the troposphere as an indicator of {OH} radical abundance},
	Volume = 267,
	Year = 1977}

@article{Loyning97,
	Author = {T. B. L{\o}yning and J. E. Weber},
	Journal = {J. Geophys. Res.},
	Pages = {27875--27885},
	Title = {Thermobaric effect on buoyancy-driven convection in cold seawater},
	Volume = {102C},
	Year = 1997}

@article{Lu07,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {J. Lu and G. A. Vecchi and T. Reichler},
	File = {../../Papers/lu07.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2006GL028443},
	Pages = {L06805},
	Title = {Expansion of the {H}adley cell under global warming},
	Volume = 34,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfghsdTA3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRHxwjAmpgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwjCJFgAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bHUwNy5wZGYAAA4AEgAIAGwAdQAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL2x1MDcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL2x1MDcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@article{Lu98,
	Author = {P. Lu and J. P. {McCreary, Jr.} and B. A. Klinger},
	File = {../../Papers/lu98.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {62--84},
	Title = {Meridional Circulation Cells and the Source Waters of the {Pacific} Equatorial Undercurrent},
	Volume = {28},
	Year = {1998},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfghsdTk4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRH0xeUFbgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxeVn3gAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bHU5OC5wZGYAAA4AEgAIAGwAdQA5ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL2x1OTgucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL2x1OTgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@article{Luetkepohl85,
	Annote = {Filed under AR Modeling. Tests a variety of order
                  selection criteria using different low-dimensional,
                  low-order AR processes. Schwarz' BC performs best.},
	Author = {H. L{\"u}tkepohl},
	Journal = {J. Time Ser. Anal.},
	Note = {Correction, {\bf 8} (1987), 373.},
	Pages = {35--52},
	Title = {Comparison of Criteria for Estimating the Order of a Vector Autoregressive Process},
	Volume = 6,
	Year = 1985}

@book{Luetkepohl93,
	Address = {Berlin},
	Annote = {Xerox filed under AR Modeling.},
	Author = {H. L{\"u}tkepohl},
	Edition = {2nd},
	Pages = 545,
	Publisher = {Springer-Verlag},
	Title = {Introduction to Multiple Time Series Analysis},
	Year = 1993}

@article{Lukas93,
	Annote = {Not on file.},
	Author = {M. A. Lukas},
	Journal = {Numer. Math.},
	Pages = {41--66},
	Title = {Asymptotic optimality of generalized cross-validation for choosing the regularization parameter},
	Volume = 66,
	Year = 1993}

@article{Luo04a,
	Author = {Z. Luo and W. B. Rossow},
	Date-Modified = {2010-06-11 16:44:04 -0700},
	File = {../../Papers/luo04.pdf},
	Journal = {J. Climate},
	Pages = {4541--4563},
	Title = {Characterizing Tropical Cirrus Life Cycle, Evolution, and Interaction with Upper-Tropospheric Water Vapor Using {L}agrangian Trajectory Analysis of Satellite Observations},
	Volume = 17,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpsdW8wNGEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRH3yDgYKgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyDh6mgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bHVvMDRhLnBkZgAADgAWAAoAbAB1AG8AMAA0AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL2x1bzA0YS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvbHVvMDRhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Luo98,
	Annote = {Filed under Imputation of Missing Values.},
	Author = {Z. Luo and G. Wahba and D. R. Johnson},
	Journal = {J. Climate},
	Pages = {18--28},
	Title = {Spatial-temporal analysis of temperature using smoothing spline {ANOVA}},
	Volume = 11,
	Year = 1998}

@article{Luyten83,
	Author = {J. R. Luyten and J. Pedlosky and H. Stommel},
	Journal = {J. Phys. Oceanogr.},
	Pages = {292--309},
	Title = {The Ventilated Thermocline},
	Volume = {13},
	Year = {1983}}

@article{Madden76,
	Annote = {Filed under Predictability.},
	Author = {R. A. Madden},
	Journal = {Mon. Wea. Rev.},
	Pages = {942--952},
	Title = {Estimates of the Natural Variability of Time-Averaged Sea-Level Pressure},
	Volume = 104,
	Year = 1976}

@article{Madden94,
	Author = {Madden, R. A. and Julian, P. R.},
	File = {../../Papers/madden94.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {814--837},
	Title = {Observations of the 40--50-day tropical oscillation---{A} review},
	Volume = 122,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxtYWRkZW45NC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRH6wS4AzFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwS5jPAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFkZGVuOTQucGRmAAAOABoADABtAGEAZABkAGUAbgA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL21hZGRlbjk0LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9tYWRkZW45NC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Magalhaes02,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {J. A. Magalh{\~a}es and A. Seiff and R. E. Young},
	File = {../../Papers/magalhaes02.pdf},
	Journal = {Icarus},
	Pages = {410--433},
	Title = {The Stratification of {J}upiter's Troposphere at the {Galileo} Probe Entry Site},
	Volume = 158,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9tYWdhbGhhZXMwMi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRH7w7ZvVgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7bf1gAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFnYWxoYWVzMDIucGRmAA4AIAAPAG0AYQBnAGEAbABoAGEAZQBzADAAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbWFnYWxoYWVzMDIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbWFnYWxoYWVzMDIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Magalhaes89,
	Author = {Magalh{\~a}es, J. A. and Weir, A. L. and Conrath, B. J. and Gierasch, P. J. and Leroy, S. S.},
	File = {../../Papers/magalhaes89.pdf},
	Journal = {Nature},
	Pages = {444--447},
	Title = {Slowly moving thermal features on {Jupiter}},
	Volume = {337},
	Year = {1989},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9tYWdhbGhhZXM4OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRH8xJlZfQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxJm77QAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFnYWxoYWVzODkucGRmAA4AIAAPAG0AYQBnAGEAbABoAGEAZQBzADgAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbWFnYWxoYWVzODkucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbWFnYWxoYWVzODkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Magnusdottir00,
	Author = {G. Magnusdottir and C. Walker},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {2725--2745},
	Title = {On the effects of the {Hadley} circulation and westerly equatorial flow on planetary-wave reflection},
	Volume = 126,
	Year = 2000}

@article{Magnusdottir96,
	Author = {G. Magnusdottir and P. H. Haynes},
	Journal = {J. Atmos. Sci.},
	Pages = {2317--2353},
	Title = {Wave Activity Diagnostics Applied to Barolinic Wave Life Cycles},
	Volume = 53,
	Year = 1996}

@article{Magnusdottir99,
	Annote = {Changes in latent heat transport go hand in hand
                  with changes in dry static energy of opposite sign.},
	Author = {G. Magnusdottir and R. Saravanan},
	Journal = {Tellus},
	Pages = {815--832},
	Title = {The response of atmospheric heat transport to zonally-averaged {SST} trends},
	Volume = {51A},
	Year = 1999}

@incollection{Mahlman92,
	Author = {J. D. Mahlman},
	Booktitle = {Climate Change and Energy Policy},
	Editor = {L. Rosen and R. Glasser},
	Publisher = {American Institute of Physics},
	Title = {Assessing Global Climate Change: When Will We Have Better Evidence},
	Year = 1992}

@article{Mahlman97a,
	Annote = {Review of stratosphere-troposphere exchange etc.},
	Author = {J. D. Mahlman},
	Journal = {Science},
	Pages = {1079--1083},
	Title = {Dynamics of Transport Processes in the Upper Troposphere},
	Volume = 276,
	Year = 1997}

@article{Mahlman97b,
	Annote = {Review of climate change issues before the Kyoto
                  summit.},
	Author = {J. D. Mahlman},
	Journal = {Science},
	Pages = {1416--1417},
	Title = {Uncertainties in Projections of Human-Caused Climate Warming},
	Volume = 278,
	Year = 1997}

@article{Mahlman98,
	Annote = {Jerry's personal view of the global warming debate.},
	Author = {J. D. Mahlman},
	File = {../../Papers/mahlman98.pdf},
	Journal = {Annu. Rev. Energy Environ.},
	Pages = {83--105},
	Title = {Science and Nonscience Concerning Human-Caused Climate Warming},
	Volume = 23,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1tYWhsbWFuOTgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRH9vJAdnQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvJCOHQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFobG1hbjk4LnBkZgAOABwADQBtAGEAaABsAG0AYQBuADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbWFobG1hbjk4LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL21haGxtYW45OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Majda01a,
	Annote = {Linear analysis of convection parameterization
                  schemes. Artificial waves in Lagrangian particle
                  adjustment scheme.},
	Author = {A. J. Majda and M. G. Shefter},
	Journal = {J. Atmos. Sci.},
	Pages = {896--914},
	Title = {Waves and Instabilities for Model Tropical Convective Parameterizations},
	Volume = 58,
	Year = 2001}

@article{Majda01b,
	Author = {A. J. Majda and M. G. Shefter},
	Journal = {J. Atmos. Sci.},
	Pages = {1567--1584},
	Title = {Models for Stratiform Instability and Convectively Coupled Waves},
	Volume = 58,
	Year = 2001}

@article{Majda02,
	Author = {A. Majda and I. Timofeyev and E. Vanden-Eijnden},
	Journal = {Physica D},
	Pages = {206--252},
	Title = {A priori test of a stochastic mode reduction strategy},
	Volume = 170,
	Year = 2002}

@article{Majda03a,
	Author = {A. Majda and R. Klein},
	Journal = {J. Atmos. Sci.},
	Pages = {393--408},
	Title = {Systematic Multiscale Models for the {T}ropics},
	Volume = 60,
	Year = 2003}

@article{Majda03b,
	Author = {A. J. Majda and I. Timofeyev and E. Vanden-Eijnden},
	Journal = {J. Atmos. Sci.},
	Pages = {1705--1722},
	Title = {Systematic Strategies for Stochastic Mode Reduction in Climate},
	Volume = 60,
	Year = 2003}

@article{Majda04,
	Annote = {MJO theory.},
	Author = {A. J. Majda and J. A. Biello},
	Journal = {Proc. Nat. Acad. Sci.},
	Pages = {4736--4741},
	Title = {A multiscale model for tropical interseasonal oscillations},
	Volume = 101,
	Year = 2004}

@article{Majda97a,
	Annote = {Theory of weak turbulence.},
	Author = {A. J. Majda and D. W. McLaughlin and E. G. Tabak},
	Journal = {J. Nonlinear Sci.},
	Pages = {9--44},
	Title = {A One-Dimensional Model for Dispersive Wave Turbulence},
	Volume = 6,
	Year = 1997}

@unpublished{Majda97b,
	Annote = {Proceedings of NCAR Workshop on Rotating Stratified
                  Turbulence},
	Author = {A. J. Majda and P. Embid},
	Note = {Preprint},
	Title = {Averaging over Fast Gravity Waves for Geophysical Flows with Unbalanced Inital Data},
	Year = 1997}

@article{Mak82,
	Author = {M. Mak},
	File = {../../Papers/mak82.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2028--2037},
	Title = {On Moist Quasigeostrophic Baroclinic Instability},
	Volume = 39,
	Year = 1982,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgltYWs4Mi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIAvrdatAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvre9JAAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFrODIucGRmAA4AFAAJAG0AYQBrADgAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvbWFrODIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvbWFrODIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Maloney98,
	Author = {Maloney, E. D. and Hartmann, D. L.},
	File = {../../Papers/maloney98.pdf},
	Journal = {J. Climate},
	Pages = {2387--2403},
	Title = {Frictional Moisture Convergence in a Composite Life Cycle of the {M}adden--{J}ulian Oscillation},
	Volume = 11,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1tYWxvbmV5OTgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRICwS37+FBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwS5eaAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFsb25leTk4LnBkZgAOABwADQBtAGEAbABvAG4AZQB5ADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbWFsb25leTk4LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL21hbG9uZXk5OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Manabe64,
	Author = {S. Manabe and R. F. Strickler},
	Journal = {J. Atmos. Sci.},
	Pages = {361--385},
	Title = {Thermal Equilibrium of the Atmosphere with a Convective Adjustment},
	Volume = 21,
	Year = 1964}

@article{Manabe65,
	Author = {S. Manabe and J. Smagorinsky and R. F. Strickler},
	Journal = {Mon. Wea. Rev.},
	Pages = {769--798},
	Title = {Simulated Climatology of a General Circulation Model with a Hydrologic Cycle},
	Volume = 93,
	Year = 1965}

@article{Manabe67,
	Annote = {Compute radiative-convective equilibrium of the
                  atmosphere and sensitivity of surface temperature to
                  changes in external forcing, such as CO_2 doubling.},
	Author = {S. Manabe and R. T. Wetherald},
	File = {../../Papers/manabe67.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {241--259},
	Title = {Thermal Equilibrium of the Atmosphere with a Given Distribution of Relative Humidity},
	Volume = 24,
	Year = 1967,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxtYW5hYmU2Ny5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIEw1s/pVBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw1uwJQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFuYWJlNjcucGRmAAAOABoADABtAGEAbgBhAGIAZQA2ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL21hbmFiZTY3LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9tYW5hYmU2Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Manabe85,
	Author = {S. Manabe and A. J. Broccoli},
	File = {../../Papers/manabe85.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {2167--2190},
	Title = {The Influence of Continental Ice Sheets on the Climate of an {I}ce {A}ge},
	Volume = {90D},
	Year = 1985,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxtYW5hYmU4NS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIGwdWk7wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwdYVbwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFuYWJlODUucGRmAAAOABoADABtAGEAbgBhAGIAZQA4ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL21hbmFiZTg1LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9tYW5hYmU4NS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Manabe91,
	Annote = {Not on file.},
	Author = {S. Manabe and R. J. Stouffer and M. J. Spelman and K. Bryan},
	Journal = {J. Climate},
	Pages = {785--818},
	Title = {Transient Response of a Coupled Ocean-Atmosphere Model to Gradual Changes of Atmospheric $\mbox{CO}_2$. {P}art {I}: {A}nnual Mean Response},
	Volume = 4,
	Year = 1991}

@article{Manabe93,
	Author = {S. Manabe and R. J. Stouffer},
	Journal = {Nature},
	Pages = {215--218},
	Title = {Century-Scale Effects of Increased Atmospheric {$\rm CO_2$} on the Ocean-Atmosphere System},
	Volume = 364,
	Year = 1993}

@article{Manabe94,
	Author = {S. Manabe and R. J. Stouffer},
	Journal = {J. Climate},
	Pages = {5--23},
	Title = {Multiple-Century Response of a Coupled Ocean-Atmosphere Model to an Increase of Atmospheric Carbon Dioxide},
	Volume = 7,
	Year = 1994}

@article{Manabe96,
	Annote = {Not on file.},
	Author = {S. Manabe and R. J. Stouffer},
	Journal = {J. Climate},
	Pages = {376--393},
	Title = {Low-frequency variability of surface air temperature in a 1000-year integration of a coupled atmosphere-ocean-land surface model},
	Volume = 9,
	Year = 1996}

@article{Mann95,
	Author = {M. E. Mann and J. Park and R. S. Bradley},
	Journal = {Nature},
	Pages = {266-270},
	Title = {Global interdecadal and century-scale climate oscillations during the past five centuries},
	Volume = 378,
	Year = 1995}

@article{Mann96,
	Author = {M. E. Mann and J. M. Lees},
	Journal = {Climatic Change},
	Pages = {409--445},
	Title = {Robust estimation of background noise and signal detection in climatic time series},
	Volume = 33,
	Year = 1996}

@article{Mann98,
	Annote = {Filed under Mann.},
	Author = {M. E. Mann and R. S. Bradley and M. K. Hughes},
	Journal = {Nature},
	Pages = {779--787},
	Title = {Global-scale temperature patterns and climate forcing over the past centuries},
	Volume = 392,
	Year = 1998}

@article{Mann99,
	Annote = {Not on file.},
	Author = {M. E. Mann and R. S. Bradley and M. K. Hughes},
	Journal = {Geophys. Res. Lett.},
	Pages = {759--762},
	Title = {Northern hemisphere temperatures during the past millennium: Inferences, uncertainties, and limitations},
	Volume = 26,
	Year = 1999}

@article{Mapes01,
	Author = {B. E. Mapes},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {2353--2366},
	Title = {Water's two height scales: The moist adiabat and the radiative troposphere},
	Volume = 127,
	Year = 2001}

@article{Mapes05,
	Annote = {Monsoon delayed by a about a month compared with
                  equilibrium response to seasonal forcing},
	Author = {Mapes, B. E. and Liu, P. and Buenning, N.},
	File = {../../Papers/mapes05.pdf},
	Journal = {J. Climate},
	Pages = {1109--1115},
	Title = {Indian Monsoon Onset and the {A}mericas Midsummer Drought: Out-of-Equilibrium Responses to Smooth Seasonal Forcing},
	Volume = 18,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgttYXBlczA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRINwR5YmlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwR67CgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFwZXMwNS5wZGYADgAYAAsAbQBhAHAAZQBzADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvbWFwZXMwNS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9tYXBlczA1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Mapes96,
	Annote = {Not on file. Hypothesize that radiatively-driven
                  subsidence (over timescale of a few days) is
                  responsible for generation of dry tongues. Simpler
                  explanation (lateral displacement with moistening of
                  boundary layer from below) given by Cau05.},
	Author = {B. Mapes and P. Zuidema},
	File = {../../Papers/mapes96.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {620--638},
	Title = {Radiative-Dynamical Consequences of Dry Tongues in the Tropical Troposphere},
	Volume = 53,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgttYXBlczk2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIOv3VicQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3XE4QAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFwZXM5Ni5wZGYADgAYAAsAbQBhAHAAZQBzADkANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvbWFwZXM5Ni5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9tYXBlczk2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@book{Mardia79,
	Address = {San Diego, CA},
	Author = {K. V. Mardia and J. T. Kent and J. M. Bibby},
	Pages = 518,
	Publisher = {Academic Press},
	Series = {Series in Probability and Mathematical Statistics},
	Title = {Multivariate Analysis},
	Year = 1979}

@article{Marquardt70,
	Annote = {Not on file. Classic paper on ridge regression.},
	Author = {D. W. Marquardt},
	Journal = {Technometrics},
	Pages = {591--612},
	Title = {Generalized inverses, ridge regression, biased linear estimation, and nonlinear estimation},
	Volume = 12,
	Year = 1970}

@article{Marquet95,
	Annote = {Filed under Available Potential Energy. Relation
                  between APE and exergy.},
	Author = {P. Marquet},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {455--459},
	Title = {On the concept of pseudo-energy of {T.\ G.\ Shepherd}},
	Volume = 121,
	Year = 1995}

@article{Marsden01a,
	Author = {J. E. Marsden and M. West},
	Journal = {Acta Numerica},
	Pages = {357--514},
	Title = {Discrete Mechanics and Variational Integrators},
	Volume = 10,
	Year = 2001}

@article{Marsden01b,
	Author = {J. E. Marsden and S. Shkoller},
	Journal = {Phil. Trans. R. Soc. Lond. A},
	Pages = {1449--1468},
	Title = {Global well-posedness for the {L}agrangian averaged {N}avier-{S}tokes ({LANS-$\alpha$}) equations on bounded domains},
	Volume = 359,
	Year = 2001}

@incollection{Marsden99,
	Author = {J. E. Marsden},
	Booktitle = {???},
	Pages = {337--430},
	Publisher = {American Mathematical Society},
	Series = {{IAS}/{P}ark {C}ity Mathematics Series},
	Title = {{P}ark {C}ity Lectures on Mechanics, Dynamics, and Symmetry},
	Volume = 7,
	Year = 1999}

@article{Marshall00,
	Author = {D. P. Marshall},
	Journal = {J. Phys. Oceanogr.},
	Pages = {3102--3112},
	Title = {Vertical Fluxes of Potential Vorticity and the Structure of the Thermocline},
	Volume = 30,
	Year = 2000}

@article{Marshall01a,
	Annote = {Uses Bernoulli theorem of Schaer93 to diagnose PV
                  fluxes.},
	Author = {J. Marshall and D. Jamous and J. Nilsson},
	Journal = {J. Phys. Oceanogr.},
	Pages = {777--789},
	Title = {Entry, Flux, and Exit of Potential Vorticity in Ocean Circulation},
	Volume = 31,
	Year = 2001}

@article{Marshall01b,
	Author = {J. Marshall and H. Johnson and J. Goodman},
	Journal = {J. Climate},
	Pages = {1399--1421},
	Title = {A study of the interaction of the {N}orth {A}tlantic {O}scillation with ocean circulation},
	Volume = 14,
	Year = 2001}

@article{Marshall01c,
	Annote = {Review of NAO phenomenology.},
	Author = {J. Marshall and Y. Kushnir and D. Battisti and P. Chang and A. Czaja and R. Dickson and J. Hurrell and M. McCartney and R. Saravanan and M. Visbeck},
	Journal = {Int. J. Climatology},
	Pages = {1863--1898},
	Title = {North {A}tlantic Climate Variability: {P}henomena, impacts and mechanisms},
	Volume = 21,
	Year = 2001}

@article{Marshall02,
	Author = {J. Marshall and H. Jones and R. Karsten and R. Wardle},
	Journal = {J. Phys. Oceanogr.},
	Pages = {26--38},
	Title = {Can eddies set ocean stratification?},
	Volume = 32,
	Year = 2002}

@article{Marshall07,
	Author = {J. Marshall and D. Ferreira and J.-M. Campin and D. Enderton},
	File = {../../Papers/marshall07.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {4270--4286},
	Title = {Mean Climate and Variablity of the Atmosphere and Ocean on an Aquaplanet},
	Volume = 64,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5tYXJzaGFsbDA3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIUw60aOQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw62KuQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFyc2hhbGwwNy5wZGYAAA4AHgAOAG0AYQByAHMAaABhAGwAbAAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL21hcnNoYWxsMDcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL21hcnNoYWxsMDcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Marshall85,
	Annote = {Filed under Ornstein-Uhlenbeck
                  Processes. First-passage times.},
	Author = {T. W. Marshall and E. J. Watson},
	Journal = {J. Phys. A: Math. Gen.},
	Pages = {3531--3559},
	Title = {A drop of ink falls from my pen \dots {It} comes to earth, I know not when},
	Volume = 18,
	Year = 1985}

@article{Marshall92,
	Author = {J. C. Marshall and A. J. G. Nurser},
	Journal = {J. Phys. Oceanogr.},
	Pages = {583--595},
	Title = {Fluid Dynamics of Oceanic Thermocline Ventilation},
	Volume = 22,
	Year = 1992}

@article{Marshall97,
	Author = {D. Marshall},
	Journal = {J. Mar. Res.},
	Pages = {201--222},
	Title = {Subduction of Water Masses in an Eddying Ocean},
	Volume = 55,
	Year = 1997}

@article{Marston08a,
	Author = {J. B. Marston and E. Conover and T. Schneider},
	Date-Modified = {2010-06-11 12:15:10 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {1955--1966},
	Title = {Statistics of an unstable barotropic jet from a cumulant expansion},
	Volume = {65},
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5tYXJzdG9uMDhhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIVxHKxqwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxHMUGwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFyc3RvbjA4YS5wZGYAAA4AHgAOAG0AYQByAHMAdABvAG4AMAA4AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL21hcnN0b24wOGEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL21hcnN0b24wOGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Maslowe86,
	Author = {S. A. Maslowe},
	File = {../../Papers/maslowe86.pdf},
	Journal = {Ann. Rev. Fluid Mech.},
	Pages = {405--432},
	Title = {Critical layers in shear flows},
	Volume = 18,
	Year = 1986,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1tYXNsb3dlODYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIWwjqJogAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwjrsEgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWFzbG93ZTg2LnBkZgAOABwADQBtAGEAcwBsAG8AdwBlADgANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbWFzbG93ZTg2LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL21hc2xvd2U4Ni5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Matsuno66,
	Author = {Matsuno, T.},
	File = {../../Papers/matsuno66.pdf},
	Journal = {J. Meteor. Soc. Japan},
	Pages = {25--42},
	Title = {Quasi-geostrophic motions in the equatorial area},
	Volume = {44},
	Year = {1966},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1tYXRzdW5vNjYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIXxGW/SwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxGYhuwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWF0c3VubzY2LnBkZgAOABwADQBtAGEAdABzAHUAbgBvADYANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbWF0c3VubzY2LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL21hdHN1bm82Ni5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Matsuno71,
	Annote = {Wave--mean flow interaction responsible for breakup
                  of stratospheric polar vortex and sudden warming.},
	Author = {T. Matsuno},
	Journal = {J. Atmos. Sci.},
	Pages = {1479--1494},
	Title = {A Dynamical Model of the Stratospheric Sudden Warming},
	Volume = 28,
	Year = 1971}

@article{Maurizi05,
	Annote = {Filed under Stochastic Lagrangian Models of Turbulence.},
	Author = {A. Maurizi and G. Pagnini and F. Tampieri},
	File = {../../Papers/maurizi05.pdf},
	Journal = {???},
	Pages = {???},
	Title = {The dependence of relative dispersion on turbulence scales in {L}agrangian stochastic models},
	Volume = {???},
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1tYXVyaXppMDUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIZv5GVaVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5IF6QAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWF1cml6aTA1LnBkZgAOABwADQBtAGEAdQByAGkAegBpADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbWF1cml6aTA1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL21hdXJpemkwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@book{McComb90,
	Address = {Oxford, UK},
	Author = {W. D. McComb},
	Pages = 572,
	Publisher = {Clarendon Press},
	Series = {Oxford Engineering Science Series},
	Title = {The Physics of Fluid Turbulence},
	Volume = 25,
	Year = 1990}

@article{McComb95,
	Annote = {Filed under Turbulence Closure Theories. Review of
                  renormalization group methods.},
	Author = {W. D. McComb},
	Journal = {Rep. Prog. Phys.},
	Pages = {1117--1206},
	Title = {Theory of Turbulence},
	Volume = 58,
	Year = 1995}

@article{McCreary91,
	Annote = {Filed under Anderson.},
	Author = {J. P. {McCreary, Jr.} and D. L. T. Anderson},
	Journal = {J. Geophys. Res.},
	Pages = {3125--3150},
	Title = {An Overview of Coupled Ocean-Atmosphere Models of {E}l {N}i{\~n}o and the {S}outhern {O}scillation},
	Volume = {96 {\rm Supplement}},
	Year = 1991}

@article{McCreary94,
	Author = {J. P. {McCreary, Jr.} and P. Lu},
	File = {../../Papers/mccreary94.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {466--497},
	Title = {Interaction between the Subtropical and Equatorial Ocean Circulations: The Subtropical Cell},
	Volume = {24},
	Year = {1994},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5tY2NyZWFyeTk0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIcxeSeXgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxeUAzgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWNjcmVhcnk5NC5wZGYAAA4AHgAOAG0AYwBjAHIAZQBhAHIAeQA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL21jY3JlYXJ5OTQucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL21jY3JlYXJ5OTQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@book{McCullagh89,
	Address = {London},
	Author = {P. McCullagh and J.~A. Nelder},
	Edition = {2nd},
	Publisher = {Chapman \& Hall},
	Title = {Generalized Linear Models},
	Year = 1989}

@article{McDougall01,
	Annote = {Part 2 of 2: see McDougall96},
	Author = {T. J. McDougall and P. C. McIntosh},
	File = {../../Papers/mcdougall01.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1222--1246},
	Title = {The temporal-residual-mean velocity. {P}art {II}: Isopycnal Interpretation and the Tracer and Momentum Equations},
	Volume = 31,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9tY2RvdWdhbGwwMS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIdvk6d9QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvk8OdQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWNkb3VnYWxsMDEucGRmAA4AIAAPAG0AYwBkAG8AdQBnAGEAbABsADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbWNkb3VnYWxsMDEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbWNkb3VnYWxsMDEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{McDougall88,
	Annote = {Review of neutral surfaces. PV conservation with
                  saline and thermal effects in equation of state.},
	Author = {T. J. McDougall},
	Journal = {Prog. Oceanogr.},
	Pages = {185--221},
	Title = {Neutral-surface potential vorticity},
	Volume = 20,
	Year = 1988}

@article{McDougall96,
	Annote = {Part 1 of 2: see McDougall01.},
	Author = {T. J. McDougall and P. C. McIntosh},
	File = {../../Papers/mcdougall96.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {2653--2665},
	Title = {The temporal-residual-mean velocity. {P}art {I}: {D}erivation and the scalar conservation equations},
	Volume = 26,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9tY2RvdWdhbGw5Ni5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIevk6deAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvk8N+AAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWNkb3VnYWxsOTYucGRmAA4AIAAPAG0AYwBkAG8AdQBnAGEAbABsADkANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbWNkb3VnYWxsOTYucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbWNkb3VnYWxsOTYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{McElroy86,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {M. B. {McElroy} and R. J. Salawitch and S. C. Wofsy and J. A. Logan},
	Journal = {Nature},
	Pages = {759--762},
	Title = {Reductions of {A}ntarctic ozone due to synergistic interactions of chlorine and bromine},
	Volume = 321,
	Year = 1986}

@article{McIntosh96,
	Annote = {Filed under McDougall. See also McDougall96.},
	Author = {P. C. McIntosh and T. J. McDougall},
	File = {../../Papers/mcintosh96.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1655--1660},
	Title = {Isopycnal averaging and the residual mean circulation},
	Volume = 26,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5tY2ludG9zaDk2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIgvk6dpQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvk8OJQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWNpbnRvc2g5Ni5wZGYAAA4AHgAOAG0AYwBpAG4AdABvAHMAaAA5ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL21jaW50b3NoOTYucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL21jaW50b3NoOTYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{McIntyre00,
	Author = {M. E. McIntyre and W. A. Norton},
	Journal = {J. Atmos. Sci.},
	Pages = {1214--1235},
	Title = {Potential Vorticity Inversion on a Hemisphere},
	Volume = 57,
	Year = 2000}

@article{McIntyre80b,
	Author = {McIntyre, ME},
	File = {../../Papers/mcintyre80b.pdf},
	Journal = {Pure Appl. Geophys.},
	Pages = {152--176},
	Title = {An introduction to the generalized {L}agrangian-mean description of wave, mean-flow interaction},
	Volume = {118},
	Year = {1980},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9tY2ludHlyZTgwYi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIixGmIOAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxGnqqAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWNpbnR5cmU4MGIucGRmAA4AIAAPAG0AYwBpAG4AdAB5AHIAZQA4ADAAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbWNpbnR5cmU4MGIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbWNpbnR5cmU4MGIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{McIntyre82,
	Author = {McIntyre, M. E.},
	File = {../../Papers/mcintyre82_part1.pdf},
	Journal = {J. Meteor. Soc. Japan},
	Pages = {37--65},
	Title = {How well do we understand the dynamics of stratospheric warmings?},
	Volume = {60},
	Year = {1982},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYYAAAAAAYYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhRtY2ludHlyZTgyX3BhcnQxLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIjxMVIdwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxMWq5wAAAAEADAAJDH4ACE6zAACS8wACADNNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWNpbnR5cmU4Ml9wYXJ0MS5wZGYAAA4AKgAUAG0AYwBpAG4AdAB5AHIAZQA4ADIAXwBwAGEAcgB0ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAnVXNlcnMvdGFwaW8vUGFwZXJzL21jaW50eXJlODJfcGFydDEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAhLi4vLi4vUGFwZXJzL21jaW50eXJlODJfcGFydDEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAioCLAIxAjoCRQJJAlcCXgJnAosCkAKTAqACpQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAK3}}

@article{McIntyre83,
	Author = {M. E. {McIntyre} and T. N. Palmer},
	Journal = {Nature},
	Pages = {593--600},
	Title = {Breaking planetary waves in the stratosphere},
	Volume = 305,
	Year = 1983}

@article{McIntyre87,
	Author = {M. E. McIntyre and T. G. Shepherd},
	Journal = {J. Fluid Mech.},
	Pages = {527--565},
	Title = {An exact local conservation theorem for finite-amplitude disturbances to non-parallel shear flows, with remarks on {Hamiltonian} structure and on {Arnol'd}'s stability theorems},
	Volume = 181,
	Year = 1987}

@inproceedings{McIntyre92,
	Author = {M. E. McIntyre},
	Booktitle = {Proc. Int. School Phys. ``Enrico Fermi''},
	Editor = {J. C. Gille and G. Visconti},
	Pages = {313--386},
	Publisher = {North-Holland},
	Title = {Atmospheric Dynamics: Some Fundamentals, with Observational Implications},
	Year = 1992}

@book{McLachlan92,
	Address = {New York},
	Author = {G. J. McLachlan},
	Pages = 544,
	Publisher = {Wiley},
	Series = {Series in Probability and Mathematical Statistics},
	Title = {Discriminant Analysis and Statistical Pattern Recognition},
	Year = 1992}

@article{McPhaden02,
	Annote = {Slowdown of overturning circulation is speculated to
                  have led to decrease in upwelling and warming of
                  equatorial Pacific.},
	Author = {M. J. McPhaden and D. Zhang},
	Journal = {Nature},
	Pages = {603--608},
	Title = {Slowdown of the meridional overturning circulation in the upper {P}acific {O}cean},
	Volume = 415,
	Year = 2002}

@article{McWilliams06,
	Author = {McWilliams, J. C.},
	Journal = {J. Fluid Mech.},
	Pages = {21--43},
	Title = {The emergence of isolated coherent vortices in turbulent flow},
	Volume = {146},
	Year = {2006}}

@article{McWilliams84,
	Author = {J. C. McWilliams},
	File = {../../Papers/mcwilliams84.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {21--43},
	Title = {The emergence of isolated coherent vortices},
	Volume = 146,
	Year = 1984,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBtY3dpbGxpYW1zODQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRInxlgYCwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxlh6ewAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWN3aWxsaWFtczg0LnBkZgAADgAiABAAbQBjAHcAaQBsAGwAaQBhAG0AcwA4ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL21jd2lsbGlhbXM4NC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvbWN3aWxsaWFtczg0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Mccabe01,
	Author = {McCabe, G.J. and Clark, M.P. and Serreze, M.C.},
	File = {../../Papers/mccabe01.pdf},
	Journal = {J. Climate},
	Pages = {2763--2768},
	Title = {Trends in Northern Hemisphere Surface Cyclone Frequency and Intensity},
	Volume = {14},
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxtY2NhYmUwMS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIbxAbgDwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxAdCfwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWNjYWJlMDEucGRmAAAOABoADABtAGMAYwBhAGIAZQAwADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL21jY2FiZTAxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9tY2NhYmUwMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@incollection{Meehl07,
	Address = {Cambridge, UK, and New York, NY, USA},
	Author = {G. A. Meehl and T. F. Stocker and W. D. Collins and P. Friedlingstein and A. T. Gaye and J. M. Gregory and A. Kitoh and R. Knutti and J. M. Murphy and A. Noda and S. C. B. Raper and I. G. Watterson and A. J. Weaver and Z.-C. Zhao},
	Booktitle = {Climate Change 2007: The Physical Science Basis. Contribution of Working Group I to the Fourth Assessment Report of the Intergovernmental Panel on Climate Change},
	Editor = {S. Solomon and D. Qin and M. Manning and Z. Chen and M. Marquis and K.B. Averyt and M. Tignor and H.L. Miller},
	Pages = {747--845},
	Publisher = {Cambridge Univ. Press},
	Title = {Global Climate Projections},
	Year = 2007}

@article{Mentz98,
	Annote = {Filed under AR modeling. Bias in LS estimates is
                  smaller than bias in Yule-Walker estimates. YW may
                  be poor when process has roots close to unity. Give
                  asymptotic formulas for bias.},
	Author = {R. P. Mentz and P. A. Morettin and C. M. C. Toloi},
	Journal = {J. Time Series Anal.},
	Pages = {187--208},
	Title = {On residual variance estimation in autoregressive models},
	Volume = 19,
	Year = 1998}

@article{Merlis09a,
	Author = {T. M. Merlis and T. Schneider},
	Date-Modified = {2010-06-11 12:14:45 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {1821--1833},
	Title = {Scales of linear baroclinic instability and macroturbulence in dry atmospheres},
	Volume = 66,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1tZXJsaXMwOWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIsxmS/rAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxmUiHAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWVybGlzMDlhLnBkZgAOABwADQBtAGUAcgBsAGkAcwAwADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbWVybGlzMDlhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL21lcmxpczA5YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Merlis10,
	Author = {T. M. Merlis and T. Schneider},
	Journal = {J. Adv. Model. Earth Sys.},
	Note = {doi:10.3894/JAMES.2009.?.??. Submitted.},
	Pages = {Art. \#xx, xx pp.},
	Title = {Atmospheric dynamics of Earth-like tidally locked aquaplanets},
	Volume = 2,
	Year = 2010}

@article{Merryfield01,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow. Statistical mechanics without prior
                  distribution. Gives linear relationship between
                  streamfunction and potential vorticity.},
	Author = {W. J. Merryfield and P. F. Cummins and G. Holloway},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1880--1890},
	Title = {Equilibrium Statistical Mechanics of Barotropic Flow over Finite Topography},
	Volume = 31,
	Year = 2001}

@article{Merryfield98,
	Author = {W. J. Merryfield},
	Journal = {J. Fluid Mech.},
	Pages = {345--356},
	Title = {Effects of stratification on quasi-geostrophic inviscid equilibria},
	Volume = 354,
	Year = 1998}

@article{Meyers93,
	Annote = {Filed under Wavelets.},
	Author = {S. D. Meyers and B. G. Kelly and J. J. {O'Brien}},
	Journal = {Mon. Wea. Rev.},
	Pages = {2858--2866},
	Title = {An Introduction to Wavelet Analysis in Oceanography and Meteorology: With Application to the Dispersion of {Y}anai Waves},
	Volume = 121,
	Year = 1993}

@article{Meyers99,
	Annote = {Not on file. Imputation of missing values. Uses EOF
                  reconstruction technique of Smith95. Determine rank
                  of reconstruction (number of included EOFs) by
                  cross-validation with different dataset. This
                  cross-validation, however, cannot cover the entire
                  period for which a reconstruction is sought, for
                  otherwise there would be data available and no
                  reconstruction would be necessary.},
	Author = {S. D. Meyers and J. J. {O'Brien} and E. Thelin},
	Journal = {Mon. Wea. Rev.},
	Pages = {1599--1612},
	Title = {Reconstruction of monthly SST in the tropical Pacific Ocean during 1868-1993 using adaptive climate basis functions},
	Volume = 127,
	Year = 1999}

@article{Miller70,
	Annote = {Not on file. Choice of regularization parameter as a
                  function of observational error.},
	Author = {K. Miller},
	Journal = {SIAM J. Math. Anal.},
	Pages = {52--74},
	Title = {Least squares methods for ill-posed problems with a prescribed bound},
	Volume = 1,
	Year = 1970}

@article{Miller84,
	Annote = {Filed under Regression Analysis. AIC biased if used
                  for variable selection.},
	Author = {A. J. Miller},
	Journal = {J. Roy. Statist. Soc. A},
	Pages = {389--425},
	Title = {Selection of Subsets of Regression Variables},
	Volume = {147},
	Year = 1984}

@article{Miller90,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {J. Miller},
	Journal = {Phys. Rev. Lett.},
	Pages = {2137--2140},
	Title = {Statistical Mechanics of Euler Equations in Two Dimensions},
	Volume = 65,
	Year = 1990}

@article{Milne22,
	Annote = {Filed under General Circulation History.},
	Author = {E. A. Milne},
	File = {../../Papers/milne22.pdf},
	Journal = {Phil. Mag.},
	Pages = {872--896},
	Title = {Radiative Equilibrium: the Insolation of an Atmosphere},
	Volume = 44,
	Year = 1922,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgttaWxuZTIyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRItvzIxnAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzKUDAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWlsbmUyMi5wZGYADgAYAAsAbQBpAGwAbgBlADIAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvbWlsbmUyMi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9taWxuZTIyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Mitas05,
	Author = {C. M. Mitas and A. Clement},
	File = {../../Papers/mitas05.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2004GL021765},
	Pages = {L03809},
	Title = {Has the {H}adley cell been strengthening in recent decades?},
	Volume = 32,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgttaXRhczA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIvv9szEAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv9ujkAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWl0YXMwNS5wZGYADgAYAAsAbQBpAHQAYQBzADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvbWl0YXMwNS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9taXRhczA1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Mitchell95a,
	Annote = {Filed under Climate Change Detection.},
	Author = {J. F. B. Mitchell and T. C. Johns and J. M. Gregory and S. F. B. Tett},
	Journal = {Nature},
	Pages = {501--504},
	Title = {Climate response to increasing levels of greenhouse gases and sulphate aerosols},
	Volume = 376,
	Year = 1995}

@article{Mitchell95b,
	Annote = {Filed under Climate Change Detection. Compare Hadley
                  Centre climate simulations with observations. Model
                  is too sensitive. Only equilibrium response to CO2
                  and aerosol changes is considered; hence, thermal
                  inertia of oceans is neglected, which contributes to
                  the overestimation of the warming. Better agreement
                  between simulations and observations when radiative
                  cooling effect of aerosols is doubled.},
	Author = {J. F. B. Mitchell and R. A. Davis and W. J. Ingram and C. A. Senior},
	Journal = {J. Climate},
	Pages = {2364--2386},
	Title = {On Surface Temperature, Greenhouse Gases, and Aerosols: Models and Observations},
	Volume = 8,
	Year = 1995}

@article{Mitchell97,
	Annote = {Filed under Climate Change Detection.},
	Author = {J. F. B. Mitchell and T. C. Johns},
	Journal = {J. Climate},
	Pages = {245--267},
	Title = {On Modification of Global Warming by Sulfate Aerosols},
	Volume = 10,
	Year = 1997}

@article{Mkhadri97,
	Annote = {Filed under Discriminant Analysis.},
	Author = {A. Mkhadri and G. Celeux and A. Nasroallah},
	Journal = {Comput. Statist. Data Anal.},
	Pages = {403--423},
	Title = {Regularization in discriminant analysis: an overview},
	Volume = 23,
	Year = 1997}

@article{Mo96,
	Author = {K. C. Mo and R. W. Higgins},
	File = {../../Papers/mo96.pdf},
	Journal = {J. Climate},
	Pages = {1531--1545},
	Title = {Large-Scale Atmospheric Moisture Transport as Evaluated in the {NCEP}/{NCAR} and the {NASA}/{DAO} Reanalyses},
	Volume = 9,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfghtbzk2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRI2vDxT+AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvDzEeAAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bW85Ni5wZGYAAA4AEgAIAG0AbwA5ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL21vOTYucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL21vOTYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@article{Mokkadem89,
	Annote = {Filed under Entropy Estimation.},
	Author = {A. Mokkadem},
	Journal = {IEEE Trans. Inform. Theory},
	Pages = {193--196},
	Title = {Estimation of the Entropy and Information of Absolutely Continuous Random Variables},
	Volume = 35,
	Year = 1989}

@article{Molina87,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {L. T. Molina and M. J. Molina},
	Journal = {J. Phys. Chem.},
	Pages = {433--436},
	Title = {Production of $\mathrm{Cl}_s\mathrm{O}_2$ from the self-reaction of the $\mathrm{ClO}$ radical},
	Volume = 91,
	Year = 1987}

@article{Molteni93,
	Annote = {File under Predictability.},
	Author = {F. Molteni and T. N. Palmer},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {269--298},
	Title = {Predictability and finite-time instability of the northern winter circulation},
	Volume = 119,
	Year = 1993}

@book{Monin71,
	Address = {Cambridge, MA},
	Author = {A. S. Monin and A. M. Yaglom},
	Note = {Updated, augmented, and revised translation of \emph{Statisicheskaya gidromekhanika --- Mekhanika Turbulentnosti} (Nauka Press, Moscow, 1965).},
	Pages = 769,
	Publisher = {MIT Press},
	Title = {Statistical Fluid Mechanics: Mechanics of Turbulence},
	Volume = 1,
	Year = 1971}

@incollection{Morf78,
	Address = {New York},
	Annote = {Not on file.},
	Author = {M. Morf},
	Booktitle = {Modern Spectrum Analysis},
	Editor = {D. G. Childers},
	Pages = {172--181},
	Publisher = {IEEE Press},
	Title = {???},
	Year = 1978}

@article{Morrison98,
	Annote = {Filed under Hamiltonian Balanced Dynamics.},
	Author = {P. J. Morrison},
	Journal = {Rev. Mod. Phys.},
	Pages = {467--521},
	Title = {Hamiltonian description of the ideal fluid},
	Volume = 70,
	Year = 1998}

@book{Morse53,
	Address = {New York},
	Annote = {(2 vols.)},
	Author = {P. M. Morse and H. Feshbach},
	Pages = 1978,
	Publisher = {McGraw-Hill},
	Series = {International Series in Pure and Applied Physics},
	Title = {Methods of Theoretical Physics},
	Year = 1953}

@article{Munk50,
	Annote = {Classic paper on wind-driven circulation.},
	Author = {W. H. Munk},
	Journal = {J. Meteorol.},
	Pages = {79--93},
	Title = {On the wind-driven ocean circulation},
	Volume = 7,
	Year = 1950}

@article{Muraki99,
	Annote = {Filed under Quasigeostrophy -- Alternatives and
                  Higher Order Corrections.},
	Author = {D. J. Muraki and C. Snyder and R. Rotunno},
	Journal = {J. Atmos. Sci.},
	Pages = {1547--1560},
	Title = {The next-order corrections to quasigeostrophic theory},
	Volume = 56,
	Year = 1999}

@article{Mureau93,
	Annote = {Filed under Predictability.},
	Author = {R. Mureau and F. Molteni and T. N. Palmer},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {299--323},
	Title = {Ensemble prediction using dynamically conditioned perturbations},
	Volume = 119,
	Year = 1993}

@article{Murphy88,
	Annote = {Filed under Predictability.},
	Author = {J. M. Murphy},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {463--493},
	Title = {The Impact of Ensemble Forecasts on Predictability},
	Volume = 114,
	Year = 1988}

@article{Nakamura01,
	Annote = {Introduces Eulerian mixing efficieny.},
	Author = {N. Nakamura},
	Journal = {J. Atmos. Sci.},
	Pages = {3685--3701},
	Title = {A new look at eddy diffusivity as a mixing diagnostic},
	Volume = 58,
	Year = 2001}

@article{Nakamura89,
	Author = {N. Nakamura and I. M. Held},
	Journal = {J. Atmos. Sci.},
	Pages = {3055--3064},
	Title = {Nonlinear Equilibration of Two-Dimensional {E}ady Waves},
	Volume = 46,
	Year = 1989}

@article{Nakamura93,
	Annote = {Effects of barotropic shear on the nonlinear
                  evolution of baroclinic waves.},
	Author = {N. Nakamura},
	Journal = {J. Atmos. Sci.},
	Pages = {2159--2179},
	Title = {Momentum Flux, Flow Symmetry, and the Nonlinear Barotropic Governor},
	Volume = 50,
	Year = 1993}

@article{Nakamura95,
	Annote = {Not on file. Introduces a meridional coordinate that
                  is a function of the mass-weighted average of area
                  between contours of conserved tracer. Derives
                  transport equations in this coordinate. The mean of
                  the N2O mixing ratio in this coordinate clearly
                  indicates the edge of the polar vortex. Can also use
                  PV as tracer, which also results in better
                  diagnostic of vortex edge than Eulerian mean.},
	Author = {N. Nakamura},
	Journal = {J. Atmos. Sci.},
	Pages = {2096--2108},
	Title = {Modified {L}agrangian-Mean Diagnostics of the Stratospheric Polar Vortices. {P}art {I}: Formulation and Analysis of {GFDL} {SKYHI} {GCM}},
	Volume = 52,
	Year = 1995}

@article{Nakamura96,
	Author = {N. Nakamura},
	Journal = {J. Atmos. Sci.},
	Pages = {1524--1537},
	Title = {Two-Dimensional Mixing, Edge Formation, and Permeability Diagnosed in an Area Coordinate},
	Volume = 53,
	Year = 1996}

@article{Nakamura97a,
	Author = {N. Nakamura and J. Ma},
	Journal = {J. Geophys. Res.},
	Pages = {25721--25735},
	Title = {Modified {L}agrangian-Mean Diagnostics of the Stratospheric Polar Vortices. 2. {N}itrous Oxide and Seasonal Barrier Migration in the Cryogenic Limb Array Etalon Spectrometer and {SKYHI} General Circulation Model},
	Volume = {102D},
	Year = 1997}

@article{Nakamura97b,
	Author = {H. Nakamura and M. Nakamura and J. L. Anderson},
	Journal = {Mon. Wea. Rev.},
	Pages = {2074--2093},
	Title = {The Role of High- and Low-Frequency Dynamics in Blocking Formation},
	Volume = 125,
	Year = 1997}

@incollection{Nakamura98,
	Author = {N. Nakamura},
	Booktitle = {Dynamics of Atmospheric Flows: Atmospheric Transport and Diffusion Processes},
	Chapter = 5,
	Editor = {M. Rahman},
	Pages = {193--246},
	Publisher = {Computational Mechanics Publications},
	Series = {Advances in Fluid Mechanics},
	Title = {Leaky containment vessels of air: A {L}agrangian-mean approach to the stratospheric tracer transport},
	Volume = 18,
	Year = 1998}

@article{Nakamura99,
	Author = {N. Nakamura},
	Journal = {J. Atmos. Sci.},
	Pages = {2246--2260},
	Title = {Baroclinic-barotropic Adjustments in a Meridionally Wide Domain},
	Volume = 56,
	Year = 1999}

@article{Nankervis88,
	Annote = {Not on file. Univariate AR(1) model with
                  intercept. Least squares estimates of AR coefficient
                  are biased such that t-distribution is not a good
                  approximation of distribution of empirical
                  t-ratios. Correcting the bias of the estimates
                  empirically and adjusting standard deviation of
                  t-ratios gives a statistic that is approximately
                  distributed like Student's t.},
	Author = {J. C. Nankervis and N. E. Savin},
	Journal = {Econometrica},
	Pages = {119--145},
	Title = {The {S}tudent's $t$ approximation in a stationary first order autoregressive model},
	Volume = 56,
	Year = 1988}

@article{Navarra02,
	Annote = {Filed under Boccaletti.},
	Author = {A. Navarra and G. Boccaletti},
	File = {../../Papers/navarra02.pdf},
	Journal = {Cli. Dyn.},
	Pages = {467--483},
	Title = {Numerical general circulation experiments of sensitivity to {E}arth rotation rate},
	Volume = 19,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1uYXZhcnJhMDIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJAwE7qBAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwE9ahAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmF2YXJyYTAyLnBkZgAOABwADQBuAGEAdgBhAHIAcgBhADAAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbmF2YXJyYTAyLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL25hdmFycmEwMi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Neelin03,
	Author = {J. D. Neelin and C. Chou and H. Su},
	File = {../../Papers/neelin03.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2003GL018625},
	Pages = 2275,
	Title = {Tropical drought regions in global warming and {El} {Ni{\~n}o} teleconnections},
	Volume = 30,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxuZWVsaW4wMy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJCvWXhawAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvWZD2wAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmVlbGluMDMucGRmAAAOABoADABuAGUAZQBsAGkAbgAwADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL25lZWxpbjAzLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9uZWVsaW4wMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Neelin06,
	Author = {J. D. Neelin and M. M{\"u}nnich and H. Su and J. E. Meyerson and C. E. Holloway},
	File = {../../Papers/neelin06.pdf},
	Journal = {Proc. Nat. Acad. Sci.},
	Pages = {6110--6115},
	Title = {Tropical drying trends in global warming models and observations},
	Volume = 103,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxuZWVsaW4wNi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJDxXPdqAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxXROKAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmVlbGluMDYucGRmAAAOABoADABuAGUAZQBsAGkAbgAwADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL25lZWxpbjA2LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9uZWVsaW4wNi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@incollection{Neelin07a,
	Address = {Princeton, NJ},
	Author = {J. D. Neelin},
	Booktitle = {The Global Circulation of the Atmosphere},
	Chapter = 10,
	Editor = {T. Schneider and A. H. Sobel},
	Pages = {267--301},
	Publisher = {Princeton University Press},
	Title = {Moist Dynamics of Tropical Convection Zones in Monsoons, Teleconnections, and Global Warming},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1uZWVsaW4wN2EucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJEwooc0wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwop/QwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmVlbGluMDdhLnBkZgAOABwADQBuAGUAZQBsAGkAbgAwADcAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbmVlbGluMDdhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL25lZWxpbjA3YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Neelin08,
	Author = {J. D. Neelin and O. Peters and J. W.-B. Lin and K. Hales and C. E. Holloway},
	File = {../../Papers/neelin08.pdf},
	Journal = {Phil. Trans. Roy. Soc. A},
	Pages = {2581--2604},
	Title = {Rethinking convective quasi-equilibrium: observational constraints for stochastic convective schemes in climate models},
	Volume = 366,
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxuZWVsaW4wOC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJFxXPcTwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxXRMzwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmVlbGluMDgucGRmAAAOABoADABuAGUAZQBsAGkAbgAwADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL25lZWxpbjA4LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9uZWVsaW4wOC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Neelin09a,
	Author = {J. D. Neelin and O. Peters and K. Hales},
	File = {../../Papers/neelin09a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2367--2384},
	Title = {The transition to strong convection},
	Volume = 66,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1uZWVsaW4wOWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJGxqCDqAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxqDmGAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmVlbGluMDlhLnBkZgAOABwADQBuAGUAZQBsAGkAbgAwADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbmVlbGluMDlhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL25lZWxpbjA5YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Neelin87a,
	Annote = {Gross moist stability is, to a large extent,
                  determinant of position of convective zones
                  (low-level mass flux convergence).},
	Author = {J. D. Neelin and I. M. Held},
	File = {../../Papers/neelin87a.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {3--12},
	Title = {Modeling Tropical Convergence Based on the Moist Static Energy Budget},
	Volume = 115,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1uZWVsaW44N2EucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJHwcGawwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwcILQwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmVlbGluODdhLnBkZgAOABwADQBuAGUAZQBsAGkAbgA4ADcAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbmVlbGluODdhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL25lZWxpbjg3YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Neelin87b,
	Author = {J. D. Neelin and I. M. Held and K. H. Cook},
	File = {../../Papers/neelin87b.pdf},
	Journal = {J. Atmos. Sci},
	Pages = {2341--2348},
	Title = {Evaporation-wind feedback and low-frequency variability in the tropical atmosphere},
	Volume = {44},
	Year = {1987},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1uZWVsaW44N2IucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJIwS3zJ1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwS5VlwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmVlbGluODdiLnBkZgAOABwADQBuAGUAZQBsAGkAbgA4ADcAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbmVlbGluODdiLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL25lZWxpbjg3Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Neelin91,
	Annote = {Not on file.},
	Author = {J. D. Neelin},
	Journal = {J. Atmos. Sci.},
	Pages = {584--606},
	Title = {The Slow Sea Surface Temperature Mode and the Fast-Wave Limit: {A}nalytic Theory for Tropical Interannual Oscillations and Experiments in a Hybrid Coupled Model},
	Volume = 48,
	Year = 1991}

@article{Neelin93,
	Annote = {Second of a series of three papers by these authors},
	Author = {J. D. Neelin and F.-F. Jin},
	Journal = {J. Atmos. Sci.},
	Pages = {3504--3522},
	Title = {Modes of Interannual Tropical Ocean-Atmosphere Interaction --- a Unified View. {P}art {II}: {A}nalytical Results in the Weak-Coupling Limit},
	Volume = 50,
	Year = 1993}

@article{Neelin94,
	Author = {J. D. Neelin and M. Latif and F.-F. Jin},
	File = {../../Papers/neelin94.pdf},
	Journal = {Annu. Rev. Fluid Mech.},
	Pages = {617--59},
	Title = {Dynamics of Coupled Ocean-Atmosphere models: {T}he Tropical Problem},
	Volume = {26},
	Year = {1994},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxuZWVsaW45NC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJJwwzG8lBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAww0pYgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmVlbGluOTQucGRmAAAOABoADABuAGUAZQBsAGkAbgA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL25lZWxpbjk0LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9uZWVsaW45NC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Neelin95,
	Annote = {Not on file.},
	Author = {J. D. Neelin and H. A. Dijkstra},
	Journal = {J. Climate},
	Pages = {1325--1342},
	Title = {Ocean-Atmosphere Interaction and the Tropical Climatology. {P}art {I}: {T}he Dangers of Flux Correction},
	Volume = 8,
	Year = 1995}

@incollection{Neelin97,
	Address = {Netherlands},
	Annote = {Filed under Moist Convection. Introduces
                  QTCM. Discussion of
                  quasi-equilibrium. Moist-convective damping of
                  waves.},
	Author = {J. D. Neelin},
	Booktitle = {The Physics and Parameterization of Moist Atmospheric Convection},
	Editor = {R. K. Smith},
	Pages = {413--446},
	Publisher = {Kluwer Academic Publishers},
	Title = {Implications of Convective Quasi-Equilibrium for the Large-Scale Flow},
	Year = 1997}

@article{Neelin98,
	Annote = {Review of ENSO dynamics.},
	Author = {J. D. Neelin and D. S. Battisti and A. C. Hirst and F.-F. Jin and Y. Wakata and T. Yamagata and S. E. Zebiak},
	Journal = {J. Geophys. Res.},
	Pages = {14261--14290},
	Title = {{ENSO} Theory},
	Volume = {103C},
	Year = 1998}

@incollection{Neiburger61,
	Address = {Berkeley, Los Angeles, CA; London, England},
	Annote = {History of discovery of trade inversion.},
	Author = {M. Neiburger and D. S. Johnson and C.-W. Chien},
	Booktitle = {University of California Publications in Meteorology},
	Editor = {Z. Sekera and J. Bjerknes and Y. Mintz},
	Pages = {1--94},
	Publisher = {University of California Press and Cambridge University Press},
	Title = {Studies of the structure of the atmosphere over the eastern {Pacific} ocean in summer. I. {The} Inversion over the Eastn North Pacific Ocean},
	Volume = 1,
	Year = 1961}

@article{Nellis96,
	Author = {W. J. Nellis and S. T. Weir and A. C. Mitchell},
	Journal = {Science},
	Pages = {936--938},
	Title = {Metallization and electrical conductivity of hydrogen in {Jupiter}},
	Volume = {273},
	Year = {1996}}

@unpublished{Nelson94,
	Annote = {Filed under Baker.},
	Author = {J. T. Nelson and M. B. Baker},
	Note = {Preprint},
	Title = {A New Theoretical Framework for Studies of Vapor Growth and Evaporation of Small ice Crystals in the Atmosphere},
	Year = 1994}

@article{Neufeld00,
	Annote = {Filed under Chaotic Advection.},
	Author = {Z. Neufeld and P. H. Haynes and G. Picard},
	Journal = {Phys. Fluids},
	Pages = {2506--2513},
	Title = {The effect of forcing on the spatial structure and spectra of chaotically advected passive scalars},
	Volume = 12,
	Year = 2000}

@article{Neumaier01a,
	Author = {A. Neumaier and T. Schneider},
	Date-Modified = {2010-06-11 12:13:42 -0700},
	Journal = {ACM Trans. Math. Softw.},
	Pages = {27--57},
	Title = {Estimation of parameters and eigenmodes of multivariate autoregressive models},
	Volume = 27,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9uZXVtYWllcjAxYS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJOt7fYpAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAt7g7FAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmV1bWFpZXIwMWEucGRmAA4AIAAPAG4AZQB1AG0AYQBpAGUAcgAwADEAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbmV1bWFpZXIwMWEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbmV1bWFpZXIwMWEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@unpublished{Neumaier94,
	Author = {A. Neumaier},
	Note = {Unpublished Manuscript},
	Title = {From Thermodynamics to Quantum Theory. {P}art {I}: Equilibrium},
	Year = 1994}

@unpublished{Neumaier95,
	Author = {A. Neumaier},
	Note = {Preprint},
	Title = {Invariant confidence regions for nonlinear parameter estimation problems},
	Year = 1995}

@article{Neumaier98,
	Annote = {Filed under Regularization.},
	Author = {A. Neumaier},
	Journal = {SIAM Rev.},
	Pages = {636--666},
	Title = {Solving ill-conditioned and singular linear systems: A tutorial on regularization},
	Volume = 40,
	Year = 1998}

@article{Neumaier98a,
	Author = {A. Neumaier and E. Groeneveld},
	Journal = {Genetics Selection Evolution},
	Pages = {3--26},
	Title = {Restricted maximum likelihood estimation of covariances in sparse linear models},
	Volume = {30},
	Year = 1998}

@article{Nevison99,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {C. D. Nevison and S. Solomon and R. S. Gao},
	Journal = {J. Geophys. Res.},
	Pages = {3741--3754},
	Title = {Buffering interactions in the modeled response of stratospheric $\mathrm{O}_3$ to increased $\mathrm{NO}_x$ and $\mathrm{HO}_x$},
	Volume = {104D},
	Year = 1999}

@article{Newell92,
	Author = {R. E. Newell and N. E. Newell and Y. Zhu and C. Scott},
	File = {../../Papers/newell92.pdf},
	Journal = {Geophys. Res. Lett.},
	Pages = {2401--2404},
	Title = {Tropospheric Rivers? --- {A} Pilot Study},
	Volume = 12,
	Year = 1992,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxuZXdlbGw5Mi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJUv9ApXwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv9CZ3wAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmV3ZWxsOTIucGRmAAAOABoADABuAGUAdwBlAGwAbAA5ADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL25ld2VsbDkyLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9uZXdlbGw5Mi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Newell99,
	Annote = {Laminar structure of tracers (?).},
	Author = {R. E. Newell and V. Thouret and J. Y. N. Cho and P. Stoller and A. Marenco and H. G. Smit},
	Journal = {Nature},
	Pages = {316--319},
	Title = {Ubiquity of quasi-horizontal layers in the troposphere},
	Volume = 398,
	Year = 1999}

@article{Ngan99a,
	Annote = {Filed under Shepherd.},
	Author = {K. Ngan and T. G. Shepherd},
	Journal = {J. Atmos. Sci.},
	Pages = {4134--4152},
	Title = {A closer look at chaotic advection in the stratosphere. {P}art {I}: {G}eometric structure},
	Volume = 56,
	Year = 1999}

@article{Ngan99b,
	Annote = {Filed under Shepherd.},
	Author = {K. Ngan and T. G. Shepherd},
	Journal = {J. Atmos. Sci.},
	Pages = {4153--4166},
	Title = {A closer look at chaotic advection in the stratosphere. {P}art {II}: {S}tatistical diagnostics},
	Volume = 56,
	Year = 1999}

@incollection{Nicholls96,
	Address = {Cambridge, UK},
	Author = {N. Nicholls and G. V. Gruza and J. Jouzel and T. R. Karl and L. A. Ogallo and D. E. Parker},
	Booktitle = {Climate Change 1995: The Science of Climate Change},
	Editor = {J. T. Houghton and L. G. {Meira Filho} and B. A. Callander and N. Harris and A. Kattenberg and K. Maskell},
	Pages = {132--192},
	Publisher = {Intergovernmental Panel on Climate Change, Cambridge University Press},
	Title = {Observed Climate Variability and Change},
	Year = 1996}

@article{Nicolis95,
	Annote = {Filed under Predictability.},
	Author = {C. Nicolis and S. Vannitsem and J.-F. Royer},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {705--722},
	Title = {Short-Range Predictability of the Atmosphere: Mechanisms for Superexponential Error Growth},
	Volume = 121,
	Year = 1995}

@article{Nielsen84,
	Annote = {Filed under Barotropic Point Jet and Schoeberl.},
	Author = {J. E. Nielsen and M. R. Schoeberl},
	File = {../../Papers/nielsen84.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2869--2881},
	Title = {A Numerical Simulation of Barotropic Instability. {P}art {II}: Wave-Wave Interaction},
	Volume = 41,
	Year = 1984,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1uaWVsc2VuODQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJWwhD4O1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwhFouwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bmllbHNlbjg0LnBkZgAOABwADQBuAGkAZQBsAHMAZQBuADgANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbmllbHNlbjg0LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL25pZWxzZW44NC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Niemela00,
	Annote = {Filed under Rayleigh-Benard convection. Measurements
                  of scaling laws in convection over 10 orders of
                  magnitude. Find that Nu \sim Ra^{0.309} (consistent
                  with weakly nonlinear scaling).},
	Author = {J. J. Niemela and L. Skrbek and K. R. Sreenivasan and R. J. Donnelly},
	Journal = {Nature},
	Pages = {837--840},
	Title = {Turbulent convection at very high {R}ayleigh numbers},
	Volume = 404,
	Year = 2000}

@article{North79,
	Author = {G. R. North and J. A. Coakley, Jr.},
	File = {../../Papers/north79.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1189--1204},
	Title = {Differences between Seasonal and Mean Annual Energy Balance Model Calculations of Climate and Climate Sensitivity},
	Volume = 36,
	Year = 1979,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtub3J0aDc5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJaw9SfpQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw9UQJQAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bm9ydGg3OS5wZGYADgAYAAsAbgBvAHIAdABoADcAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvbm9ydGg3OS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9ub3J0aDc5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{North81,
	Annote = {Filed under Predictability.},
	Author = {G. R. North and R. F. Cahalan},
	File = {../../Papers/north81.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {504--513},
	Title = {Predictability in a Solvable Stochastic Climate Model},
	Volume = 38,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtub3J0aDgxLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJbvhavmAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvhcgGAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bm9ydGg4MS5wZGYADgAYAAsAbgBvAHIAdABoADgAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvbm9ydGg4MS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9ub3J0aDgxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{North83,
	Author = {G. R. North and J. G. Mengel and D. A. Short},
	Journal = {J. Geophys. Res.},
	Pages = {6576--6586},
	Title = {Simple Energy Balance Model Resolving the Seasons and the Continents: Application to the Astronomical Theory of the Ice Ages},
	Volume = 88,
	Year = 1983}

@article{North98,
	Annote = {Filed under Climate Change Detection. Another review
                  of ``optimal signal detection'' methods. Then try to
                  detect solar cycle, volcanic forcing, GHG, and
                  aerosol ``signal'' in observational
                  record. Represent all data in frequency domain. Show
                  that the component of the solar cycle signal that is
                  perpendicular to the other signals is very weak in
                  the observational record. By way of contrast, the
                  componentens of the volcanic signal and the GHG
                  signal perpendicular to the other signals are
                  robustly manifest in the observational record.},
	Author = {G. R. North and M. J. Stevens},
	Journal = {J. Climate},
	Pages = {563--577},
	Title = {Detecting Climate Signals in the Surface Temperature Record},
	Volume = 11,
	Year = 1998}

@article{Nozawa97a,
	Annote = {Filed under 2D Turbulence.},
	Author = {T. Nozawa and S. Yoden},
	File = {../../Papers/nozawa97a.pdf},
	Journal = {Pys. Fluids},
	Pages = {2081--2093},
	Title = {Formation of zonal band structure in forced two-dimensional turbulence on a rotating sphere},
	Volume = 9,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ub3phd2E5N2EucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJdvW9uGAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvW/QiAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bm96YXdhOTdhLnBkZgAOABwADQBuAG8AegBhAHcAYQA5ADcAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbm96YXdhOTdhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL25vemF3YTk3YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Nozawa97b,
	Annote = {Filed under 2D Turbulence.},
	Author = {T. Nozawa and S. Yoden},
	File = {../../Papers/nozawa97b.pdf},
	Journal = {Pys. Fluids},
	Pages = {3834--3842},
	Title = {Spectral anisotropy in forced two-dimensional turbulence on a rotating sphere},
	Volume = 9,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1ub3phd2E5N2IucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJevW9uawAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvW/Q2wAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bm96YXdhOTdiLnBkZgAOABwADQBuAG8AegBhAHcAYQA5ADcAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvbm96YXdhOTdiLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL25vemF3YTk3Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Numaguti95,
	Annote = {Filed under Monsoon Dynamics. Studies location of
                  precipitation zones given fixed SST. With
                  sinusoidally varying latitude of SST maximum,
                  precipitation zones jump nonlinearly if SST maximum
                  reaches sufficiently high latitude (about 15 deg),
                  but details depend on convection scheme. WISHE
                  feedback important (jump not there if WISHE feedback
                  disabled). Discusses relative importance of
                  boundary layer convergence (Lindzen-Nigam) and moist
                  static energy budget.},
	Author = {A. Numaguti},
	File = {../../Papers/numaguti95.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1128--1141},
	Title = {Dynamics and Energy Balance of the {H}adley Circulation and the Tropical Precipitation Zones. {P}art~{II}: Sensitivity to Meridional {SST} Distribution},
	Volume = 52,
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5udW1hZ3V0aTk1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJgwAGoBlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwAIYhgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bnVtYWd1dGk5NS5wZGYAAA4AHgAOAG4AdQBtAGEAZwB1AHQAaQA5ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL251bWFndXRpOTUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL251bWFndXRpOTUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{OGorman03,
	Annote = {Not on file.},
	Author = {P. A. O'Gorman and D. I. Pullin},
	File = {../../Papers/ogorman03.pdf},
	Journal = {Phys. Fluids},
	Pages = {280--291},
	Title = {The velocity-scalar cross spectrum of stretched spiral vortices},
	Volume = 15,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1vZ29ybWFuMDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJov6FScFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv6HC8AAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6b2dvcm1hbjAzLnBkZgAOABwADQBvAGcAbwByAG0AYQBuADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvb2dvcm1hbjAzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL29nb3JtYW4wMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{OGorman06a,
	Author = {P. A. O'Gorman and T. Schneider},
	Date-Modified = {2010-06-11 12:12:45 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {2992--3005},
	Title = {Stochastic Models for the Kinematics of Moisture Transport and Condensation in Homogeneous Turbulent Flows},
	Volume = {63},
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9vJ2dvcm1hbjA2YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJhwZXgugAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwZZROgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bydnb3JtYW4wNmEucGRmAA4AIAAPAG8AJwBnAG8AcgBtAGEAbgAwADYAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbydnb3JtYW4wNmEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbydnb3JtYW4wNmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{OGorman07a,
	Author = {P. A. O'Gorman and T. Schneider},
	Date-Modified = {2010-06-11 12:13:22 -0700},
	Journal = {Geophys. Res. Lett.},
	Pages = {L22801},
	Title = {Recovery of atmospheric flow statistics in a general circulation model without nonlinear eddy--eddy interactions},
	Volume = {34},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9vJ2dvcm1hbjA3YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJiw2ZpjQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw2baDQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bydnb3JtYW4wN2EucGRmAA4AIAAPAG8AJwBnAG8AcgBtAGEAbgAwADcAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbydnb3JtYW4wN2EucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbydnb3JtYW4wN2EucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{OGorman08a,
	Author = {P. A. O'Gorman and T. Schneider},
	Journal = {J. Atmos. Sci.},
	Pages = {524--535},
	Title = {Weather-layer dynamics of baroclinic eddies and multiple jets in an idealized general circulation model},
	Volume = {65},
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9vJ2dvcm1hbjA4YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJjw+hz3gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw+jkXgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bydnb3JtYW4wOGEucGRmAA4AIAAPAG8AJwBnAG8AcgBtAGEAbgAwADgAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbydnb3JtYW4wOGEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbydnb3JtYW4wOGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{OGorman08b,
	Author = {P. A. O'Gorman and T. Schneider},
	Journal = {J. Climate},
	Pages = {3815--3832},
	Title = {The hydrological cycle over a wide range of climates simulated with an idealized {GCM}},
	Volume = {21},
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9vJ2dvcm1hbjA4Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJkxMU8ygAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxMWfOgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bydnb3JtYW4wOGIucGRmAA4AIAAPAG8AJwBnAG8AcgBtAGEAbgAwADgAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbydnb3JtYW4wOGIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbydnb3JtYW4wOGIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{OGorman08c,
	Author = {P. A. O'Gorman and T. Schneider},
	Journal = {J. Climate},
	Pages = {5797--5806},
	Title = {Energy of midlatitude transient eddies in idealized simulations of changed climates},
	Volume = {21},
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9vJ2dvcm1hbjA4Yy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJlxVFZPgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxVHJvgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bydnb3JtYW4wOGMucGRmAA4AIAAPAG8AJwBnAG8AcgBtAGEAbgAwADgAYwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbydnb3JtYW4wOGMucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbydnb3JtYW4wOGMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{OGorman09a,
	Author = {P. A. O'Gorman and T. Schneider},
	Journal = {J. Climate},
	Pages = {5676--5685},
	Title = {Scaling of precipitation extremes over a wide range of climates simulated with an idealized {GCM}},
	Volume = {22},
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9vJ2dvcm1hbjA5YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJmxxBemwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxxDBCwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bydnb3JtYW4wOWEucGRmAA4AIAAPAG8AJwBnAG8AcgBtAGEAbgAwADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbydnb3JtYW4wOWEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbydnb3JtYW4wOWEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{OGorman09b,
	Author = {P. A. O'Gorman and T. Schneider},
	Journal = {Proc. Nat. Acad. Sci.},
	Pages = {14773--14777},
	Title = {The physical basis for increases in precipitation extremes in simulations of 21st-century climate change},
	Volume = {106},
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9vJ2dvcm1hbjA5Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJnxrGYyAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxrH7OAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bydnb3JtYW4wOWIucGRmAA4AIAAPAG8AJwBnAG8AcgBtAGEAbgAwADkAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvbydnb3JtYW4wOWIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvbydnb3JtYW4wOWIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@techreport{Oort71,
	Annote = {Not on file.},
	Author = {A. H. Oort and E. M. Rasmusson},
	Institution = {U.S. Dept. of Commerce, National Oceanic and Atmospheric Administration,},
	Number = 5,
	Title = {Atmospheric Circulation Statistics},
	Type = {Professional Paper},
	Year = 1971}

@article{Oort94,
	Author = {A. H. Oort and L. A. Anderson and J. P. Peixoto},
	Journal = {J. Geophys. Res.},
	Pages = {7665--7688},
	Title = {Estimates of the Energy Cycle of the Oceans},
	Volume = {99C},
	Year = 1994}

@unpublished{Oort96,
	Annote = {Basically follows his book with Peixoto.},
	Author = {A. H. Oort},
	Note = {Lecture Notes},
	Title = {Climate Dynamics},
	Year = {Spring 1996}}

@article{Orlanski98,
	Author = {Orlanski, I.},
	File = {../../Papers/orlanski98.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2577--2602},
	Title = {Poleward Deflection of Storm Tracks},
	Volume = {55},
	Year = {1998},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5vcmxhbnNraTk4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJxxaOmogAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxaQXIgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6b3JsYW5za2k5OC5wZGYAAA4AHgAOAG8AcgBsAGEAbgBzAGsAaQA5ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL29ybGFuc2tpOTgucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL29ybGFuc2tpOTgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Orszag70,
	Author = {S. A. Orszag},
	Journal = {J. Fluid Mech.},
	Pages = {363--386},
	Title = {Analytical theories of turbulence},
	Volume = 41,
	Year = 1970}

@incollection{Orszag73,
	Author = {S. A. Orszag},
	Booktitle = {Fluid Dynamics},
	Editor = {R. Balian and J.-L. Peube},
	Pages = {237--374},
	Publisher = {Gordon and Breach},
	Title = {Lectures on the Statistical Theory of Turbulence},
	Year = 1973}

@unpublished{Orszag95,
	Author = {S. A. Orszag},
	Note = {Lecture notes},
	Title = {Hydrodynamic Stability and Turbulence},
	Year = {Fall 1995}}

@unpublished{Orszag96,
	Author = {S. A. Orszag and I. Staroselsky and W. S. Flannery and Y. Zhang},
	Note = {Preprint},
	Title = {Introduction to Renormalization Group Modeling of Turbulence},
	Year = 1996}

@article{Orton94,
	Author = {Orton, G. S. and Friedson, A. J. and Yanamandra-Fisher, P. A. and Caldwell, J. and Hammel, H. B. and Baines, K. H. and Bergstralh, J. T. and Martin, T. Z. and West, R. A. and Veeder, G. J. and others},
	File = {../../Papers/orton94.pdf},
	Journal = {Science},
	Pages = {625--631},
	Title = {Spatial Organization and Time Dependence of {Jupiter's} Tropospheric Temperatures, 1980--1993},
	Volume = {265},
	Year = {1994},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtvcnRvbjk0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJyxJldGwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxJm/iwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6b3J0b245NC5wZGYADgAYAAsAbwByAHQAbwBuADkANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvb3J0b245NC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9vcnRvbjk0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Oseledec68,
	Annote = {Not on file. Existence of Liapunov exponents in
                  great generality.},
	Author = {V. I. Oseledec},
	Journal = {Trans. Moscow Math. Soc},
	Pages = {197--231},
	Title = {A multiplicative ergodic theorem: {L}iapunov characteristic numbers for dynamical systems},
	Volume = 19,
	Year = 1968}

@article{Ozawa01,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {H. Ozawa and S. Shimokawa and H. Sakuma},
	Journal = {Phys. Rev. E},
	Pages = 026303,
	Title = {Thermodynamics of fluid turbulence: {A} unifired approach to maximum transport properties},
	Volume = 64,
	Year = 2001}

@article{Ozawa03,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {H. Ozawa and A. Ohmura and R. D. Lorenz. and T. Pujol},
	Journal = {Rev. Geophys.},
	Note = {doi:10.1029/2002RG000113},
	Title = {The second law of thermodynamics and the global climate system: {A} review of the maximum entropy production principle},
	Volume = 41,
	Year = 2003}

@article{Pacala01,
	Annote = {Filed under Carbon Flux Estimates.},
	Author = {S. W. Pacala and Coauthors},
	Journal = {Science},
	Pages = {2316--2320},
	Title = {Consistent land- and atmosphere-based {U.S.} carbon sink estimates},
	Volume = 292,
	Year = 2001}

@article{Pall07,
	Annote = {Filed under Precipitation Statistics. Claim precip
                  extremes scales with precipitable water and hence
                  with saturation vapor pressure (?).},
	Author = {P. Pall and M. R. Allen and D. A. Stone},
	File = {../../Papers/pall07.pdf},
	Journal = {Climate Dyn.},
	Pages = {351--363},
	Title = {Testing the {C}lausius-{C}lapeyron constraint on changes in extreme precipitation under $\mathrm{CO_2}$ warming},
	Volume = 28,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpwYWxsMDcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJ4wdWoBVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwdYYhQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGFsbDA3LnBkZgAADgAWAAoAcABhAGwAbAAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3BhbGwwNy5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvcGFsbDA3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@incollection{Palmer96,
	Address = {Berlin},
	Annote = {Only preprint on file. Filed under
                  Predictability. Nice review of the concept of
                  predictability in nonlinear systems, distinguishing,
                  as Lorenz did, predictability of the first and
                  second kind. Review of singular vectors, Lyapunov
                  exponents, etc. Criticism of breeding vector
                  approach.},
	Author = {T. N. Palmer},
	Booktitle = {Decadal Climate Variability: Dynamics and Predictability},
	Editor = {D. L. T. Anderson and J. Willebrand},
	Pages = {83--155},
	Publisher = {Springer},
	Series = {{NATO} {ASI} Series},
	Title = {Predictability of the Atmosphere and Oceans: From Days to Decades},
	Volume = {I 44},
	Year = 1996}

@unpublished{Palmer98a,
	Annote = {Filed under Predictability.},
	Author = {T. N. Palmer},
	Note = {Submitted to {\em J . Climate}},
	Title = {A Nonlinear Dynamical Perspective on Climate Prediction},
	Year = 1997}

@article{Palmer98b,
	Annote = {Filed under Predictability. Address the question as
                  to what extent simpler metrics approximate the
                  analysis error covariance metric.},
	Author = {T. N. Palmer and R. Gelaro and J. Barkmeijer and R. Buizza},
	Journal = {J. Atmos. Sci.},
	Pages = {633--653},
	Title = {Singular Vectors, Metrics, and Adaptive Observations},
	Volume = 55,
	Year = 1998}

@article{Paltridge01,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {G. W. Paltridge},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {305--313},
	Title = {A physical basis for a maximum of thermodynamic dissipation of the climate system},
	Volume = 127,
	Year = 2001}

@article{Panareda08,
	Author = {A. Agust\'i-Panareda and {Coauthors}},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {submitted},
	Title = {Radiosonde humidity bias correction over the West African region for the special {AMMA} reanalysis at {ECMWF}},
	Volume = 134,
	Year = 2008}

@article{Panetta87,
	Annote = {Study to what extent a critical latitude at a lower
                  level affects wave propagation at upper levels (if
                  there are no critical latitudes there)},
	Author = {R. L Panetta and I. M. Held and R. T. Pierrehumbert},
	File = {../../Papers/panetta87.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2924--2933},
	Title = {External {R}ossby waves in the two-layer model},
	Volume = 44,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1wYW5ldHRhODcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJ8wO+5HAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwPAbjAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGFuZXR0YTg3LnBkZgAOABwADQBwAGEAbgBlAHQAdABhADgANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcGFuZXR0YTg3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3BhbmV0dGE4Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Panetta93,
	Author = {R. L. Panetta},
	Journal = {J. Atmos. Sci.},
	Pages = {2073--2106},
	Title = {Zonal Jets in Wide Baroclinically Unstable Regions: Persistence and Scale Separation},
	Volume = 50,
	Year = 1993}

@article{Paparella97,
	Annote = {Filed under Smith.},
	Author = {F. Paparella and A. Provenzale and L. A. Smith and C. Taricco and R. Vio},
	Journal = {Phys. Lett. A},
	Pages = {233--240},
	Title = {Local Random Analogue Prediction of Nonlinear Processes},
	Volume = 235,
	Year = 1997}

@book{Papoulis91,
	Address = {New York},
	Annote = {In GFDL Library: QA273.P2},
	Author = {A. Papoulis},
	Edition = {3rd},
	Pages = 666,
	Publisher = {McGraw Hill},
	Title = {Probability, Random Variables, and Stochastic Processes},
	Year = 1991}

@article{Park81,
	Annote = {Filed under Regression Analysis.},
	Author = {S. H. Park},
	Journal = {Technometrics},
	Pages = {289--295},
	Title = {Collinearity and Optimal Restrictions on Regression Parameters for Estimating Responses},
	Volume = 23,
	Year = 1981}

@article{Parker94,
	Annote = {Not on file.},
	Author = {D. E. Parker and P. D. Jones and C. K. Folland and A. Bevan},
	Journal = {J. Geophys. Res.},
	Pages = {14373--14399},
	Title = {Interdecadal changes of surface temperature since the late nineteenth century},
	Volume = {99D},
	Year = 1994}

@article{Parker95,
	Annote = {Not on file.},
	Author = {D. E. Parker and C. K. Folland and M. Jackson},
	Journal = {Climatic Change},
	Pages = {559--600},
	Title = {Marine surface temperature: {O}bserved variations and data requirements},
	Volume = 31,
	Year = 1995}

@book{Parlett80,
	Address = {London},
	Annote = {QA188.P37. Classic reference on eigenvalue
                  problems.},
	Author = {B. N. Parlett},
	Pages = 348,
	Publisher = {Prentice Hall},
	Series = {Series in Computational Mathematics},
	Title = {The Symmetric Eigenvalue Problem},
	Year = 1980}

@article{Pasquero03,
	Annote = {Filed under Tziperman.},
	Author = {C. Pasquero and E. Tziperman},
	Journal = {J. Phys. Oceanogr.},
	Note = {(in press)},
	Pages = {??},
	Title = {Effects of a wind driven gyre on thermohaline circulation variability},
	Volume = {??},
	Year = 2003}

@article{Patterson71,
	Annote = {Filed under Parameter Estimation.},
	Author = {H.~D. Patterson and R. Thompson},
	Journal = {Biometrika},
	Key = {parameter estimation, classic on restricted maximum likelihood},
	Pages = {545--554},
	Title = {Recovery of inter-block information when block sizes are unequal},
	Volume = 58,
	Year = 1971}

@article{Paulsen85,
	Annote = {Not on file.},
	Author = {J. Paulsen and D. Tj{\o}stheim},
	Journal = {J. Roy. Stat. Soc. B},
	Pages = {216--228},
	Title = {On the estimation of residual variance and order in autoregressive time series},
	Volume = 47,
	Year = 1985}

@article{Pauluis00,
	Author = {O. Pauluis and V. Balaji and I. M. Held},
	File = {../../Papers/pauluis00.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {989--994},
	Title = {Frictional Dissipation in a Precipitating Atmosphere},
	Volume = 57,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1wYXVsdWlzMDAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRJ/v/qUpVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv/sFJQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGF1bHVpczAwLnBkZgAOABwADQBwAGEAdQBsAHUAaQBzADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcGF1bHVpczAwLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3BhdWx1aXMwMC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Pauluis02a,
	Annote = {Convection as heat engine
                  vs. dehumidifier. Differences in entropy budget
                  between moist and dry convection.},
	Author = {O. Pauluis and I. M. Held},
	File = {../../Papers/pauluis02a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {125--139},
	Title = {Entropy Budget of an Atmosphere in Radiative-Convective Equilibrium. {P}art {I}: {M}aximum Work and Frictional Dissipation},
	Volume = 59,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5wYXVsdWlzMDJhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKAv/qUJFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv/sEpAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGF1bHVpczAyYS5wZGYAAA4AHgAOAHAAYQB1AGwAdQBpAHMAMAAyAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3BhdWx1aXMwMmEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3BhdWx1aXMwMmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Pauluis02b,
	Annote = {.},
	Author = {O. Pauluis and I. M. Held},
	File = {../../Papers/pauluis02b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {140--149},
	Title = {Entropy Budget of an Atmosphere in Radiative-Convective Equilibrium. {P}art {II}: {L}atent heat transport and moist processes},
	Volume = 59,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5wYXVsdWlzMDJiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKBv/qUY1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv/sE4wAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGF1bHVpczAyYi5wZGYAAA4AHgAOAHAAYQB1AGwAdQBpAHMAMAAyAGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3BhdWx1aXMwMmIucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3BhdWx1aXMwMmIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Pauluis04,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {O. Pauluis},
	File = {../../Papers/pauluis04.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1161--1173},
	Title = {Boundary Layer Dynamics and Cross-Equatorial {H}adley Circulation},
	Volume = 61,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1wYXVsdWlzMDQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKCvZNyJgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvZPUlgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGF1bHVpczA0LnBkZgAOABwADQBwAGEAdQBsAHUAaQBzADAANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcGF1bHVpczA0LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3BhdWx1aXMwNC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Pavan96a,
	Annote = {Filed under Baroclinic Eddy Parameterizations.},
	Author = {V. Pavan},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {55--72},
	Title = {Sensitivity of a multi-layer quasi-geostrophic $\beta$--channel to the vertical structure of the equilibrium meridional temperature gradient},
	Volume = 122,
	Year = 1996}

@article{Pavan96b,
	Annote = {Filed under Baroclinic Eddy Parameterizations.},
	Author = {V. Pavan and I. M. Held},
	Journal = {J. Atmos. Sci.},
	Pages = {1262--1272},
	Title = {The diffusive approximation for eddy fluxes in baroclinically unstable jets},
	Volume = 53,
	Year = 1996}

@article{Pearson01,
	Annote = {Tropics warmer than previously thought in Late
                  Cretaceous and Eocene.},
	Author = {P. N. Pearson and P. W. Ditchfield and J. Singano and K. G. Harcourt-Brown and C. J. Nicholas and R. K. Olsson and N. J. Shackleton and M. A. Hall},
	Journal = {Nature},
	Pages = {481--487},
	Title = {Warm tropical sea surface temperatures in the {L}ate {C}retaceous and {E}ocene epochs},
	Volume = 413,
	Year = 2001}

@article{Pedlosky70,
	Annote = {Weakly nonlinear waves in two-layer model.},
	Author = {J. Pedlosky},
	File = {../../Papers/pedlosky70.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {15--30},
	Title = {Finite-amplitude baroclinic waves},
	Volume = 27,
	Year = 1970,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5wZWRsb3NreTcwLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKNwvcAfFBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwvdi7AAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGVkbG9za3k3MC5wZGYAAA4AHgAOAHAAZQBkAGwAbwBzAGsAeQA3ADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3BlZGxvc2t5NzAucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3BlZGxvc2t5NzAucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Pedlosky75,
	Annote = {Marginally stable at minimum critical shear unstable
                  to perturbations with meridional scale of order
                  Rossby radius.},
	Author = {J. Pedlosky},
	File = {../../Papers/pedlosky75.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {603--607},
	Title = {On secondary instability and the meridional scale of motion in the ocean},
	Volume = 5,
	Year = 1975,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5wZWRsb3NreTc1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKOwOJ0YwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwOLW0wAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGVkbG9za3k3NS5wZGYAAA4AHgAOAHAAZQBkAGwAbwBzAGsAeQA3ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3BlZGxvc2t5NzUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3BlZGxvc2t5NzUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Pedlosky76,
	Annote = {Weakly nonlinear waves in two-layer model.},
	Author = {J. Pedlosky},
	File = {../../Papers/pedlosky76.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {621--637},
	Title = {On the dynamics of finite-amplitude baroclinic waves as a function of supercriticality},
	Volume = 78,
	Year = 1976,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5wZWRsb3NreTc2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKPvizuZgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvi1e5gAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGVkbG9za3k3Ni5wZGYAAA4AHgAOAHAAZQBkAGwAbwBzAGsAeQA3ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3BlZGxvc2t5NzYucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3BlZGxvc2t5NzYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Pedlosky79,
	Annote = {Weakly nonlinear waves in Charney model.},
	Author = {J. Pedlosky},
	File = {../../Papers/pedlosky79.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1908--1924},
	Title = {Finite-amplitude baroclinic waves in a continuous model of the atmosphere},
	Volume = 36,
	Year = 1979,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5wZWRsb3NreTc5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKQvip3BwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvirnhwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGVkbG9za3k3OS5wZGYAAA4AHgAOAHAAZQBkAGwAbwBzAGsAeQA3ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3BlZGxvc2t5NzkucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3BlZGxvc2t5NzkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Pedlosky82a,
	Annote = {.},
	Author = {J. Pedlosky},
	File = {../../Papers/pedlosky82a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {555--562},
	Title = {Finite-amplitude baroclinic waves at minimum critical shear},
	Volume = 39,
	Year = 1982,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9wZWRsb3NreTgyYS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKTvIcLwgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvId8QgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGVkbG9za3k4MmEucGRmAA4AIAAPAHAAZQBkAGwAbwBzAGsAeQA4ADIAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvcGVkbG9za3k4MmEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvcGVkbG9za3k4MmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Pedlosky82b,
	Annote = {.},
	Author = {J. Pedlosky},
	File = {../../Papers/pedlosky82b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2119--2127},
	Title = {A minimum model for nonlinear critical layers in an unstable baroclinic wave},
	Volume = 39,
	Year = 1982,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9wZWRsb3NreTgyYi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKUvIcMbAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvId87AAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGVkbG9za3k4MmIucGRmAA4AIAAPAHAAZQBkAGwAbwBzAGsAeQA4ADIAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvcGVkbG9za3k4MmIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvcGVkbG9za3k4MmIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@book{Pedlosky87,
	Address = {New York},
	Author = {J. Pedlosky},
	Edition = {2nd},
	Pages = 710,
	Publisher = {Springer},
	Title = {Geophysical Fluid Dynamics},
	Year = 1987}

@book{Peixoto92,
	Author = {J. P. Peixoto and A. H. Oort},
	Pages = 555,
	Publisher = {American Institute of Physics},
	Title = {Physics of Climate},
	Year = 1992}

@article{Peixoto96,
	Author = {J. P. Peixoto and A. H. Oort},
	File = {../../Papers/peixoto96.pdf},
	Journal = {J. Climate},
	Pages = {3443--3463},
	Title = {The Climatology of Relative Humidity in the Atmosphere},
	Volume = 9,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1wZWl4b3RvOTYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKWvsnNlQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvsowBQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGVpeG90bzk2LnBkZgAOABwADQBwAGUAaQB4AG8AdABvADkANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcGVpeG90bzk2LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3BlaXhvdG85Ni5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Penland89,
	Author = {C. Penland},
	Journal = {Mon. Wea. Rev.},
	Pages = {2165--2185},
	Title = {Random Forcing and Forecasting Using {P}rincipal {O}scillation {P}attern Analysis},
	Volume = 117,
	Year = 1989}

@article{Penland94,
	Annote = {Fluctuation-dissipation theorem.},
	Author = {C. Penland and L. Matrosova},
	Journal = {J. Climate},
	Pages = {1352--1372},
	Title = {A Balance Condition for Stochastic Numerical Models with Applications to the {E}l {N}i{\~n}o-{S}outhern {O}scillation},
	Volume = 7,
	Year = 1994}

@article{Penland95a,
	Annote = {Consider error propagation from errors in matrix
                  entries to eigenvectors and eigenvalues. To estimate
                  errors in eigenmodes of AR process, they use a
                  Monte-Carlo method first to get errors in
                  coefficient matrix and then consider error
                  propagation. Expensive, in particular because they
                  use Ornstein-Uhlenbeck processes and integrate by
                  direct simulation.},
	Author = {C. Penland and P. D. Sardeshmukh},
	Journal = {J. Climate},
	Pages = {1988--1998},
	Title = {Error and Sensitivity Analysis of Geophysical Eigensystems},
	Volume = 8,
	Year = 1995}

@article{Penland95b,
	Annote = {AR(1) modeling of SST anomalies. No diagnostic
                  checking.},
	Author = {C. Penland and P. D. Sardeshmukh},
	Journal = {J. Climate},
	Pages = {1999--2024},
	Title = {The Optimal Growth of Tropical Sea Surface Temperature Anomalies},
	Volume = 8,
	Year = 1995}

@article{Peters05,
	Annote = {Filed under Bretherton.},
	Author = {M. E. Peters and C. S. Bretherton},
	File = {../../Papers/peters05.pdf},
	Journal = {J. Climate},
	Pages = {4216--4234},
	Title = {A Simplified Model of the {Walker} Circulation with an Interactive Ocean Mixed Layer and Cloud-Radiative Feedbacks},
	Volume = 18,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxwZXRlcnMwNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKdv6o8SQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv6qsyQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGV0ZXJzMDUucGRmAAAOABoADABwAGUAdABlAHIAcwAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3BldGVyczA1LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9wZXRlcnMwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@book{Petty06,
	Address = {Madison, Wisconsin},
	Author = {G. W. Petty},
	Edition = {2nd},
	Pages = {470},
	Publisher = {Sundog Publishing},
	Title = {A First Course in Atmospheric Radiation},
	Year = 2006}

@article{Pfeffer81,
	Author = {R. L. Pfeffer},
	Journal = {J. Atmos. Sci.},
	Pages = {1340--1359},
	Title = {Wave-mean flow interaction in the atmosphere},
	Volume = 38,
	Year = 1981}

@unpublished{Philander96,
	Annote = {Mainly student seminar. Term paper on Jin-Neelin
                  model of ENSO.},
	Author = {S. G. Philander},
	Note = {Lecture Notes},
	Title = {Physical Oceanography},
	Year = {Spring 1996}}

@article{Phillips54,
	Annote = {Classic paper on two-layer model.},
	Author = {N. A. Phillips},
	File = {../../Papers/phillips54.pdf},
	Journal = {Tellus},
	Pages = {273--286},
	Title = {Energy Transformations and Meridional Circulations Associated with Simple Baroclinic Waves in a Two-Level, Quasi-Geostrophic Model},
	Volume = 6,
	Year = 1954,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5waGlsbGlwczU0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKhxAafcAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxAcB4AAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGhpbGxpcHM1NC5wZGYAAA4AHgAOAHAAaABpAGwAbABpAHAAcwA1ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3BoaWxsaXBzNTQucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3BoaWxsaXBzNTQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Phillips56,
	Annote = {Filed under General Circulation History.},
	Author = {N. A. Phillips},
	File = {../../Papers/phillips56.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {123--164},
	Title = {The general circulation of the atmosphere: a numerical experiment},
	Volume = 82,
	Year = 1956,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5waGlsbGlwczU2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKiw7m0PFBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7okvAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGhpbGxpcHM1Ni5wZGYAAA4AHgAOAHAAaABpAGwAbABpAHAAcwA1ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3BoaWxsaXBzNTYucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3BoaWxsaXBzNTYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Phillips96,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {L. Phillips},
	Journal = {J. Plasma Phys.},
	Pages = {531--551},
	Title = {States of minimum dissipation in magnetohydrodynamics: a review},
	Volume = 56,
	Year = 1996}

@article{Piegorsch98,
	Annote = {Filed under Climate Change Detection. Review of
                  evironmetrics after 1992.},
	Author = {W. W. Piegorsch and E. P. Smith and D. Edwards and R. L. Smith},
	Journal = {Statist. Sci.},
	Pages = {186--208},
	Title = {Statistical Advances in Environmental Sciences},
	Volume = 13,
	Year = 1998}

@article{Pierrehumbert,
	Annote = {Filed under Snowball Earth.},
	Author = {R. T. Pierrehumbert},
	Journal = {Nature},
	Title = {High levels of atmospheric carbon dioxide necessary for the termination of global glaciation},
	Volume = 429,
	Year = 2004}

@article{Pierrehumbert00,
	Author = {R. T. Pierrehumbert},
	File = {../../Papers/pierrehumbert00.pdf},
	Journal = {Proc. Natl. Acad. Sci.},
	Note = {doi:10.1073/pnas.97.4.1355},
	Pages = {1355-1358},
	Title = {Climate change and the tropical {P}acific: The sleeping dragon wakes},
	Volume = 97,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYAAAAAAAYAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhNwaWVycmVodW1iZXJ0MDAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKjxfZUcgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxfa24gAAAAEADAAJDH4ACE6zAACS8wACADJNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGllcnJlaHVtYmVydDAwLnBkZgAOACgAEwBwAGkAZQByAHIAZQBoAHUAbQBiAGUAcgB0ADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACZVc2Vycy90YXBpby9QYXBlcnMvcGllcnJlaHVtYmVydDAwLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAgLi4vLi4vUGFwZXJzL3BpZXJyZWh1bWJlcnQwMC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACJAImAisCNAI/AkMCUQJYAmEChAKJAowCmQKeAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAArA=}}

@article{Pierrehumbert02,
	Annote = {Review of possible Snowball Earth dynamics; water
                  vapor feedbacks.},
	Author = {R. T. Pierrehumbert},
	File = {../../Papers/pierrehumbert02.pdf},
	Journal = {Nature},
	Pages = {191--198},
	Title = {The hydrologic cycle in deep-time climate problems},
	Volume = 419,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYAAAAAAAYAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhNwaWVycmVodW1iZXJ0MDIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKkwnvS8lBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwnw1YgAAAAEADAAJDH4ACE6zAACS8wACADJNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGllcnJlaHVtYmVydDAyLnBkZgAOACgAEwBwAGkAZQByAHIAZQBoAHUAbQBiAGUAcgB0ADAAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACZVc2Vycy90YXBpby9QYXBlcnMvcGllcnJlaHVtYmVydDAyLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAgLi4vLi4vUGFwZXJzL3BpZXJyZWh1bWJlcnQwMi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACJAImAisCNAI/AkMCUQJYAmEChAKJAowCmQKeAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAArA=}}

@incollection{Pierrehumbert07a,
	Address = {Princeton, NJ},
	Author = {R. T. Pierrehumbert and H. Brogniez and R. Roca},
	Booktitle = {The Global Circulation of the Atmosphere},
	Date-Modified = {2010-06-12 10:17:27 -0700},
	Editor = {T. Schneider and A. H. Sobel},
	Pages = {143--185},
	Publisher = {Princeton University Press},
	Title = {On the Relative Humidity of the Atmosphere},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYYAAAAAAYYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhRwaWVycmVodW1iZXJ0MDdhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKmwoR65QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwoTdVQAAAAEADAAJDH4ACE6zAACS8wACADNNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGllcnJlaHVtYmVydDA3YS5wZGYAAA4AKgAUAHAAaQBlAHIAcgBlAGgAdQBtAGIAZQByAHQAMAA3AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAnVXNlcnMvdGFwaW8vUGFwZXJzL3BpZXJyZWh1bWJlcnQwN2EucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAhLi4vLi4vUGFwZXJzL3BpZXJyZWh1bWJlcnQwN2EucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAioCLAIxAjoCRQJJAlcCXgJnAosCkAKTAqACpQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAK3}}

@article{Pierrehumbert91,
	Annote = {Introduction to chaotic mixing concepts.},
	Author = {R. Pierrehumbert},
	File = {../../Papers/pierrehumbert91.pdf},
	Journal = {Geophys. Astrophys. Fluid. Dyn.},
	Pages = {285--320},
	Title = {Chaotic Mixing of Tracer and Vorticity by Modulated Traveling Rossby Waves},
	Volume = 58,
	Year = 1991,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYAAAAAAAYAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhNwaWVycmVodW1iZXJ0OTEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKoxJuHAwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxJvpcwAAAAEADAAJDH4ACE6zAACS8wACADJNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGllcnJlaHVtYmVydDkxLnBkZgAOACgAEwBwAGkAZQByAHIAZQBoAHUAbQBiAGUAcgB0ADkAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACZVc2Vycy90YXBpby9QYXBlcnMvcGllcnJlaHVtYmVydDkxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAgLi4vLi4vUGFwZXJzL3BpZXJyZWh1bWJlcnQ5MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACJAImAisCNAI/AkMCUQJYAmEChAKJAowCmQKeAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAArA=}}

@article{Pierrehumbert93,
	Annote = {Considers mixing of passive tracers on 315K
                  isentrope. Barrier to mixing at the boundary of
                  tropics and extratropics (critical
                  layer?). Coarse-grained homogenization of tracer
                  outside the tropics on time scales of order 50
                  days. Generation of microstructure by coarse-grained
                  advecting velocity field. Meridional mixing is
                  diffusive on time scales longer than about 30 days
                  (i.e., the meridional tracer variance increases
                  linearly). By way of contrast, zonal mixing is
                  superdiffusive. (That means that diffusive closure
                  of zonal mean flow might be possible, but zonal
                  variations are more difficult to take into account.)
                  Mixing regions are zonally symmetric (e.g., no
                  signatures of storm tracks visible).},
	Author = {R. T. Pierrehumbert and H. Yang},
	File = {../../Papers/pierrehumbert93.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2462--2480},
	Title = {Global chaotic mixing on isentropic surfaces},
	Volume = 50,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYAAAAAAAYAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhNwaWVycmVodW1iZXJ0OTMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKpv7ZBKgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv7axqgAAAAEADAAJDH4ACE6zAACS8wACADJNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGllcnJlaHVtYmVydDkzLnBkZgAOACgAEwBwAGkAZQByAHIAZQBoAHUAbQBiAGUAcgB0ADkAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACZVc2Vycy90YXBpby9QYXBlcnMvcGllcnJlaHVtYmVydDkzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAgLi4vLi4vUGFwZXJzL3BpZXJyZWh1bWJlcnQ5My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACJAImAisCNAI/AkMCUQJYAmEChAKJAowCmQKeAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAArA=}}

@article{Pierrehumbert94,
	Annote = {Filed under Held.},
	Author = {R. T. Pierrehumbert and I. M. Held},
	Journal = {Chaos, Solitons \& Fractals},
	Pages = {1111--1116},
	Title = {Spectra of Local and Nonlocal Two-dimensional Turbulence},
	Volume = 4,
	Year = 1994}

@article{Pierrehumbert95,
	Annote = {Review of baroclinic instability:
                  linear models, (Eady, Charney), nonlinear
                  lifecycles, equilibration.},
	Author = {R. T. Pierrehumbert and K. L. Swanson},
	Date-Modified = {2010-06-11 10:58:34 -0700},
	File = {../../Papers/pierrehumbert95.pdf},
	Journal = {Annu. Rev. Fluid Mech.},
	Pages = {419--467},
	Title = {Baroclinic Instability},
	Volume = 27,
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYAAAAAAAYAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhNwaWVycmVodW1iZXJ0OTUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKqvxkZkwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvxl8AwAAAAEADAAJDH4ACE6zAACS8wACADJNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGllcnJlaHVtYmVydDk1LnBkZgAOACgAEwBwAGkAZQByAHIAZQBoAHUAbQBiAGUAcgB0ADkANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACZVc2Vycy90YXBpby9QYXBlcnMvcGllcnJlaHVtYmVydDk1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAgLi4vLi4vUGFwZXJzL3BpZXJyZWh1bWJlcnQ5NS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACJAImAisCNAI/AkMCUQJYAmEChAKJAowCmQKeAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAArA=}}

@article{Pierrehumbert95b,
	Author = {R. T. Pierrehumbert},
	File = {../../Papers/pierrehumbert95b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1784--1806},
	Title = {Thermostats, Radiator Fins, and the local Runaway Greenhouse},
	Volume = 52,
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYYAAAAAAYYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhRwaWVycmVodW1iZXJ0OTViLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKrwT1kxgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwT3HNgAAAAEADAAJDH4ACE6zAACS8wACADNNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGllcnJlaHVtYmVydDk1Yi5wZGYAAA4AKgAUAHAAaQBlAHIAcgBlAGgAdQBtAGIAZQByAHQAOQA1AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAnVXNlcnMvdGFwaW8vUGFwZXJzL3BpZXJyZWh1bWJlcnQ5NWIucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAhLi4vLi4vUGFwZXJzL3BpZXJyZWh1bWJlcnQ5NWIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAioCLAIxAjoCRQJJAlcCXgJnAosCkAKTAqACpQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAK3}}

@article{Pierrehumbert98a,
	Author = {R. T. Pierrehumbert},
	Date-Modified = {2010-06-11 10:59:52 -0700},
	File = {../../Papers/pierrehumbert98a.pdf},
	Journal = {Geophys. Res. Lett.},
	Pages = {151--154},
	Title = {Lateral mixing as a source of subtropical water vapor},
	Volume = 25,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYYAAAAAAYYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhRwaWVycmVodW1iZXJ0OThhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKsxfZWmwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxfa5CwAAAAEADAAJDH4ACE6zAACS8wACADNNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGllcnJlaHVtYmVydDk4YS5wZGYAAA4AKgAUAHAAaQBlAHIAcgBlAGgAdQBtAGIAZQByAHQAOQA4AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAnVXNlcnMvdGFwaW8vUGFwZXJzL3BpZXJyZWh1bWJlcnQ5OGEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAhLi4vLi4vUGFwZXJzL3BpZXJyZWh1bWJlcnQ5OGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAioCLAIxAjoCRQJJAlcCXgJnAosCkAKTAqACpQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAK3}}

@article{Pierrehumbert98b,
	Author = {R. T. Pierrehumbert and R. Roca},
	Journal = {Geophys. Res. Lett.},
	Pages = {4537--4540},
	Title = {Evidence for Control of {A}tlantic Subtropical Humidity by Large Scale Advection},
	Volume = 25,
	Year = 1998}

@incollection{Pierrehumbert99,
	Address = {Washington, D.C.},
	Author = {R. T. Pierrehumbert},
	Booktitle = {Mechanisms of Global Change at Millennial Time Scales},
	Editor = {P. U. Clark and R. S. Webb and L. D. Keigwin},
	File = {../../Papers/pierrehumbert99.pdf},
	Pages = 394,
	Publisher = {American Geophysical Union},
	Title = {Subtropical water vapor as a mediator of rapid global climate change},
	Volume = 112,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYAAAAAAAYAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhNwaWVycmVodW1iZXJ0OTkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKtvChvIAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvCjfoAAAAAEADAAJDH4ACE6zAACS8wACADJNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGllcnJlaHVtYmVydDk5LnBkZgAOACgAEwBwAGkAZQByAHIAZQBoAHUAbQBiAGUAcgB0ADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACZVc2Vycy90YXBpby9QYXBlcnMvcGllcnJlaHVtYmVydDk5LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAgLi4vLi4vUGFwZXJzL3BpZXJyZWh1bWJlcnQ5OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACJAImAisCNAI/AkMCUQJYAmEChAKJAowCmQKeAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAArA=}}

@incollection{Platzman90,
	Address = {Boston, MA},
	Annote = {Interview with Charney.},
	Author = {G. W. Platzman},
	Booktitle = {The Atmosphere --- A Challenge. The Science of Jule Gregory Charney},
	Editor = {R. S. Lindzen and E. N. Lorenz and G. W. Platzman},
	Pages = {11--82},
	Publisher = {Amer. Meteor. Soc.},
	Series = {Historical Monograph Series},
	Title = {The Atmosphere --- {A} Challenge},
	Year = 1990}

@article{Plumb02,
	Annote = {Review of stratospheric transport.},
	Author = {R. A. Plumb},
	Journal = {J. Meteor. Soc. Japan},
	Pages = {793-809},
	Title = {Stratospheric transport},
	Volume = 80,
	Year = 2002}

@article{Plumb03,
	Annote = {Shows that downward migrating zonal wind anomalies
                  can arise by vertically local wave-mean flow
                  interaction, without the need for reflection of
                  waves or "downward control."},
	Author = {R. A. Plumb and K. Semeniuk},
	File = {../../Papers/plumb03.pdf},
	Journal = {J. Geophys. Res.},
	Note = {doi:10.1029/2002JD002773},
	Pages = {4223},
	Title = {Downward migration of extratropical zonal wind anomalies},
	Volume = {108D},
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtwbHVtYjAzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRKzwIUvEAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwIWRgAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGx1bWIwMy5wZGYADgAYAAsAcABsAHUAbQBiADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvcGx1bWIwMy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9wbHVtYjAzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Plumb05,
	Author = {R. A. Plumb and R. Ferrari},
	File = {../../Papers/plumb05.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {165--174},
	Title = {Transformed Eulerian-mean theory. {I}: Non-quasigeostrophic theory for eddies on a zonal mean flow},
	Volume = {35},
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtwbHVtYjA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRK0vnyHmAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvnzqCAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGx1bWIwNS5wZGYADgAYAAsAcABsAHUAbQBiADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvcGx1bWIwNS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9wbHVtYjA1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@incollection{Plumb07a,
	Address = {Princeton, NJ},
	Author = {R. A. Plumb},
	Booktitle = {The Global Circulation of the Atmosphere},
	Editor = {T. Schneider and A. H. Sobel},
	Pages = {252--266},
	Publisher = {Princeton University Press},
	Title = {Dynamical Constraints on Monsoon Circulations},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxwbHVtYjA3YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRK2woWdRwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwoX/twAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGx1bWIwN2EucGRmAAAOABoADABwAGwAdQBtAGIAMAA3AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3BsdW1iMDdhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9wbHVtYjA3YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Plumb07b,
	Author = {R. A. Plumb},
	Journal = {Rev. Geophys.},
	Pages = {RG4005},
	Title = {Tracer Interrelationships in the Stratosphere},
	Volume = 45,
	Year = 2007}

@article{Plumb79,
	Author = {R. A. Plumb},
	Journal = {J. Atmos. Sci.},
	Pages = {1699--1704},
	Title = {Eddy Fluxes of Conserved Quantities by Small-Amplitude Waves},
	Volume = {36},
	Year = {1979}}

@article{Plumb83,
	Annote = {Different conversions in TEM dynamics.},
	Author = {R. A. Plumb},
	Journal = {J. Atmos. Sci.},
	Pages = {1669--1688},
	Title = {A new look at the energy cycle},
	Volume = 40,
	Year = 1983}

@article{Plumb86,
	Author = {R. A. Plumb},
	File = {../../Papers/plumb86.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1657--1678},
	Title = {Three-Dimensional Propagation of Transient Quasi-Geostrophic Eddies and Its Relationship with the Eddy Forcing of the Time-Mean Flow},
	Volume = 43,
	Year = 1986,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtwbHVtYjg2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRK6w+jIJFBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw+k4pAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGx1bWI4Ni5wZGYADgAYAAsAcABsAHUAbQBiADgANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvcGx1bWI4Ni5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9wbHVtYjg2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Plumb87,
	Author = {R. A. Plumb and J. D. Mahlman},
	Journal = {J. Atmos. Sci.},
	Pages = {298--327},
	Title = {The Zonally Averaged Transport Characteristics of the {GFDL} General Circulation/Transport Model},
	Volume = 44,
	Year = 1987}

@article{Plumb92,
	Author = {R. A. Plumb and A. Y. Hou},
	File = {../../Papers/plumb92.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1790--1799},
	Title = {The response of a zonally symmetric atmosphere to subtropical thermal forcing: {T}hreshold behavior},
	Volume = 49,
	Year = 1992,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtwbHVtYjkyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRK7v00PG1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv01xiwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cGx1bWI5Mi5wZGYADgAYAAsAcABsAHUAbQBiADkAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvcGx1bWI5Mi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9wbHVtYjkyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Plumb99,
	Annote = {Filed under Hadley Cell Dynamics. Stratospheric
                  "Hadley cell" dynamics. Role of extratropical wave
                  drag and tropical heating in tropical
                  upwelling. Small viscous effects essential in
                  tropics to allow wave-driven circulation to cross
                  angular momentum contours.},
	Author = {R. A. Plumb and J. Eluszkiewicz},
	Journal = {J. Atmos. Sci.},
	Pages = {868--890},
	Title = {The {Brewer}-{Dobson} Circulation: Dynamics of the Tropical Upwelling},
	Volume = 56,
	Year = 1999}

@article{Polvani02a,
	Annote = {Cooling in polar stratosphere induces poleward
                  movement of tropospheric jet. Dynamical connection
                  between stratosphere and troposphere not
                  clear. (Does not appear to be "downward control.)"},
	Author = {L. M. Polvani and P. J. Kushner},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.129/2001/GL014284},
	Title = {Tropospheric response to stratospheric perturbations in a relatively simple general circulation model},
	Volume = 29,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5wb2x2YW5pMDJhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRK+yEUBsQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEVkIQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cG9sdmFuaTAyYS5wZGYAAA4AHgAOAHAAbwBsAHYAYQBuAGkAMAAyAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3BvbHZhbmkwMmEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3BvbHZhbmkwMmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Polvani02b,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {L. M. Polvani and A. H. Sobel},
	Journal = {J. Atmos. Sci.},
	Pages = {1744--1752},
	Title = {The {H}adley Circulation and the Weak Temperature Gradient Approximation},
	Volume = 59,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5wb2x2YW5pMDJiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRK/yEUBkwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEVkAwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cG9sdmFuaTAyYi5wZGYAAA4AHgAOAHAAbwBsAHYAYQBuAGkAMAAyAGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3BvbHZhbmkwMmIucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3BvbHZhbmkwMmIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Polyakov01,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {I. Polyakov},
	Journal = {J. Phys. Oceanogr.},
	Pages = {2255--2270},
	Title = {An eddy parameterization based on maximum entropy production with application to modeling of the {A}rctic {O}cean circulation},
	Volume = 31,
	Year = 2001}

@article{Pope94,
	Annote = {Filed under Stochastic Lagrangian Models of
                  Turbulence. Review of pdf methods, Langevin
                  equation, particle representations. Brief mention of
                  passive scalar problem.},
	Author = {S. B. Pope},
	File = {../../Papers/pope94.pdf},
	Journal = {Annu. Rev. Fluid Mech.},
	Pages = {23--63},
	Title = {Lagrangian PDF Methods for Turbulent Flows},
	Volume = 26,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpwb3BlOTQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLDv5GlZ1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5IV5wAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cG9wZTk0LnBkZgAADgAWAAoAcABvAHAAZQA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3BvcGU5NC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvcG9wZTk0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Porco03,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {Porco, C.C. and West, R.A. and McEwen, A. and {Del~Genio}, A.D. and Ingersoll, A.P. and Thomas, P. and Squyres, S. and Dones, L. and Murray, C.D. and Johnson, T.V. and others},
	File = {../../Papers/porco03.pdf},
	Journal = {Science},
	Pages = {1541--1547},
	Title = {Cassini Imaging of {J}upiter's atmosphere, satellites, and rings},
	Volume = 299,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtwb3JjbzAzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLFw1AcCFBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw1B+eAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cG9yY28wMy5wZGYADgAYAAsAcABvAHIAYwBvADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvcG9yY28wMy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9wb3JjbzAzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@book{PrakasaRao83,
	Address = {Orlando, FL},
	Annote = {Excerpted copies filed under Entropy Estimation.},
	Author = {B. L. S. {Prakasa Rao}},
	Pages = 522,
	Publisher = {Academic Press},
	Series = {Series in Probability and Mathematical Statistics},
	Title = {Nonparametric Functional Estimation},
	Year = 1983}

@inproceedings{Prandtl05,
	Address = {Teubner, Leipzig},
	Author = {L. Prandtl},
	Booktitle = {Verhandlungen des dritten internationalen Mathematiker-Kongresses (Heidelberg 1904)},
	File = {../../Papers/prandtl05.pdf},
	Pages = {484--491},
	Title = {{\"U}ber {F}l{\"u}ssigkeitsbewegung bei sehr kleiner {R}eibung},
	Year = 1905,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1wcmFuZHRsMDUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLIvnh4qgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvnjbGgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cHJhbmR0bDA1LnBkZgAOABwADQBwAHIAYQBuAGQAdABsADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcHJhbmR0bDA1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3ByYW5kdGwwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@book{Press92,
	Author = {W. H. Press and S. A. Teukolsky and W. T. Vetterling and B. P. Flannery},
	Edition = {2nd},
	Pages = 963,
	Publisher = {Cambridge University Press},
	Title = {Numerical Recipes},
	Year = 1992}

@article{Previdi07,
	Author = {M. Previdi and B. G. Liepert},
	File = {../../Papers/previdi07.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2007GL031243},
	Pages = {L22701},
	Title = {Annular modes and {H}adley cell expansion under global warming},
	Volume = 34,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1wcmV2aWRpMDcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLJxcR8VwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxcTs1wAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cHJldmlkaTA3LnBkZgAOABwADQBwAHIAZQB2AGkAZABpADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcHJldmlkaTA3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3ByZXZpZGkwNy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Prive07a,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {N. C. Priv{\'e} and R. A. Plumb},
	File = {../../Papers/prive07a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1417--1430},
	Title = {Monsoon dynamics with interactive forcing. {P}art~{I}: {A}xisymmetric studies},
	Volume = {64},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxwcml2ZTA3YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLKwnEKoQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwnFtEQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cHJpdmUwN2EucGRmAAAOABoADABwAHIAaQB2AGUAMAA3AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3ByaXZlMDdhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9wcml2ZTA3YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Prive07b,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {N. C. Priv{\'e} and R. A. Plumb},
	File = {../../Papers/prive07b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1431--1442},
	Title = {Monsoon dynamics with interactive forcing. {P}art~{II}: {I}mpact of eddies and asymmetric geometries},
	Volume = {64},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxwcml2ZTA3Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLLwnEK0QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwnFtQQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cHJpdmUwN2IucGRmAAAOABoADABwAHIAaQB2AGUAMAA3AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3ByaXZlMDdiLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9wcml2ZTA3Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Pullin00,
	Author = {D. I. Pullin},
	Journal = {Phys. Fluids},
	Pages = {2311--2319},
	Title = {A vortex-based model for the subgrid flux of a passive scalar},
	Volume = 12,
	Year = 2000}

@article{Pullin01,
	Author = {D. I. Pullin and T. S. Lundgren},
	Journal = {Phys. Fluids},
	Pages = {2552--2563},
	Title = {Axial motion and scalar transport in stretched spiral vortices},
	Volume = 13,
	Year = 2001}

@incollection{Quan04,
	Author = {Quan, X. W. and Diaz, H. F. and Hoerling, M. P.},
	Booktitle = {The Hadley Circulation: Past, Present, and Future},
	Editor = {Diaz, Henry F. and Bradley, Raymond S.},
	File = {../../Papers/quan04.pdf},
	Pages = {85--120},
	Publisher = {Springer},
	Series = {Advances in Global Change Research},
	Title = {Change in the tropical {Hadley} cell since 1950},
	Volume = 21,
	Year = {2004},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpxdWFuMDQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLMx8kCTwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx8lkvwAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cXVhbjA0LnBkZgAADgAWAAoAcQB1AGEAbgAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3F1YW4wNC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvcXVhbjA0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Rahmstorf02,
	Annote = {Filed under Paleo-Climate Reviews.},
	Author = {S. Rahmstorf},
	Journal = {Nature},
	Pages = {207--214},
	Title = {Ocean circulation and climate during the past 120,000 years},
	Volume = 419,
	Year = 2002}

@article{Rahmstorf95b,
	Annote = {Not on file. Study sensitivity of North Atlantic
                  thermohaline circulatio to changes in the input of
                  freshwater using global ocean circulation model
                  coupled to a simplified model atmosphere. Transition
                  between equilibrium states result from moderate
                  changes in freshwater input.},
	Author = {S. Rahmstorf},
	Journal = {Nature},
	Pages = {145--149},
	Title = {Bifurcations of the {A}tlantic Thermohaline Circulation in Response to Changes in the Hydrological Cycle},
	Volume = 378,
	Year = 1995}

@article{Ramanathan01,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {V. Ramanathan and P. J. Crutzen and J. T. Kiehl and D. Rosenfeld},
	Journal = {Science},
	Pages = {2119--2124},
	Title = {Aerosols, Climate, and the Hydrological Cycle},
	Volume = 294,
	Year = 2001}

@incollection{Randall07,
	Address = {Cambridge, UK, and New York, NY, USA},
	Author = {D. A. Randall and R. A. Wood and S. Bony and R. Colman and T. Fichefet and J. Fyfe and V. Kattsov and A. Pitman and J. Shukla and J. Srinivasan and R. J. Stouffer and A. Sumi and K. E. Taylor},
	Booktitle = {Climate Change 2007: The Physical Science Basis. Contribution of Working Group I to the Fourth Assessment Report of the Intergovernmental Panel on Climate Change},
	Editor = {S. Solomon and D. Qin and M. Manning and Z. Chen and M. Marquis and K.B. Averyt and M. Tignor and H.L. Miller},
	Pages = {590--662},
	Publisher = {Cambridge Univ. Press},
	Title = {Climate Models and Their Evaluation},
	Year = 2007}

@article{Randall92,
	Author = {Randall, D. A. and Cess, R. D. and Blanchet, J. P. and Boer, G. J. and Dazlich, D. A. and {DelGenio}, A. D. and Deque, M. and Dymnikov, V. and Galin, V. and Ghan, S. J. and others},
	Date-Modified = {2010-06-11 11:00:46 -0700},
	File = {../../Papers/randall92.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {3711--3724},
	Title = {Intercomparison and interpretation of surface energy fluxes in atmospheric general circulation models},
	Volume = {97D},
	Year = {1992},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1yYW5kYWxsOTIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLPxT4YxAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxT6JRAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmFuZGFsbDkyLnBkZgAOABwADQByAGEAbgBkAGEAbABsADkAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcmFuZGFsbDkyLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3JhbmRhbGw5Mi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Randel91a,
	Author = {W. J. Randel and I. M. Held},
	Date-Modified = {2010-06-21 10:37:17 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {688--697},
	Title = {Phase speed spectra of transient eddy fluxes and critical layer absorption},
	Volume = 48,
	Year = 1991,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1yYW5kZWw5MWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLUyETxQgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyEVTsgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmFuZGVsOTFhLnBkZgAOABwADQByAGEAbgBkAGUAbAA5ADEAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcmFuZGVsOTFhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3JhbmRlbDkxYS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Randerson02,
	Author = {J. T. Randerson and C. J. Still and J. J. Ball{\'e} and I. Y. Fung and S. C. Doney and P. P. Tans and T. J. Conway and J. W. C. White and B. Vaughn and N. Suits and A. S. Denning},
	Journal = {Global Biogeochem. Cycles},
	Pages = {10.1029/2001GB001435},
	Title = {Carbon isotope discrimination of arctic and boreal biomes inferred from remote atmospheric measurements and a biosphere--atmosphere model},
	Volume = 16,
	Year = 2002}

@article{Raval89,
	Annote = {Filed under Water Vapor Feedback (Feedback and
                  Kinematics).},
	Author = {A. Raval and V. Ramanathan},
	Journal = {Nature},
	Pages = {758--761},
	Title = {Observational Determination of the Greenhouse Effect},
	Volume = 342,
	Year = 1989}

@article{Read04,
	Annote = {Experiment with rotating tank onto which denser
                  liquid was sprayed, leading to vortices, an inverse
                  energy cascade, and the formation of zonal jets. No
                  large-scale temperature (density) gradient in experiment.},
	Author = {P. L. Read and Y. H. Yamazaki and S. R. Lewis and P. D. Williams and K. Miki-Yamazaki and J. Sommeria and H. Didelle and A. Fincham},
	File = {../../Papers/read04.pdf},
	Journal = {Geophys. Res. Lett.},
	Title = {Jupiter's and {Saturn}'s convectively banded jets in the laboratory},
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpyZWFkMDQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLbwst65VBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsvdVQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmVhZDA0LnBkZgAADgAWAAoAcgBlAGEAZAAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3JlYWQwNC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvcmVhZDA0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Read06,
	Author = {P. L. Read and P. J. Gierasch and B. J. Conrath and A. Simon-Miller and T. Fouchet and Y. H. Yamazaki},
	File = {../../Papers/read06.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1577--1603},
	Title = {Mapping potential-vorticity dynamics on {Jupiter}. {I}. {Z}onal-mean circulation from {Cassini} and {Voyager}~1 data},
	Volume = 132,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpyZWFkMDYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLcw18qswAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw1+bMwAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmVhZDA2LnBkZgAADgAWAAoAcgBlAGEAZAAwADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3JlYWQwNi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvcmVhZDA2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Read06b,
	Author = {P. L. Read and P. J. Gierasch and B. J. Conrath},
	File = {../../Papers/read06b.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1605--1625},
	Title = {Mapping potential-vorticity dynamics on Jupiter. {II}: the {Great} {Red} {Spot} from {Voyager 1} and 2 data},
	Volume = {132},
	Year = {2006},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtyZWFkMDZiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLdxkXCcgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxkYk4gAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmVhZDA2Yi5wZGYADgAYAAsAcgBlAGEAZAAwADYAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvcmVhZDA2Yi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9yZWFkMDZiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Read09,
	Author = {P. L. Read and T. E. Dowling and G. Schubert},
	File = {../../Papers/read09.pdf},
	Journal = {Nature},
	Pages = {608--610},
	Title = {Saturn's rotation period from its atmospheric planetary-wave configuration},
	Volume = 460,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpyZWFkMDkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLfxzVP5gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxzXAZgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmVhZDA5LnBkZgAADgAWAAoAcgBlAGEAZAAwADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3JlYWQwOS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvcmVhZDA5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Read09b,
	Author = {P. L. Read and B. J. Conrath and L. N. Fletcher and P. J. Gierasch and A. A. Simon-Miller and L. C. Zuchowski},
	File = {../../Papers/read09b.pdf},
	Journal = {Planet. Space Sci.},
	Pages = {1682--1698},
	Title = {Mapping potential vorticity dynamics on saturn: Zonal mean circulation from {Cassini} and {Voyager} data},
	Volume = 57,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtyZWFkMDliLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLgx2wBPAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx2xxvAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmVhZDA5Yi5wZGYADgAYAAsAcgBlAGEAZAAwADkAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvcmVhZDA5Yi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9yZWFkMDliLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Read86a,
	Author = {P. L. Read},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {231--251},
	Title = {Super-rotation and diffusion of axial angular momentum: {I}. '{S}peed limits' for axisymmetric flow in a rotating cylindrical fluid annulus},
	Volume = 112,
	Year = 1986}

@article{Read86b,
	Author = {P. L. Read},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {253--272},
	Title = {Super-rotation and diffusion of axial angular momentum: {II}. {A} review of quasi-axisymmetric models of planetary atmospheres},
	Volume = 112,
	Year = 1986}

@article{Read86c,
	Author = {P. L. Read},
	Journal = {J. Fluid. Mech.},
	Pages = {255--289},
	Title = {Regimes of axisymmetric flow in an internally heated rotating fluid},
	Volume = 168,
	Year = 1986}

@article{Reed88,
	Author = {Reed, R. J. and Simmons, A. J. and Albright, M. D. and Und{\'e}n, P.},
	Journal = {Wea. Forecast.},
	Pages = {217--229},
	Title = {The Role of Latent Heat Release in Explosive Cyclogenesis: {T}hree Examples Based on {ECMWF} Operational Forecasts},
	Volume = {3},
	Year = {1988}}

@article{Reid96,
	Annote = {Not on file.},
	Author = {G. C. Reid and K. S. Gage},
	Journal = {J. Geophys. Res.},
	Pages = {21233--21241},
	Title = {The tropical tropopause over the western {P}acific: Wave driving, convection, and the annual cycle},
	Volume = {101D},
	Year = 1996}

@article{Renwick95,
	Annote = {Filed under Predictability. Use a 'predictable
                  component analysis' as we did; only read paper in
                  2002.},
	Author = {J. A. Renwick and J. M. Wallace},
	Journal = {Mon. Wea. Rev.},
	Pages = {2114--2131},
	Title = {Predictable Anomaly Patterns and the Forecast Skill of {N}orthern {H}emisphere Wintertime 500-mb Height Fields},
	Volume = 123,
	Year = 1995}

@article{Reynolds02,
	Annote = {Filed under Stochastic Lagrangian Models of Turbulence.},
	Author = {A. M. Reynolds},
	File = {../../Papers/reynolds02.pdf},
	Journal = {Phys. Fluids},
	Pages = {1442--1449},
	Title = {Lagrangian stochastoc modeling of anomalous diffusion in two-dimensional turbulence},
	Volume = 14,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5yZXlub2xkczAyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLmv5Gf01BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5IQUwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmV5bm9sZHMwMi5wZGYAAA4AHgAOAHIAZQB5AG4AbwBsAGQAcwAwADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3JleW5vbGRzMDIucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3JleW5vbGRzMDIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@book{Reza61,
	Address = {New York},
	Author = {F. M. Reza},
	Pages = {496},
	Publisher = {McGraw-Hill},
	Title = {An Introduction to Information Theory},
	Year = 1961}

@article{Reznik01,
	Annote = {Filed under Quasigeostrophy -- Alternatives and
                  Higher Order Corrections.},
	Author = {G. M. Reznik and V. Zeitlin and M. Ben Jelloul},
	Journal = {J. Fluid Mech.},
	Pages = {93--120},
	Title = {Nonlinear theory of geostrophic adjustment. {Part 1}. Rotating shallow-water model},
	Volume = 445,
	Year = 2001}

@article{Rhines75,
	Annote = {Introduces Rhines scale.},
	Author = {P. B. Rhines},
	File = {../../Papers/rhines75.pdf},
	Journal = {J. Fluid. Mech.},
	Pages = {417--443},
	Title = {Waves and Turbulence on a $\beta$-plane},
	Volume = 69,
	Year = 1975,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxyaGluZXM3NS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLow3rWVAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw3tG1AAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmhpbmVzNzUucGRmAAAOABoADAByAGgAaQBuAGUAcwA3ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3JoaW5lczc1LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9yaGluZXM3NS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Rhines79,
	Annote = {Filed under Geostrophic Turbulence.},
	Author = {P. B. Rhines},
	Journal = {Ann. Rev. Fluid Mech.},
	Pages = {401--441},
	Title = {Geostrophic Turbulence},
	Volume = 11,
	Year = 1979}

@article{Rhines79b,
	Annote = {Downgradient mixing of PV generates enstrophy
                  cascade.},
	Author = {P. B. Rhines and W. R. Holland},
	Journal = {Dyn. Atmos. Oceans},
	Pages = {289--325},
	Title = {A Theoretical Discussion of Eddy-driven Mean Flows},
	Volume = 3,
	Year = 1979}

@article{Rhines82,
	Author = {P. B. Rhines and W. R. Young},
	Journal = {J. Fluid. Mech.},
	Pages = {347--367},
	Title = {Homogenization of potential vorticity in planetary gyres},
	Volume = 122,
	Year = 1982}

@article{Rhines89,
	Annote = {Topographic influence on planetary-scale flow (flow
                  on scale much larger than Rossby radius) might help
                  shape the ocean general circulation. Not necessary
                  to invoke turbulent diffusion.},
	Author = {P. B. Rhines},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1449--1470},
	Title = {Deep Planetary Circulation and Topography: Simple Models of Midocean Flows},
	Volume = 19,
	Year = 1989}

@article{Rhines94,
	Annote = {Review of jet formation.},
	Author = {P. B. Rhines},
	File = {../../Papers/rhines94.pdf},
	Journal = {Chaos},
	Pages = {313--339},
	Title = {Jets},
	Volume = 4,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxyaGluZXM5NC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLqw7fCiVBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7gzCQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmhpbmVzOTQucGRmAAAOABoADAByAGgAaQBuAGUAcwA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3JoaW5lczk0LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9yaGluZXM5NC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Riehl58,
	Author = {H. Riehl and J. S. Malkus},
	File = {../../Papers/riehl58.pdf},
	Journal = {Geophysica},
	Pages = {503--538},
	Title = {On the heat balance in the equatorial trough zone},
	Volume = 6,
	Year = 1958,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtyaWVobDU4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLrxG7ObwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxG8w3wAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmllaGw1OC5wZGYADgAYAAsAcgBpAGUAaABsADUAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvcmllaGw1OC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9yaWVobDU4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Rind86,
	Author = {Rind, D.},
	File = {../../Papers/rind86.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3--25},
	Title = {The dynamics of warm and cold climates},
	Volume = {43},
	Year = {1986},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpyaW5kODYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLsxizo6AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxi1LWAAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmluZDg2LnBkZgAADgAWAAoAcgBpAG4AZAA4ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3JpbmQ4Ni5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvcmluZDg2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Rind98,
	Annote = {Filed under Hadley Cell Dynamics. Response of GCM to
                  changes in SST gradient and global mean SST. Hadley
                  cell strength increases with increased temperature
                  gradient (tropics moisten, subtropics dry).},
	Author = {D. Rind},
	Journal = {J. Geophys. Res.},
	Pages = {5943--5971},
	Title = {Latitudinal temperature gradients and climate change},
	Volume = {103D},
	Year = 1998}

@book{Ripley96,
	Address = {Cambridge},
	Annote = {QA76.87.R56 1996. In GFDL library.},
	Author = {B. D. Ripley},
	Pages = 403,
	Publisher = {Cambridge University Press},
	Title = {Pattern Recognition and Neural Networks},
	Year = 1996}

@article{Risi08,
	Author = {Risi, C. and Bony, S. and Vimeux, F.},
	File = {../../Papers/risi08.pdf},
	Journal = {J. Geophys. Res.},
	Title = {Influence of convective processes on the isotopic composition ($\delta^18\mathrm{O}$ and $\delta \mathrm{D}$) of precipitation and water vapor in the tropics: 2. Physical interpretation of the amount effect},
	Volume = {D113},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpyaXNpMDgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLtxT3msgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxT5XMgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cmlzaTA4LnBkZgAADgAWAAoAcgBpAHMAaQAwADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3Jpc2kwOC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvcmlzaTA4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Roads98,
	Address = {Silver Spring, MD},
	Author = {Roads, J. and Chen, S. C. and Marshall, S. and Oglesby, R.},
	File = {../../Papers/roads98.pdf},
	Journal = {GEWEX News},
	Pages = {1,7--10},
	Publisher = {International GEWEX Project Office},
	Title = {Atmospheric moisture cycling rate trends from model runs},
	Volume = {8},
	Year = {1998},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtyb2Fkczk4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLux/dtrwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx/fQHwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cm9hZHM5OC5wZGYADgAYAAsAcgBvAGEAZABzADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvcm9hZHM5OC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9yb2Fkczk4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Robert91,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {R. Robert and J. Sommeria},
	Journal = {J. Fluid Mech.},
	Pages = {291--310},
	Title = {Statistical Equilibrium States for Two-Dimensional Flows},
	Volume = 229,
	Year = 1991}

@article{Robert92,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {R. Robert and J. Sommeria},
	Journal = {Phys. Rev. Lett.},
	Pages = {2776--2779},
	Title = {Relaxation towards a statistical equilibrium in two-dimensional perfect fluid dynamics},
	Volume = 69,
	Year = 1992}

@article{Robert97,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {R. Robert and C. Rosier},
	Journal = {J. Statist. Phys.},
	Pages = {481--515},
	Title = {The Modeling of Small Scales in Two-Dimensional Turbulent Flows:{A} Statistical Mechanics Approach},
	Volume = 86,
	Year = 1997}

@article{Robinson02,
	Author = {W. A. Robinson},
	File = {../../Papers/robinson02.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2001GL014158},
	Title = {On the midlatitude thermal response to tropical warmth},
	Volume = 29,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5yb2JpbnNvbjAyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRLyvyeOcwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvyfw4wAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cm9iaW5zb24wMi5wZGYAAA4AHgAOAHIAbwBiAGkAbgBzAG8AbgAwADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3JvYmluc29uMDIucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3JvYmluc29uMDIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Robinson02b,
	Annote = {Show that cooling of eastern U.S. may be dynamical
                  response to warming of tropical Pacific (which leads
                  to increased cloud cover over U.S.).},
	Author = {W. A. Robinson and R. Reudy},
	Date-Modified = {2010-08-19 18:04:36 -0700},
	Journal = {J. Geophys. Res.},
	Pages = {??},
	Title = {{GCM} simulations of recent cooling in the {E}ast-central {U}nited {S}tates},
	Volume = {??D},
	Year = 2002}

@article{Robinson97,
	Annote = {Jets shift poleward as surface drag is decreased.},
	Author = {W. A. Robinson},
	Journal = {J. Climate},
	Pages = {176--182},
	Title = {Dissipation Dependence of the Jet Latitude},
	Volume = 10,
	Year = 1997}

@article{Rodwell01,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {M. J. Rodwell and B. J. Hoskins},
	File = {../../Papers/rodwell01.pdf},
	Journal = {J. Climate},
	Pages = {3192--3211},
	Title = {Subtropical Anticyclones and Summer Monsoons},
	Volume = 14,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1yb2R3ZWxsMDEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRL2xwuRHgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxwvzjgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cm9kd2VsbDAxLnBkZgAOABwADQByAG8AZAB3AGUAbABsADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvcm9kd2VsbDAxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3JvZHdlbGwwMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Rodwell96,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {M. J. Rodwell and B. J. Hoskins},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1385--1404},
	Title = {Monsoons and the Dynamics of Deserts},
	Volume = 122,
	Year = 1996}

@article{Rosenthal83a,
	Annote = {Filed under Lindzen.},
	Author = {A. J. Rosenthal and R. S. Lindzen},
	File = {../../Papers/rosenthal83a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {509--520},
	Title = {Instabilities in a Stratified Fluid Having One Critical Level. {P}art {I}: {R}esults},
	Volume = 40,
	Year = 1983,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhByb3NlbnRoYWw4M2EucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRL9wtc4q1BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwtebGwAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cm9zZW50aGFsODNhLnBkZgAADgAiABAAcgBvAHMAZQBuAHQAaABhAGwAOAAzAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3Jvc2VudGhhbDgzYS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvcm9zZW50aGFsODNhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Rosenthal83b,
	Annote = {Filed under Lindzen.},
	Author = {A. J. Rosenthal and R. S. Lindzen},
	File = {../../Papers/rosenthal83b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {521--529},
	Title = {Instabilities in a Stratified Fluid Having One Critical Level. {P}art {II}: {E}xplanation of Gravity Wave Instabilites Using the Concept of Overreflection},
	Volume = 40,
	Year = 1983,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhByb3NlbnRoYWw4M2IucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRL+wtc421BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwtebSwAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cm9zZW50aGFsODNiLnBkZgAADgAiABAAcgBvAHMAZQBuAHQAaABhAGwAOAAzAGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3Jvc2VudGhhbDgzYi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvcm9zZW50aGFsODNiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Rosenthal83c,
	Annote = {Filed under Lindzen.},
	Author = {A. J. Rosenthal and R. S. Lindzen},
	Journal = {J. Atmos. Sci.},
	Pages = {530--542},
	Title = {Instabilities in a Stratified Fluid Having One Critical Level. {P}art {III}: {K}elvin-{H}elmholtz Instabilities as Overreflected Waves},
	Volume = 40,
	Year = 1983}

@incollection{Rossby59,
	Address = {New York},
	Author = {C.-G. Rossby},
	Booktitle = {The Rossby Memorial Volume},
	Pages = {9--50},
	Publisher = {Rockefeller Institute Press},
	Title = {Current Problems in Meteorology},
	Year = 1959}

@article{Rossow99,
	Annote = {Filed under Cloud Observations.},
	Author = {W. B. Rossow and R. A. Schiffer},
	File = {../../Papers/rossow99.pdf},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {2261--2287},
	Title = {Advances in Understanding Clouds from {ISCCP}},
	Volume = 80,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxyb3Nzb3c5OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRL/wCU2DwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwCWmjwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cm9zc293OTkucGRmAAAOABoADAByAG8AcwBzAG8AdwA5ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3Jvc3Nvdzk5LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9yb3Nzb3c5OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Rotunno99,
	Annote = {Filed under Lee Vortex Generation.},
	Author = {R. Rotunno and V. Grubi\v{s}i\'{c} and P. K. Smolarkiewicz},
	Journal = {J. Atmos. Sci.},
	Pages = {2796--2810},
	Title = {Vorticity and Potential Vorticity in Mountain Wakes},
	Volume = 56,
	Year = 1999}

@article{Rowell98,
	Annote = {Filed under Predictability.},
	Author = {D. P. Rowell},
	Journal = {J. Climate},
	Pages = {109--120},
	Title = {Assessing Potential Seasonal Predictability with an Ensemble of Multidecadal {GCM} Simulations},
	Volume = {11},
	Year = 1998}

@article{Rubin76,
	Annote = {Not on file.},
	Author = {D. B. Rubin},
	Journal = {Biometrika},
	Pages = {581--592},
	Title = {Inference and missing data},
	Volume = 63,
	Year = 1976}

@article{Ruiz-Barradas05,
	Annote = {Not on file.},
	Author = {A. Ruiz-Barradas and S. Nigam},
	File = {../../Papers/ruiz-barradas05.pdf},
	Journal = {J. Climate},
	Pages = {1808--1830},
	Title = {Warm Season Rainfall Variability over the {U.~S.} {G}reat {P}lains in Observations, {NCEP} and {ERA-40} Reanalyses, and {NCAR} and {NASA} Atmospheric Model Simulations},
	Volume = 18,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYAAAAAAAYAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhNydWl6LWJhcnJhZGFzMDUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMBv3VNIQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3WvkQAAAAEADAAJDH4ACE6zAACS8wACADJNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cnVpei1iYXJyYWRhczA1LnBkZgAOACgAEwByAHUAaQB6AC0AYgBhAHIAcgBhAGQAYQBzADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACZVc2Vycy90YXBpby9QYXBlcnMvcnVpei1iYXJyYWRhczA1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAgLi4vLi4vUGFwZXJzL3J1aXotYmFycmFkYXMwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACJAImAisCNAI/AkMCUQJYAmEChAKJAowCmQKeAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAArA=}}

@article{Rutherford03,
	Annote = {Filed under Mann. See also Reviews.},
	Author = {S. Rutherford and M. E. Mann and T. L. Delworth and R. J. Stouffer},
	Journal = {J. Climate},
	Pages = {462--479},
	Title = {Climate Field Reconstruction under Stationary and Nonstationary Forcing},
	Volume = 16,
	Year = 2003}

@article{Ryoo08,
	Author = {J.-M. Ryoo and D. W. Waugh and A. Gettelman},
	File = {../../Papers/ryoo08.pdf},
	Journal = {Atmos. Chem. Phys.},
	Pages = {2643--2655},
	Title = {Variability of subtropical upper tropospheric humidity},
	Volume = {8},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpyeW9vMDgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMExfvC7QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxfwlXQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cnlvbzA4LnBkZgAADgAWAAoAcgB5AG8AbwAwADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3J5b28wOC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvcnlvbzA4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Ryoo09,
	Author = {J.-M. Ryoo and T. Igusa and D. W. Waugh},
	File = {../../Papers/ryoo09.pdf},
	Journal = {J. Climate},
	Note = {In press},
	Pages = {??},
	Title = {{PDF}s of Tropical Tropospheric Humidity: Measurements and Theory},
	Volume = {22},
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpyeW9vMDkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMFxfvGXgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxfwozgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6cnlvbzA5LnBkZgAADgAWAAoAcgB5AG8AbwAwADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3J5b28wOS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvcnlvbzA5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Sabelfeld98,
	Annote = {Filed under Stochastic Lagrangian Models of Turbulence.},
	Author = {K. Sabelfeld and O. Kurbanmuradov},
	File = {../../Papers/sabelfeld98.pdf},
	Journal = {???},
	Pages = {???},
	Title = {One-particle Stochastic {L}agrangian Model for Turbulent Dispersion in Horizontally Homogeneous Turbulence},
	Volume = {???},
	Year = {???},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zYWJlbGZlbGQ5OC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMGv5GUVVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5IE1QAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FiZWxmZWxkOTgucGRmAA4AIAAPAHMAYQBiAGUAbABmAGUAbABkADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2FiZWxmZWxkOTgucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2FiZWxmZWxkOTgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Sadourny85,
	Annote = {Not on file.},
	Author = {R. Sadourny and C. Basdevant},
	Journal = {J. Atmos. Sci.},
	Pages = {1353--1363},
	Title = {Parameterization of subgrid scale barotropic and baroclinic eddies in quasi-geostrophic models: {A}nticipated potential vorticity method},
	Volume = 42,
	Year = 1985}

@article{Salathe97,
	Author = {Salath{\'e}, Jr., E. P. and Hartman, D. L.},
	File = {../../Papers/salathe97.pdf},
	Journal = {J. Climate},
	Pages = {2533--2547},
	Title = {A Trajectory Analysis of Tropical Upper-Tropospheric Moisture and Convection},
	Volume = 10,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zYWxhdGhlOTcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMJv7tPuwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv7vAOwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FsYXRoZTk3LnBkZgAOABwADQBzAGEAbABhAHQAaABlADkANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc2FsYXRoZTk3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3NhbGF0aGU5Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Salby84,
	Annote = {Gave presentation on this in Kevin's class. Solves
                  for modes of Laplace's Tidal equation numerically in
                  a hierarchy of cases with varying complexity. Thus
                  obtained modes agree fairly well with observed modes
                  in lower troposphere.},
	Author = {M. L. Salby},
	Journal = {Rev. Geophys. Space Phys.},
	Pages = {209--236},
	Title = {Survey of Planetary-Scale Traveling Waves: {T}he State of Theory and Observations},
	Volume = {22},
	Year = {1984}}

@article{Salmon80,
	Annote = {Filed under Geostrophic Turbulence.},
	Author = {R. Salmon},
	File = {../../Papers/salmon80.pdf},
	Journal = {Geophys. Astrophys. Fluid Dyn.},
	Pages = {167--211},
	Title = {Baroclinic Instability and Geostrophic Turbulence},
	Volume = 15,
	Year = 1980,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzYWxtb244MC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMLvRhW4AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRi5UAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FsbW9uODAucGRmAAAOABoADABzAGEAbABtAG8AbgA4ADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NhbG1vbjgwLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zYWxtb244MC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@incollection{Salmon82,
	Address = {Bologna, Italy},
	Annote = {Filed under Geostrophic Turbulence.},
	Author = {R. Salmon},
	Booktitle = {Topics in Ocean Physics},
	Editors = {A. R. Osborne and P. M. Rizzoli},
	Pages = {30--78},
	Publisher = {Soc. Italiana di Fisica},
	Title = {Geostrophic Turbulence},
	Year = 1982}

@book{Salmon98,
	Address = {New York},
	Author = {R. Salmon},
	Pages = 378,
	Publisher = {Oxford University Press},
	Title = {Lectures on Geophysical Fluid Dynamics},
	Year = 1998}

@article{Salyk06,
	Author = {C. Salyk and A. P. Ingersoll and J. Lorre and A. Vasavada and A. D. {Del~Genio}},
	File = {../../Papers/salyk06.pdf},
	Journal = {Icarus},
	Pages = {430--442},
	Title = {Interaction between eddies and mean flow in {J}upiter's atmosphere: {A}nalysis of {Cassini} imaging data},
	Volume = 185,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzYWx5azA2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMNw1AGbFBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw1Bo3AAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FseWswNi5wZGYADgAYAAsAcwBhAGwAeQBrADAANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc2FseWswNi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zYWx5azA2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Samelson97,
	Annote = {Filed under Vallis.},
	Author = {R. M. Samelson and G. K. Vallis},
	Journal = {J. Mar. Res.},
	Pages = {223--275},
	Title = {Large-scale circulation with small diapycnal diffusion: {T}he two-thermocline limit},
	Volume = 55,
	Year = 1997}

@article{Sanchez-Lavega08,
	Author = {A. S{\'a}nchez-Lavega and G. S. Orton and R. Hueso and E. Garc{\'\i}{\'a}-Melendo and S. P{\'e}rez-Hoyos and A. Simon-Miller and J. F. Rojas and J. M. G{\'o}mez and P. Yanamandra-Fisher and L. Fletcher and J. Joels and J. Kemerer and J. Hora and E. Karkoschka and I. de Pater and M. H. Wong and P. S. Marcus and N. Pinilla-Alonso and F. Carvalho and C. Goand D. Parker and M. Salway and M. Valimberti and A. Wesley and and Z. Pujic},
	File = {../../Papers/sanchez-lavega08.pdf},
	Journal = {Nature},
	Pages = {437--440},
	Title = {Depth of a strong {Jovian} jet from a planetary-scale disturbance driven by storms},
	Volume = 451,
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYYAAAAAAYYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhRzYW5jaGV6LWxhdmVnYTA4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMRw9OdrQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw9QOLQAAAAEADAAJDH4ACE6zAACS8wACADNNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FuY2hlei1sYXZlZ2EwOC5wZGYAAA4AKgAUAHMAYQBuAGMAaABlAHoALQBsAGEAdgBlAGcAYQAwADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAnVXNlcnMvdGFwaW8vUGFwZXJzL3NhbmNoZXotbGF2ZWdhMDgucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAhLi4vLi4vUGFwZXJzL3NhbmNoZXotbGF2ZWdhMDgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAioCLAIxAjoCRQJJAlcCXgJnAosCkAKTAqACpQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAK3}}

@article{Santer03a,
	Annote = {Filed under Tropopause Dynamics.},
	Author = {B. D. Santer and R. Sausen and T. M. L. Wigley and J. S. Boyle and K. AchutaRao and C. Doutriaux and J. E. Hansen and G. A. Meehl and E. Roeckner and R. Ruedy and G. Schmidt and K. E. Taylor},
	File = {../../Papers/santer03a.pdf},
	Journal = {J. Geophys. Res.},
	Note = {doi:10.1029/2002JD002258},
	Pages = 4002,
	Title = {Behavior of tropopause height and atmospheric temperature in models, reanalyses, and observations: Decadal changes},
	Volume = {108D},
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zYW50ZXIwM2EucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMWwCEFAQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwCF1gQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FudGVyMDNhLnBkZgAOABwADQBzAGEAbgB0AGUAcgAwADMAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc2FudGVyMDNhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3NhbnRlcjAzYS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Santer03b,
	Annote = {Filed under Tropopause Dynamics.},
	Author = {B. D. Santer and M. F. Wehner and T. M. L. Wigley and R. Sausen and G. A. Meehl and K. E. Taylor and C. Ammann and J. Arblaster and W. M. Washington and J. S. Boyle and W. Bruggemann},
	File = {../../Papers/santer03b.pdf},
	Journal = {Science},
	Pages = {479--483},
	Title = {Contributions of Anthropogenic and Natural Forcing to Recent Tropopause Height Changes},
	Volume = 301,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zYW50ZXIwM2IucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMXwCEEpwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwCF1JwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FudGVyMDNiLnBkZgAOABwADQBzAGEAbgB0AGUAcgAwADMAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc2FudGVyMDNiLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3NhbnRlcjAzYi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Santer04,
	Annote = {Filed under Tropopause Dynamics.},
	Author = {B. D. Santer and T. M. L. Wigley and A. J. Simmons and P. W. Kallberg and G. A. Kelly and S. M. Uppala and C. Ammann and J. S. Boyle and W. Bruggemann and C. Doutriaux and M. Fiorino and C. Mears and G. A. Meehl and R. Sausen and K. E. Taylor and W. M. Washington and M. F. Wehner and F. J. Wentz},
	File = {../../Papers/santer04.pdf},
	Journal = {J. Geophys. Res.},
	Note = {doi:10.1029/2004JD005075},
	Pages = {art. D21104},
	Title = {Identification of anthropogenic climate change using a second-generation reanalysis},
	Volume = {109D},
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzYW50ZXIwNC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMYvjEVjQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvjGGDQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FudGVyMDQucGRmAAAOABoADABzAGEAbgB0AGUAcgAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NhbnRlcjA0LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zYW50ZXIwNC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Santer93,
	Annote = {Filed under Climate Change Detection. Try to
                  establish if a time-independent signal pattern
                  becomes increasingly manifest in observational
                  record. Signal pattern is defined as difference
                  between equilibrium response of 2xCO2 simulation and
                  1xC02 simulation. Authors suppose that correlation
                  between signal and data should increase with time,
                  `as GHG signal emerges from the background of
                  natural variability.' Use various correlation
                  statistics. Point out normalization problem (`common
                  factor effect') with existing statistics. Show that
                  Barnett87 correlation statistic mainly accounts for
                  changes in mean temperature. Thus, correlation
                  statistics can be decomposed into those that contain
                  information about the `emergence' of a multivariate
                  pattern of climate change [their R(t)] and those
                  that contain information about mean strength of
                  signal [Barnett87 C(t)], i.e., information about the
                  climate sensitivity. State that reliable estimation
                  of time-dependent GHG change signal would require
                  large ensemble of model runs.},
	Author = {B. D. Santer and T. M. L. Wigley and P. D. Jones},
	Journal = {Climate Dyn.},
	Pages = {265--276},
	Title = {Correlation Methods in Fingerprint Detection Studies},
	Volume = 8,
	Year = 1993}

@article{Santer94,
	Annote = {Filed under Climate Change Detection. Analyze IPCC
                  scenario runs and equilibrium response run of ECHAM
                  climate model. Do various principal component
                  analyses: of control run ('noise EOFs') and of
                  difference between scenario run and control run
                  ('signal EOFs'). Signal and noise EOFs differ most
                  for SAT and are similar for SLP.},
	Author = {B. D. Santer and W. Br{\"u}ggemann and U. Cubasch and K. Hasselmann and H. H{\"o}ck},
	Journal = {Climate Dyn.},
	Pages = {267--285},
	Title = {Signal-to-noise analysis of time-dependent greenhouse warming experiments},
	Volume = 9,
	Year = 1994}

@article{Santer95,
	Annote = {Filed under Climate Change Detection. Test
                  significance of trends in correlations between
                  `climate change signal' and record of
                  observations. The `climate change signal' is taken
                  to be the equilibrium response (relative to a
                  pre-industrial control run) of a coupled GCM to (i)
                  present-day CO2 concentration, (ii) present-day
                  sulfate [?] emissions, and (iii) combined sulfate
                  and CO2 effects. Trends in global mean are
                  significant in all seasons [detection], but trends
                  in pattern correlation are only marginally
                  significant on the 40--50 time scale. In this as
                  well as other papers by the authors a `static' view
                  of global change prevails: An `evolving expression
                  of a ... signal pattern' is thought to emerge in the
                  observed data.},
	Author = {B. D. Santer and K. E. Taylor and T. M. L. Wigley and J. E. Penner and P. D. Jones and U. Cubasch},
	Journal = {Climate Dyn.},
	Pages = {77-100},
	Title = {Towards the detection and attribution of an anthropogenic effect on climate},
	Volume = 12,
	Year = 1995}

@incollection{Santer96,
	Address = {Cambridge, UK},
	Author = {B. D. Santer and T. M. L. Wigley and T. P. Barnett and E. Anyamba},
	Booktitle = {Climate Change 1995: The Science of Climate Change},
	Editor = {J. T. Houghton and L. G. {Meira Filho} and B. A. Callander and N. Harris and A. Kattenberg and K. Maskell},
	Pages = {408--443},
	Publisher = {Intergovernmental Panel on Climate Change, Cambridge University Press},
	Title = {Detection of Climate Change and Attribution of Causes},
	Year = 1996}

@article{Santer99,
	Annote = {Filed under Climate Change Detection. Biases in
                  reanalysis data before (pre-satellite era).},
	Author = {B. D. Santer and J. J. Hnilo and T. M. L. Wigley and J. S. Boyle and C. Doutriaux and M. Fiorino and D. E. Parker and K. E. Taylor},
	Journal = {J. Geophys. Res.},
	Pages = {6405--6333},
	Title = {Uncertainties in observationally based estimates of temperature change in the free atmosphere},
	Volume = {104D},
	Year = 1999}

@article{Sarachik85,
	Author = {E. S. Sarachik},
	File = {../../Papers/sarachik85.pdf},
	Journal = {Pure Appl. Geophys.},
	Pages = {261--271},
	Title = {A Simple Theory for the Vertical Structure of the Tropical Atmosphere},
	Volume = 123,
	Year = 1985,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zYXJhY2hpazg1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMbvzTW9gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvzU5ZgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FyYWNoaWs4NS5wZGYAAA4AHgAOAHMAYQByAGEAYwBoAGkAawA4ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3NhcmFjaGlrODUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3NhcmFjaGlrODUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Saravanan93,
	Author = {R. Saravanan},
	File = {../../Papers/saravanan93.pdf},
	Journal = {J. Atmos. Sci.},
	Number = 9,
	Pages = {1211--1227},
	Title = {Equatorial superrotation and maintenance of the general circulation in two-level models},
	Volume = 50,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zYXJhdmFuYW45My5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMcwTYh3VBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwTaETQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FyYXZhbmFuOTMucGRmAA4AIAAPAHMAYQByAGEAdgBhAG4AYQBuADkAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2FyYXZhbmFuOTMucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2FyYXZhbmFuOTMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Sardeshmukh85,
	Author = {P. D. Sardeshmukh and B. J. Hoskins},
	File = {../../Papers/sardeshmukh85.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {261--278},
	Title = {Vorticity balances in the tropics during the 1982--1983 {El} {Ni\~no}--{S}outhern {O}scillation event},
	Volume = 111,
	Year = 1985,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXgAAAAAAXgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhFzYXJkZXNobXVraDg1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMewS5F7FBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwS6oXAAAAAEADAAJDH4ACE6zAACS8wACADBNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FyZGVzaG11a2g4NS5wZGYADgAkABEAcwBhAHIAZABlAHMAaABtAHUAawBoADgANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACRVc2Vycy90YXBpby9QYXBlcnMvc2FyZGVzaG11a2g4NS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHi4uLy4uL1BhcGVycy9zYXJkZXNobXVraDg1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIcAh4CIwIsAjcCOwJJAlACWQJ6An8CggKPApQAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACpg==}}

@article{Sardeshmukh88,
	Author = {P. D. Sardeshmukh and B. J. Hoskins},
	File = {../../Papers/sardeshmukh88.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1228--1251},
	Title = {The Generation of Global Rotational Flow by Steady Idealized Tropical Divergence},
	Volume = 45,
	Year = 1988,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXgAAAAAAXgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhFzYXJkZXNobXVraDg4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMfwS5FYFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwS6n0AAAAAEADAAJDH4ACE6zAACS8wACADBNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2FyZGVzaG11a2g4OC5wZGYADgAkABEAcwBhAHIAZABlAHMAaABtAHUAawBoADgAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACRVc2Vycy90YXBpby9QYXBlcnMvc2FyZGVzaG11a2g4OC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHi4uLy4uL1BhcGVycy9zYXJkZXNobXVraDg4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIcAh4CIwIsAjcCOwJJAlACWQJ6An8CggKPApQAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACpg==}}

@article{Sarmiento96,
	Annote = {In a model without biological processes, CO2 uptake
                  by oceans in reduced in global warming scenarios due
                  to breakdown of thermohaline circulation.},
	Author = {J. L. Sarmiento and C. {Le Qu{\'e}r{\'e}}},
	Journal = {Science},
	Pages = {1346--1350},
	Title = {Oceanic Carbon Dioxide Uptake in a Model of Century-Scale Global Warming},
	Volume = 274,
	Year = 1996}

@article{Sarmiento98,
	Author = {J. L. Sarmiento and T. M. C. Hughes and R. J. Stouffer and S. Manabe},
	Journal = {Nature},
	Pages = {245--249},
	Title = {Simulated Response of the Ocean Carbon Cycle to Anthropogenic Climate Warming},
	Volume = 393,
	Year = 1998}

@article{Satoh01,
	Annote = {Relaxation model for mean pv. Model cannot work for
                  thermal relaxation towards statically unstable
                  thermal stratification.},
	Author = {M. Satoh and Z. Neufeld},
	Journal = {Geophys. Res. Lett.},
	Pages = {163--166},
	Title = {The latitudinal gradient of potential vorticity in the mid-latitudes of the troposphere},
	Volume = 28,
	Year = 2001}

@article{Satoh92,
	Author = {M. Satoh and Y.-Y. Hayashi},
	Journal = {J. Atmos. Sci.},
	Pages = {1202--1220},
	Title = {Simple Cumulus Models in One-Dimensional Radiative Convective Equilibrium Problems},
	Volume = 49,
	Year = 1992}

@article{Satoh94,
	Annote = {Filed under Hadley Cell Dynamics. Studies
                  axisymmetric Hadley circulations with moist
                  convection.},
	Author = {M. Satoh},
	Journal = {J. Atmos. Sci.},
	Pages = {1947--1968},
	Title = {{H}adley Circulations in Radiative--Convective Equilibrium in an Axially Symmetric Atmosphere},
	Volume = 51,
	Year = 1994}

@article{Satoh95,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {M. Satoh and M. Shiobara and M. Takahashi},
	Journal = {Tellus},
	Pages = {548--560},
	Title = {{H}adley circulations and their r{\^o}les in the global angular momentum budget in two- and three-dimensional models},
	Volume = {47A},
	Year = 1995}

@article{Sawford01,
	Annote = {Filed under Stochastic Lagrangian Models of
                  Turbulence. Review of turbulent dispersion,
                  including summary of two-particle Lagrangian
                  stochastic models. Two-point closures and kinematic simulation.},
	Author = {B. Sawford},
	File = {../../Papers/sawford01.pdf},
	Journal = {Annu. Rev. Fluid Mech.},
	Pages = {289--317},
	Title = {Turbulent Relative Dispersion},
	Volume = 33,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zYXdmb3JkMDEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMgv5GhjlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5ISDgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2F3Zm9yZDAxLnBkZgAOABwADQBzAGEAdwBmAG8AcgBkADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc2F3Zm9yZDAxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3Nhd2ZvcmQwMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Schaer93a,
	Annote = {Filed under Lee Vortex Generation.},
	Author = {C. Sch{\"a}r and R. B. Smith},
	Journal = {J. Atmos. Sci.},
	Pages = {1373--1400},
	Title = {Shallow-Water Flow past Isolated Topography. {P}art {I}: Vorticity Production and Wake Formation},
	Volume = 50,
	Year = 1993}

@article{Schaer93b,
	Author = {C. Sch{\"a}r},
	Journal = {J. Atmos. Sci.},
	Pages = {1437--1443},
	Title = {A Generalization of {B}ernoulli's Theorem},
	Volume = 50,
	Year = 1993}

@article{Schaer97,
	Annote = {Filed under Lee Vortex Generation.},
	Author = {C. Sch{\"a}r and D. R. Durran},
	Journal = {J. Atmos. Sci.},
	Pages = {534--554},
	Title = {Vortex Formation and Vortex Shedding in Continuously Stratified Flows past Isolated Topography},
	Volume = 54,
	Year = 1997}

@book{Schafer97,
	Author = {J. L. Schafer},
	Pages = 430,
	Publisher = {Chapman and Hall},
	Series = {Monographs on Statistics and Applied Probability},
	Title = {Analysis of Incomplete Multivariate Data},
	Volume = 72,
	Year = 1997}

@article{Schaller09a,
	Author = {E.~L. Schaller and H.~G.\ Roe and T.\ Schneider and M.~E.\ Brown},
	Date-Modified = {2010-06-11 12:09:59 -0700},
	Journal = {Nature},
	Pages = {873--875},
	Title = {Storms in the Tropics of {Titan}},
	Volume = 460,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zY2hhbGxlcjA5YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMmxqiFQwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxqjnswAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NoYWxsZXIwOWEucGRmAA4AIAAPAHMAYwBoAGEAbABsAGUAcgAwADkAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2NoYWxsZXIwOWEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2NoYWxsZXIwOWEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Schar03,
	Annote = {Filed under Lee Vortex Generation.},
	Author = {C. Sch{\"a}r and M. Sprenger and D. L{\"u}th and Q. Jiang and R. B. Smith and R. Benoit},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {825--855},
	Title = {Structure and dynamics of an {Alpine} potential-vorticity banner},
	Volume = 129,
	Year = 2003}

@article{Schimel01,
	Annote = {Filed under Carbon Flux Estimates},
	Author = {D. S. Schimel and Coauthors},
	Journal = {Nature},
	Pages = {169--172},
	Title = {Recent patterns and mechanisms of carbon exchange by terrestrial ecosystems},
	Volume = 414,
	Year = 2001}

@incollection{Schimel96,
	Address = {Cambridge, UK},
	Author = {D. Schimel and Coauthors},
	Booktitle = {Climate Change 1995: The Science of Climate Change},
	Editor = {J. T. Houghton and L. G. {Meira Filho} and B. A. Callander and N. Harris and A. Kattenberg and K. Maskell},
	Pages = {65--131},
	Publisher = {Intergovernmental Panel on Climate Change, Cambridge University Press},
	Title = {Radiative Forcing of Climate Change},
	Year = 1996}

@book{Schlittgen87,
	Address = {M{\"u}nchen, Wien},
	Annote = {don't have it},
	Author = {R. Schlittgen and B. Streitberg},
	Publisher = {Oldenbourg Verlag},
	Title = {Zeitreihenanalyse},
	Year = 1987}

@article{Schneider01a,
	Author = {T. Schneider and I. M. Held},
	Journal = {J. Climate},
	Pages = {249--254},
	Title = {Discriminants of twentieth-century changes in {E}arth surface temperatures},
	Volume = 14,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwMWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMoubdkAwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAubfGcwAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDFhLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAAxAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjAxYS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDFhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@misc{Schneider01aa,
	Annote = {Online appendix to Schneider, T. and I. M. Held,
                  2001: Discriminants of twentieth-century changes in
                  Earth surface temperatures, J. Climate, 14,
                  249--254.},
	Author = {T. Schneider and I. M. Held},
	Title = {Higher-order discriminants of twentieth-century changes in {E}arth surface temperatures},
	Url = {www.caltech.edu/\~{}tapio/papers},
	Year = 2001,
	Bdsk-Url-1 = {www.caltech.edu/%5C~%7B%7Dtapio/papers}}

@article{Schneider01b,
	Author = {T. Schneider},
	Journal = {J. Climate},
	Pages = {853--871},
	Title = {Analysis of incomplete climate data: Estimation of mean values and covariance matrices and imputation of missing values},
	Volume = 14,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwMWIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMpuZDdNgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAuZE/pgAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDFiLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAAxAGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjAxYi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDFiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider01c,
	Author = {T. Schneider and A. Neumaier},
	Journal = {ACM Trans. Math. Softw.},
	Pages = {58--65},
	Title = {Algorithm 808: {AR}fit --- {A} {M}atlab package for the estimation of parameters and eigenmodes of multivariate autoregressive models},
	Volume = 27,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwMWMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMqt7fgAgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAt7hCcgAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDFjLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAAxAGMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjAxYy5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDFjLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider03,
	Author = {T. Schneider and I. M. Held and S. T. Garner},
	File = {../../Papers/schneider03.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1024--1040},
	Title = {Boundary effects in potential vorticity dynamics},
	Volume = {60},
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zY2huZWlkZXIwMy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMrv9bctgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv9dNNgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDMucGRmAA4AIAAPAHMAYwBoAG4AZQBpAGQAZQByADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2NobmVpZGVyMDMucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2NobmVpZGVyMDMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Schneider04a,
	Author = {T. Schneider},
	Date-Modified = {2010-06-11 11:51:41 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {1317--1340},
	Title = {The tropopause and the thermal stratification in the extratropics of a dry atmosphere},
	Volume = 61,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwNGEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMsvPoH5gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvPpqVgAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDRhLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA0AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA0YS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDRhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider05a,
	Author = {T. Schneider},
	Date-Modified = {2010-06-11 11:51:32 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {1884--1900},
	Title = {Zonal momentum balance, potential vorticity dynamics, and mass fluxes on near-surface isentropes},
	Volume = 62,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwNWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMturpPCAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAurqxeAAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDVhLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA1AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA1YS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDVhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider06a,
	Author = {T. Schneider and C. C. Walker},
	Journal = {J. Atmos. Sci.},
	Pages = {1569--1586},
	Title = {Self-Organization of Atmospheric Macroturbulence into Critical States of Weak Nonlinear Eddy--Eddy Interactions},
	Volume = {63},
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwNmEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMuwLhQBQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwLiydQAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDZhLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA2AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA2YS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDZhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider06b,
	Author = {T. Schneider},
	Journal = {Ann. Rev. Earth Planet. Sci.},
	Pages = {655-688},
	Title = {The General Circulation of the Atmosphere},
	Volume = {34},
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwNmIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMvx6g4dAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx6io9AAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDZiLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA2AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA2Yi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDZiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider06c,
	Author = {T. Schneider and K. L. Smith and P. A. O'Gorman and C. C. Walker},
	Journal = {J. Climate},
	Pages = {5918--5933},
	Title = {A Climatology of Tropospheric Zonal-Mean Water Vapor Fields and Fluxes in Isentropic Coordinates},
	Volume = {19},
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwNmMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMwwZ0qWAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwZ2a2AAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDZjLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA2AGMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA2Yy5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDZjLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider06d,
	Author = {T. Schneider and A. H. Sobel},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {807-809},
	Title = {The Global Circulation of the Atmosphere (2004)},
	Volume = {87},
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwNmQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMxwMsArAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwMtjHAAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDZkLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA2AGQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA2ZC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDZkLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider06e,
	Author = {T. Schneider},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {1410--1411},
	Title = {Analysis of incomplete data: Readings from the statistics literature},
	Volume = 87,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwNmUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMywRH2DgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwRJYfgAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDZlLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA2AGUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA2ZS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDZlLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@book{Schneider07e,
	Address = {Princeton, NJ},
	Date-Modified = {2010-06-11 12:06:43 -0700},
	Editor = {T. Schneider and A. H. Sobel},
	Pages = {400},
	Publisher = {Princeton University Press},
	Title = {The Global Circulation of the Atmosphere},
	Year = 2007}

@incollection{Schneider07a,
	Address = {Princeton, NJ},
	Author = {T. Schneider},
	Booktitle = {The Global Circulation of the Atmosphere},
	Date-Modified = {2010-06-11 12:02:52 -0700},
	Editor = {T. Schneider and A. H. Sobel},
	Pages = {47--77},
	Publisher = {Princeton University Press},
	Title = {The thermal stratification of the extratropical troposphere},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwN2EucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRMzwoRe4AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwoTBUAAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDdhLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA3AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA3YS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDdhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider07b,
	Author = {T. Schneider},
	Date-Modified = {2010-06-11 12:05:55 -0700},
	Journal = {Nature},
	Pages = {doi:10.1038/nature05707},
	Title = {Uncertainty in Climate-Sensitivity Estimates},
	Volume = 446,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwN2IucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRM0wgsVkAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwguGEAAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDdiLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA3AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA3Yi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDdiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@inproceedings{Schneider07c,
	Address = {Honolulu, HI},
	Author = {T. Schneider and P. A. O'Gorman},
	Booktitle = {Extreme Events},
	Date-Modified = {2010-06-11 12:06:10 -0700},
	Editor = {P. M{\"u}ller and C. Garrett and D. Henderson},
	Pages = {61--66},
	Publisher = {University of Hawaii at Manoa},
	Series = {Proceedings 'Aha Huliko'a Hawaiian Winter Workshop},
	Title = {Precipitation and its extremes in changed climates},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwN2MucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRM1w71QtgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw73BNgAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDdjLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA3AGMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA3Yy5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDdjLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider07d,
	Author = {T. Schneider},
	Date-Modified = {2010-06-11 12:06:35 -0700},
	Journal = {Nonlin. Processes Geophys.},
	Pages = {1--2},
	Title = {Comment on ``Spatio-temporal filling of missing points in geophysical data sets'' by D. Kondrashov and M. Ghil, Nonlin. Processes Geophys., 13, 151--159, 2006},
	Volume = 14,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwN2QucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRM2wdDvDgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwdFfjgAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDdkLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA3AGQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA3ZC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDdkLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider08a,
	Author = {T. Schneider and S. Bordoni},
	Journal = {J. Atmos. Sci.},
	Pages = {915--934},
	Title = {Eddy-mediated regime transitions in the seasonal cycle of a {H}adley circulation and implications for monsoon dynamics},
	Volume = {65},
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwOGEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRM3xBMWmQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxBN5CQAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDhhLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA4AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA4YS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDhhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider08b,
	Author = {T. Schneider and C. C. Walker},
	Journal = {J. Atmos. Sci.},
	Pages = {2153--2173},
	Title = {Scaling laws and regime transitions of macroturbulence in dry atmospheres},
	Volume = {65},
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwOGIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRM4xKoPwAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxKpyMAAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDhiLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA4AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA4Yi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDhiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider08c,
	Author = {T. Schneider and P. A. O'Gorman},
	Journal = {J. Atmos. Sci.},
	Pages = {3571--3583},
	Title = {Moist convection and the thermal stratification of the extratropical troposphere},
	Volume = {65},
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwOGMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRM5xUoJqwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxUp6KwAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDhjLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA4AGMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA4Yy5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDhjLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider08z,
	Author = {T. Schneider and T. M. Merlis},
	Journal = {J. Atmos. Sci.},
	Note = {In preparation. Available at www.gps.caltech.edu/\~{}tapio.},
	Title = {Further Results on Self-Organization of Atmospheric Macroturbulence into Critical States of Weak Nonlinear Eddy--Eddy Interactions},
	Year = 2008}

@article{Schneider09a,
	Author = {T. Schneider and J. J. Liu},
	Journal = {J. Atmos. Sci.},
	Pages = {579--601},
	Title = {Formation of jets and equatorial superrotation on {J}upiter},
	Volume = {66},
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIwOWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRM6xfLnJAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxfNJlAAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMDlhLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMAA5AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjA5YS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMDlhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider10a,
	Author = {T. Schneider and P. A. O'Gorman and X. J. Levine},
	Date-Modified = {2010-07-02 04:51:14 -0700},
	Journal = {Rev. Geophys.},
	Note = {doi:10.1029/2009RG000302},
	Pages = {RG3001},
	Title = {Water Vapor and the Dynamics of Climate Changes},
	Volume = {48},
	Year = 2010,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXIxMGEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAJfHyyFMdAgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAyFN/cgAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyMTBhLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAMQAwAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjEwYS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyMTBhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schneider81,
	Author = {Schneider, E. K.},
	File = {../../Papers/schneider81.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2142--2149},
	Title = {On the Amplitudes Reached by Baroclinically Unstable Disturbances},
	Volume = {38},
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zY2huZWlkZXI4MS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRM+w43kJlBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw45UpgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyODEucGRmAA4AIAAPAHMAYwBoAG4AZQBpAGQAZQByADgAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2NobmVpZGVyODEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2NobmVpZGVyODEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Schneider99a,
	Author = {T. Schneider and S. M. Griffies},
	Date-Modified = {2010-06-11 11:52:31 -0700},
	Journal = {J. Climate},
	Pages = {3133--3155},
	Title = {A Conceptual Framework for Predictability Studies},
	Volume = 12,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2huZWlkZXI5OWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNCuZDdewAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAuZE/6wAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NobmVpZGVyOTlhLnBkZgAADgAiABAAcwBjAGgAbgBlAGkAZABlAHIAOQA5AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaG5laWRlcjk5YS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NobmVpZGVyOTlhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@unpublished{Schneider99b,
	Author = {T. Schneider},
	Title = {Analysis of incomplete climate data: Matlab code},
	Url = {www.caltech.edu/\~{}tapio/imputation},
	Year = {cited 2000},
	Bdsk-Url-1 = {www.caltech.edu/%5C~%7B%7Dtapio/imputation}}

@article{SchneiderEK03,
	Author = {E. K. Schneider and L. Bengtsson and Z.-Z. Hu},
	Journal = {J. Atmos. Sci.},
	Pages = {1504--1521},
	Title = {Forcing of {N}orthern {H}emisphere Climate Trends},
	Volume = 60,
	Year = 2003}

@article{SchneiderEK76,
	Annote = {Filed under Hadley Cell Dynamics. Linear viscous
                  Hadley cell.},
	Author = {E. K. Schneider and R. S. Lindzen},
	Journal = {J. Atmos. Sci.},
	Pages = {1301--1307},
	Title = {The Influence of Stable Stratification on the Thermally Driven Tropical Boundary Layer},
	Volume = 33,
	Year = 1976}

@article{SchneiderEK77a,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {E. K. Schneider and R. S. Lindzen},
	Journal = {J. Atmos. Sci.},
	Pages = {263--279},
	Title = {Axially Symmetric Steady-State Models of the Basic State for Instability and Climate Studies. {P}art~{I}. {L}inearized Calculations},
	Volume = 34,
	Year = 1977}

@article{SchneiderEK77b,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {E. K. Schneider},
	Journal = {J. Atmos. Sci.},
	Pages = {280--296},
	Title = {Axially Symmetric Steady-State Models of the Basic State for Instability and Climate Studies. {P}art~{II}. {N}onlinear Calculations},
	Volume = 34,
	Year = 1977}

@article{SchneiderEK83,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {E. K. Schneider},
	Journal = {Icarus},
	Pages = {302--331},
	Title = {Martian Great Dust Storms: Interpretive Axially Symmetric Models},
	Volume = 55,
	Year = 1983}

@article{SchneiderEK84,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {E. K. Schneider},
	Journal = {J. Atmos. Sci.},
	Pages = {1093--1115},
	Title = {Response of the Annual and Zonal Mean Winds and Temperatures to Variations in the Heat and Momentum Sources},
	Volume = 41,
	Year = 1984}

@article{SchneiderEK87,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {E. K. Schneider},
	Journal = {J. Atmos. Sci.},
	Pages = {3311--3328},
	Title = {A simplified model of the modified {H}adley circulation},
	Volume = 44,
	Year = 1987}

@article{SchneiderEK99,
	Author = {E. K. Schneider and B. P. Kirtman and R. S. Lindzen},
	Journal = {J. Atmos. Sci.},
	Pages = {1649--1658},
	Title = {Tropospheric Water Vapor and Climate Sensitivity},
	Volume = 56,
	Year = 1999}

@article{Schnur93,
	Annote = {Not on file.},
	Author = {R. Schnur and G. Schmitz and N. Grieger and H. {von Storch}},
	Journal = {J. Atmos. Sci.},
	Pages = {2386--2400},
	Title = {Normal Modes of the Atmosphere as estimated by {P}rincipal {O}scillation {P}atterns and derived from Quasigeostrophic Theory},
	Volume = {50},
	Year = 1993}

@article{Schoeberl84,
	Annote = {Filed under Barotropic Point Jet and Schoeberl.},
	Author = {M. R. Schoeberl and R. S. Lindzen},
	File = {../../Papers/schoeberl84.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1368--1379},
	Title = {A Numerical Simulation of Barotropic Instability. {P}art {I}: Wave-Mean Flow Interaction},
	Volume = 41,
	Year = 1984,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zY2hvZWJlcmw4NC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNDwhD4ElBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwhFokgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2Nob2ViZXJsODQucGRmAA4AIAAPAHMAYwBoAG8AZQBiAGUAcgBsADgANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2Nob2ViZXJsODQucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2Nob2ViZXJsODQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Schoeberl86,
	Annote = {Filed under Barotropic Point Jet.},
	Author = {M. R. Schoeberl and J. E. Nielsen},
	File = {../../Papers/schoeberl86.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1045--1050},
	Title = {A Numerical Simulation of Barotropic Instability. {P}art {III}: Wave-Wave Interaction in the Presence of Dissipation},
	Volume = 43,
	Year = 1986,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zY2hvZWJlcmw4Ni5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNEwthLnFBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwtiuDAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2Nob2ViZXJsODYucGRmAA4AIAAPAHMAYwBoAG8AZQBiAGUAcgBsADgANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2Nob2ViZXJsODYucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2Nob2ViZXJsODYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Schubert01,
	Annote = {Defines potential vorticity with gradient of virtual
                  potential temperature. Claims that this potential
                  vorticity is adequate for a non-hydrostatic moist
                  atmosphere because it is not affected by
                  baroclinicity and it can be inverted to infer
                  balanced flow fields. However, this 'virtual
                  potential vorticity' is not conserved in moist
                  dynamics, not even in pseudoadiabatic dynamics, so
                  it is questionably how useful it really is. Only the
                  density effects of moisture are taken into account,
                  not the thermal effects (latent heat release).},
	Author = {W. H. Schubert and S. A. Hausman and M. Garcia and K. V. Ooyama and H.-C. Kuo},
	File = {../../Papers/schubert01.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3148--3157},
	Title = {Potential Vorticity in a Moist Atmosphere},
	Volume = 58,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zY2h1YmVydDAxLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNGvEWlywAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvEYWSwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NodWJlcnQwMS5wZGYAAA4AHgAOAHMAYwBoAHUAYgBlAHIAdAAwADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3NjaHViZXJ0MDEucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3NjaHViZXJ0MDEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Schubert95,
	Annote = {Rossby adjustment of inversion layer. Inversion
                  height cannot slope strongly from subtropics to
                  tropics.},
	Author = {W. H. Schubert and P. E. Ciesielski and C. Lu and R. H. Johnson},
	File = {../../Papers/schubert95.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2941--2952},
	Title = {Dynamical Adjustment of the Trade Wind Inversion Layer},
	Volume = 52,
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zY2h1YmVydDk1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNHvkd2iAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvkfnCAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NodWJlcnQ5NS5wZGYAAA4AHgAOAHMAYwBoAHUAYgBlAHIAdAA5ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3NjaHViZXJ0OTUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3NjaHViZXJ0OTUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Schubert99,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {W. H. Schubert and M. T. Montgomery and R. K. Taft and T. A. Guinn and S. R. Fulton and J. P. Kossin and J. P. Edwards},
	File = {../../Papers/schubert99.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1197--1222},
	Title = {Polygonal eyewalls, asymmetric eye contraction, and potential vorticity mixing in hurricanes},
	Volume = 56,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zY2h1YmVydDk5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNIwsRRkVBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsS0AQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NodWJlcnQ5OS5wZGYAAA4AHgAOAHMAYwBoAHUAYgBlAHIAdAA5ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3NjaHViZXJ0OTkucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3NjaHViZXJ0OTkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Schumacher03,
	Annote = {Filed under Cloud Observations.},
	Author = {C. Schumacher and R. A. Houze, Jr.},
	File = {../../Papers/schumacher03.pdf},
	Journal = {J. Appl. Meteor.},
	Pages = {1519--1524},
	Title = {The {TRMM} Precipitation Radar's View of Shallow, Isolated Rain},
	Volume = 42,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzY2h1bWFjaGVyMDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNJwGAkSAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwGCGuAAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NodW1hY2hlcjAzLnBkZgAADgAiABAAcwBjAGgAdQBtAGEAYwBoAGUAcgAwADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3NjaHVtYWNoZXIwMy5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc2NodW1hY2hlcjAzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Schwarz78,
	Annote = {Not on file.},
	Author = {G. Schwarz},
	Journal = {Ann. Stat.},
	Pages = {461--464},
	Title = {Estimating the Dimension of a Model},
	Volume = 6,
	Year = 1978}

@article{Schwarzschild1906,
	Author = {K. Schwarzschild},
	File = {../../Papers/schwarzschild1906.pdf},
	Journal = {Nachrichten von der K{\"o}niglichen Gesellschaft der Wissenschaften zu G{\"o}ttingen. Math.-phys.\ Klasse},
	Pages = {41--53},
	Title = {{\"U}ber das {G}leich\-ge\-wicht der {S}onnen\-atmo\-sph{\"a}re},
	Volume = 195,
	Year = 1906,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYgAAAAAAYgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhVzY2h3YXJ6c2NoaWxkMTkwNi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNKv021kVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv04YAQAAAAEADAAJDH4ACE6zAACS8wACADRNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2Nod2FyenNjaGlsZDE5MDYucGRmAA4ALAAVAHMAYwBoAHcAYQByAHoAcwBjAGgAaQBsAGQAMQA5ADAANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAChVc2Vycy90YXBpby9QYXBlcnMvc2Nod2FyenNjaGlsZDE5MDYucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfECIuLi8uLi9QYXBlcnMvc2Nod2FyenNjaGlsZDE5MDYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAiwCLgIzAjwCRwJLAlkCYAJpAo4CkwKWAqMCqAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAK6}}

@article{Scinocca98,
	Annote = {Filed under Haynes.},
	Author = {J. F. Scinocca and P. H. Haynes},
	Journal = {J. Atmos. Sci.},
	Pages = {2361--2392},
	Title = {Dynamical Forcing of Stratospheric Waves by the Tropospheric Circulation},
	Volume = 55,
	Year = 1998}

@article{Scott08,
	Author = {Scott, R. K. and Polvani, L. M.},
	File = {../../Papers/scott08.pdf},
	Journal = {Geophys. Res. Lett.},
	Pages = {L24202},
	Title = {Equatorial superrotation in shallow atmospheres},
	Volume = {35},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzY290dDA4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNMxqHwTwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxqJSvwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NvdHQwOC5wZGYADgAYAAsAcwBjAG8AdAB0ADAAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc2NvdHQwOC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zY290dDA4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==},
	Bdsk-File-2 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zY290dDA4X3BybC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNPw/jEcVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw/k08QAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NvdHQwOF9wcmwucGRmAA4AIAAPAHMAYwBvAHQAdAAwADgAXwBwAHIAbAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2NvdHQwOF9wcmwucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2NvdHQwOF9wcmwucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc},
	Bdsk-File-3 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYAAAAAAAYAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhNzY290dDA4X2dybF9yZXYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNOxWKf6gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxWMQagAAAAEADAAJDH4ACE6zAACS8wACADJNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NvdHQwOF9ncmxfcmV2LnBkZgAOACgAEwBzAGMAbwB0AHQAMAA4AF8AZwByAGwAXwByAGUAdgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACZVc2Vycy90YXBpby9QYXBlcnMvc2NvdHQwOF9ncmxfcmV2LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAgLi4vLi4vUGFwZXJzL3Njb3R0MDhfZ3JsX3Jldi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACJAImAisCNAI/AkMCUQJYAmEChAKJAowCmQKeAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAArA=},
	Bdsk-File-4 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zY290dDA4X2dybC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNNxPij7wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxPkGXwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2NvdHQwOF9ncmwucGRmAA4AIAAPAHMAYwBvAHQAdAAwADgAXwBnAHIAbAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2NvdHQwOF9ncmwucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2NvdHQwOF9ncmwucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@book{Scott92,
	Author = {D. W. Scott},
	Pages = 317,
	Publisher = {Wiley},
	Series = {Series in Probability and Mathematical Statistics},
	Title = {Multivariate Density Estimation: Theory, Practice, and Visualization},
	Year = 1992}

@article{Seager02,
	Author = {R. Seager and D. S. Battisti and J. Yin and N. Gordon and N. Naik and A. C. Clement and M. A. Cane},
	File = {../../Papers/seager02.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {???},
	Title = {Is the {G}ulf {S}tream responsible for {E}urope's mild winters},
	Volume = 128,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzZWFnZXIwMi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNQxnjitQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxnlFJQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2VhZ2VyMDIucGRmAAAOABoADABzAGUAYQBnAGUAcgAwADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NlYWdlcjAyLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zZWFnZXIwMi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Seager03,
	Annote = {Follow-up to Robinson02a. Try to account for
                  extratropical cooling in response to tropical
                  warming by considering eddy-driven Eulerian mean
                  meridional circulation. Claim that changes in
                  momentum fluxes, due to changes in zonal winds, are
                  responsible for change of circulation that leads to
                  cooling.},
	Author = {R. Seager and N. Harnik and Y. Kushnir and W. Robinson and J. Miller},
	File = {../../Papers/seager03.pdf},
	Journal = {J. Climate},
	Pages = {??},
	Title = {Mechanisms of hemispherically symmetric climate variability},
	Volume = {??},
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzZWFnZXIwMy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNRv92UWFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv94E2AAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2VhZ2VyMDMucGRmAAAOABoADABzAGUAYQBnAGUAcgAwADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NlYWdlcjAzLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zZWFnZXIwMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Seager07,
	Author = {Richard Seager and Mingfang Ting and Isaac Held and Yochanan Kushnir and Jian Lu and Gabriel Vecchi and Huei-Ping Huang and Nili Harnik and Ants Leetmaa and Ngar-Cheung Lau and Cuihua Li and Jennifer Velez and Naomi Naik},
	File = {../../Papers/seager07.pdf},
	Journal = {Science},
	Pages = {1181--1184},
	Title = {Model Projections of an Imminent Transition to a More Arid Climate in Southwestern {N}orth {A}merica},
	Volume = 316,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzZWFnZXIwNy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNTwoXUxAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwoY3NAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2VhZ2VyMDcucGRmAAAOABoADABzAGUAYQBnAGUAcgAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NlYWdlcjA3LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zZWFnZXIwNy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@incollection{Seager07a,
	Address = {Princeton, NJ},
	Author = {R. Seager and D. S. Battisti},
	Booktitle = {The Global Circulation of the Atmosphere},
	Date-Modified = {2010-06-11 11:43:35 -0700},
	Editor = {T. Schneider and A. H. Sobel},
	Pages = {331--371},
	Publisher = {Princeton University Press},
	Title = {Challenges to Our Understanding of the General Circulation: {A}brupt Climate Change},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zZWFnZXIwN2EucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNUwoPJZQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwoQr1QAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2VhZ2VyMDdhLnBkZgAOABwADQBzAGUAYQBnAGUAcgAwADcAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc2VhZ2VyMDdhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3NlYWdlcjA3YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Seidel01,
	Author = {D. J. Seidel and R. J. Ross and J. K. Angell and G. C. Reid},
	File = {../../Papers/seidel01.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {7857--7878},
	Title = {Climatological characteristics of the tropical tropopause as revealed by radiosondes},
	Volume = {106},
	Year = {2001},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzZWlkZWwwMS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNWxgK6+AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxgMdaAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2VpZGVsMDEucGRmAAAOABoADABzAGUAaQBkAGUAbAAwADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NlaWRlbDAxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zZWlkZWwwMS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Seidel07,
	Author = {D. J. Seidel and W. J. Randel},
	File = {../../Papers/seidel07.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {D20113},
	Title = {Recent widening of the tropical belt: Evidence from tropopause observations},
	Volume = 112,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzZWlkZWwwNy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNYw67KdlBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw6869gAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2VpZGVsMDcucGRmAAAOABoADABzAGUAaQBkAGUAbAAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NlaWRlbDA3LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zZWlkZWwwNy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Seidel08,
	Author = {D. J. Seidel and Q. Fu and W. J. Randel and T. J. Reichler},
	File = {../../Papers/seidel08.pdf},
	Journal = {Nature Geosci.},
	Pages = {21--24},
	Title = {Widening of the tropical belt in a changing climate},
	Volume = 1,
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzZWlkZWwwOC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNZw6VOpVBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw6W/JQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2VpZGVsMDgucGRmAAAOABoADABzAGUAaQBkAGUAbAAwADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NlaWRlbDA4LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zZWlkZWwwOC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Seiff96,
	Annote = {Filed under Jupiter dynamics.},
	Author = {Seiff, A. and Kirk, D.B. and Knight, T.C.D. and Mihalov, J.D. and Blanchard, R.C. and Young, R.E. and Schubert, G. and von Zahn, U. and Lehmacher, G. and Milos, F.S. and Wang, J.},
	File = {../../Papers/seiff96.pdf},
	Journal = {Science},
	Pages = {844--845},
	Title = {Structure of the Atmosphere of {J}upiter: {Galileo} Probe Measurements},
	Volume = {272},
	Year = {1996},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzZWlmZjk2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNaw7Z72AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7bsWAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2VpZmY5Ni5wZGYADgAYAAsAcwBlAGkAZgBmADkANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc2VpZmY5Ni5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zZWlmZjk2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Seiff97,
	Annote = {Filed under Jupiter dynamics.},
	Author = {Seiff, A. and Kirk, D.B. and Knight, T.C.D. and Young, L.A. and Milos, F.S. and Venkatapathy, E. and Mihalov, J.D. and Blanchard, R.C. and Young, R.E. and Schubert, G.},
	File = {../../Papers/seiff97.pdf},
	Journal = {Science},
	Pages = {102--104},
	Title = {Thermal Structure of {J}upiter's Upper Atmosphere Derived from the {Galileo} probe},
	Volume = {276},
	Year = {1997},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzZWlmZjk3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNbw7Z5ygAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7bqSgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2VpZmY5Ny5wZGYADgAYAAsAcwBlAGkAZgBmADkANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc2VpZmY5Ny5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zZWlmZjk3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Sellers69,
	Annote = {Considers energy balance at surface to obtain
                  zonally averaged surface temperature and estimates
                  of climate sensitivity.},
	Author = {W. D. Sellers},
	Journal = {J. Appl. Meteor.},
	Pages = {392--400},
	Title = {A Global Climatic Model Based on the Energy Balance of the {E}arth-Atmosphere System},
	Volume = 8,
	Year = 1969}

@article{Seltzer02,
	Annote = {Filed under Paleo-Climate Reviews. Warming of Andes
                  preceded major temperature change in the Northern
                  Hemisphere by at least 5000 yrs. Late Pleistocene in
                  tropical Andes was wet.},
	Author = {G. O. Seltzer and D. T. Rodbell and P. A. Baker and S. C. Fritz and P. M. Tapia and H. D. Rowe and R. B. Dunbar},
	Journal = {Science},
	Pages = {1685--1686},
	Title = {Early Warming of Tropical {S}outh {A}merica at the Last Glacial-Interglacial Transition},
	Volume = 296,
	Year = 2002}

@article{Semeniuk01a,
	Annote = {Filed under Shepherd.},
	Author = {K. Semeniuk and T. G. Shepherd},
	Journal = {J. Atmos. Sci.},
	Pages = {3077--3096},
	Title = {The Middle-Atmosphere {H}adley Circulation and Equatorial Inertial Adjustment},
	Volume = 58,
	Year = 2001}

@article{Semeniuk01b,
	Annote = {Filed under Shepherd.},
	Author = {K. Semeniuk and T. G. Shepherd},
	Journal = {J. Atmos. Sci.},
	Pages = {3097--3115},
	Title = {Mechanism for Tropical Upwelling in the Stratosphere},
	Volume = 58,
	Year = 2001}

@article{Sen98,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {B. Sen and G. C. Toon and G. B. Osterman and J.-F. Blavier and J. J. Margitan and R. J. Salawitch and G. K. Yue},
	Journal = {J. Geophys. Res.},
	Pages = {3571--3585},
	Title = {Measurements of reactive nitrogen in the stratosphere},
	Volume = {103D},
	Year = 1998}

@article{Shannon48,
	Annote = {Classic paper on Shannon information.},
	Author = {C. E. Shannon},
	Crossref = {Shannon49},
	Journal = {Bell Syst. Tech. J.},
	Note = {Reprinted in \citet{Shannon49}.},
	Pages = {370--423, 623--656},
	Title = {A Mathematical Theory of Communication},
	Volume = 27,
	Year = 1948}

@book{Shannon49,
	Address = {Urbana},
	Annote = {Classical book on information theory. Contains
                  Shannon48 plus an introductory paper by Weaver.},
	Author = {C. E. Shannon and W. Weaver},
	Pages = {117},
	Publisher = {University of Illinois Press},
	Title = {The Mathematical Theory of Communication},
	Year = 1949}

@book{Shaw30,
	Address = {London, UK},
	Author = {N. Shaw},
	Pages = 445,
	Publisher = {Cambridge University Press},
	Title = {Manual of Meteorology. Vol.~III. The Physical Processes of Weather},
	Year = 1930}

@article{Shea87,
	Annote = {Filed under AR Modeling.},
	Author = {B. L. Shea},
	Journal = {J. Time Series Anal.},
	Pages = {95--110},
	Title = {Estimation of Multivariate Time Series},
	Volume = 8,
	Year = 1987}

@article{Shell04,
	Author = {Shell, K. M. and Held, I. M.},
	File = {../../Papers/shell04.pdf},
	Journal = {J. Atmos. Sci.},
	Number = 23,
	Pages = {2928--2935},
	Title = {Abrupt transition to strong superrotation in an axisymmetric model of the upper troposphere},
	Volume = 61,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzaGVsbDA0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNfwTYhulBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwTaEKgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hlbGwwNC5wZGYADgAYAAsAcwBoAGUAbABsADAANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc2hlbGwwNC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zaGVsbDA0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Shepherd00,
	Annote = {Review of middle atmosphere dynamics and chemistry.},
	Author = {T. G. Shepherd},
	Journal = {J. Atmos. Sol.-Terr. Phys.},
	Pages = {1587--1601},
	Title = {The middle atmosphere},
	Volume = 62,
	Year = 2000}

@article{Shepherd02,
	Annote = {Review.},
	Author = {T. G. Shepherd},
	Journal = {J. Meteor. Soc. Japan},
	Pages = {769--792},
	Title = {Issues in stratosphere-troposphere coupling},
	Volume = 80,
	Year = 2002}

@article{Shepherd87a,
	Annote = {Atmospheric turbulence spectra from observational
                  data.},
	Author = {T. G. Shepherd},
	File = {../../Papers/shepherd87a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1166--1178},
	Title = {A Spectral View of Nonlinear Fluxes and Stationary-Transient Interaction in the Atmosphere},
	Volume = 44,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zaGVwaGVyZDg3YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNhvbVOLAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvbW+rAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hlcGhlcmQ4N2EucGRmAA4AIAAPAHMAaABlAHAAaABlAHIAZAA4ADcAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2hlcGhlcmQ4N2EucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2hlcGhlcmQ4N2EucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Shepherd87b,
	Author = {T. G. Shepherd},
	File = {../../Papers/shepherd87b.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {467--509},
	Title = {Rossby waves and two-dimensional turbulence in a large-scale zonal jet},
	Volume = 183,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zaGVwaGVyZDg3Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNixCfQUQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxCgywQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hlcGhlcmQ4N2IucGRmAA4AIAAPAHMAaABlAHAAaABlAHIAZAA4ADcAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2hlcGhlcmQ4N2IucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2hlcGhlcmQ4N2IucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Shepherd87c,
	Author = {T. G. Shepherd},
	File = {../../Papers/shepherd87c.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {289--302},
	Title = {Non-ergodicity of inviscid two-dimensional flow on a beta-plane and on the surface of a rotating sphere},
	Volume = 184,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zaGVwaGVyZDg3Yy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNjwjqPAgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwjrxcgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hlcGhlcmQ4N2MucGRmAA4AIAAPAHMAaABlAHAAaABlAHIAZAA4ADcAYwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2hlcGhlcmQ4N2MucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2hlcGhlcmQ4N2MucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Shepherd88a,
	Annote = {Bounds on saturation from nonlinear pseudomomentum
                  and pseudoenergy conservation.},
	Author = {T. G. Shepherd},
	Journal = {J. Fluid Mech.},
	Pages = {291--322},
	Title = {Rigorous bounds on the nonlinear saturation of instabilities to parallel shear flows},
	Volume = 196,
	Year = 1988}

@article{Shepherd88b,
	Annote = {Bounds on saturation potential enstrophy from
                  nonlinear pseudomomentum conservation. Potential
                  enstrophy proportional to supercriticality.},
	Author = {T. G. Shepherd},
	Journal = {J. Atmos. Sci.},
	Pages = {2014--2025},
	Title = {Nonlinear saturation of baroclinic instability. {P}art {I}: {T}he two-layer model},
	Volume = 45,
	Year = 1988}

@article{Shepherd89,
	Annote = {Bounds on saturation surface-APE and potential
                  enstrophy from nonlinear pseudomomentum conservation
                  for stratified flows.},
	Author = {T. G. Shepherd},
	Journal = {J. Atmos. Sci.},
	Pages = {888--907},
	Title = {Nonlinear saturation of baroclinic instability. {P}art {II}: {C}ontinuously stratified flow},
	Volume = 46,
	Year = 1989}

@article{Shepherd93,
	Annote = {APE is non-kinetic part of pseudo-energy. Quadratic
                  in vicinity of equilibrium.},
	Author = {T. G. Shepherd},
	File = {../../Papers/shepherd93.pdf},
	Journal = {Atmos.-Ocean},
	Pages = {1--26},
	Title = {A Unified Theory of Available Potential Energy},
	Volume = 31,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zaGVwaGVyZDkzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNkvE0lbAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvE2V7AAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hlcGhlcmQ5My5wZGYAAA4AHgAOAHMAaABlAHAAaABlAHIAZAA5ADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3NoZXBoZXJkOTMucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3NoZXBoZXJkOTMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Shepherd93b,
	Annote = {Rigorous bounds on eddy energies on two-layer model;
                  comparison with weakly nonlinear theory: same
                  scaling behavior.},
	Author = {T. G. Shepherd},
	File = {../../Papers/shepherd93b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2697--2709},
	Title = {Nonlinear saturation of baroclinic instability. {Part~III}: {B}ounds on the energy},
	Volume = 50,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zaGVwaGVyZDkzYi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNlvivXLAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvixHrAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hlcGhlcmQ5M2IucGRmAA4AIAAPAHMAaABlAHAAaABlAHIAZAA5ADMAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2hlcGhlcmQ5M2IucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2hlcGhlcmQ5M2IucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Sherman49,
	Annote = {Sherman-Morrison formula for computation of inverse},
	Author = {J. Sherman and W. J. Morrison},
	Journal = {Ann. Math. Statist.},
	Pages = 621,
	Title = {Adjustment of an inverse matrix corresponding to changes in the elements of a given column or given row of the original matrix},
	Volume = 20,
	Year = 1949}

@article{Sherwood00,
	Author = {S. C. Sherwood},
	Journal = {J. Geophys. Res.},
	Pages = {29489--29500},
	Title = {Climate signals from station arrays with missing data, and an application to winds},
	Volume = {105D},
	Year = 2000}

@article{Sherwood01,
	Annote = {Dehydration at tropical tropopause.},
	Author = {S. C. Sherwood and A. E. Dessler},
	Journal = {J. Atmos. Sci.},
	Pages = {765--779},
	Title = {A Model for Transport across the Tropical Tropopause},
	Volume = 58,
	Year = 2001}

@article{Sherwood02,
	Annote = {Smaller ice crystals in upper troposphere sink more
                  slowly and sublimate more easily, thus may lead to
                  increase in upper tropospheric and stratospheric
                  relative humidity; smaller ice crystals may be due
                  to aerosols produced by biomass burning.},
	Author = {S. Sherwood},
	Journal = {Science},
	Pages = {1272--1275},
	Title = {A Microphysical Connection Among Biomass Burning, Cumulus Clouds, and Stratospheric Moisture},
	Volume = 295,
	Year = 2002}

@article{Sherwood06b,
	Author = {S. C. Sherwood and C. L. Meyer},
	Date-Modified = {2010-06-11 11:01:42 -0700},
	File = {../../Papers/sherwood06b.pdf},
	Journal = {J. Climate},
	Pages = {6278--6290},
	Title = {The General Circulation and Robust Relative Humidity},
	Volume = 19,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zaGVyd29vZDA2Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNnxoC3BAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxoEZdAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hlcndvb2QwNmIucGRmAA4AIAAPAHMAaABlAHIAdwBvAG8AZAAwADYAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2hlcndvb2QwNmIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2hlcndvb2QwNmIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Sherwood09,
	Author = {S. C. Sherwood and R.~Roca and T.~M.~Weckwerth and N.~G.~Andronova},
	Journal = {Rev. Geophys.},
	Note = {In press.},
	Pages = {??},
	Title = {Tropospheric water vapor, convection and climate: a critical review},
	Volume = {??},
	Year = 2009}

@article{Sherwood96a,
	Author = {S. C. Sherwood},
	File = {../../Papers/sherwood96a.pdf},
	Journal = {J. Climate},
	Pages = {2903--2918},
	Title = {Maintenance of the Free-Tropospheric Tropical Water Vapor Distribution. {P}art~{I}: {C}lear Regime Budget},
	Volume = 9,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zaGVyd29vZDk2YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNpwHmv9FBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwHoSZAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hlcndvb2Q5NmEucGRmAA4AIAAPAHMAaABlAHIAdwBvAG8AZAA5ADYAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2hlcndvb2Q5NmEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2hlcndvb2Q5NmEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Sherwood96b,
	Author = {S. C. Sherwood},
	File = {../../Papers/sherwood96b.pdf},
	Journal = {J. Climate},
	Pages = {2919--2934},
	Title = {Maintenance of the Free-Tropospheric Tropical Water Vapor Distribution. {P}art~{II}: {S}imulation by Large-Scale Advection},
	Volume = 9,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zaGVyd29vZDk2Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNqwHmwQVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwHoSsQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hlcndvb2Q5NmIucGRmAA4AIAAPAHMAaABlAHIAdwBvAG8AZAA5ADYAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc2hlcndvb2Q5NmIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc2hlcndvb2Q5NmIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Shibata76,
	Annote = {Not on file.},
	Author = {R. Shibata},
	Journal = {Biometrika},
	Pages = {117--126},
	Title = {Selection of the Order of an Autoregressive Model by {A}kaike's {I}nformation {C}riterion},
	Volume = 63,
	Year = 1976}

@article{Shige01,
	Annote = {Gravity-wave mediated mechanism for westward
                  generation of convective bands.},
	Author = {S. Shige and T. Satomura},
	Journal = {J. Atmos. Sci.},
	Pages = {3724--3740},
	Title = {Westward Generation of Eastward-Moving Tropical Convective Bands in {TOGA} {COARE}},
	Volume = 58,
	Year = 2001}

@article{Shine91,
	Author = {K. P. Shine and A. Shina},
	Journal = {Nature},
	Pages = {382--384},
	Title = {Sensitivity of the {E}arth's climate to height-dependent changes in water vapour mixing ratio},
	Volume = 354,
	Year = 1991}

@article{Short00,
	Annote = {Filed under Cloud Observations.},
	Author = {D. A. Short and K. Nakamura},
	File = {../../Papers/short00.pdf},
	Journal = {J. Climate},
	Pages = {4107--4124},
	Title = {{TRMM} Radar Observations of Shallow Precipitation over the Tropical Oceans},
	Volume = 13,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzaG9ydDAwLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNtwGAkUgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwGCGwgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hvcnQwMC5wZGYADgAYAAsAcwBoAG8AcgB0ADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc2hvcnQwMC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zaG9ydDAwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Showman07,
	Author = {A. P. Showman},
	File = {../../Papers/showman07.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3132--3157},
	Title = {Numerical Simulations of Forced Shallow-Water Turbulence: Effects of Moist Convection on the Large-Scale Circulation of {J}upiter and {S}aturn},
	Volume = 64,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zaG93bWFuMDcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNvwy8pJFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwy+LlAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hvd21hbjA3LnBkZgAOABwADQBzAGgAbwB3AG0AYQBuADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc2hvd21hbjA3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3Nob3dtYW4wNy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Showman98,
	Author = {Showman, A.P. and Ingersoll, A.P.},
	File = {../../Papers/showman98.pdf},
	Journal = {Icarus},
	Pages = {205--220},
	Title = {Interpretation of {Galileo} Probe Data and Implications for {Jupiter}'s Dry Downdrafts},
	Volume = {132},
	Year = {1998},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zaG93bWFuOTgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNxxGmIgQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxGnq8QAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2hvd21hbjk4LnBkZgAOABwADQBzAGgAbwB3AG0AYQBuADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc2hvd21hbjk4LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3Nob3dtYW45OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Shraiman00,
	Annote = {Filed under Turbulence Reviews.},
	Author = {B. I. Shraiman and E. D. Siggia},
	Journal = {Nature},
	Pages = {639--646},
	Title = {Scalar Turbulence},
	Volume = 405,
	Year = 2000}

@article{Shukla81,
	Annote = {Not on file.},
	Author = {J. Shukla},
	Journal = {J. Atmos. Sci.},
	Pages = {2547--2572},
	Title = {Dynamical Predictability of Monthly Means},
	Volume = 38,
	Year = 1981}

@incollection{Shukla85,
	Annote = {Not on file.},
	Author = {J. Shukla},
	Booktitle = {Advances in Geophysics},
	Pages = {87--122},
	Publisher = {Academic Press},
	Title = {Predictability},
	Volume = {28b},
	Year = 1985}

@article{Shukla98,
	Annote = {Filed under Predictability. Features of tropical
                  circulation are strongly determined by lower
                  boundary condition and so do not depend sensitively
                  on initial conditions.},
	Author = {J. Shukla},
	File = {../../Papers/Shukla98.pdf},
	Journal = {Science},
	Pages = {728--731},
	Title = {Predictability in the Midst of Chaos: A Scientific Basis for Climate Forecasting},
	Volume = 282,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxTaHVrbGE5OC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRNyvAI1SQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvAKlyQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6U2h1a2xhOTgucGRmAAAOABoADABTAGgAdQBrAGwAYQA5ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL1NodWtsYTk4LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9TaHVrbGE5OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Shutts81,
	Annote = {Filed under Maximum Entropy Production Principles.},
	Author = {G. J. Shutts},
	File = {../../Papers/shutts81.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {503--520},
	Title = {Maximum entropy production states in quasi-geostrophic dynamical systems},
	Volume = 107,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzaHV0dHM4MS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRN4vFqekQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvFsPEQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2h1dHRzODEucGRmAAAOABoADABzAGgAdQB0AHQAcwA4ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NodXR0czgxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zaHV0dHM4MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Siebesma03,
	Author = {A. P. Siebesma and C. S. Bretherton and A. Brown and A. Chlond and J. Cuxart and P. G. Duynkerke and H. Jiang and M. Khairoutdinov and D. Lewellen and C. H. Moeng and E. Sanchez and B. Stevens and D. E. Stevens},
	File = {../../Papers/siebesma03.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1201--1219},
	Title = {A large eddy simulation intercomparison study of shallow cumulus convection},
	Volume = {60},
	Year = {2003},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zaWViZXNtYTAzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRN5x7FfjQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx7HQDQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2llYmVzbWEwMy5wZGYAAA4AHgAOAHMAaQBlAGIAZQBzAG0AYQAwADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3NpZWJlc21hMDMucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3NpZWJlc21hMDMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Siebesma07,
	Author = {A. P. Siebesma and P. M. M. Soares and J. Teixeira},
	File = {../../Papers/siebesma07.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1230--1248},
	Title = {A combined eddy-diffusivity mass-flux approach for the convective boundary layer},
	Volume = {64},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zaWViZXNtYTA3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRN6x0gnxwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx0iYRwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2llYmVzbWEwNy5wZGYAAA4AHgAOAHMAaQBlAGIAZQBzAG0AYQAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3NpZWJlc21hMDcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3NpZWJlc21hMDcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Siggia94,
	Annote = {Filed under Rayleigh-Benard Convection.},
	Author = {E. D. Siggia},
	File = {../../Papers/siggia94.pdf},
	Journal = {Ann. Rev. Fluid. Mech.},
	Pages = {137--168},
	Title = {High {R}ayleigh Number Convection},
	Volume = 26,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzaWdnaWE5NC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRN8u+q+ggAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAu+svAgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2lnZ2lhOTQucGRmAAAOABoADABzAGkAZwBnAGkAYQA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NpZ2dpYTk0LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zaWdnaWE5NC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Sigman00,
	Annote = {Filed under Paleo-Climate Reviews.},
	Author = {D. M. Sigman and E. A. Boyle},
	Journal = {Nature},
	Pages = {859--869},
	Title = {Glacial/interglacial variations in atmospheric carbon dioxide},
	Volume = 407,
	Year = 2000}

@book{Silverman86,
	Address = {London},
	Author = {B. W. Silverman},
	Pages = 175,
	Publisher = {Chapman and Hall},
	Title = {Density Estimation for Statistics and Data Analysis},
	Year = 1986}

@article{Simmons74,
	Annote = {Normal modes in two-layer QG model with meridional
                  shear in upper layer. If meridional scale of zonal
                  flow is order Rossby radius, so is meridional scale
                  of most unstable wave. If meridional scale of zonal
                  flow is greater, meridional scale of most unstable
                  wave is greater than Rossby radius (but smaller than
                  meridional scale of zonal flow).},
	Author = {A. J. Simmons},
	File = {../../Papers/simmons74.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1515--1525},
	Title = {The meridional scale of baroclinic waves},
	Volume = 31,
	Year = 1974,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zaW1tb25zNzQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRN+wOJymAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwOLVCAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2ltbW9uczc0LnBkZgAOABwADQBzAGkAbQBtAG8AbgBzADcANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc2ltbW9uczc0LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3NpbW1vbnM3NC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Simmons76,
	Author = {A. J. Simmons and B. J. Hoskins},
	File = {../../Papers/simmons76.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1454--1477},
	Title = {Baroclinic Instability on the Sphere: {N}ormal Modes of the Primitive and Quasigeostrophic Equations},
	Volume = 33,
	Year = 1976,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zaW1tb25zNzYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRN/vUprNgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvUrNpgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2ltbW9uczc2LnBkZgAOABwADQBzAGkAbQBtAG8AbgBzADcANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc2ltbW9uczc2LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3NpbW1vbnM3Ni5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Simmons77,
	Annote = {Normal modes of primitive equations linearized about
                  a climatological mean state.},
	Author = {A. J. Simmons and B. J. Hoskins},
	Journal = {J. Atmos. Sci.},
	Pages = {581--588},
	Title = {Baroclinic Instability on the Sphere: Solutions with a More Realistic Tropopause},
	Volume = 34,
	Year = 1977}

@article{Simmons78,
	Annote = {Nonlinear life cycle simulations of baroclinic
                  waves. Nonlinear development leads to increased
                  upper-level amplitude of wave (and fluxes).},
	Author = {A. J. Simmons and B. J. Hoskins},
	Journal = {J. Atmos. Sci.},
	Pages = {414--432},
	Title = {The Life Cycles of Some Nonlinear Baroclinic Waves},
	Volume = 35,
	Year = 1978}

@article{Simmons80,
	Annote = {Secondary barotropic instability can alter
                  baroclinic life cycles significantly.},
	Author = {A. J. Simmons and B. J. Hoskins},
	Journal = {J. Atmos. Sci.},
	Pages = {1679--1684},
	Title = {Barotropic Influences on the Growth and Decay of Nonlinear Baroclinic Waves},
	Volume = 37,
	Year = 1980}

@article{Simmons81,
	Author = {A. J. Simmons and D. M. Burridge},
	File = {../../Papers/simmons81.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {758--766},
	Title = {An Energy and Angular-Momentum Conserving Vertical Finite-Difference Scheme and Hybrid Vertical Coordinates},
	Volume = 109,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zaW1tb25zODEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROCxLwZ3QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxLx8TQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2ltbW9uczgxLnBkZgAOABwADQBzAGkAbQBtAG8AbgBzADgAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc2ltbW9uczgxLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3NpbW1vbnM4MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Simmons99,
	Annote = {Filed under ECMWF Data.},
	Author = {A. J. Simmons and A. Untch and C. Jakob and P. K{\aa}llberg and P. Und{\'e}n},
	File = {../../Papers/simmons99.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {353--386},
	Title = {Stratospheric water vapour and tropical tropopause temperatures in {ECMWF} analyses and multi-year simulations},
	Volume = 125,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zaW1tb25zOTkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROEv3MIZlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3Nq1gAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2ltbW9uczk5LnBkZgAOABwADQBzAGkAbQBtAG8AbgBzADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc2ltbW9uczk5LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3NpbW1vbnM5OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Simon-Miller06,
	Author = {A. A. Simon-Miller and B. J. Conrath and P. J. Gierasch and G. S. Orton and R. K. Achterberg and F. M. Flasar and B. M. Fisher},
	File = {../../Papers/simon-miller06.pdf},
	Journal = {Icarus},
	Pages = {98--112},
	Title = {Jupiter's atmospheric temperatures: From {Voyager} {IRIS} to {Cassini} {CIRS}},
	Volume = 180,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAX4AAAAAAX4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhJzaW1vbi1taWxsZXIwNi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROFwxxMyVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwxyvOQAAAAEADAAJDH4ACE6zAACS8wACADFNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c2ltb24tbWlsbGVyMDYucGRmAAAOACYAEgBzAGkAbQBvAG4ALQBtAGkAbABsAGUAcgAwADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAlVXNlcnMvdGFwaW8vUGFwZXJzL3NpbW9uLW1pbGxlcjA2LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHy4uLy4uL1BhcGVycy9zaW1vbi1taWxsZXIwNi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACIgIkAikCMgI9AkECTwJWAl8CgQKGAokClgKbAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAq0=}}

@article{Smagorinsky63,
	Author = {J. Smagorinsky},
	File = {../../Papers/smagorinsky63.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {99--164},
	Title = {General Circulation Experiments with the Primitive Equations. I. The Basic Experiment},
	Volume = 91,
	Year = 1963,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXgAAAAAAXgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhFzbWFnb3JpbnNreTYzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROIv9hoEgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv9jYkgAAAAEADAAJDH4ACE6zAACS8wACADBNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c21hZ29yaW5za3k2My5wZGYADgAkABEAcwBtAGEAZwBvAHIAaQBuAHMAawB5ADYAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACRVc2Vycy90YXBpby9QYXBlcnMvc21hZ29yaW5za3k2My5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHi4uLy4uL1BhcGVycy9zbWFnb3JpbnNreTYzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIcAh4CIwIsAjcCOwJJAlACWQJ6An8CggKPApQAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACpg==}}

@article{Smagorinsky65,
	Author = {J. Smagorinsky and S. Manabe and Holloway, Jr., J. L.},
	File = {../../Papers/smagorinsky65.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {727--768},
	Title = {Numerical Results from a Nine-Level General Circulation Model of the Atmosphere},
	Volume = 93,
	Year = 1965,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXgAAAAAAXgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhFzbWFnb3JpbnNreTY1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROJwkaMOFBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwkbuqAAAAAEADAAJDH4ACE6zAACS8wACADBNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c21hZ29yaW5za3k2NS5wZGYADgAkABEAcwBtAGEAZwBvAHIAaQBuAHMAawB5ADYANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACRVc2Vycy90YXBpby9QYXBlcnMvc21hZ29yaW5za3k2NS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QHi4uLy4uL1BhcGVycy9zbWFnb3JpbnNreTY1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIcAh4CIwIsAjcCOwJJAlACWQJ6An8CggKPApQAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACpg==}}

@article{Smith01,
	Author = {K. S. Smith and G. K. Vallis},
	Journal = {J. Phys. Oceanogr.},
	Pages = {554--571},
	Title = {The Scales and Equilibration of Midocean Eddies: Freely Evolving Flow},
	Volume = 31,
	Year = 2001}

@article{Smith02a,
	Author = {K. S. Smith and G. K. Vallis},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1699--1720},
	Title = {The Scales and Equilibration of Midocean Eddies: Forced-Dissipative Flow},
	Volume = 32,
	Year = 2002}

@article{Smith02b,
	Author = {K. S. Smith and G. Boccaletti and C. C. Henning and I. N. Marinov and C. Y. Tam and I. M. Held and G. K. Vallis},
	File = {../../Papers/smith02b.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {13--48},
	Title = {Turbulent diffusion in the geostrophic inverse energy cascade},
	Volume = 469,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzbWl0aDAyYi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROLvRebtwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRf+JwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c21pdGgwMmIucGRmAAAOABoADABzAG0AaQB0AGgAMAAyAGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NtaXRoMDJiLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zbWl0aDAyYi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Smith80,
	Annote = {Filed under Lee Vortex Generation.},
	Author = {R. B. Smith},
	Journal = {Tellus},
	Pages = {348--364},
	Title = {Linear theory of stratified hydrostatic flow past an isolated mountain},
	Volume = {32A},
	Year = 1980}

@article{Smith80a,
	Annote = {Filed under Regression Analysis. In the discussion,
                  Marquardt argues for centering and scaling.},
	Author = {G. Smith and F. Campbell},
	Journal = {J. Amer. Statist. Assoc.},
	Pages = {74--103 (including discussion)},
	Title = {A Critique of Some Ridge Regression Methods},
	Volume = 75,
	Year = 1980}

@article{Smith88,
	Annote = {Filed under Lee Vortex Generation. Collapse of
                  density surfaces on leeward slope.},
	Author = {R. B. Smith},
	Journal = {J. Atmos. Sci.},
	Pages = {3889--3396},
	Title = {Linear Theory of Stratified Flow past an Isolated Mountain in Isosteric Coordinates},
	Volume = 45,
	Year = 1988}

@incollection{Smith89a,
	Annote = {Filed under Lee Vortex Generation.},
	Author = {R. B. Smith},
	Booktitle = {Advances in Geophysics},
	Editor = {B. Saltzman},
	Pages = {1--41},
	Publisher = {Academic Press},
	Title = {Hydrostatic Airflow over Mountains},
	Volume = {31},
	Year = 1989}

@article{Smith89b,
	Annote = {Filed under Lee Vortex Generation. Comment on
                  Smolarkiewicz89: PV does not seem to be materially
                  conserved in simulations. Need dissipation?},
	Author = {R. B. Smith},
	Journal = {J. Atmos. Sci.},
	Pages = {3611--3613},
	Title = {Comment on ``{L}ow {F}roude Number Flow past Three-Dimensional Obstacles. {P}art {I}: Baroclinically Generated Lee Vortices''},
	Volume = 46,
	Year = 1989}

@article{Smith96,
	Annote = {Simple, non-iterative EOF reconstruction of
                  SST. Method is likely to exaggerate correlation
                  structure of data and certainly leads to biased
                  covariance matrix estimates.},
	Author = {T. M. Smith and R. W. Reynolds and R. E. Livezey and D. C. Stokes},
	Journal = {J. Climate},
	Pages = {1403--1420},
	Title = {Reconstruction of historical sea surface temperatures using empirical orthogonal functions},
	Volume = 9,
	Year = 1996}

@inproceedings{Smith97,
	Address = {Amsterdam},
	Annote = {Review of predictability in dynamical systems.},
	Author = {L. A. Smith},
	Booktitle = {Past and Present Variability of Solar-Terrestrial System: Measurement, Data Analysis and Theoretical Models},
	Editor = {G. C. Castagnoli and A. Provenzale},
	Organization = {Italian Physical Society},
	Pages = {177--246},
	Publisher = {IOS Press},
	Title = {The Maintenance of Uncertainty},
	Year = 1997}

@article{Smith99,
	Annote = {Linear waves in various models with small Rossby
                  number ("geostrophic potential vorticity",
                  quasigeostrophic, planetary geostrophic.},
	Author = {K. S. Smith and G. K. Vallis},
	File = {../../Papers/smith99.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1579--1593},
	Title = {Linear baroclinic instability in extended regime geostrophic models},
	Volume = 56,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzbWl0aDk5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROTvhnQWgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvhpA2gAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c21pdGg5OS5wZGYADgAYAAsAcwBtAGkAdABoADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc21pdGg5OS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zbWl0aDk5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Smith99a,
	Annote = {Filed under Predictability.},
	Author = {L. A. Smith and C. Ziehmann and K. Fraedrich},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {2855--2886},
	Title = {Uncertainty dynamics and predictability in chaotic systems},
	Volume = 125,
	Year = 1999}

@article{Smith_RD99,
	Annote = {Filed under Turbulence Closure Theories.},
	Author = {R. D. Smith},
	File = {../../Papers/smith_rd99.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1865--1880},
	Title = {The Primitive Equations in the Stochastic Theory of Adiabatic Stratified Turbulence},
	Volume = 29,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zbWl0aF9yZDk5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROVwOzzXAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwO1VzAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c21pdGhfcmQ5OS5wZGYAAA4AHgAOAHMAbQBpAHQAaABfAHIAZAA5ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3NtaXRoX3JkOTkucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3NtaXRoX3JkOTkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Smolarkiewicz89,
	Annote = {Filed under Lee Vortex Generation. Generation of lee
                  vortices in adiabatic and frictionless flow.},
	Author = {P. K. Smolarkiewicz and R. Rotunno},
	Journal = {J. Atmos. Sci.},
	Pages = {1154--1164},
	Title = {Low {F}roude Number Flow past Three-Dimensional Obstacles. {P}art {I}: Baroclinically Generated Lee Vortices},
	Volume = 46,
	Year = 1989}

@article{Smolarkiewicz90,
	Annote = {Filed under Lee Vortex Generation.},
	Author = {P. K. Smolarkiewicz and R. Rotunno},
	Journal = {J. Atmos. Sci.},
	Pages = {1498--1511},
	Title = {Low {F}roude Number Flow past Three-Dimensional Obstacles. {P}art {II}: Upwind Flow Reversal Zone},
	Volume = 47,
	Year = 1990}

@article{Soares04,
	Author = {P. M. M. Soares and P. M. A Miranda and A. P. Siebesma and J. Teixeira},
	File = {../../Papers/soares04.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {3365--3384},
	Title = {An eddy-diffusivity/mass-flux parametrization for dry and shallow cumulus convection},
	Volume = {130},
	Year = {2004},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzb2FyZXMwNC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROWx0gnrQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx0iYLQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c29hcmVzMDQucGRmAAAOABoADABzAG8AYQByAGUAcwAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NvYXJlczA0LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zb2FyZXMwNC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Sobel00,
	Author = {A. H. Sobel and C. Bretherton},
	File = {../../Papers/sobel00.pdf},
	Journal = {J. Climate},
	Pages = {4378--4392},
	Title = {Modeling Tropical Precipitation in a Single Column},
	Volume = {13},
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzb2JlbDAwLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROXwC4gwQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwC6RQQAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c29iZWwwMC5wZGYADgAYAAsAcwBvAGIAZQBsADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc29iZWwwMC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zb2JlbDAwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Sobel01,
	Author = {A. H. Sobel and J. Nilsson and L. M. Polvani},
	File = {../../Papers/sobel01.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3650--3665},
	Title = {The weak temperature gradient approximation and balanced tropical moisture waves},
	Volume = {58},
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzb2JlbDAxLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROYvsDe1gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvsFBRgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c29iZWwwMS5wZGYADgAYAAsAcwBvAGIAZQBsADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc29iZWwwMS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zb2JlbDAxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Sobel02,
	Annote = {Review of basic tropical dynamics, WTG
                  approximation, water vapor in troposphere},
	Author = {A. H. Sobel},
	File = {../../Papers/sobel02.pdf},
	Journal = {Chaos},
	Pages = {??},
	Title = {Water vapor as an active scalar in tropical atmospheric dynamics},
	Volume = {??},
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzb2JlbDAyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROZvsDfSQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvsFBuQAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c29iZWwwMi5wZGYADgAYAAsAcwBvAGIAZQBsADAAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc29iZWwwMi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zb2JlbDAyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Sobel03,
	Author = {A. H. Sobel},
	Journal = {J. Climate},
	Pages = {1003--1009},
	Title = {On the Coexistence of an Evaporation Minimum and Precipitation Maximum in the Warm Pool},
	Volume = 16,
	Year = 2003}

@article{Sobel06a,
	Author = {A. H. Sobel and J. D. Neelin},
	File = {../../Papers/sobel06a.pdf},
	Journal = {Theor. Comput. Fluid Dyn.},
	Pages = {323--350},
	Title = {The boundary layer contribution to intertropical convergence zones in the quasi-equilibrium tropical circulation model framework},
	Volume = 20,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzb2JlbDA2YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRObwYsi91BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwYuTdwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c29iZWwwNmEucGRmAAAOABoADABzAG8AYgBlAGwAMAA2AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NvYmVsMDZhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zb2JlbDA2YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@incollection{Sobel07a,
	Address = {Princeton, NJ},
	Author = {A. H. Sobel},
	Booktitle = {The Global Circulation of the Atmosphere},
	Chapter = {8},
	Editor = {T. Schneider and A. H. Sobel},
	Pages = {219--251},
	Publisher = {Princeton University Press},
	Title = {Simple models of ensemble-averaged tropical precipitation and surface wind, given the sea surface temperature},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxTb2JlbDA3YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROcwoR8MgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwoTeogAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6U29iZWwwN2EucGRmAAAOABoADABTAG8AYgBlAGwAMAA3AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL1NvYmVsMDdhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9Tb2JlbDA3YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Sobel09a,
	Author = {A. H. Sobel and T. Schneider},
	Date-Modified = {2010-06-11 12:08:49 -0700},
	Journal = {J. Adv. Model. Earth Sys.},
	Note = {doi:10.3894/JAMES.2009.1.10},
	Pages = {Art. \#10, 11 pp.},
	Title = {Single-layer axisymmetric model for a {H}adley circulation with parameterized eddy momentum forcing},
	Volume = 1,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzb2JlbDA5YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROfxuA9xAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxuCgNAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c29iZWwwOWEucGRmAAAOABoADABzAG8AYgBlAGwAMAA5AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3NvYmVsMDlhLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zb2JlbDA5YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Sobel99,
	Author = {A. H. Sobel},
	File = {../../Papers/sobel99.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2571--2584},
	Title = {Diffusion versus Nonlocal Models of Stratospheric Mixing, in Theory and Practice},
	Volume = 56,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzb2JlbDk5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROgwDIn3gAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwDKYXgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c29iZWw5OS5wZGYADgAYAAsAcwBvAGIAZQBsADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc29iZWw5OS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zb2JlbDk5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Soden05,
	Annote = {Filed under Water Vapor (Feedback and
                  Kinematics).},
	Author = {B. J. Soden and D. L. Jackson and V. Ramaswamy and M. D. Schwarzkopf and X. Hung},
	File = {../../Papers/soden05.pdf},
	Journal = {Science},
	Pages = {841--844},
	Title = {The Radiative Signature of Upper Tropospheric Moistening},
	Volume = 310,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzb2RlbjA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROhv5AUCwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5CEiwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c29kZW4wNS5wZGYADgAYAAsAcwBvAGQAZQBuADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc29kZW4wNS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zb2RlbjA1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Soden98,
	Author = {B. J. Soden},
	Journal = {J. Geophys. Res.},
	Pages = {17069--17081},
	Title = {Tracking upper tropospheric water vapor radiances: {A} satellite perspective},
	Volume = {103D},
	Year = 1998}

@article{Solomon01a,
	Author = {A. Solomon and P. H. Stone},
	Journal = {J. Atmos. Sci.},
	Pages = {561--574},
	Title = {Equilibration in an Eddy Resolving Model with Simplified Physics},
	Volume = {58},
	Year = 2001}

@article{Solomon01b,
	Annote = {One copy filed under Reviews.},
	Author = {A. Solomon and P. H. Stone},
	Journal = {J. Atmos. Sci.},
	Pages = {2395--2410},
	Title = {A study of the sensitivity of the equilibrated state of an intermediate model of the mid-latitude troposphere to changes in radiative forcing},
	Volume = {58},
	Year = 2001}

@article{Solomon86,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {S. Solomon and R. R. Garcia and F. S. Rowland and D. J. Wuebbles},
	Journal = {Nature},
	Pages = {755--758},
	Title = {On the depletion of {A}ntarctic ozone},
	Volume = 321,
	Year = 1986}

@article{Sommeria77,
	Author = {G. Sommeria and J. W. Deardorff},
	File = {../../Papers/sommeria77.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {344--355},
	Title = {Subgrid-scale condensation in models of nonprecipitating clouds},
	Volume = {34},
	Year = {1977},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zb21tZXJpYTc3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROkx1uTCAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx1wDiAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c29tbWVyaWE3Ny5wZGYAAA4AHgAOAHMAbwBtAG0AZQByAGkAYQA3ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3NvbW1lcmlhNzcucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3NvbW1lcmlhNzcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@incollection{Sommeria98,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {J. Sommeria},
	Booktitle = {Ocean Modeling and Parameterization},
	Editor = {E. P. Chassignet and J. Verron},
	Pages = {303--326},
	Publisher = {Kluwer Acad. Publishers},
	Title = {Statistical Mechanics of Potential Vorticity for Parameterizing Mesoscale Eddies},
	Year = 1998}

@article{Song00,
	Annote = {Filed under Nakamura. Semi-geostrophic stability
                  problems with meridional variations.},
	Author = {Y. Song and N. Nakamura},
	File = {../../Papers/song00.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {46--65},
	Title = {Eady Instability of Isolated Baroclinic Jets with Meridionally Varying Tropopause Height},
	Volume = 57,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgpzb25nMDAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROpwOz2gAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwO1Y8AAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c29uZzAwLnBkZgAADgAWAAoAcwBvAG4AZwAwADAALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3NvbmcwMC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvc29uZzAwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Spencer97,
	Author = {R. W. Spencer and W. D. Braswell},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {1097--1106},
	Title = {How Dry is the Tropical Free Troposphere? {I}mplications for Global Warming Theory},
	Volume = 78,
	Year = 1997}

@article{Spiegel60,
	Author = {E. A. Spiegel and G. Veronis},
	Journal = {Astrophys. J},
	Pages = {442--447},
	Title = {On the {B}oussinesq approximation for a compressible fluid},
	Volume = 131,
	Year = 1960}

@article{Sromovsky02,
	Author = {L. A. Sromovsky and P. M. Fry},
	Journal = {Icarus},
	Pages = {373--400},
	Title = {Jupiter's cloud structure as constrained by {G}alileo {P}robe and {HST} observations},
	Volume = 157,
	Year = 2002}

@article{Sromovsky98,
	Annote = {Filed under Jupiter Dynamics.},
	Author = {L. A. Sromovsky and A. D. Collard and P. M. Fry and G. S. Orton and M. T. Lemmon and M. G. Tomasko and R. S. Freedman},
	File = {../../Papers/sromovsky98.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {22929--22977},
	Title = {Galileo probe measurements of thermal and solar radiation fluxes in the {Jovian} atmosphere},
	Volume = 103,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zcm9tb3Zza3k5OC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROwwxhmSAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwxjIuAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3JvbW92c2t5OTgucGRmAA4AIAAPAHMAcgBvAG0AbwB2AHMAawB5ADkAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc3JvbW92c2t5OTgucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc3JvbW92c2t5OTgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Staley77,
	Annote = {Filed under Baroclinic Instability.},
	Author = {D. O. Staley and R. L. Gall},
	File = {../../Papers/staley77.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1679--1688},
	Title = {On the Wavelength of Maximum Baroclinic Instability},
	Volume = 34,
	Year = 1977,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzdGFsZXk3Ny5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROxvwpeFwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvwrAhwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RhbGV5NzcucGRmAAAOABoADABzAHQAYQBsAGUAeQA3ADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3N0YWxleTc3LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zdGFsZXk3Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Stammer97,
	Annote = {Eddy scales and spectra in the ocean. Length scales
                  consistent with Rossby radius. Rhines scale
                  sometimes smaller.},
	Author = {D. Stammer},
	File = {../../Papers/stammer97.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1743-1769},
	Title = {Global characteristics of ocean variability estimated from regional {TOPEX}/{POSEIDON} altimeter measurements},
	Volume = 27,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zdGFtbWVyOTcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACROyva0ODgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAva1+jgAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RhbW1lcjk3LnBkZgAOABwADQBzAHQAYQBtAG0AZQByADkANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc3RhbW1lcjk3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3N0YW1tZXI5Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Stenzel04,
	Annote = {Filed under Hadley Cell Dynamics.},
	Author = {O. J. Stenzel and J.-S. von Storch},
	File = {../../Papers/stenzel04.pdf},
	Journal = {Climate Dyn.},
	Pages = {415--427},
	Title = {On the effect of thermal forcing on the global atmospheric angular momentum and the general circulation},
	Volume = 22,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zdGVuemVsMDQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRO2v9bdgQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv9dOAQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RlbnplbDA0LnBkZgAOABwADQBzAHQAZQBuAHoAZQBsADAANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc3RlbnplbDA0LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3N0ZW56ZWwwNC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Stephens05,
	Author = {G. L. Stephens},
	File = {../../Papers/stephens05.pdf},
	Journal = {J. Climate},
	Pages = {237--273},
	Title = {Cloud Feedbacks in the Climate System: A Critical Review},
	Volume = 18,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zdGVwaGVuczA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRO3wTWdEQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwTX/gQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RlcGhlbnMwNS5wZGYAAA4AHgAOAHMAdABlAHAAaABlAG4AcwAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3N0ZXBoZW5zMDUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3N0ZXBoZW5zMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Stephens08a,
	Author = {G. L. Stephens and T. D. Ellis},
	File = {../../Papers/stephens08a.pdf},
	Journal = {J. Climate},
	Pages = {6141--6155},
	Title = {Controls of Global-Mean Precipitation Increases in Global Warming {GCM} Experiments},
	Volume = 21,
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zdGVwaGVuczA4YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRO4xd4EIQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxd5mkQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RlcGhlbnMwOGEucGRmAA4AIAAPAHMAdABlAHAAaABlAG4AcwAwADgAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc3RlcGhlbnMwOGEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc3RlcGhlbnMwOGEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Stephenson93,
	Annote = {Filed under Held.},
	Author = {D. B. Stephenson and I. M. Held},
	Journal = {J. Climate},
	Pages = {1859--1870},
	Title = {{GCM} Response of Northern Winter Stationary Waves and Storm Tracks to Increasing Amounts of Carbon Dioxide},
	Volume = 6,
	Year = 1993}

@article{Stephenson97,
	Annote = {Filed under Predictability. States that Mahalanobis
                  metric is invariant under arbitrary linear
                  transformations of the data.},
	Author = {B. D. Stephenson},
	Journal = {Tellus},
	Pages = {513--527},
	Title = {Correlation of spatial climate/weather maps and the advantages of using the {M}ahalanobis metric in predictions},
	Volume = {49A},
	Year = 1997}

@article{Stern95,
	Annote = {Filed under Predictability.},
	Author = {W. F. Stern and K. Miyakoda},
	Journal = {J. Climate},
	Pages = {1071--1085},
	Title = {The Feasibility of Seasonal Forecasts Inferred from multiple {GCM} Simulations},
	Volume = 8,
	Year = 1995}

@article{Stevens02,
	Annote = {Taking entrainment of momentum into boundary layer
                  into account gives more accurate model of
                  near-surface winds.},
	Author = {B. Stevens and J. Duan and J. C. McWilliams and M. M{\"u}nnich and J. D. Neelin},
	File = {../../Papers/stevens02.pdf},
	Journal = {J. Climate},
	Pages = {30--44},
	Title = {Entrainment, {R}ayleigh friction, and boundary layer winds over the tropical {P}acific},
	Volume = 15,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zdGV2ZW5zMDIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRO7wju9DAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwjwffAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RldmVuczAyLnBkZgAOABwADQBzAHQAZQB2AGUAbgBzADAAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc3RldmVuczAyLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3N0ZXZlbnMwMi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Stevens03,
	Author = {B. Stevens and D. H. Lenschow and G. Vali and H. Gerber and A. Bandy and B. Blomquist and J.-L. Brenguier and C. S. Bretherton and F. Burnet and T. Campos and S. Chai and I. Faloona and others},
	File = {../../Papers/stevens03.pdf},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {579--593},
	Title = {Dynamics and chemistry of marine stratocumulus--{DYCOMS-II}},
	Volume = {84},
	Year = {2003},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zdGV2ZW5zMDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRO8x7Fd7wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx7HObwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RldmVuczAzLnBkZgAOABwADQBzAHQAZQB2AGUAbgBzADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc3RldmVuczAzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3N0ZXZlbnMwMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Stevens05,
	Author = {B. Stevens},
	File = {../../Papers/stevens05.pdf},
	Journal = {Annu. Rev. Earth Planet. Sci.},
	Pages = {604--643},
	Title = {Atmospheric Moist Convection},
	Volume = 33,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zdGV2ZW5zMDUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRO9vuWdMAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvuX/oAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RldmVuczA1LnBkZgAOABwADQBzAHQAZQB2AGUAbgBzADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc3RldmVuczA1LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3N0ZXZlbnMwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Stevens07,
	Author = {Stevens, B. and Beljaars, A. and Bordoni, S. and Holloway, C. and K{\"o}hler, M. and Krueger, S. and Savic-Jovcic, V. and Zhang, Y.},
	File = {../../Papers/stevens07.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {985--1005},
	Title = {On the structure of the lower troposphere in the summertime stratocumulus regime of the northeast {Pacific}},
	Volume = {135},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg1zdGV2ZW5zMDcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRO+x7FcCAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx7HMiAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RldmVuczA3LnBkZgAOABwADQBzAHQAZQB2AGUAbgBzADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvc3RldmVuczA3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3N0ZXZlbnMwNy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Stewartson81,
	Annote = {Review of critical layer theory.},
	Author = {K. Stewartson},
	File = {../../Papers/stewartson81.pdf},
	Journal = {IMA J. Appl. Math.},
	Pages = {133--175},
	Title = {Marginally stable inviscid flows with critical layers},
	Volume = 27,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhBzdGV3YXJ0c29uODEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPCwjrJZAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwjsr1AAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3Rld2FydHNvbjgxLnBkZgAADgAiABAAcwB0AGUAdwBhAHIAdABzAG8AbgA4ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3N0ZXdhcnRzb244MS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvc3Rld2FydHNvbjgxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@incollection{Stocker01,
	Address = {Cambridge, UK},
	Author = {T. F. Stocker and G. K. C. Clarke and H. Le Treut and R. S. Lindzen and V. P. Meleshko and R. K. Mugara and T. N. Palmer and R. T. Pierrehumbert and P. J. Sellers and K. E. Trenberth and J. Willebrand},
	Booktitle = {Climate Change 2001: The Scientific Basis},
	Chapter = 7,
	Editor = {J. T. Houghton and Y. Ding and D. J. Griggs and M. Noguer and P. J. van der Linden and X. Dai and K. Maskell and C. A. Johnson},
	Pages = {417--470},
	Publisher = {Intergovernmental Panel on Climate Change},
	Title = {Physical Climate Processes and Feedbacks},
	Year = 2001}

@article{Stohl04,
	Annote = {Filed under Water Vapor (Feedback and Kinematics).},
	Author = {A. Stohl and P. James},
	File = {../../Papers/stohl04.pdf},
	Journal = {J. Hydrometeor.},
	Pages = {656--678},
	Title = {A {L}agrangian Analysis of the Atmospheric Branch of the Global Water Cycle. {P}art~I: {M}ethod Description, Validation, and Demonstration for the {A}ugust 2002 flooding in Central {E}urope},
	Volume = 5,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzdG9obDA0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPHv5ZsvgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5bdPgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RvaGwwNC5wZGYADgAYAAsAcwB0AG8AaABsADAANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc3RvaGwwNC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zdG9obDA0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Stohlgren98,
	Annote = {Not on file. Regional cooling due to increases in
                  irrigation, etc.},
	Author = {T. J. Stohlgren and T. N. Chase and R. A. Pielke and T. G. F. Kittel and J. S. Baron},
	Journal = {Glob. Change Biol.},
	Pages = {495--504},
	Title = {Evidence that local land use practices influence regional climate, vegetation, and stream flow patterns in adjacent natural areas},
	Volume = 4,
	Year = 1998}

@article{Stommel58,
	Author = {H. Stommel and A. B. Arons and A. J. Faller},
	Journal = {Tellus},
	Pages = {179--187},
	Title = {Some Examples of Stationary Planetary Flow Patterns in Bounded Basins},
	Volume = {10},
	Year = {1958}}

@article{Stommel84,
	Annote = {Simple historical overview on the ventilated
                  thermocline, subtropical gyre circulation, {R}ossby
                  waves. Crafoord Prize Lecture.},
	Author = {H. Stommel},
	Journal = {Tellus},
	Pages = {111-119},
	Title = {The delicate interplay between wind-stress and buoyancy input in ocean circulation: the {G}oldsbrough variations},
	Volume = {36A},
	Year = {1984}}

@article{Stone72,
	Author = {P. H. Stone},
	File = {../../Papers/stone72.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {405--418},
	Title = {A Simplified Radiative-Dynamical Model for the Static Stability of Rotating Atmospheres},
	Volume = 29,
	Year = 1972,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzdG9uZTcyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPLvHbsmQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvHddGQAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RvbmU3Mi5wZGYADgAYAAsAcwB0AG8AbgBlADcAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc3RvbmU3Mi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zdG9uZTcyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Stone73,
	Author = {P. H. Stone},
	File = {../../Papers/stone73.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {521--529},
	Title = {Effects of Large-Scale Eddies on Climate Change},
	Volume = 30,
	Year = 1973,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzdG9uZTczLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPNvtB0LwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvtDWnwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RvbmU3My5wZGYADgAYAAsAcwB0AG8AbgBlADcAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc3RvbmU3My5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zdG9uZTczLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Stone78,
	Annote = {Not on file.},
	Author = {P. H. Stone},
	Journal = {J. Atmos. Sci.},
	Pages = {561--571},
	Title = {Baroclinic Adjustment},
	Volume = 35,
	Year = 1978}

@article{Stone79,
	Annote = {Extratropical lapse rate close to critical lapse
                  rate from two-layer model. Tropical lapse rate close
                  to moist adiabat.},
	Author = {P. H. Stone and J. H. Carlson},
	File = {../../Papers/stone79.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {415--423},
	Title = {Atmospheric Lapse Rate Regimes and Their Parameterization},
	Volume = 36,
	Year = 1979,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzdG9uZTc5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPPvmSJpwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvmT6JwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RvbmU3OS5wZGYADgAYAAsAcwB0AG8AbgBlADcAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc3RvbmU3OS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zdG9uZTc5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Stone80,
	Author = {P. H. Stone and D. A. Miller},
	File = {../../Papers/stone80.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1708--1721},
	Title = {Empirical relations between seasonal changes in meridional temperature gradients and meridional fluxes of heat},
	Volume = 37,
	Year = 1980,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzdG9uZTgwLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPQv/vtzgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv/xeTgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RvbmU4MC5wZGYADgAYAAsAcwB0AG8AbgBlADgAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc3RvbmU4MC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zdG9uZTgwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Stone87,
	Annote = {Also moisture flux parameterization (relating
                  moisture fluxes to heat fluxes by linearizing
                  specific humidity variations.},
	Author = {P. H. Stone and M.-S. Yao},
	File = {../../Papers/stone87.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3769--3786},
	Title = {Development of a Two-Dimensional Zonally Averaged Statistical-Dynamical Model. {Part}~II: {The} Role of Eddy Momentum Fluxes in the General Circulation and their Parameterization},
	Volume = 44,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtzdG9uZTg3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPRvmSIZwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvmT45wAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RvbmU4Ny5wZGYADgAYAAsAcwB0AG8AbgBlADgANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvc3RvbmU4Ny5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9zdG9uZTg3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Stone92,
	Author = {P. H. Stone and L. Branscome},
	Journal = {J. Atmos. Sci.},
	Pages = {355--367},
	Title = {Diabatically Forced, Nearly Inviscid Eddy Regimes},
	Volume = 49,
	Year = 1992}

@article{Stone96,
	Annote = {Compute isentropic slope from observations and GCM
                  runs. Isentropic slope not strongly
                  season-dependent, although heat fluxes are strongly
                  season-dependent. Suggests that baroclinic
                  adjustment is important at intermediate levels in
                  midlatitudes. Models do not do well in simulating
                  variability of isentropic slope: model slope varies
                  more strongly than observed slope. Thus, models may
                  not simulate climate sensitivity accurately.},
	Author = {P. H. Stone and B. Nemet},
	Journal = {J. Atmos. Sci.},
	Pages = {1663--1674},
	Title = {Baroclinic Adjustment: A Comparison between Theory, Observations, and Models},
	Volume = 53,
	Year = 1996}

@article{Stott00,
	Annote = {Filed under Climate Change Detection.},
	Author = {P. A. Stott and S. F. B. Tett and G. S. Jones and M. R. Allen and J. F. B. Mitchell and G. J. Jenkins},
	Journal = {Science},
	Pages = {2133--2137},
	Title = {External Control of 20th Century Temperature by Natural and Anthropogenic Forcings},
	Volume = 290,
	Year = 2000}

@article{Stott02,
	Annote = {Filed under Paleo-Climate Reviews.},
	Author = {L. Stott and C. Poulsen and S. Lund and R. Thunell},
	Journal = {Science},
	Pages = {222--226},
	Title = {Super {ENSO} and Global Climate Oscillations at Millennial Time Scales},
	Volume = 297,
	Year = 2002}

@article{Stott98,
	Annote = {Filed under Climate Change Detection. Use ensembles
                  of 4 climate change simulations to investigate on
                  which spatial and temporal scales a climate change
                  is detectable. Climate change can be detected in
                  30-yr- and 50-yr-trends on spatial scales greater
                  than 5000 km. Compute trends from ensemble
                  means. Show that, if the model is forced with GHG
                  only, the model simulations are inconsistent with
                  observed record on spatial scales smaller than 2000
                  km. The simulations are consistent with observed
                  record if aerosol forcing is included.},
	Author = {P. A. Stott and S. F. B. Tett},
	Journal = {J. Climate},
	Pages = {3282--3294},
	Title = {Scale-Dependent Detection of Climate Change},
	Volume = 11,
	Year = 1998}

@article{Stouffer00,
	Annote = {Filed under Climate Change Detection.},
	Author = {R. J. Stouffer and G. Hegerl and S. F. B. Tett},
	Journal = {J. Climate},
	Pages = {513--537},
	Title = {A comparison of surface air temperature variability in three 1000-yr coupled ocean-atmosphere model integrations},
	Volume = 13,
	Year = 2000}

@article{Stouffer94,
	Annote = {Filed under Manabe.},
	Author = {R. J. Stouffer and S. Manabe and K. Ya. Vinnikov},
	Journal = {Nature},
	Pages = {634--635},
	Title = {Model Assessment of the Role of Natural Variability in Recent Global Warming},
	Volume = 367,
	Year = 1994}

@article{Straus99,
	Annote = {Filed under Atmospheric Turbulence Spectra. Energy
                  spectra from reanalysis data.},
	Author = {D. M. Straus and P. Ditlevsen},
	File = {../../Papers/straus99.pdf},
	Journal = {Tellus},
	Pages = {749--772},
	Title = {Two-dimensional turbulence properties of the {ECMWF} reanalyses},
	Volume = {51A},
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzdHJhdXM5OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPXv1EKHFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv1FsjAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3RyYXVzOTkucGRmAAAOABoADABzAHQAcgBhAHUAcwA5ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3N0cmF1czk5LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zdHJhdXM5OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@unpublished{Strichartz91,
	Annote = {Filed under Wavelets. Expanded version to appear in
                  Wavelets, ed. M. Frazier.},
	Author = {R. S. Strichartz},
	Note = {Unpublished},
	Title = {How to Make Wavelets},
	Year = 1991}

@unpublished{Strong97,
	Annote = {Filed under Entropy Estimation. See also deRuyter97},
	Author = {S. P. Strong and R. Koberle and R. R. {de Ruyter van Steveninck} and W. Bialek},
	Month = {June},
	Note = {Preprint; to appear in {\em Phys. Rev.}},
	Title = {Entropy and Information in Neural Spike Trains},
	Year = 1997}

@article{Stuart58,
	Annote = {Classic paper on weakly nonlinear stability theory
                  (with application to Poiseuille flow).},
	Author = {J. T. Stuart},
	File = {../../Papers/stuart58.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {1--21},
	Title = {On the non-linear mechanics of hydrodynamic stability},
	Volume = 4,
	Year = 1958,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzdHVhcnQ1OC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPYwphjAQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwpjFcQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3R1YXJ0NTgucGRmAAAOABoADABzAHQAdQBhAHIAdAA1ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3N0dWFydDU4LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zdHVhcnQ1OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Stuart71,
	Annote = {Review of weakly nonlinear stability theory.},
	Author = {J. T. Stuart},
	File = {../../Papers/stuart71.pdf},
	Journal = {Ann. Rev. Fluid Mech.},
	Pages = {347--370},
	Title = {Nonlinear Stability Theory},
	Volume = {3},
	Year = 1971,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzdHVhcnQ3MS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPawphlIAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwpjHkAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3R1YXJ0NzEucGRmAAAOABoADABzAHQAdQBhAHIAdAA3ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3N0dWFydDcxLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zdHVhcnQ3MS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Suarez76,
	Annote = {Filed under Climate Stability/Energy Balance Models.},
	Author = {M. J. Suarez and I. M. Held},
	File = {../../Papers/suarez76.pdf},
	Journal = {Nature},
	Pages = {46--47},
	Title = {Modelling climatic response to orbital parameter variations},
	Volume = 263,
	Year = 1976,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzdWFyZXo3Ni5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPbvhaFjgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvhb2DgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3VhcmV6NzYucGRmAAAOABoADABzAHUAYQByAGUAegA3ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3N1YXJlejc2LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zdWFyZXo3Ni5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Suarez79,
	Annote = {Filed under Climate Stability/Energy Balance Models.},
	Author = {M. J. Suarez and I. M. Held},
	File = {../../Papers/suarez79.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {4825--44836},
	Title = {The sensitivity of an energy balance climate model to variations in the orbital parameters},
	Volume = 84,
	Year = 1979,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzdWFyZXo3OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPcvhavDgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvhcfjgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3VhcmV6NzkucGRmAAAOABoADABzAHUAYQByAGUAegA3ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3N1YXJlejc5LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zdWFyZXo3OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Suarez92,
	Author = {M. J. Suarez and D. G> Duffy},
	File = {../../Papers/suarez92.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1541--1554},
	Title = {Terrestrial superrotation: {A} bifurcation of the general circulation},
	Volume = 49,
	Year = 1992,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxzdWFyZXo5Mi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPdwTYjEVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwTaFgQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3VhcmV6OTIucGRmAAAOABoADABzAHUAYQByAGUAegA5ADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3N1YXJlejkyLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9zdWFyZXo5Mi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Sudradjat05,
	Annote = {Comparison of ERA-40, NCEP reanalyses with NASA
                  Water Vapor Project Data. ERA-40 better than NCEP renanalysis.},
	Author = {A. Sudradjat and R. R. Ferraro and M. Fiorino},
	File = {../../Papers/sudradjat05.pdf},
	Journal = {J. Climate},
	Pages = {1790--1807},
	Title = {A Comparison of Total Precipitable Water between Reanalyses and {NVAP}},
	Volume = 18,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg9zdWRyYWRqYXQwNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPevuGOXQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvuHwzQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3VkcmFkamF0MDUucGRmAA4AIAAPAHMAdQBkAHIAYQBkAGoAYQB0ADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvc3VkcmFkamF0MDUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvc3VkcmFkamF0MDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Sun06,
	Annote = {Filed under Precipitation Statistics. In GCMs, light
                  rain generally too frequent, heavy rain not intense
                  enough.},
	Author = {Y. Sun and S. Solomon and A. Dai and R. W. Portmann},
	File = {../../Papers/sun06.pdf},
	Journal = {J. Climate},
	Pages = {919--934},
	Title = {How often does it rain?},
	Volume = 19,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglzdW4wNi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPkwaSnMgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwaUXsgAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3VuMDYucGRmAA4AFAAJAHMAdQBuADAANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvc3VuMDYucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvc3VuMDYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Sun93,
	Author = {D.-Z. Sun and R.~S. Lindzen},
	File = {../../Papers/sun93.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1643--1660},
	Title = {Distribution of tropical tropospheric water vapor},
	Volume = 50,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfglzdW45My5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPlxPQz0wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxPSWQwAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3VuOTMucGRmAA4AFAAJAHMAdQBuADkAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvc3VuOTMucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvc3VuOTMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Sun94,
	Annote = {Filed under Lindzen.},
	Author = {D.-Z. Sun and R. S. Lindzen},
	Journal = {J. Atmos. Sci.},
	Pages = {757--772},
	Title = {A {PV} View of the Zonal Mean Distribution of Temperature and Wind in the Extratropical Troposphere},
	Volume = 51,
	Year = 1994}

@article{Sun96,
	Annote = {Filed under Water Vapor Feedback (Feedback and
                  Kinematics).},
	Author = {D.-Z. Sun and I. M. Held},
	Journal = {J. Climate},
	Pages = {665--675},
	Title = {A Comparison of Modeled and Observed Relationships between Interannual Variations of Water Vapor and Temperature},
	Volume = 9,
	Year = 1996}

@article{SunDZ93,
	Annote = {Filed under Lindzen.},
	Author = {D.-Z. Sun and R. S. Lindzen},
	Journal = {J. Atmos. Sci.},
	Pages = {1643--1660},
	Title = {Distribution of tropical tropospheric water vapor},
	Volume = 50,
	Year = 1993}

@article{SunZP93,
	Author = {Sun, Z. P. and Schubert, G. and Glatzmaier, G. A.},
	Journal = {Science},
	Pages = {661--664},
	Title = {Banded Surface Flow Maintained by Convection in a Model of the Rapidly Rotating Giant Planets},
	Volume = {260},
	Year = {1993}}

@article{Swanson00,
	Annote = {Equivalent barotropic model of low-frequency variability.},
	Author = {K. L. Swanson},
	Journal = {J. Atmos. Sci.},
	Pages = {2262--2280},
	Title = {Stationary Wave Accumulation and the Generation of Low-Frequency Variability on Zonally Varying Flows},
	Volume = 57,
	Year = 2000}

@incollection{Swanson07a,
	Address = {Princeton, NJ},
	Author = {K. L. Swanson},
	Booktitle = {The Global Circulation of the Atmosphere},
	Date-Modified = {2010-06-11 11:45:04 -0700},
	Editor = {T. Schneider and A. H. Sobel},
	Pages = {78--103},
	Publisher = {Princeton University Press},
	Title = {Storm Track Dynamics},
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zd2Fuc29uMDdhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPnwjseIAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwjuAkAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3dhbnNvbjA3YS5wZGYAAA4AHgAOAHMAdwBhAG4AcwBvAG4AMAA3AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3N3YW5zb24wN2EucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3N3YW5zb24wN2EucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@unpublished{Swanson94,
	Annote = {Filed under Baker.},
	Author = {B. D. Swanson and M. B. Baker},
	Note = {Preprint},
	Title = {Laboratory Measurements of Ice Crystal Evaporation Rates},
	Year = 1994}

@article{Swanson97a,
	Author = {K. L. Swanson and P. J. Kushner and I. M. Held},
	File = {../../Papers/swanson97a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {791--810},
	Title = {Dynamics of Barotropic Storm Tracks},
	Volume = 54,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zd2Fuc29uOTdhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPpwE74zQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwE9pTQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3dhbnNvbjk3YS5wZGYAAA4AHgAOAHMAdwBhAG4AcwBvAG4AOQA3AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3N3YW5zb245N2EucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3N3YW5zb245N2EucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Swanson97b,
	Annote = {Filed under Surface Heat Flux
                  Parameterizations. Temperature fluctuations damp to
                  the underlying oceanic temperature with a timescale
                  of approximately 1 day, but dynamics still play the
                  dominant role in determining atmospheric heat flux.},
	Author = {K. L. Swanson and R. T. Pierrehumbert},
	File = {../../Papers/swanson97b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1533--1543},
	Title = {Lower-tropospheric heat transport in the {P}acific storm track},
	Volume = 54,
	Year = 1997,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5zd2Fuc29uOTdiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPqwuVIi1BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwuWq+wAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6c3dhbnNvbjk3Yi5wZGYAAA4AHgAOAHMAdwBhAG4AcwBvAG4AOQA3AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3N3YW5zb245N2IucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3N3YW5zb245N2IucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Sweldens96,
	Annote = {Filed under Wavelets. Nicely written and containing
                  lots of quotes.},
	Author = {W. Sweldens},
	Journal = {Proc. IEEE},
	Pages = {680--685},
	Title = {Wavelets: {W}hat Next},
	Volume = {84},
	Year = {1996}}

@article{Talagrand87,
	Annote = {Filed under Adjoint Methods.},
	Author = {O. Talagrand and P. Courtier},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1311--1328},
	Title = {Variational assimilation of meteorological observations with the adjoint vorticity equation. {I}: {T}heory},
	Volume = 113,
	Year = 1987}

@article{Tanaka04,
	Author = {Tanaka, H. L. and Ishizaki, N. and Kitoh, A.},
	File = {../../Papers/tanaka04.pdf},
	Journal = {Tellus},
	Pages = {250--269},
	Title = {Trend and interannual variability of {Walker}, monsoon and {Hadley} circulations defined by velocity potential in the upper troposphere},
	Volume = {56A},
	Year = {2004},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx0YW5ha2EwNC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPwxaIlDQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxaKVjQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGFuYWthMDQucGRmAAAOABoADAB0AGEAbgBhAGsAYQAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3RhbmFrYTA0LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy90YW5ha2EwNC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Tanaka05,
	Abstract = {In this study, intensities and trends of Hadley,
                  Walker, and monsoon circulations are compared for
                  the IPCC 20th Century simulations and for 21st
                  Century simulations, using the upper tropospheric
                  velocity potential data. As a result, we showed
                  significantly weaker biases in Walker and monsoon
                  circulations for the JJA climate in the IPCC 20th
                  Century simulations. The dispersal in the scatter
                  diagram of the model biases is considerably
                  large. The same analyses are applied for the IPCC
                  21st Century simulations to investigate the trends
                  of these tropical circulations in response to the
                  projected global warming. As a result, it is
                  anticipated that Hadley, Walker, and monsoon
                  circulations are weakened by 9, 8, and 14%,
                  respectively, by the late 21st Century, according to
                  the ensemble mean of the IPCC model
                  simulations. Considering the large model biases
                  demonstrated for the IPCC 20th Century simulations,
                  further studies are needed to quantify those
                  trends.},
	Author = {Tanaka, H. L. and Ishizaki, N. and Nohara, D.},
	File = {../../Papers/tanaka05.pdf},
	Journal = {SOLA},
	Note = {doi:10.2151/sola.2005-021},
	Pages = {77--80},
	Title = {Intercomparison of the intensities and trends of {Hadley}, {Walker} and monsoon circulations in the global warming projections},
	Volume = 1,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx0YW5ha2EwNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPxxbB5zAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxbDqTAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGFuYWthMDUucGRmAAAOABoADAB0AGEAbgBhAGsAYQAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3RhbmFrYTA1LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy90YW5ha2EwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Tao99,
	Annote = {Simulation of radiative-convective equilibrium.},
	Author = {W.-K. Tao and J. Simpson and C.-H. Sui and C.-L. Shie and B. Zhou and K. M. Lau and M. Moncrieff},
	Journal = {J. Atmos. Sci.},
	Pages = {3128--3139},
	Title = {Equilibrium States Simulated by Cloud-Resolving Models},
	Volume = 56,
	Year = 1999}

@article{Tarantola84,
	Annote = {Filed under Adjoint Methods.},
	Author = {A. Tarantola},
	Journal = {Geophys.},
	Pages = {1259--1266},
	Title = {Inversion of seismic reflection data in the acoustic approximation},
	Volume = 49,
	Year = 1984}

@book{Tarantola87,
	Address = {New York},
	Annote = {Bayesian approach to inverse problems},
	Author = {A. Tarantola},
	Pages = 613,
	Publisher = {Elsevier},
	Title = {Inverse Problem Theory: Methods for Data Fitting and Model Parameter Estimation},
	Year = 1987}

@article{Teixeira02,
	Author = {J. Teixeira and T. F. Hogan},
	File = {../../Papers/teixeira02.pdf},
	Journal = {J. Climate},
	Pages = {1261--1276},
	Title = {Boundary layer clouds in a global atmospheric model: {Simple} cloud cover parameterizations},
	Volume = {15},
	Year = {2002},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg50ZWl4ZWlyYTAyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRP2x7FxkgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAx7HiEgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGVpeGVpcmEwMi5wZGYAAA4AHgAOAHQAZQBpAHgAZQBpAHIAYQAwADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3RlaXhlaXJhMDIucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3RlaXhlaXJhMDIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Tett96,
	Annote = {Not on file.},
	Author = {S. F. B. Tett and J. F. B. Mitchell and D. E. Parker and M. R. Allen},
	Journal = {Science},
	Note = {Corrections in \citet{Allen99}.},
	Pages = {1170--1173},
	Title = {Human Influence on the Atmospheric Vertical Temperature Structure: Detection and Observations},
	Volume = 247,
	Year = 1996}

@article{Tett99,
	Annote = {Filed under Climate Change Detection.},
	Author = {S. F. B. Tett and P. A. Stott and M. R. Allen and W. J. Ingram and J. F. B. Mitchell},
	Journal = {Nature},
	Pages = {569--572},
	Title = {Causes of twentieth-century temperature change near the {E}arth's surface},
	Volume = 399,
	Year = 1999}

@article{Thacker96a,
	Annote = {Confusing presentation of various ways to decompose
                  multivariate fields.},
	Author = {W. C. Thacker and R. Lewandowicz},
	Journal = {J. Climate},
	Pages = {1942--1958},
	Title = {Climatic Indices, Principal Components, and the {G}auss-{M}arkov Theorem},
	Volume = 9,
	Year = 1996}

@article{Thacker96b,
	Annote = {Essentially computes left and right eigenvectors of
                  Fisher's discriminant matrix. Obtains in this way a
                  metric-independent decomposition of data.},
	Author = {W. C. Thacker},
	Journal = {Tellus},
	Pages = {584--592},
	Title = {Metric-based Principal Components: Data Uncertainties},
	Volume = {48A},
	Year = 1996}

@article{Theiss06,
	Annote = {Filed under Geostrophic Turbulence. Considers
                  limitations on Rhines scale by finite deformation
                  radius in shallow-water model. However, this misses
                  the barotropic mode, which can cascade.},
	Author = {J. Theiss},
	File = {../../Papers/theiss06.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2005GL025379},
	Pages = {L08809},
	Title = {A generalized {Rhines} effect and storms on {J}upiter},
	Volume = 33,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx0aGVpc3MwNi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRP6w7I+hwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7KvBwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGhlaXNzMDYucGRmAAAOABoADAB0AGgAZQBpAHMAcwAwADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3RoZWlzczA2LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy90aGVpc3MwNi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Thompson01,
	Annote = {NAM affects not only Atlantic, but also Pacific,
                  modulating storm tracks.},
	Author = {D. W. J. Thompson and J. M. Wallace},
	Journal = {Science},
	Pages = {85--89},
	Title = {Regional Climate Impacts of the {N}orthern {H}emisphere annular mode},
	Volume = 293,
	Year = 2001}

@article{Thompson02a,
	Author = {D. W. J. Thompson and S. Solomon},
	Journal = {Science},
	Pages = {895--899},
	Title = {Interpretation of Recent {S}outhern {H}emisphere Climate Change},
	Volume = 296,
	Year = 2002}

@article{Thompson02b,
	Annote = {Find negative correlation between 'onset' of
                  stratospheric polar vortex strengthening and
                  subsequent surface temperature anomalies.},
	Author = {D. W. J. Thompson and M. P. Baldwin and J. M. Wallace},
	Journal = {J. Climate},
	Pages = {1421--1428},
	Title = {Stratospheric Connection to {N}orthern {H}emisphere Wintertime Weather: Implications for Prediction},
	Volume = 15,
	Year = 2002}

@article{Thompson06,
	Annote = {Filed under Baroclinic Eddy Flux
                  Parameterizations. Shows that dual-cascade picture
                  is inadequate on f-plane. Eddy flux scaling must
                  take properties of coherent vortices into account.},
	Author = {A. F. Thompson and W. R. Young},
	File = {../../Papers/thompson06.pdf},
	Journal = {J. Phys. Oceanogr.},
	Pages = {720--738},
	Title = {Scaling Baroclinic Eddy Fluxes: Vortices and Energy Balance},
	Volume = 36,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg50aG9tcHNvbjA2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQBwL2SowAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwL31EwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGhvbXBzb24wNi5wZGYAAA4AHgAOAHQAaABvAG0AcABzAG8AbgAwADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3Rob21wc29uMDYucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3Rob21wc29uMDYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Thompson98,
	Annote = {.},
	Author = {D. W. J. Thompson and J. M. Wallace},
	Journal = {Geophys. Res. Lett.},
	Pages = {1297--1300},
	Title = {The {A}rctic {O}scillation Signature in the Wintertime Geopotential Height and Temperature Fields},
	Volume = 25,
	Year = 1998}

@inproceedings{Thomson1857,
	Address = {London},
	Annote = {Filed under General Circulation History.},
	Author = {J. Thomson},
	Booktitle = {Report of the Meeting of the British Association for the Advancement of Science},
	File = {../../Papers/thomson1857.pdf},
	Note = {[Abstract of paper read at British Association meeting. Full account of theory given in \citet{Thomson1892}.]},
	Organization = {British Association},
	Pages = {38--39},
	Title = {On the Grand Currents of Atmospheric Circulation},
	Year = 1857,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg90aG9tc29uMTg1Ny5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQFvvrAlwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvvsjBwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGhvbXNvbjE4NTcucGRmAA4AIAAPAHQAaABvAG0AcwBvAG4AMQA4ADUANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdGhvbXNvbjE4NTcucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdGhvbXNvbjE4NTcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Thomson1892,
	Annote = {Filed under General Circulation History.},
	Author = {J. Thomson},
	File = {../../Papers/thomson1892.pdf},
	Journal = {Phil. Trans. Roy. Soc. A},
	Pages = {653--684},
	Title = {Bakerian Lecture: On the Grand Currents of Atmospheric Circulation},
	Volume = 183,
	Year = 1892,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg90aG9tc29uMTg5Mi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQGvvF0QAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvvHWsAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGhvbXNvbjE4OTIucGRmAA4AIAAPAHQAaABvAG0AcwBvAG4AMQA4ADkAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdGhvbXNvbjE4OTIucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdGhvbXNvbjE4OTIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Thomson87,
	Annote = {Filed under Stochastic Lagrangian Models of
                  Turbulence. Classic paper introducing well-mixed
                  criterion for determination of drift term in
                  Langevin models of turbulence.},
	Author = {D. J. Thomson},
	File = {../../Papers/thomson87.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {529--556},
	Title = {Criteria for the selection of stochastic models of particle trajectories in turbulent flows},
	Volume = 180,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg10aG9tc29uODcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQHv5TvsQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5VgMQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGhvbXNvbjg3LnBkZgAOABwADQB0AGgAbwBtAHMAbwBuADgANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvdGhvbXNvbjg3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3Rob21zb244Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Thomson90,
	Annote = {Filed under Stochastic Lagrangian Models of
                  Turbulence. Classic paper introducing well-mixed
                  criterion for models of dispersion.},
	Author = {D. J. Thomson},
	File = {../../Papers/thomson90.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {113--153},
	Title = {A stochastic model for the motion of particle pairs in isotropic high-{R}eynolds-number turbulence, and its application to the problem of concentration variance},
	Volume = 210,
	Year = 1990,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg10aG9tc29uOTAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQIv5Tv8QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5VgcQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGhvbXNvbjkwLnBkZgAOABwADQB0AGgAbwBtAHMAbwBuADkAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvdGhvbXNvbjkwLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3Rob21zb245MC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Thorncroft93,
	Annote = {Filed under Hoskins.},
	Author = {C. D. Thorncroft and B. J. Hoskins and M. E. McIntyre},
	File = {../../Papers/thorncroft93.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {17--55},
	Title = {Two paradigms of baroclinic-wave life-cycle behaviour},
	Volume = 119,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhB0aG9ybmNyb2Z0OTMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQJwefLAAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAweg7gAAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGhvcm5jcm9mdDkzLnBkZgAADgAiABAAdABoAG8AcgBuAGMAcgBvAGYAdAA5ADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3Rob3JuY3JvZnQ5My5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvdGhvcm5jcm9mdDkzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Thorpe89,
	Author = {A. J. Thorpe and R. Rotunno},
	File = {../../Papers/thorpe89.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1285--1299},
	Title = {Nonlinear Aspects of Symmetric Instability},
	Volume = 46,
	Year = 1989,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx0aG9ycGU4OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQMvrccPAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvrd+rAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGhvcnBlODkucGRmAAAOABoADAB0AGgAbwByAHAAZQA4ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3Rob3JwZTg5LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy90aG9ycGU4OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Thorpe95,
	Annote = {Unnecessarily complicated analogy between pv and
                  charge in electrostatics.},
	Author = {A. J. Thorpe and C. H. Bishop},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1477--1495},
	Title = {Potential vorticity and the electrostatics analogy: {E}rtel--{R}ossby formulation},
	Volume = 121,
	Year = 1995}

@article{Thuburn00,
	Annote = {Filed under Tropopause Dynamics.},
	Author = {J. Thuburn and G. C. Craig},
	File = {../../Papers/thuburn00.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {17--28},
	Title = {Stratospheric Influence on Tropopause Height: The Radiative Constraint},
	Volume = 57,
	Year = {2000},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg10aHVidXJuMDAucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQOw0WILAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw0XqnAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGh1YnVybjAwLnBkZgAOABwADQB0AGgAdQBiAHUAcgBuADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvdGh1YnVybjAwLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3RodWJ1cm4wMC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Thuburn97,
	Annote = {Filed under Tropopause Dynamics.},
	Author = {J. Thuburn and G. C. Craig},
	File = {../../Papers/thuburn97.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {869--882},
	Title = {{GCM} Tests of Theories for the Height of the Tropopause},
	Volume = 54,
	Year = {1997},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg10aHVidXJuOTcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQQvuR6lAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvuTdBAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGh1YnVybjk3LnBkZgAOABwADQB0AGgAdQBiAHUAcgBuADkANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvdGh1YnVybjk3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3RodWJ1cm45Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Thuburn99,
	Author = {J. Thuburn and V. Lagneau},
	Journal = {J. Atmos. Sci.},
	Pages = {689--710},
	Title = {Eulerian Mean, Contour Integral, and Finite-Amplitude Wave Activity Diagnostics Applied to a Single-Layer Model of the Winter Stratosphere},
	Volume = 56,
	Year = 1999}

@article{Tiao81,
	Annote = {Filed under AR Modeling. Systematic approach to
                  order selection estimation: tentative specification,
                  estimation, diagnostic checking.},
	Author = {G. C. Tiao and G. E. P Box},
	Journal = {J. Amer. Stat. Assoc.},
	Pages = {802--816},
	Title = {Modeling Multiple Time Series With Applications},
	Volume = 76,
	Year = 1981}

@article{Tiedtke89,
	Annote = {Convection scheme used by ECMWF},
	Author = {M. Tiedtke},
	File = {../../Papers/tiedtke89.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {1779--1800},
	Title = {A comprehensive mass flux scheme for cumulus parameterization in large-scale models},
	Volume = 117,
	Year = 1989,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg10aWVkdGtlODkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQRxpx0XAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxpzWzAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGllZHRrZTg5LnBkZgAOABwADQB0AGkAZQBkAHQAawBlADgAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvdGllZHRrZTg5LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3RpZWR0a2U4OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Tiedtke93,
	Annote = {Cloud and grid-scale condensation/evaporation scheme used by ECMWF},
	Author = {M. Tiedtke},
	File = {../../Papers/tiedtke93.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {3040--3061},
	Title = {Representation of clouds in large-scale models},
	Volume = 121,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg10aWVkdGtlOTMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQSxpxxUQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxpzTwQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGllZHRrZTkzLnBkZgAOABwADQB0AGkAZQBkAHQAawBlADkAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvdGllZHRrZTkzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3RpZWR0a2U5My5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@book{Tikhonov77,
	Address = {Washington},
	Author = {A. N. Tikhonov and V. Y. Arsenin},
	Pages = 258,
	Publisher = {V. H. Winston and Sons},
	Series = {Scripta Series in Mathematics},
	Title = {Solution of Ill-Posed Problems},
	Year = 1977}

@article{Tippett03,
	Annote = {Filed under Predictability.},
	Author = {M. K. Tippett and P. Chang},
	File = {../../Papers/tippett03.pdf},
	Journal = {Tellus},
	Pages = {148--157},
	Title = {Some theoretical considerations on predictability of linear stochastic dynamics},
	Volume = {55A},
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg10aXBwZXR0MDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQWxLb6cAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxLdc4AAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGlwcGV0dDAzLnBkZgAOABwADQB0AGkAcABwAGUAdAB0ADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvdGlwcGV0dDAzLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3RpcHBldHQwMy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Tjostheim83,
	Annote = {Filed under AR Modeling. Study bias of Yule-Walker
                  and least squares estimates for univariate and
                  multivariate autoregressive processes. Simulations
                  and theory indicate that Yule-Walker estimates are
                  inferior to least squares. Yule-Walker estimates can
                  be severely biased for marginally stable processes.},
	Author = {D. Tj{\o}stheim and J. Paulsen},
	Journal = {Biometrika},
	Pages = {389--399},
	Title = {Bias of some commonly used time series estimates},
	Volume = 70,
	Year = 1983}

@article{Tokano02,
	Author = {T. Tokano and F. M. Neubauer},
	File = {../../Papers/tokano02.pdf},
	Journal = {Icarus},
	Pages = {499--515},
	Title = {Tidal Winds on {Titan} caused by {Saturn}},
	Volume = 158,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx0b2thbm8wMi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQZxgk9gwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxgmf8wAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dG9rYW5vMDIucGRmAAAOABoADAB0AG8AawBhAG4AbwAwADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3Rva2FubzAyLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy90b2thbm8wMi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Tokano09,
	Author = {Tokano, T.},
	File = {../../Papers/tokano09.pdf},
	Journal = {Phil. Trans. Roy. Soc. A},
	Pages = {633--648},
	Title = {The dynamics of {Titan}'s troposphere},
	Volume = {367},
	Year = {2009},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx0b2thbm8wOS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQexgAdygAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxgCAOgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dG9rYW5vMDkucGRmAAAOABoADAB0AG8AawBhAG4AbwAwADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3Rva2FubzA5LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy90b2thbm8wOS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Tomas94,
	Annote = {Filed under Webster. Westerly ducts also in
                  vertical, i.e., lower-level part of waves accounting
                  easterlies is sheared off while upper-level part can
                  propagate further if there are upper-level
                  westerlies and lower-level easterles.},
	Author = {R. A. Tomas and P. J. Webster},
	File = {../../Papers/tomas94.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1417--1430},
	Title = {Horizontal and Vertical Structure of Cross-Equatorial Wave Propagation},
	Volume = 51,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt0b21hczk0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQgwYokjgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwYqVDgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dG9tYXM5NC5wZGYADgAYAAsAdABvAG0AYQBzADkANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvdG9tYXM5NC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy90b21hczk0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Tomas99,
	Annote = {Filed under ITCZ Dynamics. States that flow is
                  not inertially unstable in monsoon regions, as
                  Tomas97 had suggested, but friction stabilizes
                  it. Nonetheless, nonlinear momentum advection near
                  surface can concentrate convection zones.},
	Author = {R. A. Tomas and J. R. Holton and P. J. Webster},
	File = {../../Papers/tomas99.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1107--1127},
	Title = {The influence of cross-equatorial pressure gradients on the location of near-equatorial convection},
	Volume = 125,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt0b21hczk5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQiwYsiFVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwYuSlQAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dG9tYXM5OS5wZGYADgAYAAsAdABvAG0AYQBzADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvdG9tYXM5OS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy90b21hczk5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Medeiros08,
	Author = {Medeiros, B. and Stevens, B. and Held, I. M. and Zhao, M. and Williamson, D. L. and Olson, J. G. and Bretherton, C. S.},
	File = {../../Papers/medeiros08.pdf},
	Journal = {J. Climate},
	Pages = {4974--4991},
	Title = {Aquaplanets, climate sensitivity, and low clouds},
	Volume = {21},
	Year = {2008},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg5tZWRlaXJvczA4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRIoxQrw6QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxQtTWQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6bWVkZWlyb3MwOC5wZGYAAA4AHgAOAG0AZQBkAGUAaQByAG8AcwAwADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL21lZGVpcm9zMDgucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL21lZGVpcm9zMDgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@techreport{Tompkins04c,
	Address = {[Available at http://www.ecmwf.int/publications/.]},
	Author = {A. M. Tompkins and P. Bechtold and A.C.M. Beljaars and A. Benedetti and S. Cheinet and M. Janiskov\'a and M. K\"ohler and P. Lopez and J.-J. Morcrette},
	File = {../../Papers/tompkins04c.pdf},
	Institution = {European Centre for Medium-Range Weather Forecasts},
	Number = {452},
	Pages = {91},
	Series = {ECMWF Technical Memorandum},
	Title = {Moist physical processes in the {IFS}: Progress and plans},
	Year = {2004},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg90b21wa2luczA0Yy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQkxRjqSAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxRlMuAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dG9tcGtpbnMwNGMucGRmAA4AIAAPAHQAbwBtAHAAawBpAG4AcwAwADQAYwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdG9tcGtpbnMwNGMucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdG9tcGtpbnMwNGMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Tompkins07a,
	Author = {A. M. Tompkins and K. Gierens and G. R\"adel},
	File = {../../Papers/tompkins07a.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {53--63},
	Title = {Ice supersaturation in the {ECMWF} integrated forcast system},
	Volume = 133,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg90b21wa2luczA3YS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQlxRjrrwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxRlOHwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dG9tcGtpbnMwN2EucGRmAA4AIAAPAHQAbwBtAHAAawBpAG4AcwAwADcAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdG9tcGtpbnMwN2EucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdG9tcGtpbnMwN2EucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Toth91,
	Annote = {Not on file.},
	Author = {Z. Toth},
	Journal = {Mon. Wea. Rev.},
	Pages = {1501--1511},
	Title = {Circulation Patterns in Phase Space: {A} Multinormal Distribution?},
	Volume = 119,
	Year = 1991}

@article{Toth95,
	Annote = {Filed under Predictability. Estimates degrees of
                  freedom in 700 hPa circulation pattern in the
                  Northern Hemisphere during winter. Uses two methods:
                  (i) chi-squared fit to squared anomalies to get dofs
                  in chi-square distribution; (ii) 'hypersphere'
                  method. About 24 dofs in 700 hPa data. Roughly 60-90
                  dofs in large-scale global circulation.},
	Author = {Z. Toth},
	Journal = {Tellus},
	Pages = {457--472},
	Title = {Degrees of freedom in {N}orthern {H}emisphere circulation data},
	Volume = {47A},
	Year = 1995}

@article{Townsend85,
	Annote = {Filed under Isentropic Observations. Shows observed
                  isentropic mass transport streamfunctions.},
	Author = {R. D. Townsend and D. R. Johnson},
	Journal = {J. Atmos. Sci.},
	Pages = {1565--1579},
	Title = {A Diagnostic Study of the Isentropic Zonally Averaged Mass Circulation during the First {GARP} Global Experiment},
	Volume = 42,
	Year = 1985}

@article{Tran02a,
	Annote = {Bounds on energy and enstrophy dissipation rates in
                  2d turbulence that is forced in a spectrally local
                  manner. Realizability of energy- and
                  enstrophy-cascading inertial ranges.},
	Author = {C. V. Tran and T. G. Shepherd},
	Journal = {Physica D},
	Pages = {1--22},
	Title = {Constraints on the spectral distribution of energy and enstrophy dissipation in forced two-dimensional turbulence},
	Volume = 165,
	Year = 2002}

@article{Tran02b,
	Annote = {Realizability of enstrophy- and energy-cascading
                  inertial ranges depends on forcing and dissipation.},
	Author = {C. V. Tran and J. C. Bowman},
	Journal = {Physica D},
	Pages = {??--??},
	Title = {On the dual cascade in two-dimensional turbulence},
	Volume = {???},
	Year = 2003}

@article{Treguier97,
	Annote = {Filed under Held.},
	Author = {A. M. Treguier and I. M. Held and V. D. Larichev},
	Journal = {J. Phys. Oceanogr.},
	Pages = {567--580},
	Title = {On the Parameterization of Quasi-Geostrophic Eddies in Primitive Equation Ocean Models},
	Volume = 27,
	Year = 1997}

@article{Trenberth01,
	Author = {Trenberth, K.E. and Caron, J.M.},
	File = {../../Papers/trenberth01.pdf},
	Journal = {J. Climate},
	Pages = {3433--3443},
	Title = {Estimates of Meridional Atmosphere and Ocean Heat Transports},
	Volume = 14,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg90cmVuYmVydGgwMS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQnwMK+v1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwMMhLwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHJlbmJlcnRoMDEucGRmAA4AIAAPAHQAcgBlAG4AYgBlAHIAdABoADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdHJlbmJlcnRoMDEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdHJlbmJlcnRoMDEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Trenberth03,
	Author = {K. E. Trenberth and D. P. Stepaniak},
	File = {../../Papers/trenberth03.pdf},
	Journal = {J. Climate},
	Pages = {3706--3722},
	Title = {Seamless Poleward Atmospheric Energy Transports and Implications for the {Hadley} Circulation},
	Volume = 16,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg90cmVuYmVydGgwMy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQovpgmzgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvpiJPgAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHJlbmJlcnRoMDMucGRmAA4AIAAPAHQAcgBlAG4AYgBlAHIAdABoADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdHJlbmJlcnRoMDMucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdHJlbmJlcnRoMDMucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Trenberth03a,
	Author = {K. E. Trenberth and D. P. Stepaniak},
	File = {../../Papers/trenberth03a.pdf},
	Journal = {J. Climate},
	Pages = {3691--3705},
	Title = {Covariability of Components of Poleward Atmospheric Energy Transports on Seasonal and Interannual Timescales},
	Volume = 16,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhB0cmVuYmVydGgwM2EucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQpxe/+qgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxfBhGgAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHJlbmJlcnRoMDNhLnBkZgAADgAiABAAdAByAGUAbgBiAGUAcgB0AGgAMAAzAGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3RyZW5iZXJ0aDAzYS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvdHJlbmJlcnRoMDNhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Trenberth03b,
	Annote = {Filed under Precipitation Statistics.},
	Author = {K. E. Trenberth and A. Dai and R. M. Rasmussen and D. B. Parsons},
	File = {../../Papers/trenberth03b.pdf},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {1205--1217},
	Title = {The changing character of precipitation},
	Volume = 84,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhB0cmVuYmVydGgwM2IucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQqwdLQGwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwdNAmwAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHJlbmJlcnRoMDNiLnBkZgAADgAiABAAdAByAGUAbgBiAGUAcgB0AGgAMAAzAGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3RyZW5iZXJ0aDAzYi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvdHJlbmJlcnRoMDNiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Trenberth05a,
	Annote = {Column water vapor appears to be relatively reliable
                  in ERA-40 and other reanalysis data after 1979.},
	Author = {K. E. Trenberth and L. Smith},
	File = {../../Papers/trenberth05a.pdf},
	Journal = {J. Climate},
	Pages = {864--875},
	Title = {The mass of the atmosphere: A constraint on global analyses},
	Volume = 18,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhB0cmVuYmVydGgwNWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQrv3VmMAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3XIoAAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHJlbmJlcnRoMDVhLnBkZgAADgAiABAAdAByAGUAbgBiAGUAcgB0AGgAMAA1AGEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3RyZW5iZXJ0aDA1YS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvdHJlbmJlcnRoMDVhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Trenberth05b,
	Annote = {ERA-40 and other reanalysis data problematic over oceans.},
	Author = {K. E. Trenberth and J. Fasullo and L. Smith},
	File = {../../Papers/trenberth05b.pdf},
	Journal = {Climate Dyn.},
	Pages = {741--758},
	Title = {Trends and variability in column-integrated atmospheric water vapor},
	Volume = 24,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhB0cmVuYmVydGgwNWIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQsv3VJdQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3Wr5QAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHJlbmJlcnRoMDViLnBkZgAADgAiABAAdAByAGUAbgBiAGUAcgB0AGgAMAA1AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3RyZW5iZXJ0aDA1Yi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvdHJlbmJlcnRoMDViLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Trenberth09a,
	Author = {K. E. Trenberth and J. T. Fasullo and J. Kiehl},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {311--323},
	Title = {Earth's Global Energy Budget},
	Volume = 90,
	Year = 2009}

@article{Trenberth90,
	Annote = {Not on file.},
	Author = {K. E. Trenberth},
	Journal = {Bull. Amer. Meteor. Soc.},
	Pages = {988--993},
	Title = {Recent observed interdecadal changes in the {N}orthern {H}emisphere},
	Volume = 71,
	Year = 1990}

@article{Trenberth94,
	Author = {Trenberth, K. E. and Solomon, A.},
	Journal = {Climate Dyn.},
	Pages = {107--134},
	Title = {The global heat balance: Heat transports in the atmosphere and ocean},
	Volume = {10},
	Year = {1994}}

@article{Trenberth96,
	Annote = {Fits ARMA model to El Nino time series and concludes
                  from model statistics the probability of occurence
                  of 1990--95 event. Doesn't validate model by
                  diagnostic checking; only uses AIC. Assumes noise to
                  be Gaussian. Could a noise distribution with a
                  longer tail induce more rare events such as
                  1990--95?},
	Author = {K. E. Trenberth and T. J. Hoar},
	Journal = {Geophys. Res. Lett.},
	Pages = {??},
	Title = {The 1990--1995 {E}l {N}i{\~n}o-{S}outhern {O}scillation Event: Longest on record},
	Volume = {??},
	Year = 1996}

@article{Trenberth98b,
	Author = {Trenberth, K.E.},
	File = {../../Papers/trenberth98b.pdf},
	Journal = {Climatic Change},
	Pages = {667--694},
	Title = {Atmospheric Moisture Residence Times and Cycling: Implications for Rainfall Rates and Climate Change},
	Volume = {39},
	Year = {1998},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhB0cmVuYmVydGg5OGIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQuxO74zQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxO9bPQAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHJlbmJlcnRoOThiLnBkZgAADgAiABAAdAByAGUAbgBiAGUAcgB0AGgAOQA4AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3RyZW5iZXJ0aDk4Yi5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvdHJlbmJlcnRoOThiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Trenberth99,
	Author = {K. E. Trenberth},
	File = {../../Papers/trenberth99.pdf},
	Journal = {Climatic Change},
	Pages = {327--339},
	Title = {Conceptual framework for changes of extremes of the hydrological cycle with climate change},
	Volume = 42,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg90cmVuYmVydGg5OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQvwqFI61BERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwqGrWwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHJlbmJlcnRoOTkucGRmAA4AIAAPAHQAcgBlAG4AYgBlAHIAdABoADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdHJlbmJlcnRoOTkucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdHJlbmJlcnRoOTkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Trevisan93,
	Annote = {Filed under Predictability.},
	Author = {A. Trevisan},
	Journal = {J. Atmos. Sci.},
	Pages = {1016--1028},
	Title = {Impact of Transient Error Growth on Global Average Predictability Measures},
	Volume = 50,
	Year = 1993}

@article{Troen86,
	Annote = {Simple boundary layer scheme.},
	Author = {I. B. Troen and L. Mahrt},
	File = {../../Papers/troen86.pdf},
	Journal = {Boundary-Layer Met.},
	Pages = {129--148},
	Title = {A simple model of the atmospheric boundary layer: {S}ensitivity to surface evaporation},
	Volume = 37,
	Year = 1986,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt0cm9lbjg2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQwvs5BoAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvs6kEAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHJvZW44Ni5wZGYADgAYAAsAdAByAG8AZQBuADgANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvdHJvZW44Ni5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy90cm9lbjg2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Tukey62,
	Author = {J. W. Tukey},
	Journal = {Ann. Math. Statist.},
	Pages = {1--67},
	Title = {The future of data analysis},
	Volume = 33,
	Year = 1962}

@book{Tukey77,
	Address = {Reading, MA},
	Annote = {Preface on file.},
	Author = {J. W. Tukey},
	Pages = 688,
	Publisher = {Addison-Wesley},
	Title = {Exploratory Data Analysis},
	Year = 1977}

@article{Tukey80,
	Annote = {Not on file.},
	Author = {J. W. Tukey},
	Journal = {Am. Statist.},
	Pages = {23--25},
	Title = {We need both exploratory and confirmatory},
	Volume = {34},
	Year = {1980}}

@article{Tung01,
	Annote = {Points out errors in Charney's note.},
	Author = {K. K. Tung and W. T. Welch},
	Journal = {J. Atmos. Sci.},
	Pages = {2009--2012},
	Title = {Remarks on {C}harney's Note on Geostrophic Turbulence},
	Volume = 58,
	Year = 2001}

@article{Tung03,
	Annote = {Considers overall energy spectrum (not baroclinic
                  and barotropic components). Finds k^{-5/3} spectrum
                  for large wavenumbers (larger than about Rossby
                  radius) and k^{-3} for smaller wavenumbers.},
	Author = {K. K. Tung and W. W. Orlando},
	Journal = {J. Atmos. Sci.},
	Pages = {???--???},
	Title = {The $k^{-3}$ and $k^{-5/3}$ energy spectrum of atmospheric turbulence: {Q}uasigeostrophic two-level model simulation},
	Volume = 60,
	Year = 2003}

@article{Tung86a,
	Author = {K. K. Tung},
	File = {../../Papers/tung86a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2600--2618},
	Title = {Nongeostrophic Theory of Zonally Averaged Circulation. {P}art {I}: Formulation},
	Volume = 43,
	Year = 1986,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt0dW5nODZhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQ2v+dIyVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv+e5SQAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHVuZzg2YS5wZGYADgAYAAsAdAB1AG4AZwA4ADYAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvdHVuZzg2YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy90dW5nODZhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Tung86b,
	Annote = {Filed under Atmospheric Chemistry (ESE172-02).},
	Author = {K.-K. Tung and M. K. W. Ko and J. M. Rodriguez and N. D. Sze},
	Journal = {Nature},
	Pages = {811--814},
	Title = {Are {A}ntarctic ozone variations a manifestation of dynamics or chemistry},
	Volume = 322,
	Year = 1986}

@article{Turkington01,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {B. Turkington and A. Majda and K. Haven and M. DiBattista},
	File = {../../Papers/turkington01.pdf},
	Journal = {Proc. Nat. Acad. Sci.},
	Pages = {12346--12350},
	Title = {Statistical Equilibrium Predictions of Jets and Spots on {J}upiter},
	Volume = 98,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXYAAAAAAXYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhB0dXJraW5ndG9uMDEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQ3wst6SQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsvcuQAAAAEADAAJDH4ACE6zAACS8wACAC9NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHVya2luZ3RvbjAxLnBkZgAADgAiABAAdAB1AHIAawBpAG4AZwB0AG8AbgAwADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAjVXNlcnMvdGFwaW8vUGFwZXJzL3R1cmtpbmd0b24wMS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEB0uLi8uLi9QYXBlcnMvdHVya2luZ3RvbjAxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIaAhwCIQIqAjUCOQJHAk4CVwJ3AnwCfwKMApEAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACow==}}

@article{Turkington96,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow. Algorithm for computing maximum entropy states.},
	Author = {B. Turkington and N. Whitaker},
	Journal = {SIAM J. Sci. Comp.},
	Pages = {1414--1433},
	Title = {Statistical Equilibrium Computations of Coherent Structures in Turbulent Shear Layers},
	Volume = 17,
	Year = 1996}

@article{Turkington99,
	Annote = {Filed under Equilibrium Statistical Mechanics of
                  Fluid Flow.},
	Author = {B. Turkington},
	Journal = {Comm. Pure Appl. Math.},
	Pages = {781--809},
	Title = {Statistical Equilibrium Measures and Coherent States in Two-Dimensional Turbulence},
	Volume = 52,
	Year = 1999}

@article{Turner67,
	Annote = {Filed under Kraus/Turner. Classic paper on seasonal
                  thermocline. See also Kraus67},
	Author = {J. S. Turner and E. B. Kraus},
	Journal = {Tellus},
	Pages = {88--97},
	Title = {A one-dimensional model of the seasonal thermocline: {I}. {A} laboratory experiment and its interpretation},
	Volume = 19,
	Year = 1967}

@article{Tyler82,
	Annote = {Filed under Predictability. Simultaneous
                  transformation of dependent and independent
                  variables in multivariate regression
                  model. Transformation maximizes the power of the
                  independent variables to predict the dependent
                  variables.},
	Author = {D. E. Tyler},
	Journal = {Psychometrika},
	Pages = {77--86},
	Title = {On the Optimality of the Simultaneous Redundancy Transformations},
	Volume = 47,
	Year = 1982}

@unpublished{Tziperman01,
	Author = {E. Tziperman},
	File = {../../Papers/tziperman01.pdf},
	Note = {Lecture Notes for Woods Hole GFD Progam},
	Title = {Conceptual Models in Climate Dynamics},
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg90emlwZXJtYW4wMS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQ4wVlvCVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwVnReQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dHppcGVybWFuMDEucGRmAA4AIAAPAHQAegBpAHAAZQByAG0AYQBuADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdHppcGVybWFuMDEucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdHppcGVybWFuMDEucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Tziperman89,
	Annote = {Use barotropic QG model to demonstrate that it is
                  feasible in principle to estimate uncertain model
                  parameters (e.g., mixing coefficients) and
                  stationary forcing fields (e.g, wind stress
                  fields).},
	Author = {E. Tziperman and W. C. Thacker},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1471--1485},
	Title = {An Optimal-Control/Adjoint-Equations Approach to Studying the Oceanic General Circulation},
	Volume = 19,
	Year = 1989}

@article{Tziperman92a,
	Annote = {Similar to Tziperman89, except using 3D GCM with
                  GCM-simulated pseudo-data. Problems with
                  ill-conditioning of inverse problem and multiple
                  solutions of optimization problem. Failure to get
                  good estimates of ocean circulation statistics in
                  high latitudes (because of ill-conditioning due to
                  convection).},
	Author = {E. Tziperman and W. C. Thacker and R. B. Long and S.-M. Hwang},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1434--1457},
	Title = {Oceanic Data Analysis Using a General Circulation Model. Part {I}: {S}imulation},
	Volume = 22,
	Year = 1992}

@article{Tziperman92b,
	Annote = {As Tziperman92a, but using 3D GCM with actual North
                  Atlantic data. Similar problems with
                  ill-conditioning of inverse problem and multiple
                  solutions of optimization problem as in
                  Tziperman92a.},
	Author = {E. Tziperman and W. C. Thacker and R. B. Long and S.-M. Hwang and S. R. Rintoul},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1458--1485},
	Title = {Oceanic Data Analysis Using a General Circulation Model. Part {II}: {A} {N}orth {A}tlantic Model},
	Volume = 22,
	Year = 1992}

@article{Tziperman93,
	Author = {E. Tziperman and K. Bryan},
	Journal = {J. Geophys. Res.},
	Pages = {22629--22644},
	Title = {Estimating Global Air-Sea Fluxes from Surface Properties And From Climatological Flux Data Using an Oceanic General Circulation Model},
	Volume = {98C},
	Year = 1993}

@article{Ufnar04,
	Annote = {Equable climates may have had low temperature
                  gradients because of increased latent heat transport.},
	Author = {D. F. Ufnar and L. A. Gonz{\'a}lez and G. A. Ludvigson and R. L. Brenner and B. J. Witzke},
	Journal = {Geology},
	Pages = {1049--1052},
	Title = {Evidence for increased latent heat transport during the {C}retaceous ({A}lbian) greenhouse warming},
	Volume = 32,
	Year = 2004}

@article{Uhlenbeck30,
	Annote = {Filed under Ornstein-Uhlenbeck Processes.},
	Author = {G. E. Uhlenbeck and L. S. Ornstein},
	Journal = {Phys. Rev.},
	Pages = {823--841},
	Title = {On the Theory of the {Brownian} Motion},
	Volume = 36,
	Year = 1930}

@article{Uppala05,
	Annote = {Filed under ECMWF Data.},
	Author = {S. M. Uppala and P. W. K{\aa}llberg and A. J. Simmons and U. Andrae and V. da Costa Bechtold and M. Fiorino and J. K Gibson and J. Haseler and A. Hernandez and G. A. Kelly and X. Li and K. Onogi and S. Saarinen and N. Sokka and R. P. Allan and E. Andersson and K. Arpe and M. A. Balmaseda and A. C. M. Beljaars and L. van de Berg and J. Bidlot and N. Bormann and S. Caires and F. Chevallier and A. Dethof and M. Dragsavac and M. Fisher and M. Fuentes and S. Hagemann and E. H{\'o}lm and B. J. Hoskins and L. Isaksen and P. A. E. M. Janssen and R. Jenne and A. P. McNally and J.-F. Mahfouf and J.-J. Morcrette and N. A. Rayner and R. W. Saunders and P. Simon and A. Sterl and K. E. Trenberth and A. Untch and D. Vasiljevic and P. Viterbo and J. Woolen},
	File = {../../Papers/uppala05.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {2961--3012},
	Title = {The {ERA-40} Reanalysis},
	Volume = {131},
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx1cHBhbGEwNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQ7v8KRNlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv8MBtgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dXBwYWxhMDUucGRmAAAOABoADAB1AHAAcABhAGwAYQAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3VwcGFsYTA1LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy91cHBhbGEwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Urban00,
	Author = {F. E. Urban and J. E. Cole and J. T. Overpeck},
	Journal = {Nature},
	Pages = {989--993},
	Title = {Influence of mean climate change on climate variability from a 155-year tropical {P}acific coral record},
	Volume = 407,
	Year = 2000}

@article{Valdes88,
	Annote = {Filed under Hoskins.},
	Author = {P. J. Valdes and B. J. Hoskins},
	File = {../../Papers/valdes88.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1584--1593},
	Title = {Baroclinic Instability of the Zonally Averaged Flow with Boundary Layer Damping},
	Volume = 45,
	Year = 1988,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx2YWxkZXM4OC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQ8vRs3qwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvRuaGwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dmFsZGVzODgucGRmAAAOABoADAB2AGEAbABkAGUAcwA4ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3ZhbGRlczg4LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy92YWxkZXM4OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Vallis04,
	Author = {G. K. Vallis and E. P. Gerber and P. J. Kushner and B. A. Cash},
	File = {../../Papers/vallis04.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {264--280},
	Title = {A mechanism and simple dynamical model of the {N}orth {A}tlantic {O}scillation and annular modes},
	Volume = 61,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx2YWxsaXMwNC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRQ+wCVDrQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwCW0LQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dmFsbGlzMDQucGRmAAAOABoADAB2AGEAbABsAGkAcwAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3ZhbGxpczA0LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy92YWxsaXMwNC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@book{Vallis06,
	Address = {Cambridge, UK},
	Author = {G. K. Vallis},
	File = {../../Papers/vallis_aofd.pdf},
	Pages = 771,
	Publisher = {Cambridge University Press},
	Title = {Atmospheric and Oceanic Fluid Dynamics: Fundamentals and Large-Scale Circulation},
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg92YWxsaXNfYW9mZC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRCv/+ftwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwAAQNwAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dmFsbGlzX2FvZmQucGRmAA4AIAAPAHYAYQBsAGwAaQBzAF8AYQBvAGYAZAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvdmFsbGlzX2FvZmQucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvdmFsbGlzX2FvZmQucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Vallis88,
	Annote = {Baroclinic adjustment only appropriate
                  for weakly forced flows.},
	Author = {G. K. Vallis},
	File = {../../Papers/vallis88.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {183--204},
	Title = {Numerical studies of eddy transport properties in eddy-resolving and parameterized models},
	Volume = 114,
	Year = 1988,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx2YWxsaXM4OC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRBwb/SJgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwcBCpgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dmFsbGlzODgucGRmAAAOABoADAB2AGEAbABsAGkAcwA4ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3ZhbGxpczg4LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy92YWxsaXM4OC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@incollection{Vallis93a,
	Annote = {Filed under Vallis, Geoturbulence.},
	Author = {G. K. Vallis},
	Booktitle = {Nonlinear phenomena in atmospheric and oceanic sciences},
	Editor = {C. F. Carnevale and R. Pierrehumbert},
	Pages = {1--25},
	Publisher = {Springer},
	Title = {Problems and phenomenology in two-dimensional turbulence},
	Year = 1993}

@article{Vallis93b,
	Annote = {Filed under Vallis, Geoturbulence. Generation of
                  anisotropy by inverse energy cascade.},
	Author = {G. K. Vallis and M. E. Maltrud},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1346--1362},
	Title = {Generation of Mean Flows and Jets on a Beta Plane and Over Topography},
	Volume = 23,
	Year = 1993}

@book{VanKampen01,
	Address = {Amsterdam},
	Author = {N. G. van Kampen},
	Pages = 480,
	Publisher = {North Holland},
	Title = {Stochastic Processes in Physics and Chemistry},
	Year = 2001}

@article{Vasavada05,
	Annote = {Filed under Jupiter Dynamics. Review of literature.},
	Author = {A. R. Vasavada and A. P. Showman},
	File = {../../Papers/vasavada05.pdf},
	Journal = {Rep. Prog. Phys.},
	Pages = {1935--1996},
	Title = {Jovian atmospheric dynamics: an update after {Galileo} and {Cassini}},
	Volume = 68,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg52YXNhdmFkYTA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRIwfTSGFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwfVCmAAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dmFzYXZhZGEwNS5wZGYAAA4AHgAOAHYAYQBzAGEAdgBhAGQAYQAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3Zhc2F2YWRhMDUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3Zhc2F2YWRhMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Vautard89,
	Annote = {Filed under Singular Spectrum Analysis.},
	Author = {R. Vautard and M. Ghil},
	Journal = {Physica D},
	Pages = {395--424},
	Title = {Singular Spectrum Analysis in Nonlinear Dynamics, with Applications to Paleoclimatic Time Series},
	Volume = 35,
	Year = 1989}

@article{Vautard92,
	Annote = {Filed under Singular Spectrum Analysis.},
	Author = {R. Vautard and P. Yiou and M. Ghil},
	Journal = {Physica D},
	Pages = {95--126},
	Title = {Singular-spectrum analysis: A toolkit for short, noisy chaotic signals},
	Volume = 58,
	Year = 1992}

@article{Vecchi06,
	Author = {G. A. Vecchi and B. J. Soden and A. T. Wittenberg and I. M. Held and A. Leetmaa and Matthew J. Harrison},
	File = {../../Papers/vecchi06.pdf},
	Journal = {Nature},
	Pages = {73--76},
	Title = {Weakening of tropical {P}acific atmospheric circulation due to anthropogenic forcing},
	Volume = 441,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx2ZWNjaGkwNi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRKwKuRA1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwKvzcwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dmVjY2hpMDYucGRmAAAOABoADAB2AGUAYwBjAGgAaQAwADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3ZlY2NoaTA2LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy92ZWNjaGkwNi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Vecchi07b,
	Author = {G. A. Vecchi and B. J. Soden},
	File = {../../Papers/vecchi07b.pdf},
	Journal = {J. Climate},
	Pages = {4316--4340},
	Title = {Global Warming and the Weakening of the Tropical Circulation},
	Volume = 20,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg12ZWNjaGkwN2IucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRLwy8cVFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwy9+xAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dmVjY2hpMDdiLnBkZgAOABwADQB2AGUAYwBjAGgAaQAwADcAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvdmVjY2hpMDdiLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3ZlY2NoaTA3Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Venzke99,
	Annote = {Not on file. Analysis formally equivalent to
                  predictable component analysis.},
	Author = {S. Venzke and M. R. Allen and R. T. Sutton and D. P. Rowell},
	Journal = {J. Climate},
	Pages = {2562--2584},
	Title = {The atmospheric response over the {N}orth {A}tlantic to decadal changes in sea surface temperature},
	Volume = 12,
	Year = 1999}

@article{VonStorch88,
	Annote = {Filed under Hasselmann.},
	Author = {H. {von Storch} and T. Bruns and I. Fischer-Bruns and K. Hasselmann},
	Journal = {J. Geophys. Res.},
	Pages = {11022--11036},
	Title = {{P}rincipal {O}scillation {P}attern analysis of the 30- to 60-day oscillation in general circulation model equatorial troposphere},
	Volume = {93D},
	Year = {1988}}

@article{Wahba77,
	Annote = {Not on file. Generalized cross-validation for
                  integral equations of the first kind},
	Author = {G. Wahba},
	Journal = {SIAM J. Numer. Anal.},
	Pages = {651--667},
	Title = {Practical approximate solutions to linear operator equations when the data are noisy},
	Volume = 14,
	Year = 1977}

@book{Wahba90,
	Address = {Philadelphia},
	Author = {G. Wahba},
	Pages = 169,
	Publisher = {Society for Industrial and Applied Mathematics},
	Series = {{CBMS-NSF} Regional Conference Series in Applied Mathematics},
	Title = {Spline Models for Observational Data},
	Volume = 59,
	Year = 1990}

@article{Wahba95,
	Annote = {Not on file. Distribution of GCV regularization
                  parameters has mass point near zero.},
	Author = {G. Wahba and Y. Wang},
	Journal = {Stat. Probabil. Lett.},
	Pages = {105--111},
	Title = {Behavior near zero of the distribution of {GCV} smoothing parameter estimates},
	Volume = 25,
	Year = 1995}

@article{Waliser08,
	Author = {D. E. Waliser and J. F. Li and J. Bacmeister and J. Chern and A. Del Genio and J. Jiang and M. Kharitondov and K. N. Liou and H. Meng and P. Minnis and W. B. Rossow and G. Stephens and S. Sun-Mack and W. K. Tao and A. Tompkins and D. Vane, C. Woods and D. Wu},
	File = {../../Papers/waliser08.pdf},
	Journal = {J. Geophys. Res.},
	Note = {in press},
	Pages = {??},
	Title = {Cloud Ice: A Climate Model Challenge With Signs and Expectations of Progress},
	Volume = {??},
	Year = 2008,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg13YWxpc2VyMDgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRWxTnHOAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxTo3uAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2FsaXNlcjA4LnBkZgAOABwADQB3AGEAbABpAHMAZQByADAAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvd2FsaXNlcjA4LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3dhbGlzZXIwOC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Waliser94,
	Annote = {Filed under ITCZ Dynamics. Contains good review of
                  theories for location of convection zones.},
	Author = {D. E. Waliser and R. C. J. Somerville},
	File = {../../Papers/waliser94.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1619--1639},
	Title = {Preferred Latitudes of the Intertropical Convergence Zone},
	Volume = 51,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg13YWxpc2VyOTQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRXwYqxdlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwYsh9gAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2FsaXNlcjk0LnBkZgAOABwADQB3AGEAbABpAHMAZQByADkANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvd2FsaXNlcjk0LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3dhbGlzZXI5NC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Walker02,
	Author = {C. Walker and G. Magnusdottir},
	Journal = {J. Atmos. Sci.},
	Pages = {2846--2859},
	Title = {Effect of the Hadley circulation on the reflection of planetary waves in three-dimensional tropospheric flows},
	Volume = 59,
	Year = 2002}

@article{Walker03,
	Author = {C. Walker and G. Magnusdottir},
	Journal = {J. Atmos. Sci.},
	Pages = {279--286},
	Title = {Nonlinear Planetary Wave Reflection in an Atmospheric {GCM}},
	Volume = 60,
	Year = 2003}

@article{Walker05a,
	Author = {C. C. Walker and T. Schneider},
	Date-Modified = {2010-06-11 11:44:30 -0700},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2004GL022304},
	Pages = {L06813},
	Title = {Response of idealized {Hadley} circulations to seasonally varying heating},
	Volume = {32},
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg13YWxrZXIwNWEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRYvkD+6QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvkFvaQAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2Fsa2VyMDVhLnBkZgAOABwADQB3AGEAbABrAGUAcgAwADUAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvd2Fsa2VyMDVhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3dhbGtlcjA1YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Walker06a,
	Author = {C. C. Walker and T. Schneider},
	Date-Modified = {2010-06-11 11:44:50 -0700},
	Journal = {J. Atmos. Sci.},
	Pages = {3333--3350},
	Title = {Eddy Influences on {Hadley} circulations: {S}imulations with an idealized {GCM}},
	Volume = {63},
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg13YWxrZXIwNmEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRZwbqoGAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwbsYmAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2Fsa2VyMDZhLnBkZgAOABwADQB3AGEAbABrAGUAcgAwADYAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvd2Fsa2VyMDZhLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3dhbGtlcjA2YS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Wallace02,
	Author = {J. M. Wallace and D. W. J. Thompson},
	Journal = {Physics Today},
	Month = {February},
	Note = {Review of NAM and SAM. Claims of predictability and stratospheric driving.},
	Pages = {28--33},
	Title = {Annular Modes and Climate Prediction},
	Year = 2002}

@article{Wallace78,
	Annote = { },
	Author = {J. M. Wallace},
	Journal = {J. Atmos. Sci.},
	Pages = {554--558},
	Title = {Trajectory Slopes, Countergradient Heat Fluxes and Mixing by Lower Stratospheric Waves},
	Volume = 35,
	Year = 1978}

@article{Wallace81,
	Author = {J. M. Wallace and D. S. Gutzler},
	Journal = {Mon. Wea. Rev.},
	Pages = {784--812},
	Title = {Teleconnections in the Geopotential Height Field during the {N}orthern {H}emisphere winter},
	Volume = 109,
	Year = 1981}

@article{Wallace95,
	Annote = {"Cold Ocean Warm Land" (COWL) Pattern. Longer
                  version Wallace96.},
	Author = {J. M. Wallace and Y. Zhang and J. A. Renwick},
	Journal = {Science},
	Pages = {780--783},
	Title = {Dynamic contribution to hemispheric mean temperature trends},
	Volume = 270,
	Year = 1995}

@article{Wallace96,
	Annote = {Long version of Wallace95; COWL pattern.},
	Author = {J. M. Wallace and Y. Zhang and L. Bajuk},
	Journal = {J. Climate},
	Pages = {249--259},
	Title = {Interpretation of interdecadal trends in {N}orthern {H}emisphere surface air temperature},
	Volume = 9,
	Year = 1996}

@article{Waple02,
	Annote = {Not on file.},
	Author = {A. M. Waple and M. E. Mann and R. S. Bradley},
	File = {../../Papers/waple02.pdf},
	Journal = {Climate Dyn.},
	Pages = {563--578},
	Title = {Long-term patterns of solar irradiance forcing in model experiments and proxy based surface temperature reconstructions},
	Volume = 18,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt3YXBsZTAyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRkwI5rZwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwI7N1wAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2FwbGUwMi5wZGYADgAYAAsAdwBhAHAAbABlADAAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvd2FwbGUwMi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy93YXBsZTAyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Ward97,
	Annote = {Filed under Predictability. Uses SVD to isolate
                  predictable modes of a system. Justification of
                  method is murky.},
	Author = {M. N. Ward and A. Navarra},
	Journal = {J. Climate},
	Pages = {2210--2220},
	Title = {Pattern Analysis of {SST}-Forced Variability in Ensemble {GCM} Simulations: Examples over {E}urope and the Tropical {P}acific},
	Volume = 10,
	Year = 1997}

@article{Wardle00,
	Author = {R. Wardle and J. Marshall},
	Journal = {J. Phys. Oceanogr.},
	Pages = {2481--2503},
	Title = {Representation of Eddies in Primitive Equation Models by a {PV} Flux},
	Volume = 30,
	Year = 2000}

@article{Warn89,
	Annote = {Weakly nonlinear baroclinic waves in two-layer model
                  near minimum critical shear.},
	Author = {T. Warn and P. Gauthier},
	File = {../../Papers/warn89.pdf},
	Journal = {Tellus},
	Pages = {115--131},
	Title = {Potential vorticity mixing by marginally unstable baroclinic disturbances},
	Volume = {41A},
	Year = 1989,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgp3YXJuODkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRmvIcK5AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvId7ZAAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2Fybjg5LnBkZgAADgAWAAoAdwBhAHIAbgA4ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3dhcm44OS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvd2Fybjg5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Warn95,
	Annote = {Filed under Quasigeostrophy -- Alternatives and Higher Order
                  Corrections.  Hierarchy of balanced models. Possible
                  breakdown of quasigeostrophic approximation in
                  long-time limit?},
	Author = {T. Warn and O. Bokhove and T. G. Shepherd and G. K. Vallis},
	File = {../../Papers/warn95.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {723--739},
	Title = {Rossby number expansions, slaving principles, and balance dynamics},
	Volume = 121,
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgp3YXJuOTUucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRnvI3SXQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvI5C3QAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2Fybjk1LnBkZgAADgAWAAoAdwBhAHIAbgA5ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3dhcm45NS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMvd2Fybjk1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Watterson87,
	Annote = {In linear model (WKB limit), meridional flow allows
                  propagation of Rossby waves through easterlies in
                  direction of meridional flow.},
	Author = {I. G. Watterson and E. K. Schneider},
	File = {../../Papers/watterson87.pdf},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {779-813},
	Title = {The effect of the {H}adley circulation on the meridional propagation of stationary waves},
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg93YXR0ZXJzb244Ny5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRpwTYdxFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwTaANAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2F0dGVyc29uODcucGRmAA4AIAAPAHcAYQB0AHQAZQByAHMAbwBuADgANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvd2F0dGVyc29uODcucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvd2F0dGVyc29uODcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Waugh05,
	Author = {D. W. Waugh},
	File = {../../Papers/waugh05.pdf},
	Journal = {J. Geophys. Res.},
	Note = {doi:10.1029/2004JD005664},
	Pages = {D11305},
	Title = {Impact of Potential Vorticity Intrusions on Subtropical Upper Tropospheric Humidity},
	Volume = {110D},
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt3YXVnaDA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRrv+HAogAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv+IxIgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2F1Z2gwNS5wZGYADgAYAAsAdwBhAHUAZwBoADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvd2F1Z2gwNS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy93YXVnaDA1LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Weare82,
	Author = {B. C. Weare and J. S. Nasstrom},
	Journal = {Mon. Wea. Rev.},
	Pages = {481--485},
	Title = {Examples of Extended Orthogonal Function Analysis},
	Volume = 110,
	Year = 1982}

@article{Weaver95,
	Annote = {Filed under Idealized GCM documentation.},
	Author = {C. P. Weaver and V. Ramanathan},
	File = {../../Papers/weaver95.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {11585--11591},
	Title = {Deductions from a simple climate model: Factors governing surface temperature and atmospheric thermal structure},
	Volume = {100D},
	Year = 1995,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx3ZWF2ZXI5NS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRtwXdsyQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwXfdSQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2VhdmVyOTUucGRmAAAOABoADAB3AGUAYQB2AGUAcgA5ADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3dlYXZlcjk1LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy93ZWF2ZXI5NS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@incollection{Webster06,
	Address = {Berlin, Germany},
	Annote = {Filed under Monsoon Dynamics.},
	Author = {P. J. Webster},
	Booktitle = {The Asian Monsoon},
	Editor = {B. Wang},
	File = {../../Papers/webster06.pdf},
	Pages = {3--66},
	Publisher = {Springer Praxis},
	Title = {The coupled monsoon system},
	Year = {2006},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg13ZWJzdGVyMDYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRvw030aAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw05W2AAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2Vic3RlcjA2LnBkZgAOABwADQB3AGUAYgBzAHQAZQByADAANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvd2Vic3RlcjA2LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3dlYnN0ZXIwNi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Webster74,
	Annote = {Filed under Regression Analysis},
	Author = {J. T. Webster and R. F. Gunst},
	Journal = {Technometrics},
	Pages = {513--522},
	Title = {Latent root regression analysis},
	Volume = 16,
	Year = 1974}

@article{Webster82,
	Annote = {Local zonal flow determines propagation
                  characteristics of Rossby waves, so Rossby waves can
                  penetrate into Tropics in regions of
                  (upper-troposphere) westerlies.},
	Author = {P. J. Webster and J. R. Holton},
	File = {../../Papers/webster82.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {722--733},
	Title = {Cross-equatorial response to middle-latitude forcing in a zonally varying basic state},
	Volume = 39,
	Year = 1982,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg13ZWJzdGVyODIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRwwOz8dAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwO1e5AAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2Vic3RlcjgyLnBkZgAOABwADQB3AGUAYgBzAHQAZQByADgAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvd2Vic3RlcjgyLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3dlYnN0ZXI4Mi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@incollection{Webster87,
	Address = {New York, NY},
	Author = {P. J. Webster},
	Booktitle = {Monsoons},
	Editor = {J. S. Fein and P. L. Stephens},
	File = {../../Papers/webster87.pdf},
	Pages = {3--32},
	Publisher = {John Wiley \& Sons},
	Title = {The Elementary Monsoon},
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg13ZWJzdGVyODcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRRywSTFL1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwSUnnwAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2Vic3Rlcjg3LnBkZgAOABwADQB3AGUAYgBzAHQAZQByADgANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvd2Vic3Rlcjg3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3dlYnN0ZXI4Ny5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Wehrl78,
	Author = {A. Wehr},
	Journal = {Rev. Mod. Phys.},
	Pages = {221--260},
	Title = {General Properties of Entropy},
	Volume = 50,
	Year = 1978}

@book{Wei94,
	Address = {Redwood City, CA},
	Annote = {Excerpted copies filed under AR Modeling.},
	Author = {W. W. S. Wei},
	Publisher = {Addison-Wesley},
	Title = {Time Series Analysis},
	Year = 1994}

@article{Welch98a,
	Author = {W. T. Welch and K. K. Tung},
	Journal = {J. Atmos. Sci.},
	Pages = {1285--1302},
	Title = {Nonlinear baroclinic adjustment and wavenumber selection in a simple case},
	Volume = 55,
	Year = 1998}

@article{Welch98b,
	Author = {W. T. Welch and K. K. Tung},
	Journal = {J. Atmos. Sci.},
	Pages = {2833--2851},
	Title = {On the equilibrium spectrum of transient waves in the atmosphere},
	Volume = 55,
	Year = 1998}

@article{Wentz00,
	Author = {F. J. Wentz and M. Schabel},
	File = {../../Papers/wentz00.pdf},
	Journal = {Nature},
	Pages = {414--416},
	Title = {Precise climate monitoring using complementary satellite data sets},
	Volume = 403,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt3ZW50ejAwLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRR2xOAqogAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxOCNEgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2VudHowMC5wZGYADgAYAAsAdwBlAG4AdAB6ADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvd2VudHowMC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy93ZW50ejAwLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Wentz07,
	Author = {F. J. Wentz and L. Ricciardulli and K. Hilburn and C. Mears},
	File = {../../Papers/wentz07.pdf},
	Journal = {Science},
	Pages = {233--235},
	Title = {How Much More Rain Will Global Warming Bring?},
	Volume = 317,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt3ZW50ejA3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRR3wsOHjgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsPp/gAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2VudHowNy5wZGYADgAYAAsAdwBlAG4AdAB6ADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvd2VudHowNy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy93ZW50ejA3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==},
	Bdsk-File-2 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAagAAAAAAagAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfh10YWthaGFzaGlfd2VudHpfY29tbWVudDA4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRPuw+w6wAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw+yrQAAAAAEADAAJDH4ACE6zAACS8wACADxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6dGFrYWhhc2hpX3dlbnR6X2NvbW1lbnQwOC5wZGYADgA8AB0AdABhAGsAYQBoAGEAcwBoAGkAXwB3AGUAbgB0AHoAXwBjAG8AbQBtAGUAbgB0ADAAOAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASADBVc2Vycy90YXBpby9QYXBlcnMvdGFrYWhhc2hpX3dlbnR6X2NvbW1lbnQwOC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QKi4uLy4uL1BhcGVycy90YWthaGFzaGlfd2VudHpfY29tbWVudDA4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAJMAk4CUwJcAmcCawJ5AoACiQK2ArsCvgLLAtAAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAC4g==}}

@article{Wernli02,
	Author = {Wernli, H. and Dirren, S. and Liniger, M. A. and Zillig, M.},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {405--429},
	Title = {Dynamical aspects of the life cycle of the winter storm {`Lothar'} (24--26 {D}ecember 1999)},
	Volume = {128},
	Year = {2002}}

@article{Wernli97,
	Annote = {Filed under Water Vapor (Feedback and Kinematics).},
	Author = {H. Wernli},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {1677--1706},
	Title = {A {L}agrangian-based analysis of extratropical cyclones.{II}: A detailed case-study},
	Volume = 123,
	Year = 1997}

@incollection{West04,
	Author = {R. A. West and K. H. Baines and A. J. Friedson and D. Banfield and B. Ragent and F. W. Taylor},
	Booktitle = {Jupiter: The Planet, Satellites and Magnetosphere},
	Editor = {F. Bagenal and T. E. Dowling and W. B. McKinnon},
	Pages = {79--104},
	Publisher = {Cambridge University Press},
	Title = {Jovian Clouds and Haze},
	Year = 2004}

@article{Wetherald75,
	Annote = {Filed under Manabe.},
	Author = {R. T. Wetherald and S. Manabe},
	Journal = {J. Atmos. Sci.},
	Pages = {2044--2059},
	Title = {The effects of changing the solar constant on the climate of a general circulation model},
	Volume = 32,
	Year = 1975}

@article{Wheeler00,
	Author = {M. Wheeler and G. N. Kiladis and P. J. Webster},
	Journal = {J. Atmos. Sci.},
	Pages = {613--640},
	Title = {Large-scale dynamical fields associated with convectively coupled equatorial waves},
	Volume = 57,
	Year = 2000}

@article{Wheeler99,
	Author = {M. Wheeler and G. N. Kiladis},
	File = {../../Papers/wheeler99.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {374--399},
	Title = {Convectively coupled equatorial waves: Analysis of clouds and temperature in the wavenumber-frequency domain},
	Volume = 56,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg13aGVlbGVyOTkucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRR5v/HeV1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv/JO1wAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2hlZWxlcjk5LnBkZgAOABwADQB3AGgAZQBlAGwAZQByADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvd2hlZWxlcjk5LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3doZWVsZXI5OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Whitaker94,
	Annote = {Not on file.},
	Author = {J. S. Whitaker and C. A. Davis},
	Journal = {J. Atmos. Sci.},
	Pages = {889--907},
	Title = {Cyclogenesis in a saturated environment},
	Volume = 51,
	Year = 1994}

@article{White77,
	Annote = {Filed under Quasigeostrophy -- Alternatives and
                  Higher Order Corrections.},
	Author = {A. A. White},
	Journal = {Quart. J. Roy. Meteor. Soc.},
	Pages = {383--396},
	Title = {Modified quasi-geostrophic equations using geometric height as vertical coordinate},
	Volume = 103,
	Year = 1977}

@article{Wigley90,
	Annote = {Filed under Climate Change Detection. Use energy
                  balance model for oceanic mixed layer to estimate
                  low-frequency variability of SST. Find that the
                  ocean may produce substantial low-frequency
                  variability, which, however, is smaller than the
                  observed trend over the last century. Claim that
                  high-frequency variability is insensitive to value
                  of climate sensitivity.},
	Author = {T. M. L. Wigley and S. C. B. Raper},
	Journal = {Nature},
	Pages = {324--327},
	Title = {Natural Variability of the Climate System and Detection of the Greenhouse Effect},
	Volume = 344,
	Year = 1990}

@article{Wigley98,
	Annote = {Filed under Climate Change Detection. Careful
                  analysis of how the correlation statistic of
                  Santer95 behaves in an idealized setting with a
                  synthetic data ensemble. Today it should be mainly
                  data coverage deficiencies that prevent us from
                  ``detecting'' an anthropogenic climate change in the
                  observational record. Claim that little is to be
                  gained by looking for time-dependent signal, instead
                  of the time-independent signal used in most studies
                  to date. Introduction has a concise review of
                  rationale and practice of current detection
                  studies.},
	Author = {T. M. L. Wigley and P. J. Jaumann and B. D. Santer and K. E. Taylor},
	Journal = {Climate Dyn.},
	Pages = {781--790},
	Title = {Relative Detectability of Greenhouse-Gas and Aerosol Climate Change Signals},
	Volume = 14,
	Year = 1998}

@article{Wilby02,
	Annote = {Filed under Precipitation Statistics. Use gamma
                  function to characterize precip pdf.},
	Author = {R. L. Wilby and T. M. L. Wigley},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2001GL013048},
	Pages = 1135,
	Title = {Future changes in the distribution of daily precipitation totals across {North} {A}merica},
	Volume = 29,
	Year = 2002}

@article{Wilcox07,
	Author = {E. M. Wilcox and L. J. Donner},
	File = {../../Papers/wilcox07.pdf},
	Journal = {J. Climate},
	Pages = {53--69},
	Title = {The Frequency of Extreme Rain Events in Satellite Rain-Rate Estimates and an Atmospheric General Circulation Model},
	Volume = 20,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx3aWxjb3gwNy5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRR9wdnAWVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwdow2QAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2lsY294MDcucGRmAAAOABoADAB3AGkAbABjAG8AeAAwADcALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3dpbGNveDA3LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy93aWxjb3gwNy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@book{Wilkinson65,
	Address = {Oxford},
	Author = {J. H. Wilkinson},
	Pages = 662,
	Publisher = {Clarendon Press},
	Series = {Monographs on Numerical Analysis},
	Title = {The Algebraic Eigenvalue Problem},
	Year = 1965}

@article{Willett07,
	Author = {Willett, K. M. and Gillett, N. P. and Jones, P. D. and Thorne, P. W.},
	File = {../../Papers/willett07.pdf},
	Journal = {Nature},
	Pages = {710--713},
	Title = {Attribution of observed surface humidity changes to human influence},
	Volume = {449},
	Year = {2007},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWgAAAAAAWgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg13aWxsZXR0MDcucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRR+xaE10AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxaGmUAAAAAEADAAJDH4ACE6zAACS8wACACxNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2lsbGV0dDA3LnBkZgAOABwADQB3AGkAbABsAGUAdAB0ADAANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACBVc2Vycy90YXBpby9QYXBlcnMvd2lsbGV0dDA3LnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAaLi4vLi4vUGFwZXJzL3dpbGxldHQwNy5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACDAIOAhMCHAInAisCOQJAAkkCZgJrAm4CewKAAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAApI=}}

@article{Williams02,
	Author = {G. P. Williams},
	File = {../../Papers/williams02.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1356--1370},
	Title = {Jovian Dynamics. {Part~II}: The Genesis and Equilibration of Vortex Sets},
	Volume = 59,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg53aWxsaWFtczAyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRR/wN3Ym1BERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwN47CwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2lsbGlhbXMwMi5wZGYAAA4AHgAOAHcAaQBsAGwAaQBhAG0AcwAwADIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3dpbGxpYW1zMDIucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3dpbGxpYW1zMDIucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Williams03a,
	Author = {G. P. Williams},
	File = {../../Papers/williams03a.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1270--1296},
	Title = {Jovian Dynamics. {Part~III}: {M}ultiple, Migrating, and Equatorial Jets},
	Volume = 60,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg93aWxsaWFtczAzYS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSAwN3WvFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwN45LAAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2lsbGlhbXMwM2EucGRmAA4AIAAPAHcAaQBsAGwAaQBhAG0AcwAwADMAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvd2lsbGlhbXMwM2EucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvd2lsbGlhbXMwM2EucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Williams03b,
	Author = {G. P. Williams},
	File = {../../Papers/williams03b.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2136--2152},
	Title = {Barotropic Instability and Equatorial Superrotation},
	Volume = 60,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAXAAAAAAAXAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg93aWxsaWFtczAzYi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSBw7e73VBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7gsXQAAAAEADAAJDH4ACE6zAACS8wACAC5NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2lsbGlhbXMwM2IucGRmAA4AIAAPAHcAaQBsAGwAaQBhAG0AcwAwADMAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACJVc2Vycy90YXBpby9QYXBlcnMvd2lsbGlhbXMwM2IucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBwuLi8uLi9QYXBlcnMvd2lsbGlhbXMwM2IucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhQCFgIbAiQCLwIzAkECSAJRAnACdQJ4AoUCigAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKc}}

@article{Williams06,
	Author = {G. P. Williams and K. Bryan},
	File = {../../Papers/williams06.pdf},
	Journal = {J. Climate},
	Pages = {1706--1715},
	Title = {Ice Age Winds: An Aquaplanet Model},
	Volume = 19,
	Year = 2006,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg53aWxsaWFtczA2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSCwNHu5lBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwNJRVgAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2lsbGlhbXMwNi5wZGYAAA4AHgAOAHcAaQBsAGwAaQBhAG0AcwAwADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3dpbGxpYW1zMDYucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3dpbGxpYW1zMDYucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ},
	Bdsk-File-2 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAYAAAAAAAYAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfhN3aWxsaWFtczA2X2NvcnIucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSDwNHyzVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwNJVPQAAAAEADAAJDH4ACE6zAACS8wACADJNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2lsbGlhbXMwNl9jb3JyLnBkZgAOACgAEwB3AGkAbABsAGkAYQBtAHMAMAA2AF8AYwBvAHIAcgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASACZVc2Vycy90YXBpby9QYXBlcnMvd2lsbGlhbXMwNl9jb3JyLnBkZgATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAgLi4vLi4vUGFwZXJzL3dpbGxpYW1zMDZfY29yci5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACJAImAisCNAI/AkMCUQJYAmEChAKJAowCmQKeAAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAArA=}}

@article{Williams79,
	Author = {G. P. Williams},
	File = {../../Papers/williams79.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {932--968},
	Title = {Planetary Circulations: 2. {The} {Jovian} Quasi-Geostrophic Regime},
	Volume = 36,
	Year = 1979,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg53aWxsaWFtczc5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSHw7e7ClBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw7grigAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2lsbGlhbXM3OS5wZGYAAA4AHgAOAHcAaQBsAGwAaQBhAG0AcwA3ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3dpbGxpYW1zNzkucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3dpbGxpYW1zNzkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Williams88a,
	Annote = {GCM simulations of circulation regimes.},
	Author = {G. P. Williams},
	Journal = {Climate Dyn.},
	Pages = {205--260},
	Title = {The dynamical range of global circulations --- {I}},
	Volume = 2,
	Year = 1988}

@article{Williams88b,
	Annote = {GCM simulations of circulation regimes.},
	Author = {G. P. Williams},
	Journal = {Climate Dyn.},
	Pages = {45--84},
	Title = {The dynamical range of global circulations --- {II}},
	Volume = 3,
	Year = 1988}

@article{Williams89,
	Annote = {Effect of deepending of mixed layer by air-sea
                  interaction on potential vorticity of thermocline.},
	Author = {R. G. Williams},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1255--1267},
	Title = {The Influence of Air-Sea Interaction on the Ventilated Thermocline},
	Volume = 19,
	Year = 1989}

@article{Williams91,
	Annote = {Can get homogenized pv in thermocline by
                  ventilation; no eddy stirring required.},
	Author = {R. G. Williams},
	Journal = {J. Phys. Oceanogr.},
	Pages = {1803--1814},
	Title = {The Role of the Mixed Layer in Setting the Potential Vorticity of the Main Thermocline},
	Volume = 21,
	Year = 1991}

@article{Wilson96,
	Annote = {Filed under Stochastic Lagrangian Models of Turbulence.},
	Author = {J. D. Wilson and B. L. Sawford},
	File = {../../Papers/wilson96.pdf},
	Journal = {Bound.-Layer Meteor.},
	Pages = {191--210},
	Title = {Review of {L}agrangian Stochastic Models for Trajectories in the Turbulent Atmosphere},
	Volume = 78,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx3aWxzb245Ni5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSJv5Tv1wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5VgVwAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d2lsc29uOTYucGRmAAAOABoADAB3AGkAbABzAG8AbgA5ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3dpbHNvbjk2LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy93aWxzb245Ni5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Wolfinger94,
	Annote = {Filed under Parameter Estimation.},
	Author = {R. Wolfinger and R. Tobias and J. Sall},
	Journal = {{SIAM} J. Sci. Comput.},
	Key = {parameter estimation},
	Pages = {1294--1310},
	Title = {Computing {G}aussian Likelihood and their Derivatives for General Linear Mixed Models},
	Volume = 15,
	Year = 1994}

@article{Wong03,
	Annote = {Filed under Tropopause Dynamics.},
	Author = {S. Wong and W.-C. Wang},
	Journal = {J. Geophys. Res.},
	Note = {doi:10.129/2001JD002016},
	Pages = 4043,
	Title = {Tropical-extratropical connection in interannual variation of the tropopause: Comparison between {NCEP/NCAR} reanalysis and an atmospheric general circulation model simulation},
	Volume = {108D},
	Year = 2003}

@article{Wood06,
	Author = {R. Wood and C. S. Bretherton},
	Journal = {J. Climate},
	Pages = {6425--6432},
	Title = {On the Relationship between Stratiform Low Cloud Cover and Lower-Tropospheric Stability},
	Volume = 19,
	Year = 2006}

@article{Wood91,
	Author = {E. F. Wood},
	Journal = {Rev. Geophys.},
	Pages = {193--201},
	Title = {Global Scale Hydrology: Advances in Land Surface Modeling},
	Volume = {{\rm Supplement}},
	Year = 1991}

@article{Wright09,
	Author = {J. S. Wright and A. H. Sobel and G. A. Schmidt},
	File = {../../Papers/wright09.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2009GL038091},
	Pages = {L12804},
	Title = {Influence of condensate evaporation on water vapor and its stable isotopes in a {GCM}},
	Volume = 36,
	Year = 2009,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx3cmlnaHQwOS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSPxn+myQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxoAJOQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d3JpZ2h0MDkucGRmAAAOABoADAB3AHIAaQBnAGgAdAAwADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3dyaWdodDA5LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy93cmlnaHQwOS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Wu04,
	Annote = {Filed under Empirical Mode Decomposition.},
	Author = {Z. Wu and N. E. Huang},
	Journal = {Proc. R. Soc. Lond. A},
	Pages = {1597--1611},
	Title = {A study of the characteristics of white noise using the empirical mode decomposition method},
	Volume = 460,
	Year = 2004}

@article{Wu07,
	Annote = {Filed under Empirical Mode Decomposition.},
	Author = {Z. Wu and N. E. Huang S. R. Long and C.-K. Peng},
	Journal = {Proc. Nat. Aacad. Sci.},
	Pages = {14889--14894},
	Title = {On the trend, detrending, and variability of nonlinear and nonstationary time series},
	Volume = 38,
	Year = 2007}

@article{Wu09,
	Author = {Wu, Y.},
	Journal = {J. Climate},
	Note = {To be submitted},
	Title = {Storm track changes in a warmer climate from {GFDL} model simulation}}

@article{Wu98,
	Author = {Wu, G. and Zhang, Y.},
	File = {../../Papers/wu98.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {913--927},
	Title = {Tibetan {P}lateau forcing and the timing of the monsoon onset over {S}outh {A}sia and the {S}outh {C}hina {S}ea},
	Volume = {126},
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgh3dTk4LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSSwS39kVBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwS5gAQAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6d3U5OC5wZGYAAA4AEgAIAHcAdQA5ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL3d1OTgucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL3d1OTgucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@article{Xie99,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {Xie, S. P. and Saiki, N.},
	File = {../../Papers/xie99.pdf},
	Journal = {J. Meteor. Soc. Japan},
	Pages = {949--968},
	Title = {Abrupt onset and slow seasonal evolution of summer monsoon in an idealized {GCM} simulation},
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgl4aWU5OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSYwSRAIFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwSSikAAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eGllOTkucGRmAA4AFAAJAHgAaQBlADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMveGllOTkucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMveGllOTkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Xu89,
	Annote = {Filed under Emanuel. Stratification in tropical atmosphere 
                  close to moist adiabat.},
	Author = {K.-M. Xu and K. A. Emanuel},
	File = {../../Papers/xu89.pdf},
	Journal = {Mon. Wea. Rev.},
	Pages = {1471--1479},
	Title = {Is the tropical atmosphere conditionally unstable?},
	Volume = 117,
	Year = 1989,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVYAAAAAAVYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgh4dTg5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSZvo6RpgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvo70FgAAAAEADAAJDH4ACE6zAACS8wACACdNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eHU4OS5wZGYAAA4AEgAIAHgAdQA4ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAbVXNlcnMvdGFwaW8vUGFwZXJzL3h1ODkucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAVLi4vLi4vUGFwZXJzL3h1ODkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfoB/AIBAgoCFQIZAicCLgI3Ak8CVAJXAmQCaQAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ7}}

@article{Xu90,
	Annote = {Not on file.},
	Author = {J. S. Xu and H. {von Storch}},
	Journal = {J. Climate},
	Pages = {1316--1329},
	Title = {Predicting the state of the {S}outhern {O}scillation using principal oscillation pattern analysis},
	Volume = 3,
	Year = 1990}

@article{Xue94,
	Annote = {Filed under Blumenthal.},
	Author = {Y. Xue and M. A. Cane and S. E. Zebiak and M. B. Blumenthal},
	Journal = {Tellus},
	Pages = {512--528},
	Title = {On the Prediction of {ENSO}: A Study with a Low-Order {M}arkov Model},
	Volume = 46,
	Year = 1994}

@article{Xue96,
	Annote = {Not on File.},
	Author = {Y. Xue and M. J. Fennessy and P. J. Sellers},
	Journal = {J. Geophys. Res.},
	Pages = {7419--7430},
	Title = {Impact of Vegetation Properties on {U.S.} Summer Weather Prediction},
	Volume = {101D},
	Year = 1996}

@article{Yamazaki05,
	Author = {Y. H. Yamazaki and P. L. Read and D. R. Skeet},
	File = {../../Papers/yamazaki05.pdf},
	Journal = {Planet. Space Sci.},
	Pages = {508--525},
	Title = {Hadley circulations and {Kelvin} wave-driven equatorial jets in the atmospheres of {Jupiter} and {Saturn}},
	Volume = 53,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg55YW1hemFraTA1LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSewst44VBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsvbUQAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFtYXpha2kwNS5wZGYAAA4AHgAOAHkAYQBtAGEAegBhAGsAaQAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3lhbWF6YWtpMDUucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3lhbWF6YWtpMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@article{Yanai73,
	Author = {M. Yanai and S. Esbensen and J.-H. Chu},
	File = {../../Papers/yanai73.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {611--627},
	Title = {Determination of bulk properties of tropical cloud clusters from large-scale heat and moisture budgets},
	Volume = 30,
	Year = 1973,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt5YW5haTczLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSfxoC5ZQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxoEb1QAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFuYWk3My5wZGYADgAYAAsAeQBhAG4AYQBpADcAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMveWFuYWk3My5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy95YW5haTczLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Yang03,
	Annote = {Filed under Hoskins.},
	Author = {G.-Y. Yang and B. Hoskins and J. Slingo},
	File = {../../Papers/yang03.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1637--1653},
	Title = {Convectively coupled equatorial waves: {A} new methodology for identifying wave structures in observational data},
	Volume = 60,
	Year = 2003,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgp5YW5nMDMucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSgwsOR3wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwsP0TwAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFuZzAzLnBkZgAADgAWAAoAeQBhAG4AZwAwADMALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3lhbmcwMy5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMveWFuZzAzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Yang07a,
	Author = {G.-Y. Yang and B. Hoskins and J. Slingo},
	File = {../../Papers/yang07a.pdf},
	Journal = {J. Atmos. Sci.},
	Note = {Filed under Hoskins.},
	Pages = {3406--3423},
	Title = {Convectively Coupled Equatorial Waves. {Part~I}: {H}orizontal and Vertical Structures},
	Volume = 64,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt5YW5nMDdhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRShw1aMCFBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw1b8iAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFuZzA3YS5wZGYADgAYAAsAeQBhAG4AZwAwADcAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMveWFuZzA3YS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy95YW5nMDdhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Yang07b,
	Author = {G.-Y. Yang and B. Hoskins and J. Slingo},
	File = {../../Papers/yang07b.pdf},
	Journal = {J. Atmos. Sci.},
	Note = {Filed under Hoskins.},
	Pages = {3424--3437},
	Title = {Convectively Coupled Equatorial Waves. {Part~II}: {P}ropagation Characteristics},
	Volume = 64,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt5YW5nMDdiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSiw1aMLVBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw1b8rQAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFuZzA3Yi5wZGYADgAYAAsAeQBhAG4AZwAwADcAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMveWFuZzA3Yi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy95YW5nMDdiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Yang07c,
	Author = {G.-Y. Yang and B. Hoskins and J. Slingo},
	File = {../../Papers/yang07c.pdf},
	Journal = {J. Atmos. Sci.},
	Note = {Filed under Hoskins.},
	Pages = {3438--3451},
	Title = {Convectively Coupled Equatorial Waves. {Part~III}: {S}ynthesis Structures and Their Forcing and Evolution},
	Volume = 64,
	Year = 2007,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt5YW5nMDdjLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSjw1aMPFBERiBwcnZ3AAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAw1b8vAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFuZzA3Yy5wZGYADgAYAAsAeQBhAG4AZwAwADcAYwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMveWFuZzA3Yy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy95YW5nMDdjLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Yang81,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {D.-S. Yang and T. N. Krishnamurti},
	File = {../../Papers/yang81.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {2676--2695},
	Title = {Potential vorticity of monsoonal low-level flows},
	Volume = 38,
	Year = 1981,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgp5YW5nODEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSkwahzfwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwajj/wAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFuZzgxLnBkZgAADgAWAAoAeQBhAG4AZwA4ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3lhbmc4MS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMveWFuZzgxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Yang90,
	Annote = {Filed under Tung.},
	Author = {H. Yang and K. K. Tung and E. Olaguer},
	Journal = {J. Atmos. Sci.},
	Pages = {215--241},
	Title = {Nongeostrophic Theory of Zonally Averaged Circulation. {P}art {II}: {Eliassen}-{Palm} Flux Divergence and Isentropic Mixing Coefficient},
	Volume = 47,
	Year = 1990}

@article{Yang94,
	Annote = {Filed under Pierrehumbert.},
	Author = {H. Yang and R. T. Pierrehumbert},
	File = {../../Papers/yang94.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3437--3454},
	Title = {Production of Dry Air by Isentropic Mixing},
	Volume = 51,
	Year = 1994,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgp5YW5nOTQucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSlv7YsMwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv7acswAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFuZzk0LnBkZgAADgAWAAoAeQBhAG4AZwA5ADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3lhbmc5NC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMveWFuZzk0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Yang96,
	Annote = {Filed under Hoskins. Sequel in Hoskins00.},
	Author = {G.-Y. Yang and B. J. Hoskins},
	File = {../../Papers/yang96.pdf},
	Journal = {J. Atmos. Sci.},
	Title = {Propagation of {Rossby} waves of nonzero frequency},
	Volume = 53,
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgp5YW5nOTYucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSmwO0B1QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwO1kRQAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFuZzk2LnBkZgAADgAWAAoAeQBhAG4AZwA5ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3lhbmc5Ni5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMveWFuZzk2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Yang98,
	Annote = {Filed under Predictability. Do EOF analysis of
                  ensemble mean and find that in some areas in the
                  extratropics the variation of the ensemble mean is
                  dominated by reproducible forced modes and not by
                  chaotic internal fluctuations.},
	Author = {X.-Q. Yang and J. L. Anderson and W. F. Stern},
	Journal = {J. Climate},
	Pages = {in press},
	Title = {Reproducible Forced Modes in {AGCM} Ensemble Integrations and Potential Predictability of Atmospheric Seasonal Variations in the Extratropics},
	Volume = 11,
	Year = 1998}

@article{Yano91,
	Author = {J.-I. Yano and K. A. Emanuel},
	File = {../../Papers/yano91.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {377--389},
	Title = {An improved model of the equatorial troposphere and its coupling with the stratosphere},
	Volume = {48},
	Year = {1991},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgp5YW5vOTEucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSowS3yVFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwS5UxAAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFubzkxLnBkZgAADgAWAAoAeQBhAG4AbwA5ADEALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3lhbm85MS5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMveWFubzkxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Yano98,
	Annote = {Filed under Monsoon Dynamics.},
	Author = {J.-I. Yano and J. L. McBride},
	File = {../../Papers/yano98.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1373--1399},
	Title = {An Aquaplanet Monsoon},
	Volume = 55,
	Year = 1998,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAV4AAAAAAV4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgp5YW5vOTgucGRmAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSqwAGnmlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwAIYGgAAAAEADAAJDH4ACE6zAACS8wACAClNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFubzk4LnBkZgAADgAWAAoAeQBhAG4AbwA5ADgALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAdVXNlcnMvdGFwaW8vUGFwZXJzL3lhbm85OC5wZGYAABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBcuLi8uLi9QYXBlcnMveWFubzk4LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAICAgQCCQISAh0CIQIvAjYCPwJZAl4CYQJuAnMAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAAChQ==}}

@article{Yao87,
	Annote = {Filed under Stone. See also Stone87.},
	Author = {M.-S. Yao and P. H. Stone},
	File = {../../Papers/yao87.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {65--82},
	Title = {Development of a Two-Dimensional Zonally Averaged Statistical-Dynamical Model. {Part}~I: {The} Parameterization of Moist Convection and its Role in the General Circulation},
	Volume = 44,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgl5YW84Ny5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSrvmSIGwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvmT4mwAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFvODcucGRmAA4AFAAJAHkAYQBvADgANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMveWFvODcucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMveWFvODcucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Yao99,
	Author = {Yao, M. S. and Del Genio, A. D.},
	File = {../../Papers/yao99.pdf},
	Journal = {J. Climate},
	Pages = {761--779},
	Title = {Effects of cloud parameterization on the simulation of climate changes in the {GISS} {GCM}},
	Volume = {12},
	Year = {1999},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgl5YW85OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSsxoPH7QAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxoQqXQAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFvOTkucGRmAA4AFAAJAHkAYQBvADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMveWFvOTkucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMveWFvOTkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Yarosh96,
	Author = {E. S. Yarosh and C. F. Ropelewski and K. E. Mitchell},
	File = {../../Papers/yarosh96.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {23289--23298},
	Title = {Comparisons of humidity observations and Eta model analyses and forecasts for water balance studies},
	Volume = {101D},
	Year = 1996,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx5YXJvc2g5Ni5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRStvsp+AQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvsrgcQAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFyb3NoOTYucGRmAAAOABoADAB5AGEAcgBvAHMAaAA5ADYALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3lhcm9zaDk2LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy95YXJvc2g5Ni5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Yarosh99,
	Author = {E. S. Yarosh and C. F. Ropelewski and E. H. Berbery},
	File = {../../Papers/yarosh99.pdf},
	Journal = {J. Geophys. Res.},
	Pages = {19349--19360},
	Title = {Biases of the observed atmospheric water budgets over the central {U}nited {S}tates},
	Volume = {104D},
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx5YXJvc2g5OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSuvsp+bAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAvsrg3AAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWFyb3NoOTkucGRmAAAOABoADAB5AGEAcgBvAHMAaAA5ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3lhcm9zaDk5LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy95YXJvc2g5OS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Yeung01,
	Annote = {Filed under Stochastic Lagrangian Models of
                  Turbulence. Discusses applicability of regression
                  model for conditional scalar diffusion (scalar
                  diffusion is function of concentration and velocity,
                  plus white noise).},
	Author = {P. K. Yeung},
	File = {../../Papers/yeung01.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {241--274},
	Title = {Lagrangian characteristics of turbulence and scalar transport in direct numerical simulations},
	Volume = 427,
	Year = 2001,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt5ZXVuZzAxLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSvv5LUSlBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5NEygAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWV1bmcwMS5wZGYADgAYAAsAeQBlAHUAbgBnADAAMQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMveWV1bmcwMS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy95ZXVuZzAxLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Yeung02,
	Annote = {Filed under Stochastic Lagrangian Models of
                  Turbulence. Has a short reviews of recent DNS
                  results on Lagrangian statistics of passive scalar
                  (based on yeung01).},
	Author = {P. K. Yeung},
	File = {../../Papers/yeung02.pdf},
	Journal = {Annu. Rev. Fluid Mech.},
	Pages = {115--142},
	Title = {Lagrangian Investigations of Turbulence},
	Volume = 34,
	Year = 2002,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt5ZXVuZzAyLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSwv5LYnFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5NJHAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWV1bmcwMi5wZGYADgAYAAsAeQBlAHUAbgBnADAAMgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMveWV1bmcwMi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy95ZXVuZzAyLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Yin05,
	Author = {J. H. Yin},
	File = {../../Papers/yin05.pdf},
	Journal = {Geophys. Res. Lett.},
	Note = {doi:10.1029/2005GL023684},
	Pages = {L18701},
	Title = {A consistent poleward shift of the storm tracks in simulations of 21st century climate},
	Volume = 32,
	Year = 2005,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgl5aW4wNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSyv/L2sQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv/NnMQAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWluMDUucGRmAA4AFAAJAHkAaQBuADAANQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMveWluMDUucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMveWluMDUucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Yin49,
	Annote = {Sudden onset of monsoon.},
	Author = {M. T. Yin},
	File = {../../Papers/yin49.pdf},
	Journal = {J. Meteor.},
	Pages = {393--400},
	Title = {Synoptic-aerologic study of the onset of the summer monsoon over {India} and {Burma}},
	Volume = 6,
	Year = 1949,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgl5aW40OS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRSzwR5bxFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwR6+NAAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eWluNDkucGRmAA4AFAAJAHkAaQBuADQAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMveWluNDkucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMveWluNDkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Yoneyama99,
	Annote = {Filed under Water Vapor (Feedback and
                  Kinematics). Dry intrusions into Tropics due to
                  baroclinic eddies.},
	Author = {K. Yoneyama and D. Parsons},
	File = {../../Papers/yoneyama99.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {1524--1546},
	Title = {A proposed mechanism for the intrusion of dry air into the tropical western {P}acific region},
	Volume = 56,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAW4AAAAAAW4AAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfg55b25leWFtYTk5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRS0v3VkTwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv3XGvwAAAAEADAAJDH4ACE6zAACS8wACAC1NYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eW9uZXlhbWE5OS5wZGYAAA4AHgAOAHkAbwBuAGUAeQBhAG0AYQA5ADkALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAhVXNlcnMvdGFwaW8vUGFwZXJzL3lvbmV5YW1hOTkucGRmAAATAAEvAAAVAAIADP//AACABdIcHR4fWCRjbGFzc2VzWiRjbGFzc25hbWWjHyAhXU5TTXV0YWJsZURhdGFWTlNEYXRhWE5TT2JqZWN0XxAbLi4vLi4vUGFwZXJzL3lvbmV5YW1hOTkucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAhICFAIZAiICLQIxAj8CRgJPAm0CcgJ1AoIChwAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAKZ}}

@incollection{Young87,
	Address = {New York, NY},
	Annote = {Filed under Monsoon Dynamics.},
	Author = {J. A. Young},
	Booktitle = {Monsoons},
	Editor = {J. S. Fein and P. L. Stephens},
	File = {../../Papers/young87.pdf},
	Pages = {211--243},
	Publisher = {John Wiley \& Sons},
	Title = {Physics of Monsoons: The Current View},
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt5b3VuZzg3LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRS1wSNn2AAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwSPKSAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eW91bmc4Ny5wZGYADgAYAAsAeQBvAHUAbgBnADgANwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMveW91bmc4Ny5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy95b3VuZzg3LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@incollection{Young87b,
	Address = {New York, NY},
	Annote = {Filed under Monsoon Dynamics.},
	Author = {J. A. Young},
	Booktitle = {Monsoon Meteorology},
	Editor = {C.-P. Chang and T. N. Krishnamurti},
	File = {../../Papers/young87b.pdf},
	Pages = {461--500},
	Publisher = {Oxford University Press},
	Series = {Monographs on Geology and Geophysics},
	Title = {Boundary Layer Dynamics of Tropical and Monsoonal Flows},
	Volume = 7,
	Year = 1987,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx5b3VuZzg3Yi5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRS2waLdmgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwaNOGgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6eW91bmc4N2IucGRmAAAOABoADAB5AG8AdQBuAGcAOAA3AGIALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3lvdW5nODdiLnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy95b3VuZzg3Yi5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@inproceedings{Young99,
	Address = {Woods Hole, MA},
	Author = {W. R. Young},
	Booktitle = {Proc. Program in Geophysical Fluid Dynamics},
	Editor = {C. Pasquero and J.-L. Thiffeault},
	Organization = {Woods Hole Oceanographic Institution},
	Title = {Stirring and Mixing},
	Year = 1999}

@article{Yu02,
	Annote = {Interaction of atmosphere with Indian Ocean can
                  influence ENSO.},
	Author = {J.-Y. Yu and C. R. Mechoso and J. C. {McWilliams} and A. Arakawa},
	Journal = {Geophys. Res. Lett.},
	Pages = {doi:0.1029/2001GL014098},
	Title = {Impacts of the {I}ndian {O}cean on the {ENSO} cycle},
	Volume = 29,
	Year = 2002}

@article{Yu93,
	Annote = {Filed under Hartmann.},
	Author = {J.-Y. Yu and D. L. Hartmann},
	Journal = {J. Atmos. Sci},
	Pages = {3244--3259},
	Title = {Zonal Flow Vacillation and Eddy Forcing in a Simple {GCM} of the Atmosphere},
	Volume = 50,
	Year = 1993}

@article{Zachos01,
	Annote = {Filed under Paleo-Climate Reviews.},
	Author = {J. Zachos and M. Pagani and L. Sloan and E. Thomas and K. Billups},
	Journal = {Sience},
	Pages = {686--693},
	Title = {Trends, Rhythms, and Aberrations in Global Climate 65 {Ma} to Present},
	Volume = 292,
	Year = 2001}

@article{Zakharov04,
	Annote = {Filed under Wave Turbulence.},
	Author = {V. Zakharov and F. Dias and A. Puskarev},
	Journal = {Phys. Rep.},
	Pages = {1--65},
	Title = {One-dimensional wave turbulence},
	Volume = 398,
	Year = 2004}

@article{Zebiak87,
	Annote = {Describes Cane-Zebiak model: Shallow water ocean
                  with embedded, fixed depth mixed layer. Upwelling in
                  SST equation carefully parameterized. Gill-type
                  atmosphere.},
	Author = {S. E. Zebiak and M. A. Cane},
	Journal = {Mon. Wea. Rev.},
	Pages = {2262--78},
	Title = {A model {E}l {N}i{\~n}o {S}outhern {O}scillation},
	Volume = 115,
	Year = 1987}

@article{Zhang04,
	Author = {C. Zhang and M. McGauley and N. A. Bond},
	File = {../../Papers/zhang04.pdf},
	Journal = {J. Climate},
	Pages = {133--139},
	Title = {Shallow Meridional Circulation in the Tropical Eastern {P}acific},
	Volume = 17,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt6aGFuZzA0LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRS6wcsXSwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwcuHywAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6emhhbmcwNC5wZGYADgAYAAsAegBoAGEAbgBnADAANAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvemhhbmcwNC5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy96aGFuZzA0LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Zhang06,
	Author = {Zhang, M. and Song, H.},
	File = {../../Papers/zhang06.pdf},
	Journal = {Geophys. Res. Lett},
	Note = {doi:10.1029/2006GL025942},
	Pages = {L12701},
	Title = {Evidence of deceleration of atmospheric vertical overturning circulation over the tropical {P}acific},
	Volume = {33},
	Year = {2006},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt6aGFuZzA2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRS8xTXE1wAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxTY1VwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6emhhbmcwNi5wZGYADgAYAAsAegBoAGEAbgBnADAANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvemhhbmcwNi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy96aGFuZzA2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Zhang96,
	Author = {Zhang, K. and Schubert, G.},
	File = {../../Papers/zhang96.pdf},
	Journal = {Science},
	Pages = {941--943},
	Title = {Penetrative Convection and Zonal Flow on Jupiter},
	Volume = {273},
	Year = {1996},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt6aGFuZzk2LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRS/xPQ6ZQAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxPSc1QAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6emhhbmc5Ni5wZGYADgAYAAsAegBoAGEAbgBnADkANgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvemhhbmc5Ni5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy96aGFuZzk2LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Zhang99,
	Annote = {Filed under Held.},
	Author = {Y. Zhang and I. M. Held},
	File = {../../Papers/zhang99.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {3416--3435},
	Title = {A Linear Stochastic Model of a {GCM}'s Midlatitude Storm Tracks},
	Volume = 56,
	Year = 1999,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt6aGFuZzk5LnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRTAwTXiNFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwTZEpAAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6emhhbmc5OS5wZGYADgAYAAsAegBoAGEAbgBnADkAOQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvemhhbmc5OS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy96aGFuZzk5LnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Zhou93a,
	Author = {S. Zhou and P. H. Stone},
	File = {../../Papers/zhou93a.pdf},
	Journal = {J. Climate},
	Pages = {985--1000},
	Title = {The Role of Large-Scale Eddies in the Climate Equilibrium: Part{I}: Fixed Static Stability},
	Volume = 6,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt6aG91OTNhLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRTBv/vzHwAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv/xjnwAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6emhvdTkzYS5wZGYADgAYAAsAegBoAG8AdQA5ADMAYQAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvemhvdTkzYS5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy96aG91OTNhLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Zhou93b,
	Annote = {Filed under Stone.},
	Author = {S. Zhou and P. H. Stone},
	File = {../../Papers/zhou93b.pdf},
	Journal = {J. Climate},
	Pages = {1871--1880},
	Title = {The Role of Large-Scale Eddies in the Climate Equilibrium: Part {II}: Variable Static Stability},
	Volume = 6,
	Year = 1993,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgt6aG91OTNiLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRTCv/vytgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv/xjNgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6emhvdTkzYi5wZGYADgAYAAsAegBoAG8AdQA5ADMAYgAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvemhvdTkzYi5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy96aG91OTNiLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@article{Zhu00,
	Annote = {Filed under Water Vapor (Feedback and Kinematics)
                  and Newell.},
	Author = {Y. Zhu and R. E. Newell and W. G. Read},
	File = {../../Papers/zhu00.pdf},
	Journal = {J. Climate},
	Pages = {836--848},
	Title = {Factors controlling Upper-Troposphere Water Vapor},
	Volume = 13,
	Year = 2000,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAVgAAAAAAVgAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgl6aHUwMC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRTDwDeRSAAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAwDgByAAAAAEADAAJDH4ACE6zAACS8wACAChNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6emh1MDAucGRmAA4AFAAJAHoAaAB1ADAAMAAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASABxVc2Vycy90YXBpby9QYXBlcnMvemh1MDAucGRmABMAAS8AABUAAgAM//8AAIAF0hwdHh9YJGNsYXNzZXNaJGNsYXNzbmFtZaMfICFdTlNNdXRhYmxlRGF0YVZOU0RhdGFYTlNPYmplY3RfEBYuLi8uLi9QYXBlcnMvemh1MDAucGRm0hwdJCWiJSFcTlNEaWN0aW9uYXJ5EgABhqBfEA9OU0tleWVkQXJjaGl2ZXIACAARABYAHwAoADIANQA6ADwARQBLAFIAXQBlAGwAbwBxAHMAdgB4AHoAfACGAJMAmACgAfwB/gIDAgwCFwIbAikCMAI5AlICVwJaAmcCbAAAAAAAAAIBAAAAAAAAACgAAAAAAAAAAAAAAAAAAAJ+}}

@article{Zhu98,
	Annote = {Filed under Newell.},
	Author = {Y. Zhu and R. E. Newell},
	Journal = {Mon. Wea. Rev.},
	Pages = {725--735},
	Title = {A Proposed Algorithm for Moisture Fluxes from Atmospheric Rivers},
	Volume = 126,
	Year = 1998}

@article{Zurita05,
	Author = {Zurita-Gotor, P.},
	Date-Modified = {2010-06-11 11:04:48 -0700},
	File = {../../Papers/zurita05.pdf},
	Journal = {J. Atmos. Sci.},
	Pages = {4450--4458},
	Title = {Updraft/Downdraft Constraints for Moist Baroclinic Modes and Their Implications for the Short-Wave Cutoff and Maximum Growth Rate},
	Volume = {62},
	Year = {2005},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgx6dXJpdGEwNS5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRTJv/Q0FgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv/SklgAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6enVyaXRhMDUucGRmAAAOABoADAB6AHUAcgBpAHQAYQAwADUALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL3p1cml0YTA1LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy96dXJpdGEwNS5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{Zurita01,
	Annote = {PV homogenization at critical level.},
	Author = {P. Zurita and R. S. Lindzen},
	Journal = {J. Atmos. Sci.},
	Pages = {3443--3462},
	Title = {The Equilibration of Short {C}harney Waves: Implications for Potential Vorticity Homogenization in the Extratropical Troposphere},
	Volume = 58,
	Year = 2001}

@article{Zwiers87,
	Annote = {Filed under Predictability.},
	Author = {F. W. Zwiers},
	Journal = {Mon. Wea. Rev.},
	Pages = {2957--2974},
	Title = {A Potential Predictability Study Conducted with an Atmospheric General Circulation Model},
	Volume = 115,
	Year = 1987}

@article{Zwiers96,
	Annote = {Not on File.},
	Author = {F. W. Zwiers},
	Journal = {Climate Dyn.},
	Pages = {825--848},
	Title = {Interannual Variability and Predictability in an Ensemble of {AMIP} climate simulations conducted with the {CCC} {GCM2}},
	Volume = 12,
	Year = 1996}

@article{borgas04,
	Annote = {Filed under Stochastic Lagrangian Models of Turbulence.},
	Author = {M. S. Borgas and P. K. Yeung},
	File = {../../Papers/borgas04.pdf},
	Journal = {J. Fluid Mech.},
	Pages = {125-160},
	Title = {Relative dispersion in isotropic turbulence. {P}art~2. {A} new stochastic model with {R}eynolds-number dependence},
	Volume = 503,
	Year = 2004,
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWYAAAAAAWYAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgxib3JnYXMwNC5wZGYAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACQz6v5GdvFBERiBDQVJPAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAv5IOPAAAAAEADAAJDH4ACE6zAACS8wACACtNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6Ym9yZ2FzMDQucGRmAAAOABoADABiAG8AcgBnAGEAcwAwADQALgBwAGQAZgAPABgACwBNAGEAYwBCAG8AbwBrACAAUAByAG8AEgAfVXNlcnMvdGFwaW8vUGFwZXJzL2JvcmdhczA0LnBkZgAAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGS4uLy4uL1BhcGVycy9ib3JnYXMwNC5wZGbSHB0kJaIlIVxOU0RpY3Rpb25hcnkSAAGGoF8QD05TS2V5ZWRBcmNoaXZlcgAIABEAFgAfACgAMgA1ADoAPABFAEsAUgBdAGUAbABvAHEAcwB2AHgAegB8AIYAkwCYAKACCgIMAhECGgIlAikCNwI+AkcCYwJoAmsCeAJ9AAAAAAAAAgEAAAAAAAAAKAAAAAAAAAAAAAAAAAAAAo8=}}

@article{deMenocal01,
	Annote = {Filed under Paleo-Climate Reviews.},
	Author = {P. B. {deMenocal}},
	Journal = {Science},
	Pages = {667--673},
	Title = {Cultural Responses to Climate Change During the Late Holocene},
	Volume = 292,
	Year = 2001}

@article{deRuyter97,
	Annote = {Filed under Entropy Estimation. See also Strong97},
	Author = {R. R. {de Ruyter van Steveninck} and G. D. Lewen and S. P. Strong and R. Koberle and W. Bialek},
	Journal = {Science},
	Pages = {1805--1808},
	Title = {Reproducibility and Variability in Neural Spike Trains},
	Volume = 275,
	Year = 1997}

@article{joshi03,
	Author = {Joshi, M.},
	File = {../../Papers/joshi03.pdf},
	Journal = {Astrobiology},
	Pages = {415--427},
	Title = {Climate model studies of synchronously rotating planets},
	Volume = {3},
	Year = {2003},
	Bdsk-File-1 = {YnBsaXN0MDDUAQIDBAUIJidUJHRvcFgkb2JqZWN0c1gkdmVyc2lvblkkYXJjaGl2ZXLRBgdUcm9vdIABqAkKFRYXGyIjVSRudWxs0wsMDQ4RFFpOUy5vYmplY3RzV05TLmtleXNWJGNsYXNzog8QgASABqISE4ACgAOAB1lhbGlhc0RhdGFccmVsYXRpdmVQYXRo0hgNGRpXTlMuZGF0YU8RAWAAAAAAAWAAAgAAC01hY0Jvb2sgUHJvAAAAAAAAAAAAAAAAAAAAAMfUNWFIKwAAAAkMfgtqb3NoaTAzLnBkZgAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAACRFfxrtCkgAAAAAAAAAAAAIAAgAACSAAAAAAAAAAAAAAAAAAAAAGUGFwZXJzABAACAAAx9SX0QAAABEACAAAxrulAgAAAAEADAAJDH4ACE6zAACS8wACACpNYWNCb29rIFBybzpVc2Vyczp0YXBpbzpQYXBlcnM6am9zaGkwMy5wZGYADgAYAAsAagBvAHMAaABpADAAMwAuAHAAZABmAA8AGAALAE0AYQBjAEIAbwBvAGsAIABQAHIAbwASAB5Vc2Vycy90YXBpby9QYXBlcnMvam9zaGkwMy5wZGYAEwABLwAAFQACAAz//wAAgAXSHB0eH1gkY2xhc3Nlc1okY2xhc3NuYW1lox8gIV1OU011dGFibGVEYXRhVk5TRGF0YVhOU09iamVjdF8QGC4uLy4uL1BhcGVycy9qb3NoaTAzLnBkZtIcHSQloiUhXE5TRGljdGlvbmFyeRIAAYagXxAPTlNLZXllZEFyY2hpdmVyAAgAEQAWAB8AKAAyADUAOgA8AEUASwBSAF0AZQBsAG8AcQBzAHYAeAB6AHwAhgCTAJgAoAIEAgYCCwIUAh8CIwIxAjgCQQJcAmECZAJxAnYAAAAAAAACAQAAAAAAAAAoAAAAAAAAAAAAAAAAAAACiA==}}

@book{signal_process,
	Address = {Natick, Massachussetts},
	Author = {T. P. Krauss and L. Shure and J. N. Little},
	Publisher = {The MathWorks, Inc.},
	Title = {Signal Processing Toolbox},
	Year = 1994}

@book{vanFraassen80,
	Author = {Bas C. {van Fraassen}},
	Pages = 235,
	Publisher = {Oxford University Press},
	Series = {Clarendon Library of Logic and Philosophy},
	Title = {The Scientific Image},
	Year = 1980}

@article{vanHuffel87,
	Annote = {Filed under Regression Analysis. Uses
                  Golub/Klema/Stewart technique applied to augmented
                  data matrix [A b].},
	Author = {S. {van Huffel} and J. Vandewalle},
	Journal = {Lin. Alg. Appl.},
	Pages = {695--714},
	Title = {Subset Selection Using the Total Least Squares Approach in Collinearity Problems with Errors in the Variables},
	Volume = {88/89},
	Year = 1987}

@book{vanHuffel91a,
	Address = {Philadelphia},
	Annote = {QA275.H84 1991},
	Author = {S. {van Huffel} and J. Vandewalle},
	Pages = 300,
	Publisher = {Society for Industrial and Applied Mathematics},
	Series = {Frontiers in Applied Mathematics},
	Title = {The Total Least Squares Problem: Computational Aspects and Analysis},
	Volume = 9,
	Year = 1991}

@article{vanHuffel91b,
	Annote = {Filed under Regularization.},
	Author = {S. {van Huffel} and H. Zha},
	Journal = {SIAM J. Matrix Anal. Appl.},
	Pages = {292--309},
	Title = {The restricted total least squares problem: formulation, algorithm and properties},
	Volume = 12,
	Year = 1991}

@article{vanHuffel92,
	Annote = {Filed under Regularization.},
	Author = {S. {van Huffel}},
	Journal = {SIAM J. Matrix Anal. Appl.},
	Pages = {20--35},
	Title = {On the significance of nongeneric total least squares problems},
	Volume = 13,
	Year = 1992}

@article{vonStorch95,
	Annote = {Filed under Hasselmann.},
	Author = {H. {von Storch} and G. B{\"u}rger and R. Schnur and J.-S. {von Storch}},
	Journal = {J. Climate},
	Pages = {377--400},
	Title = {Principal {O}scillation {P}atterns: {A} Review},
	Volume = 8,
	Year = 1995}

@book{vonStorch99,
	Address = {Cambridge, UK},
	Author = {H. {von Storch} and F. W. Zwiers},
	Pages = 484,
	Publisher = {Cambridge University Press},
	Title = {Statistical Analysis in Climate Research},
	Year = 1999}
@article{back06,
  title={Geographic variability in the export of moist static energy and vertical motion profiles in the tropical {P}acific},
  author={L. E. Back and C. S. Bretherton},
  journal={Geophys. Res. Lett.},
  volume={33},
  pages={L17810},
  year={2006},
  publisher={American Geophysical Union}
}


@article{back09a,
  title={On the relationship between {SST} gradients, boundary layer winds, and convergence over the tropical oceans},
  author={L. E. Back and C. S. Bretherton},
  journal={J. Clim.},
  volume={22},
  pages={4182--4196},
  year={2009}
}


@article{barsugli05,
  title={{Tropical climate regimes and global climate sensitivity in a simple setting}},
  author={Barsugli, J. and Shin, S .I. and Sardeshmukh, P. D.},
  journal=JAS,
  volume={62},
  number={4},
  pages={1226--1240},
  year={2005},
  publisher={American Meteorological Society}
}

@article{bellon09,
  title={{Hadley circulation: multiple equilibria and insights into the double ITCZ problem}},
  author={Bellon, G. and Sobel, A. H.},
  journal=JoC,
  year={2009}
}

@article{Boccaletti04,
  title={The thermal structure of the upper ocean},
  author={G. Boccaletti and R. C. Pacanowski and S. G. H. Philander and A. V. Fedorov},
  journal={J. Phys. Oceanogr.},
  volume={34},
  number={4},
  pages={888-902},
  year={2004}
}

@article{Boos08a,
        Author = {William R. Boos and Kerry A. Emanuel},
        Journal = {J. Atmos. Sci.},
        Pages = {2194--2214},
        Title = {Wind-evaporation feedback and abrupt seasonal transitions of axisymmetric {H}adley circulations},
        Volume = 65,
        Year = {2008}
}

@article{Bretherton06,
  title={Interpretation of simple and cloud-resolving simulations of moist convection--radiation interaction with a mock-{W}alker circulation},
  author={C. S. Bretherton and P. N. Blossey and M. E. Peters},
  journal={Theor. Comput. Fluid Dyn.},
  volume={20},
  number={5},
  pages={421--442},
  year={2006},
  publisher={Springer}
}

@article{Chiang05,
  title={Influence of high latitude ice cover on the marine {I}ntertropical {C}onvergence {Z}one},
  author={J. C. H. Chiang and C. M. Bitz},
  journal={Clim. Dyn.},
  volume={25},
  number={5},
  pages={477--496},
  year={2005},
  publisher={Springer}
}

@article{chang93,
  title={On the Dynamics of a Storm Track},
  author={Chang, E. K. M. and Orlanski, I.},
  journal={Journal of the Atmospheric Sciences},
  volume={50},
  number={7},
  pages={999--1015},
  year={1993},
  publisher={American Meteorological Society}
}

@article{chao04,
  title={{Single and double ITCZ in an aqua-planet model with constant sea surface temperature and solar angle}},
  author={Chao, W. C. and Chen, B.},
  journal={Climate Dynamics},
  volume={22},
  number={4},
  pages={447--459},
  year={2004},
  publisher={Springer}
}

@article{Charbonneau09,
  title={A super-{E}arth transiting a nearby low-mass star},
  author={D. Charbonneau and Z. K. Berta and J. Irwin and C. J. Burke and
          P. Nutzman and L. A. Buchhave and C. Lovis and X. Bonfils and
          D. W. Latham and S. Udry and R. A. Murray-Clay and M. J. Holman and
          E. E. Falco and J. N. Winn and D. Queloz and F. Pepe and M. Mayor
          and X. Delfosse and T. Forveille},
  journal={Nature},
  volume={462},
  pages={891--894},
  year={2009}
}

@article{Charbonneau00,
  title={Detection of Planetary Transits Across a {S}un-like Star},
  author={D. Charbonneau and T. M. Brown and D. W. Latham and M. Mayor},
  journal={Astrophys. J.},
  volume={529},
  pages={L45--L48},
  year={2000}
}

@article{Chou10,
  title={Depth of convection and the weakening of tropical circulation
         in global warming},
  author={C. Chou and C.-A. Chen},
  journal={J. Clim.},
  pages={in press},
  year={2010}
}

@article{Clement96,
  title={An ocean dynamical thermostat},
  author={Clement, A. C. and Seager, R. and Cane, M. A. and Zebiak, S. E.},
  journal={J. Clim.},
  volume={9},
  pages={2190--2196},
  year={1996},
}

@article{Clement04,
  title={The importance of precessional signals in the tropical climate},
  author={A. C. Clement and A. Hall and A. J. Broccoli},
  journal={Clim. Dyn.},
  volume={22},
  number={4},
  pages={327--341},
  year={2004},
  publisher={Springer}
}

@article{cobb07,
  title={Regional-scale climate influences on temporal variations of rainwater and cave dripwater oxygen isotopes in northern {B}orneo},
  author={K. M. Cobb and J. F. Adkins and J. W. Partin and B. Clark},
  journal={Earth Planet. Sci. Lett.},
  volume={263},
  number={3-4},
  pages={207--220},
  year={2007},
  publisher={Elsevier}
}

@article{Dayem09,
  title={Lessons learned from the modern monsoon applied to the interpretation
         of paleoclimate records.},
  author={K. Dayem and D. S. Battisti and G. H. Roe and P. Molnar},
  year = {2009},
  journal={Earth Planet. Sci. Lett.},
  pages = {in press}
}

@article{Dinezio09,
  title={Climate Response of the Equatorial {P}acific to Global Warming},
  author={{DiNezio}, P. N. and Clement, A. C. and Vecchi, G. A. and Soden, B. J. and Kirtman, B. P. and Lee, S. K.},
  journal={J. Clim.},
  volume={22},
  pages={4873--4892},
  year={2009}
}

@article{Dirmeyer98,
  title={Land-sea geometry and its effect on monsoon circulations},
  author={P. A. Dirmeyer},
  journal={J. Geophys. Res.},
  year={1998},
  volume={103},
  number={D10},
  pages={11555-11572},
  publisher={American Geophysical Union}
}

@article{Drijfhout09,
  title={The atmospheric response to a {THC} collapse: Scaling relations for the {H}adley circulation and the response in a coupled climate model},
  author={S. S. Drijfhout},
  year = {2009},
  journal={J. Clim.}, 
  pages={In Press}
}

@article{Enderton09,
  title={Explorations of Atmosphere-Ocean-Ice Climates on an Aquaplanet and Their Meridional Energy Transports},
  author={D. Enderton and J. Marshall},
  journal={J. Atmos. Sci.},
  volume={66},
  pages={1593--1611},
  year={2009},
  publisher={American Meteorological Society}
}

@article{Fedorov06,
  title={The {P}liocene paradox (mechanisms for a permanent {E}l {N}i{\~n}o)},
  author={A. V. Fedorov and P. S. Dekens and M. McCarthy and A. C. Ravelo and P. B. DeMenocal and M. Barreiro and R. C. Pacanowski and S. G. Philander},
  journal={Science},
  volume={312},
  number={5779},
  pages={1485--1489},
  year={2006},
  publisher={American Association for the Advancement of Science}
}

@article{Griffies04,
  title={{A Technical Guide to MOM4}},
  author={S. M. Griffies and M. J. Harrison and R. C. Pacanowski and A. Rosati},
  journal={GFDL Ocean Group Technical Report},
  year={2004}
}

@Book{Hartmann94b,
  author =       "D. Hartmann",
  title =        "Global Physical Climatology",
  publisher =    "Academic Press",
  year =         1994,
  pages =        411
}

@article{Hartmann02,
  title={An important constraint on tropical cloud-climate feedback},
  author={Hartmann, D. L. and Larson, K.},
  journal={Geophys. Res. Lett.},
  volume={29},
  pages = {1951},
  year={2002},
  note={doi:10.1029/2002GL015835},
  publisher={American Geophysical Union}
}

@article{held10,
  title={Probing the Fast and Slow Components of Global Warming by Returning Abruptly to Preindustrial Forcing},
  author={Held, I. M. and Winton, M. and Takahashi, K. and Delworth, T. and Zeng, F. and Vallis, G. K.},
  journal={J. Clim.},
  volume={23},
  pages={2418--2427},
  year={2010}
}

@Book{Hubbard84,
   author = {W. B. Hubbard},
   title = "Planetary Interiors",
   publisher = "Van Nostrand Reinhold Co.",
   year = 1984,
   pages = 334
}

@article{Kang08,
  title={The response of the {ITCZ} to extratropical thermal forcing: Idealized slab-ocean experiments with a {GCM}},
  author={S. M. Kang and I. M. Held and D. M. W. Frierson and M. Zhao},
  journal={J. Clim.},
  volume={21},
  number={14},
  pages={3521--3532},
  year={2008},
  publisher={American Meteorological Society}
}

@article{Kang09,
  title={The tropical response to extratropical thermal forcing in an
         idealized {GCM}: The importance of radiative feedbacks and convective 
         parameterization.},
  author={S. M. Kang and D. M. W. Frierson and I. M. Held},
  journal={J. Atmos. Sci.},
  volume={66},
  pages={2812-2827},
  year={2009},
  publisher={American Meteorological Society}
}

@article{Lee98,
  title={Seasonal cycles of meridional overturning and heat transport of the {I}ndian Ocean},
  author={T. Lee and J. Marotzke},
  journal={J. Phys. Oceanogr.},
  volume={28},
  number={5},
  pages={923--943},
  year={1998},
  publisher={American Meteorological Society}
}

@article{Levine09,
  title={Response of the {H}adley circulation to climate change in an aquaplanet {GCM} coupled to ocean heat transport},
  author={X. J. Levine and T. Schneider},
  journal={J. Atmos. Sci.},
  pages={to be submitted},
  year={2009}
}

@article{Neelin88,
  title={A simple model for surface stress and low-level flow in the tropical atmosphere driven by prescribed heating},
  author={J. D. Neelin},
  journal={Quart. J. Roy. Meteor. Soc.},
  volume={114},
  pages={747--770},
  year={1988}
}

@article{ogorman10,
  title={How closely do changes in surface and column water vapor follow {C}lausius--{C}lapeyron scaling in climate change simulations?},
  author={O'Gorman, P. A. and Muller, C. J.},
  journal={Environ. Res. Lett.},
  volume={5},
  pages={025207},
  year={2010},
  publisher={IOP Publishing}
}

@article{orlanski91,
  title={The Life Cycle of a Cyclone Wave in the Southern Hemisphere. Part I: Eddy Energy Budget},
  author={Orlanski, I. and Katzfey, J.},
  journal={Journal of the Atmospheric Sciences},
  volume={48},
  number={17},
  pages={1972--1998},
  year={1991},
  publisher={American Meteorological Society}
}

#@article{peters05,
#  title={A simplified model of the {W}alker circulation with an interactive ocean mixed layer and cloud-radiative feedbacks},
#  author={M. E. Peters and C. S. Bretherton},
#  journal={J. Climate},
#  volume={18},
#  number={20},
#  pages={4216--4234},
#  year={2005},
#  publisher={American Meteorological Society}
#}

@article{peters08,
  title={Analysis of Atmospheric Energy Transport in {ERA-40} and Implications for Simple Models of the Mean Tropical Circulation},
  author={Peters, M. E. and Kuang, Z. and Walker, C. C.},
  journal={J. Clim.},
  volume={21},
  number={20},
  pages={5229--5241},
  year={2008}
}

@Book{Pierrehumbert10,
  author =       "R. T. Pierrehumbert",
  title =        "Principles of Planetary Climate",
  publisher =    "Cambridge University Press",
  year =         2010,
  pages =        688
}

@InCollection{Showman09,
  author =       {A. P. Showman and J. Y-K. Cho and K. Menou},
  title =        {Atmospheric circulation of extrasolar planets},
  booktitle =    {Exoplanets},
  publisher =    {University of Arizona Press},
  year =         2009,
  editor =       {S. Seager},
  address =      {Tucson, AZ},
}

@article{trenberth01b,
  title={The atmospheric energy budget and implications for surface fluxes and ocean heat transports},
  author={K. E. Trenberth and J. M. Caron and D. P. Stepaniak},
  journal={Clim. Dyn.},
  volume={17},
  number={4},
  pages={259--276},
  year={2001},
  publisher={Springer}
}

@article{vecchi08,
  title={Examining the tropical {P}acific's response to global warming},
  author={G. A. Vecchi and A. Clement and B. J. Soden},
  journal={Eos Trans. AGU},
  volume={89},
  number={9},
  pages={81--83},
  year={2008}
}

@article{wang08,
  title={Millennial-and orbital-scale changes in the {E}ast {A}sian monsoon over the past 224,000 years},
  author={Y. Wang and H. Cheng and R.L. Edwards and et al},
  journal={Nature},
  volume={451},
  number={7182},
  pages={1090--1093},
  year={2008},
  publisher={Nature Publishing Group},
  annote={other authors: and Kong, X. and Shao, X. and Chen, S. and Wu, J. and Jiang, X. and Wang, X. and An, Z.}
}

@article{wunsch09,
  title={A Perpetually Running {ENSO} in the {P}liocene?},
  author={C. Wunsch},
  journal={J. Clim.},
  volume={22},
  pages={3506--3510},
  year={2009}
}


@article{xie10,
  title={Global warming pattern formation: Sea surface temperature and rainfall},
  author={S.-P. Xie and C. Deser and G. A. Vecchi and J. Ma and H. Teng and A. T. Wittenberg},
  journal={J. Climate},
  volume={23},
  pages={966--986},
  year={2010},
  publisher={American Meteorological Society}
}

@article{yano02,
  title={Mean-state convective circulations over large-scale tropical SST gradients},
  author={J. I. Yano and W. W. Grabowski and M. W. Moncrieff},
  journal={J. Atmos. Sci.},
  volume={59},
  number={9},
  pages={1578--1592},
  year={2002},
  publisher={American Meteorological Society}
}



